BCS Theory in the Weak Magnetic Field Regime for Systems with Nonzero Flux and Exponential Estimates on the Adiabatic Theorem in Extended Quantum Lattice Systems

In the main part of this PhD thesis, we consider a periodically realized microscopic superconductor described by BCS theory, which is subject to external electromagnetic fields. We show that the superconductor is properly described by Ginzburg--Landau theory in the macroscopic and weak magnetic field limit. The main novelty of our results is to allow for a non-vanishing magnetic flux through the unit cell of the lattice of periodicity. These main results are supplemented by various unpublished notes in the field of BCS theory. Furthermore, we preface the presentation of these results with a comprehensive introduction suitable for master's or PhD students. Thereby, we hope to contribute to filling the gap of missing introductory literature in the field. The thesis comprises a second topic, in which we provide ideas for setting up quantum lattice systems in order to prove exponential estimates for the adiabatic theorem. These notes are the result of studies in this field, which have been conducted during a research stay at the University of British Columbia (UBC) in Vancouver, Canada.

==> 00_Titel.tex <==
%auto-ignore  % for ArXiv to process correctly

%% Deckblatt
\ThisTileWallPaper{\paperwidth}{\paperheight}{Siegelwallpaperblank.pdf}
\deckblatt
%
\thispagestyle{empty}
~\newpage
\thispagestyle{empty}

\ThisTileWallPaper{\paperwidth}{\paperheight}{Siegelwallpaper.pdf}
\deckblatt

\thispagestyle{empty}
~\newpage

%\setcounter{page}1
%\begin{minipage}{1.0 \textwidth}
%\abstract{
%\noindent
%We prove a two-term asymptotics for the canonical zero-temperature Bogolubov energy functional. The functional describes a homogeneous, dilute gas of repulsively interacting Bosons in 3 spatial dimensions in the thermodynamic limit. As a main result, we show the formula $4\pi a\rho^2 + \frac{512\sqrt{\pi}}{15} C\cdot (\rho a)^{\nicefrac 52}+ \lano(\rho a)^{\nicefrac 52}$ for the ground state energy density as $\rho a\to 0$. Here, $\rho$ is the density of the gas and $a$ is the scattering length of the two-body interaction potential $V$. The explicit constant $C > 1$ is depending on the potential. The result is in agreement with the upper bound given by \cite{ESY} and the method is inspired by \cite{Reu2}. The second order term carries a constant which is strictly larger than the one in the Lee-Huang-Yang formula.
%} 
%\end{minipage}
%
%\newpage
%
%~\thispagestyle{empty}
%\newpage
%%\setcounter{page}2
%% Inhaltsverzeichnis
%
%\tableofcontents


==> 00_Titeldeklaration.tex <==
%auto-ignore  % for ArXiv to process correctly

% Gestaltung der Kopf- und Fusszeilen
\pagestyle{fancy}
\headheight 14pt
\fancyhf{}
\fancyhead[L]{\small\slshape\leftmark}
\fancyfoot[C]{\thepage}

% subsubsections numerieren und ins Inhaltsverzeichnis aufnehmen
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%%
%% Globale Variablen
%%
\newtoks\fach               % Studiengang
\newtoks\fakultaet          % Fakultät für Sprach- und Literaturwissenschaften
\newtoks\department         % Department 2
\newtoks\arbeit             % Art der Arbeit 
\newtoks\titel              % Titel der Arbeit
\newtoks\bearbeiter         % Name des Bearbeiters
\newtoks\betreuer           % Name des Betreuers
\newtoks\abgabetermin      	% Datum der Abgabe
\newtoks\bearbeitungszeit  	% bearbeitungszeit
\newtoks\aufgabensteller    % Aufgabensteller, im Allgemeinen identisch mit dem Betreuer
\newtoks\universitaet       % im allgemeinen Ludwig Maximilians Universität
\newtoks\ort                % Wohnort des Bearbeiters

%%
%% Ausgabe des Deckblatts
%%
\newcommand{\deckblatt}{
  \begin{titlepage}

%  \vspace{-2cm}
%  \begin{center}
%   \parbox[t]{160mm}{\includegraphics[width=160mm]{lmu_cis_logo.jpg} }
%  \end{center}
\vspace*{2cm}    
  \begin{center}
      %\vspace{3cm}
      \huge
      \the\arbeit\\
      \vspace*{2cm}
      {\large in \the\fach}\\			
			{\large \the\universitaet}\\
			{\large \the\fakultaet}\\
			%{\large \the\department} 

      \vspace{2cm}\huge
      \the\titel

			
      \vspace{2.5cm}\large
			~ \\
      \the\bearbeiter  \\
      \vspace{2cm}\large
      		\the \abgabetermin \\

      \vspace{\fill}\normalsize
      supervised by:\\ \the\betreuer
%      \begin{tabular}{ll}
%        Betreuer und Aufgabensteller:        & \the\betreuer\\
%        %Aufgabensteller:        & \the\aufgabensteller\\
%        %Bearbeitungszeitraum:     & \the\bearbeitungszeit
%      \end{tabular}
    
    \end{center}
  
  \end{titlepage}
}


%%
%% Ausgabe der Erklaerung ueber die selbstaendige Anfertigung
%% einer Diplomarbeit
%%
\newcommand{\erklaerung}{
  \begin{titlepage}
    \vspace*{\fill}
    \parindent 0cm
    \begin{center}
      \textbf{Declaration of authorship}

      \vspace{1cm}
  
      \begin{minipage}{9.8cm}
%        I hereby declare that I developed this thesis without using any other sources and aid other than the ones which are declared as references.\\
%        
%        This paper was neither previously presented to another exami\-nation board nor        has been published.
        
I declare that the work presented here is, to the best of my knowledge and belief, original and the result of my own investigations, except as acknowledged. It has not been submitted, neither in whole nor partly, for a degree at this or any other university.\\

Formulations and ideas taken from other sources are cited accordingly.\\

        \vspace{1cm}
        \the\ort, \the\abgabetermin

        \vspace{1.5cm}
        \makebox[9.8cm]{\dotfill}\\
        \the\bearbeiter

      \end{minipage}
  
    \end{center}
  
    \vspace*{\fill}
  \end{titlepage}
}

\newcommand{\emptypage}{
\begin{titlepage}
\vspace*{\fill}
\end{titlepage}
}


\global\fach{Theoretical and Mathematical Physics}
\global\arbeit{Master's Thesis}
\global\titel{A Second Order Ground State Energy Expansion

\vspace{0.3cm}

for the Dilute Bose Gas}
\global\bearbeiter{Marcel Oliver Schaub}
\global\betreuer{Prof. PhD Thomas \O stergaard S\o rensen}
\global\universitaet{Ludwig-Maximilians-Universität München}
\global\fakultaet{Department Mathematisches Institut}
\global\abgabetermin{September 4, 2017}
\global\ort{Munich}


==> 1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.2_Gauge-periodic_samples.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Gauge-periodic samples}
\label{DHS1:Magnetically_Periodic_Samples}

We consider a $3$-dimensional sample of fermionic particles described by BCS theory that is subject to an external magnetic field $\Bbold := Be_3$ with strength $B>0$, pointing in the $e_3$-direction. We choose the magnetic vector potential $\Abold(x) := \frac 12 \Bbold \wedge x$ so that $\curl \Abold = \Bbold$, where $\Bbold \wedge x\in \Rbb^3$ denotes the cross product of two vectors. The corresponding magnetic momentum operator $\pi := -\i \nabla + \Abold$ commutes with the magnetic translations $T(v)$, defined by
\begin{align}
T(v)f(x) &:= \e^{\i \frac {\Bbold} 2\cdot (v\wedge x)} f(x+v), & v &\in \Rbb^3.\label{DHS1:Magnetic_Translation}
\end{align}
The family $\{T(v)\}_{v\in \Rbb^3}$ obeys the relation $T(v + w) = \e^{\i \frac{\Bbold}{2} \cdot (v \wedge w)} \; T(v) T(w)$, that is, it is a unitary representation of the Heisenberg group. We assume that our system is periodic with respect to the Bravais lattice $\Lambda_B = \sqrt{2\pi B^{-1}} \, \Zbb^3$ with fundamental cell
\begin{align}
Q_B &:= \bigl[0, \sqrt{2\pi B^{-1}}\bigr]^3 \subseteq \Rbb^3. \label{DHS1:Fundamental_cell}
\end{align}
The magnetic flux through the unit cell $Q_B$ equals $\Bbold \cdot (b_1\wedge b_2) =2\pi$, where $b_i = \sqrt{2\pi B^{-1}} \, e_i$ are the basis vectors spanning $\Lambda_B$. This assures that the abelian subgroup $\{T(\lambda)\}_{\lambda\in \Lambda_B}$ is a unitary representation of the lattice group. 
%This models a periodic system with constant nonzero magnetic flux through the unit cell $Q_B$. The magnetic flux is given by $\Bbold \cdot (b_1\wedge b_2) =2\pi$, where $b_i = \sqrt{2\pi B^{-1}} \, e_i$ are the basis vectors spanning $\Lambda_B$.

==> 1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.3_BCS-functional.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The BCS functional}
\label{DHS1:BCS_functional_Section}

In BCS theory a state is described by a generalized fermionic one-particle density matrix, that is, by a self-adjoint operator $\Gamma$ on $L^2(\mathbb{R}^3) \oplus L^2(\mathbb{R}^3)$ which satisfies $0\leq \Gamma\leq 1$ and is of the form
\begin{align}
\Gamma = \begin{pmatrix} \gamma & \alpha \\ \ov \alpha & 1 - \ov \gamma \end{pmatrix}. \label{DHS1:Gamma_introduction}
\end{align}
Here, $\ov \alpha = J \alpha J$ with the Riesz identification operator $J \colon L^2(\Rbb^3) \ra L^2(\Rbb^3)$, $f\mapsto \ov f$, realized by complex conjugation. The condition $\Gamma = \Gamma^*$ implies that the one-particle density matrix $\gamma$ is a self-adjoint operator. It also implies that the Cooper pair wave function $\alpha(x,y)$, the kernel of $\alpha$, is symmetric under the exchange of its coordinates. The symmetry of $\alpha$ is due to the fact that we exclude spin variables from our description and assume that Cooper pairs are in a spin singlet state. The condition $0\leq \Gamma \leq 1$ implies $0\leq \gamma \leq 1$ as well as that $\gamma$ and $\alpha$ are related through the operator inequality 
\begin{align}
\alpha \alpha^* \leq \gamma ( 1- \gamma). \label{DHS1:gamma_alpha_fermionic_relation}
\end{align}

A BCS state $\Gamma$ is called \emph{gauge-periodic} if $\mathbf T(\lambda) \, \Gamma \, \mathbf T(\lambda)^* = \Gamma$ holds for every $\lambda\in \Lambda_B$, with the magnetic translations $\mathbf T(\lambda)$ on $L^2(\Rbb^3)\oplus L^2(\Rbb^3)$ defined by
\begin{align*}
\mathbf T(v) &:= \begin{pmatrix}
T(v) & 0 \\ 0 & \ov{T(v)}\end{pmatrix}, & v &\in \Rbb^3.
\end{align*}
For $\gamma$ and $\alpha$, this implies $T(\lambda) \gamma T(\lambda)^* = \gamma$ and   $T(\lambda)\,\alpha \,\ov{T(\lambda)}^* = \alpha$ or, in terms of their kernels,
\begin{align}
\gamma(x, y) &= \e^{\i \frac \Bbold 2 \cdot (\lambda \wedge (x-y))} \; \gamma(x+\lambda,y+ \lambda), \notag\\
%
\alpha(x, y) &= \e^{\i \frac \Bbold 2 \cdot (\lambda \wedge (x+y))} \; \alpha(x+\lambda,y+ \lambda), & \lambda\in \Lambda_B. \label{DHS1:alpha_periodicity}
\end{align}

\begin{bem}
Since we are interested in the situation of a constant magnetic field it seems natural to consider magnetically translation-invariant BCS states, that is, states obeying $\mathbf T(v) \, \Gamma \, \mathbf T(v)^* = \Gamma$ for every $v \in \mathbb{R}^3$. However, in this case one obtains a trivial model because the Cooper pair wave function $\alpha$ of a magnetically translation-invariant state necessarily vanishes. To see this, we note that $\alpha$ satisfies $T(v)\,\alpha \,\ov{T(v)}^* = \alpha$ for all $v \in \mathbb{R}^3$. Using this and the relation $T(v+w)\,\alpha \,\ov{T(v+w)}^* =  \e^{ \i\Bbold \cdot (v \wedge w)} \, T(v) T(w) \, \alpha \, \ov{T(w)}^* \, \ov{T(v)}^* $, we conclude that $\alpha = 0$.
\end{bem}

A gauge-periodic BCS state $\Gamma$ is said to be \emph{admissible} if 
\begin{align}
\Tr \bigl[\gamma + (-\i \nabla + \Abold)^2\gamma\bigr] < \infty \label{DHS1:Gamma_admissible}
\end{align}
holds. Here $\Tr[A]$ denotes the trace per unit volume of $A$, i.e.,
\begin{align}
\Tr [A] &:= \frac{1}{|Q_B|} \Tr_{L^2(Q_B)} [\chi A \chi],  \label{DHS1:Trace_per_unit_volume_definition}
\end{align}
with the characteristic function $\chi$ of the cube $Q_B$ in \eqref{DHS1:Fundamental_cell}. By $\Tr_{L^2(Q_B)}[A]$ we denote the usual trace of an operator $A$ on $L^2(Q_B)$. The condition in \eqref{DHS1:Gamma_admissible} is meant to say that $\gamma$ and $(-\i \nabla + \Abold)^2\gamma$ are locally trace class, that is, they are trace class with respect to the trace in \eqref{DHS1:Trace_per_unit_volume_definition}. Eq.~\eqref{DHS1:Gamma_admissible}, the same inequality with $\gamma$ replaced by $\overline{\gamma}$, and the inequality in \eqref{DHS1:gamma_alpha_fermionic_relation} imply that $\alpha$, $(-\i \nabla + \Abold)\alpha$, and $(-\i \nabla + \Abold) \ov \alpha$ are locally Hilbert--Schmidt. In Section~\ref{DHS1:Preliminaries} below we will express this property in terms of $H^1$-regularity of the kernel of $\alpha$.

For any admissible BCS state $\Gamma$, we define the Bardeen--Cooper--Schrieffer free energy functional (in the following: BCS functional) at temperature $T\geq 0$ by
\begin{align}
\FBCS(\Gamma) &:= \Tr\bigl[ \bigl( (-\i \nabla + \Abold)^2 - \mu\bigr)\gamma \bigr] - T\, S(\Gamma) - \frac{1}{|Q_B|} \int_{Q_B} \dd X \int_{\Rbb^3} \dd r\; V(r) \, |\alpha(X,r)|^2,
\label{DHS1:BCS functional}
\end{align}
with the von Neumann entropy per unit volume $S(\Gamma)= - \Tr [\Gamma \ln(\Gamma)]$ and the chemical potential $\mu\in \Rbb$. The particles interact via a two-body potential $V \in L^{\nicefrac 32}(\Rbb^3) + L_{\varepsilon}^{\infty}(\mathbb{R}^3)$. Furthermore, we introduced center-of-mass and relative coordinates $X = \frac{x+y}{2}$ and $r = x-y$. Here and in the following, we abuse notation slightly by writing $\alpha(X,r)\equiv \alpha(x,y)$. 
\begin{bem}
	We opt for the above set-up because the solution of the problem for the constant magnetic field already contains the main difficulties of the case of a general magnetic field. This is related to the fact that the vector potential of any magnetic field with non-zero flux through the unit cell can be written as a sum of a vector potential of a homogeneous magnetic field and a periodic vector potential, see e.g. \cite[Proposition~4.1]{Tim_Abrikosov}. The latter can be treated in some sense as a perturbation, see \cite{Hainzl2012,Hainzl2014}. However, this is not true for the constant magnetic field, see Remark~\ref{DHS1:Remarks_Main_Result}~(a) below. To solve the general case it is therefore crucial to understand the case of a homogeneous magnetic field. To keep the presentation to a reasonable length and to be able to convey the main ideas more clearly, we therefore decided to present this case first. We plan to extend our treatment to the case of a general magnetic field in a second paper. One motivation to treat general periodic magnetic fields with non-zero flux through the unit cell stems from the fact that it is an interesting and highly relevant problem to consider magnetic fields that are chosen self-consistently.
\end{bem}

The BCS functional is bounded from below and coercive on the set of admissible states. More precisely, it can be shown that the kinetic energy dominates the entropy and the interaction energy, i.e., there is a constant $C>0$ such that for all admissible $\Gamma$, we have
\begin{align}
\FBCS(\Gamma) &\geq \frac 12 \Tr \bigl[ \gamma + (-\i \nabla + \Abold)^2 \gamma\bigr] - C. \label{DHS1:BCS functional_bounded_from_below}
\end{align}

The unique minimizer of the BCS functional among admissible states with $\alpha =0$ is given by
\begin{align}
\Gamma_0 &:= \begin{pmatrix} \gamma_0 & 0  \\ 0 &  1-\ov\gamma_0 \end{pmatrix}, & \gamma_0 &:= \frac 1{1 + \e^{ ((-\i\nabla + \Abold)^2-\mu)/T}}.  \label{DHS1:Gamma0}
\end{align}
Since $\Gamma_0$ is also the unique minimizer of the BCS functional for sufficiently large temperatures $T$, it is called the normal state.
%A direct consequence of the strict convexity of $x\mapsto x\ln x$ is the fact that $\Gamma_0$ is the unique minimizer of $\FBCS$ among states $\Gamma$ of the form \eqref{Gamma_introduction} with $\alpha =0$.
We define the BCS free energy by
\begin{align}
F^{\mathrm{BCS}}(B, T) := \inf\bigl\{ \FBCS(\Gamma) - \FBCS(\Gamma_0) : \Gamma \text{ admissible}\bigr\} \label{DHS1:BCS GS-energy}
\end{align}
%for the difference between the infimum of $\FBCS$ over all admissible states and the BCS energy of the normal state. We define 
and say that our system is superconducting if $F^{\mathrm{BCS}}(B, T) < 0$, that is, if the minimal energy is strictly smaller than that of the normal state. In this work we are interested in the regime of weak magnetic fields $0 < B \ll 1$. Our goal is to obtain an asymptotic expansion of $F^{\mathrm{BCS}}(B, T)$ in powers of $B$ that allows us to derive Ginzburg--Landau theory, and to show how the BCS critical temperature depends on the magnetic field $B$. For our main results to hold, we need the following assumptions concerning the regularity of the interaction potential $V$.
%Concerning , we need the following assumptions.
%
%As mentioned in the introduction, this is a two-scale problem and $B^{\nicefrac 12}$ plays the role of a semiclassical parameter, which expresses the ratio of the length scales between the microscopic and macroscopic scale. 
%
%and the limit $B\to 0$ can be viewed as a macroscopic limit, whose limiting model of superconductivity will be the Ginzburg--Landau model, which is defined in Section \ref{Ginzburg--Landau-functional}.
%
%The result is formulated in Theorem \ref{Main_Result}. To achieve it, we need the following additional assumptions on $V$.

\begin{asmp}
\label{DHS1:Assumption_V}
We assume that the interaction potential $V$ is a nonnegative, radial function such that $(1+|\cdot|^2) V\in L^\infty(\Rbb^3)$.
\end{asmp}

\begin{bem}
Our main results Theorem~\ref{DHS1:Main_Result} and Theorem~\ref{DHS1:Main_Result_Tc} still hold if the assumption $V\geq 0$ is dropped. We only use it in Appendix \ref{DHS1:KTV_Asymptotics_of_EV_and_EF_Section} when we investigate the spectral properties of a certain linear operator involving $V$. These statements still hold in the case of potentials without a definite sign but their proof is longer. A proof of these statements in the general setting can be found in the PhD thesis of M.~Schaub. We expect our results to be true also if $V$ has moderate local singularities. Furthermore, it may be possible to slightly weaken the decay assumptions of $V$. We choose to work with the assumptions above to keep the presentation at a reasonable length.
\end{bem}

%\subsection{Upper and lower critical temperature}
%\label{upperandlowerTc}
%
%A-priori it is not clear that there is one critical temperature $\Tc(B)$ such that one has $F^{\mathrm{BCS}}(B, T) < 0$ if $T < \Tc(B)$ and $F^{\mathrm{BCS}}(B, T) = 0$ if $T \geq \Tc(B)$. It could, in principle, be that superconductivity is present at a certain temperature, and as we increase the temperature the effect disappears and afterwards reappears again. Since we are interested in asymptotic expansions for small magnetic fields such an effect cannot be excluded. The quantities that we can make a statement about, are the upper and the lower critical temperature defined by 
%\begin{equation}
%	\overline{\Tc(B)} = \inf\{ T > 0 \ | \ \mathcal{F}^{\mathrm{BCS}}_{\bold{B},T'}(\Gamma) >  \mathcal{F}^{\mathrm{BCS}}_{\bold{B},T'}(\Gamma_0) \text{ for all } T'>T \text{ and all } \Gamma \neq \Gamma_0 \}
%\end{equation}
%and
%\begin{equation}
%	\underline{\Tc(B)} = \sup\{ T > 0 \ | \ F^{\mathrm{BCS}}(B, T') < 0 \text{ for all } T' < T \},
%\end{equation}
%respectively.

==> 1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.5_Translation_Invariant_BCS-functional.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The translation-invariant BCS functional}
\label{DHS1:BCS_functional_TI_Section}

If no external fields are present, i.e. if $\Bbold =0$, we describe the system by translation-invariant states, that is, we assume that the kernels of $\gamma$ and $\alpha$ are of the form $\gamma(x-y)$ and $\alpha(x-y)$. To define the trace per unit volume we choose a cube of side length $1$. The resulting translation-invariant BCS functional and its infimum minus the free energy of the normal state are denoted by $\mathcal{F}^{\mathrm{BCS}}_{\mathrm{ti},T}$ and $F^{\mathrm{BCS}}_{\mathrm{ti}}(T)$, respectively. This functional has been studied in detail in \cite{Hainzl2007}, see also \cite{Hainzl2015} and the references therein, where it has been shown that there is a unique critical temperature $\Tc \geq 0$ such that $\mathcal{F}^{\mathrm{BCS}}_{\mathrm{ti},T}$ has a minimizer with $\alpha \neq 0$ if $T < \Tc$. For $T\geq \Tc$ the normal state in \eqref{DHS1:Gamma0} with $B=0$ is the unique minimizer. In terms of the energy, we have $F^{\mathrm{BCS}}_{\mathrm{ti}}(T) < 0$ for $T < \Tc$, while $F^{\mathrm{BCS}}_{\mathrm{ti}}(T) = 0$ if $T\geq \Tc$.

It has also been shown in \cite{Hainzl2007} that the critical temperature $\Tc$ can be characterized via a linear criterion. More precisely, the critical temperature is determined by the unique value of $T$ such that the operator 
\begin{equation*}
	K_{T} - V 
\end{equation*}
acting on $L^2_{\mathrm{sym}}(\mathbb{R}^3)$, the space of reflection-symmetric square-integrable functions, has zero as its lowest eigenvalue. Here, $K_T = K_T(-\i \nabla)$ with the symbol 
\begin{align}
	K_T(p) := \frac{p^2 - \mu}{\tanh \frac{p^2-\mu}{2T}}. \label{DHS1:KT-symbol}
\end{align}
It should be noted that the function $T \mapsto K_T(p)$ is strictly monotone increasing for fixed $p \in \mathbb{R}^3$, and that $K_T(p) \geq 2T$ if $\mu \geq 0$ and $K_T(p)\geq |\mu|/\tanh(|\mu|/(2T))$ if $\mu < 0$. Our assumptions on $V$ guarantee that the essential spectrum of the operator $K_{T} - V$ equals $[2T, \infty)$ if $\mu \geq 0$ and $[|\mu|/\tanh(|\mu|/(2T)), \infty)$ if $\mu <0$. Accordingly, an eigenvalue at zero is necessarily isolated and of finite multiplicity.



The results in \cite{Hainzl2007} have been obtained in the case where the Cooper pair wave function $\alpha(x)$ is not necessarily an even function (as opposed to our setup), which means that $K_{\Tc}(-\i \nabla) - V$ has to be understood to act on $L^2(\mathbb{R}^3)$. The results in \cite{Hainzl2007}, however, equally hold if the symmetry of $\alpha$ is enforced. 

We are interested in the situation where (a) $\Tc > 0$ and (b) the translation-invariant BCS functional has a unique minimizer with a radial Cooper pair wave function ($s$-wave Cooper pairs) for $T$ close to $\Tc$. This is implied by the following assumption. Part~(b) should be compared to \cite[Theorem~2.8]{DeuchertGeisinger}.
%The essential spectrum of $K_T -V$ equal to that of $K_T$, i.e., $[2T, \infty)$ if $\mu \geq 0$ and $[|\mu|/\tanh(|\mu|/2T), \infty)$ if $\mu <0$. This follows from the fact that $L^{\nicefrac 32}(\Rbb^3)$ is contained in the Rollnik class, see \cite[Theorem 4.3]{LiebLoss}, and version of \cite[Theorem XIII.15]{Reedsimon4} for $K_T$. Hence, the spectrum of $K_T-V$ below $2T$ consists of isolated eigenvalues of finite multiplicity. In particular, $K_{\Tc} - V$ has a spectral gap above zero that we denote by $\kappa >0$.
%In the case of no external magnetic field, i.e., if $\Bbold =0$, we restrict our attention to translation-invariant states. That is, we assume that the kernels of $\gamma$ and $\alpha$ are of the form $\gamma(x-y)$ and $\alpha(x-y)$. 
%In this way, we obtain the translation-invariant BCS functional, which has been investigated in \cite{Hainzl2007}. There, it is shown that there is a critical temperature $\Tc$ such that for $T\geq \Tc$, the translation-invariant BCS functional is minimized by the pair $(\gamma, \alpha) = (\gamma_0, 0)$ with the normal state $\gamma_0 = (1 + \e^{\beta(-\nabla^2 - \mu)})^{-1}$, the one-particle density matrix of the free Fermi gas. For $T < \Tc$, however, there is a minimizing pair $(\gamma_T, \alpha_T)$ with $\alpha_T	\neq 0$ and strictly lower BCS energy than that of the normal state.

%By the second variational test for the BCS functional
%Furthermore, it is shown that the latter is equivalent to the existence of a negative eigenvalue for the linear operator $K_T - V$. It acts in $L^2_{\mathrm{sym}}(\Rbb^3)$, the symmetric square integrable functions, and the kinetic energy operator $K_T$ is given by the Fourier multiplier

%for $T>0$ and by $K_0(p) := |p^2-\mu|$ for $T =0$. Since the symbol $K_T$ is monotone in $T$, this is equivalent to saying that $T = \Tc$ if and only if $K_{T} - V$ has zero as its lowest eigenvalue. 

\begin{asmp}
\label{DHS1:Assumption_KTc}
\begin{enumerate}[(a)]
\item We assume that $\Tc >0$. If $V \geq 0$ and it does not vanish identically this is automatically implied, see \cite[Theorem 3]{Hainzl2007}. In the case of an interaction potential without a definite sign it is a separate assumption.

%(e.g., $V\in L^{\nicefrac 32}(\Rbb^3)$, $V\geq 0$ is sufficient, see \cite[Theorem 3]{Hainzl2007}).

\item We assume that the lowest eigenvalue of $K_{\Tc} - V$ is simple.
\end{enumerate}
\end{asmp}









%\begin{bem}
%\begin{enumerate}[(a)]
%\item 


%\item
%It is important for us to require that $V$ is radial, see Assumption \ref{Assumption_V} (b). Consequently, the unique eigenfunction $\alpha_*$ of the lowest eigenvalue of $K_{\Tc} - V$ has angular momentum zero and is therefore radial, too. This is of great importance for us in Section \ref{Lower Bound Part A}, in particular in the proof of Lemma \ref{AAstar_Positive}. Physically, the simplicity of $\alpha_*$ corresponds to an s-wave superconductor.
In the following we denote by $\alpha_*$ the unique ground state of the operator $K_{\Tc} - V$, i.e.,
\begin{align}
	K_{\Tc} \alpha_* = V\alpha_*. \label{DHS1:alpha_star_ev-equation}
\end{align}
We choose the normalization of $\alpha_*$ such that it is real-valued and $\Vert \alpha_*\Vert_{L^2(\Rbb^3)} = 1$. Since $V$ is a radial function and $\alpha_*$ is the unique solution of \eqref{DHS1:alpha_star_ev-equation} it follows that $\alpha_*$ is radial, too.
%Further regularity properties that we frequently use in this paper are summarized in \eqref{Decay_of_alphastar}.
%\end{enumerate}
%\end{bem}
%It is worth mentioning that if $(\gamma_T, \alpha_T)$ is a minimizing pair in the superconducting phase, then $\alpha_T$ vanishes at the rate $(T - \Tc)^{\nicefrac 12}$ as $T$ approaches $\Tc$, the coefficient being the eigenfunction $\alpha_*$, see \cite[Lemma 4.6]{DeuchertGeisinger}. In the temperature regime $T = \Tc (1 - DB)$ of Theorem \ref{Main_Result}, this means that $\alpha_T \sim \sqrt B \, \alpha_*$ to leading order. Hence, we may think of Theorem  \ref{Main_Result} as being a generalization to the translation-invariant case in which $\Psi$ is proportional to the constant function $\sqrt{B}$. It also motivates the choice of $\alpha_*$ in the main term in the decomposition \eqref{Thm1_decomposition} of $\alpha$.

==> 1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.7_Main_Results.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Main results}
\label{DHS1:Main_Result_Section}

Our first main result concerns the asymptotics of the BCS free energy in \eqref{DHS1:BCS GS-energy} in the regime $B \ll 1$. It also contains a statement about the asymptotics of the Cooper pair wave function of states $\Gamma$, whose energy $\FBCS(\Gamma)$ has the same asymptotic behavior as the BCS free energy (approximate minimizers). The precise statement is captured in the following theorem.
%Furthermore, the main contribution to the Cooper pair wave function $\alpha$ is given by a product wave function $\alpha_*(r) \Psi(X)$ provided the variational state $\Gamma$ has low BCS energy in the sense of \eqref{BCS_low_energy} and $T$ is sufficiently close to $\Tc$. In this case, we show that $\Psi$ has low Ginzburg--Landau energy, too.

\begin{bigthm}
\label{DHS1:Main_Result}
Let Assumptions \ref{DHS1:Assumption_V} and \ref{DHS1:Assumption_KTc} hold, let $D \in \mathbb{R}$, and let the coefficients $\Lambda_0, \Lambda_2, \Lambda_3 >0$ be given by \eqref{DHS1:GL-coefficient_1}-\eqref{DHS1:GL_coefficient_3} below. Then there are constants $C>0$ and $B_0 >0$ such that for all $0 < B \leq B_0$, we have
\begin{align}
F^{\mathrm{BCS}}(B,\, \Tc(1 - DB)) = B^2 \; \bigl( \EGLGSE + R \bigr), \label{DHS1:ENERGY_ASYMPTOTICS}
\end{align}
with $R$ satisfying the estimate
\begin{align}
CB \geq R \geq - \Rcal := -C B^{\nicefrac 1{12}}. \label{DHS1:Rcal_error_Definition}
\end{align}
%
Moreover, for any approximate minimizer $\Gamma$ of $\FBCS$ at $T = \Tc(1 - DB)$ in the sense that
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \leq B^2 \bigl( \EGLGSE + \rho\bigr) 
\label{DHS1:BCS_low_energy}
\end{align}
holds for some $\rho \geq 0$, we have the decomposition
\begin{align}
\alpha(X, r ) = \Psi(X) \, \alpha_*(r) + \sigma(X,r) \label{DHS1:Thm1_decomposition}
\end{align}
for the Cooper pair wave function $\alpha =\Gamma_{12}$. Here, $\sigma$ satisfies
\begin{align}
\frac{1}{|Q_B|} \int_{Q_B} \dd X \int_{\Rbb^3} \dd r \; |\sigma(X, r)|^2 &\leq C B^{\nicefrac {11}6}, \label{DHS1:Thm1_error_bound}
\end{align}
$\alpha_*$ is the normalized zero energy eigenstate of $K_{\Tc}-V$, and the function $\Psi$ obeys
\begin{align}
\EGL(\Psi) \leq \EGLGSE + \rho + \Rcal. \label{DHS1:GL-estimate_Psi}
\end{align}
\end{bigthm}

Our second main result concerns the shift of the BCS critical temperature that is caused by the external magnetic field. 
%The second result pertains the critical temperatures defined in \eqref{Upper_Critical_Temperature} and \eqref{Lower_Critical_Temperature}. We show that both critical temperatures converge to $\Tc$ and that they have equal slope determined by the Ginzburg--Landau model.

\begin{bigthm}
\label{DHS1:Main_Result_Tc} \label{DHS1:MAIN_RESULT_TC}
Let Assumptions \ref{DHS1:Assumption_V} and \ref{DHS1:Assumption_KTc} hold. Then there are constants $C>0$ and $B_0 >0$ such that for all $0 < B \leq B_0$ the following holds:
\begin{enumerate}[(a)]
	\item Let $0 < T_0 < \Tc$. If the temperature $T$ satisfies
	\begin{equation}
		T_0 \leq T \leq \Tc \, ( 1 - B \, ( \Dc + C \, B^{\nicefrac 1{2}}))
		\label{DHS1:eq:lowertemp}
	\end{equation}
	with $\Dc$ in \eqref{DHS1:Dc_Definition}, then we have
	\begin{equation*}
		F^{\mathrm{BCS}}(B,T) < 0.
	\end{equation*} 
	\item If the temperature $T$ satisfies
	\begin{equation}
		T \geq \Tc \, ( 1 - B \, ( \Dc - \Rcal ) )
		\label{DHS1:eq:uppertemp}
	\end{equation}
	with $\Dc$ in \eqref{DHS1:Dc_Definition} and $\Rcal$ in \eqref{DHS1:Rcal_error_Definition}, then we have
	\begin{equation*}
		\FBCS(\Gamma) - \FBCS(\Gamma_0) > 0
	\end{equation*}
	unless $\Gamma = \Gamma_0$.
\end{enumerate}
%, there are constants $B_0>0$ and $C>0$ such that for any $0 < B \leq B_0$ the critical temperatures satisfy
%\begin{align}
%-\Dc - CB^{\nicefrac 12} \leq \frac{\underline{\Tc(B)} - \Tc}{B\Tc} \leq \frac{\ov{\Tc(B)} - \Tc}{B\Tc} \leq -\Dc + \Rcal. \label{Critical_Temperature_Shift}
%\end{align}
%Here, $\Dcal_c$ is as in \eqref{Dc_Definition} and $\Rcal$ is as in \eqref{Rcal_error_Definition}.
\end{bigthm}

\begin{bems}
\label{DHS1:Remarks_Main_Result}
\begin{enumerate}[(a)]
	
\item Theorem~\ref{DHS1:Main_Result} and Theorem~\ref{DHS1:Main_Result_Tc} extend similar results in \cite[Theorem 1]{Hainzl2012} and \cite[Theorem~2.4]{Hainzl2014} to the case of a homogeneous magnetic field. Such a magnetic field has a non-periodic vector potential and a non-zero magnetic flux through the unit cell $Q_B$. The main reason why the problem with a homogeneous magnetic field is more complicated is that it cannot be treated as a perturbation of the Laplacian. More precisely, it was possible in \cite{Hainzl2012,Hainzl2014} to work with a priori bounds for low-energy states that only involve the Laplacian and not the external fields. As noticed in \cite{Hainzl2017}, see the discussion below Remark~6, this is not possible in the case of a homogeneous magnetic field. In the proof of comparable a priori estimates involving the homogeneous magnetic field, see Theorem~\ref{DHS1:Structure_of_almost_minimizers} below, we have to deal with the fact that the components of the magnetic momentum operator do not commute, which leads to significant technical difficulties.

\item If we compare Theorem~\ref{DHS1:Main_Result} to \cite[Theorem 1]{Hainzl2012} or Theorem~\ref{DHS1:Main_Result_Tc} to \cite[Theorem~2.4]{Hainzl2014} we note the following technical differences: (1) The parameter $h$ in \cite{Hainzl2012,Hainzl2014} equals $B^{\nicefrac 12}$ in our work. (2) We use microscopic coordinates while macroscopic coordinates are used in \cite{Hainzl2012,Hainzl2014}. (3) Our free energy is normalized by a volume factor, see \eqref{DHS1:Trace_per_unit_volume_definition} and \eqref{DHS1:BCS functional}. This is not the case in \cite{Hainzl2012,Hainzl2014}. (4) The leading order of the Cooper pair wave function in \cite[Theorem 1]{Hainzl2012} is of the form 
\begin{equation}
	\frac{1}{2} \alpha_*(x-y) (\Psi(x) + \Psi(y)).
	\label{DHS1:eq:remarksA1}
\end{equation}
This should be compared to \eqref{DHS1:Thm1_decomposition}, where relative and center-of-mass coordinates are used. Using the a priori bound for the $L^2$-norm of $\nabla \Psi$ below (5.61) in \cite{Hainzl2012}, one can see that \eqref{DHS1:eq:remarksA1} equals the first term in \eqref{DHS1:Thm1_decomposition} to leading order in $h$. The analogue in our setup does not seem to be correct.

\item The Ginzburg--Landau energy appears at the order $B^2$. This should be compared to the free energy of the normal state, which is of order $1$.

\item To appreciate the bound in \eqref{DHS1:Thm1_error_bound}, we note that the first term in the decomposition of $\alpha$ in \eqref{DHS1:Thm1_decomposition} obeys
\begin{align*}
	\frac{1}{|Q_B|} \int_{Q_B} \dd X \int_{\Rbb^3} \dd r \; | \Psi(X)\alpha_*(r) |^2 &= O(B).
\end{align*}

\item We stated Theorem~\ref{DHS1:Main_Result} with fixed $D\in \Rbb$. Our explicit error bounds show that $D$ is allowed to vary with $B$ as long as there is a $B$-independent constant $D_0>0$ such that $|D| \leq D_0$ holds. %In particular, the decomposition result \eqref{Thm1_decomposition} holds for more general temperatures $T$. For the sake of readability, we did not incorporate this into the statement of Theorem~\ref{Main_Result} here and refer the reader to Theorem \ref{Structure_of_almost_minimizers} for the details.
%\item From a physics point of view, the situation in Theorem~\ref{Main_Result} describes a type II superconductor above its second critical magnetic field, where the external magnetic field penetrates the superconductors bulk. \textcolor{red}{Polish and give reference.}
%\item The assumption that $V$ is a radial function is an important ingredient of our proof of the lower bound in \eqref{Energy_Asymptotics} and of Theorem~\ref{Main_Result_Tc}~(b). In these proofs we encounter operators of the form
%\begin{equation}
%	\int_{\mathbb{R}^3} \alpha_*^2(r) e^{ \i \Pi_X r/2} \mathrm{d} r,
%	\label{eq:Discussion1}
%\end{equation}
%with $\alpha_*$ in \eqref{alpha_star_ev-equation} and $\Pi_X = - \i \nabla_X + B \wedge X$ acting on $L_{\mathrm{mag}}^2(Q_B)$, the space of gauge-periodic square integrable functions on $Q_B$. Since $V$ is radial and Assumption~\ref{Assumption_KTc}~(b) holds, we know that $\alpha_*$ is radial. It is well-known that this implies that the operator \eqref{eq:Discussion1} is a function of $\Pi_X^2$, see e.g. \cite[Lemma~28]{Hainzl2017}, \cite[p.~66]{Folland} or Lemma~\ref{AAstar_Positive} below. This fact was used in \cite{Hainzl2017} and it is also used in our analysis. We expect that our results (with obvious adjustments) are still true if $V$ is not radial.
%Compare Theorem \ref{Main_Result} to \cite[Theorem 1]{Hainzl2012}, where the analogous problem was studied for the case of a bounded periodic magnetic potential. In contrast to this work, we normalized all energies to the unit volume, which removes dimensional dependencies. Furthermore, in \cite{Hainzl2012} it was not necessary to assume that $V$ is radial. Therefore, the coefficient $\Lambda_0$ (called $\mathbb B$ in \cite{Hainzl2012}) for the kinetic energy in the Ginzburg--Landau functional is a matrix with nonvanishing offdiagonal. By assuming radiality of $V\alpha_*$, the reader may recover $\Lambda_0$ as defined in \eqref{GL-coefficient_1}. This explains the slightly different looking results. The error estimate for $\sigma$ in \cite{Hainzl2012} (resized to unit volume) is $B^{\nicefrac 95}$ and the estimate for $\Rcal$ there is of the order $B^{\nicefrac 1{10}}$.

%It should be noted that the groundbreaking work \cite{Hainzl2012} greatly influences our strategy of proof from the global perspective, in particular pertaining the two-part structure of the lower bound to \eqref{Energy_Asymptotics} and the upper bound on \eqref{Critical_Temperature_Shift}. We appreciate to borrow various tediously obtained results from this paper in the scope of our proof. In particular, we make use of two powerful relative entropy inequalities \cite[Lemmas~1~\&~5]{Hainzl2012}.

%However, we also provide several considerable simplifications in comparison to the work \cite{Hainzl2012}. For example, we prove a new representation formula for the BCS functional, Proposition \ref{BCS functional_identity}, along with the fact that the relevant operator is weakly trace class, Lemma \ref{BCS functional_identity_Lemma}, whose proof we believe to be shorter and easier to understand than the corresponding result \cite{Hainzl2012}. We further note that the shape of the magnetic field treated in the present work leads to significant technical difficulties beyond \cite{Hainzl2012}, which in particular require a new approach to obtain the decomposition result Theorem \ref{Structure_of_almost_minimizers}. One of the main difficulties is that the components of the magnetic momentum do not commute, which makes it impossible to repeat the analysis as it is carried out in \cite[Lemma 3]{Hainzl2012}.

\item Theorem~\ref{DHS1:Main_Result_Tc} gives bounds on the range of temperatures where superconductivity is present, see \eqref{DHS1:eq:lowertemp}, or absent, see \eqref{DHS1:eq:uppertemp}. The interpretation of this theorem is that for small magnetic fields $B$ the critical temperature obeys the asymptotic expansion
\begin{equation}
	\Tc(B) = \Tc(1 - \Dc B) + o(B).
	\label{DHS1:eq:BemA1}
\end{equation}
We highlight that $\Tc$ is determined by the translation-invariant problem, and that $D_{\mathrm{c}}$ is given by the macroscopic (linearized) GL theory. The same result has been obtained in \cite[Theorem~4]{Hainzl2017} in the case of linearized BCS theory. Theorem~\ref{DHS1:Main_Result_Tc} can therefore be interpreted as a justification of this approximation. Eq.~\eqref{DHS1:eq:BemA1} allows us to compute the upper critical field $B_{c2}$. That is, the magnetic field, above which, for a given temperature $T$, superconductivity is absent. In particular, it allows us to compute the derivative of $B_{c2}$ with respect to $T$ at the critical temperature from the BCS functional. For more details we refer to \cite[Appendix~A]{Hainzl2017}. %In a limiting case the formulas reduce to the WHH theory, see \cite{La1990,La1991}. 

\item We expect that the assumption $0 < T_0 \leq T$ for some arbitrary but $B$-independent constant $T_0$ in Theorem~\ref{DHS1:Main_Result_Tc}~(a) is of technical nature. We need this assumption, which similarly appears in \cite[Theorem~4]{Hainzl2017}, because our trial state analysis in Section~\ref{DHS1:Upper_Bound} breaks down when the temperature $T$ approaches zero. This is related to the fact that the Fermi distribution function $f_T(x) = (\e^{x/T}+1)^{-1}$ cannot be represented by a Cauchy-integral uniformly in the temperature. We note that there is no such restriction in Theorem~\ref{DHS1:Main_Result_Tc}~(b). It is also not needed in \cite[Theorem~2.4]{Hainzl2014}.

%The assumption in part (1) that the temperature is bounded away from zero is probably technical. Note however, that our result is valid for arbitrarily small T1 > 0, as long as it is uniform in B. The reason for this restriction is that our expansions diverge as the temperature goes to zero. Remarkably, there is no such restriction in part (2) of the theorem.
%Theorem~\ref{Main_Result_Tc} should be compared with \cite[Theorem~2.4]{Hainzl2014} and \cite[Theorem~4]{Hainzl2017}.
%shows that to subleading order as $B \to 0$ the critical temperatures \eqref{Upper_Critical_Temperature} and \eqref{Lower_Critical_Temperature} indeed coincide and are equal to
%\begin{align}
%\Tc(B) := \Tc(1 - \Dc B). \label{Critical_Temperature_Shift_heuristic}
%\end{align}
%In particular, they converge to $\Tc$ and the magnetic field lowers the critical temperature below $\Tc$ by an amount of $-\Dc\Tc B$. This result was obtained in \cite{Hainzl2014} for the bounded periodic potential with the methods of \cite{Hainzl2012} and the same error bounds as remarked in part (b).

%\item In \cite{Hainzl2017}, this result has been obtained for the linearized BCS model with a weak homogeneous magnetic field like here, in all of $\Rbb^3$. There, the authors analyze the bottom of the spectrum of a certain linear operator $1 - V^{\nicefrac 12} L_{T,B} V^{\nicefrac 12}$. Since the setting is linear and $\Psi$ is thus assumed to be normalized, the error bounds obtained in \cite[Theorem 4]{Hainzl2017} differ from what we obtain in a natural way. The authors further point out connections to the so-called \emph{upper critical magnetic field} and how this result connects to the corresponding result in WHH theory in the limit $\beta_c\mu\to \infty$.

%In the present paper, the operator $L_{T,B}$ will arise rigorously as a certain linearization to the BCS functional. Thus, our result justifies the linearization in \cite{Hainzl2017} a posteriori. We put strong emphasis on the fact that we happily use many of the techniques that were developed in \cite{Hainzl2017}. In particular, we make use of the phase approximation method, which was first implemented to BCS theory in \cite{Hainzl2017}. This drives the energy calculation of the variational states $\Gamma_\Delta$ introduced in Section \ref{Upper_Bound}, even beyond the linear stage. Furthermore, many ideas that led to the decomposition result for $\alpha$ in \cite{Hainzl2017} also play a very important role here. Roughly speaking, our Theorem \ref{Structure_of_almost_minimizers} is an ``unbounded analogue'' of the decomposition result \cite[Theorem 22]{Hainzl2017}. 

%\item The proofs of the upper and lower bounds of \eqref{Energy_Asymptotics} and \eqref{Critical_Temperature_Shift} are related crosswise, which can be seen from the definitions \eqref{BCS GS-energy}, \eqref{Upper_Critical_Temperature}, and \eqref{Lower_Critical_Temperature}. In the following section, we provide a detailed explanation on the strategy of the proof of the individual bounds.

%For the upper bound on \eqref{Energy_Asymptotics} and the lower bound in \eqref{Critical_Temperature_Shift}, we are going to compute the energy of suitable variational states. Conversely, the method of proof for the lower bound on \eqref{Energy_Asymptotics} corresponds to the upper bound in \eqref{Critical_Temperature_Shift} and consists of a priori estimates on almost minimizers of the BCS functional.

%\item To leading order, \eqref{Energy_Asymptotics} decides whether the BCS model with external magnetic field is in a superconducting state or not. For, if $D >0$, then $T$ approaches the critical temperature $\Tc$ of the translation invariant model from below. In this case, $\EGLGSE < 0$, proving that $F^{\mathrm{BCS}}(B, \Tc(1-DB)) <0$ for $B$ small enough. Hence, the BCS model is in a superconducting state. If $D \leq 0$, then $\EGLGSE  =0$, which proves that $F^{\mathrm{BCS}}(B, \Tc(1 - DB))$ vanishes to leading order. Thus, the BCS model is in the normal state to leading order.

%\item Let us give a brief explanation of how to obtain the terms in the Ginzburg--Landau functional and of their order of magnitude. In \notiz{Noch nicht zu 100\% zufrieden. Soll erklären, warum sich das subleading behavior auf der Energieskala $B^{\nicefrac 12}$ abspielt...}absence of the magnetic field, the BCS energy of the normal state is a constant independent of $B$. When the magnetic field is present, the subleading correction to the normal state is taking place on the energy level $B^2$. This is driven by two effects. On the one hand, the energy perturbation due to the magnetic field is, roughly speaking, of order $B$ in the BCS functional. On the other hand, the temperature $T = \Tc(1 - DB)$ will approach $\Tc$ in such a way that the first variation of the entropy is canceled\notiz{Liegt an der Differenz, die wir nehmen}. This explains the second power of $B$ that is gained for the quadratic term in the Ginzburg--Landau functional in comparison to the normal state. 
%
%The center-of-mass coordinate of $\alpha$ displays the density of Cooper pairs $\Psi$ in the Ginzburg--Landau functional. It is no longer the constant function $1$ as opposed to the translation invariant case. However, $\Psi$ can be viewed as the reaction of the superconductor to the weak and slowly varying (even linear) external magnetic field. In the temperature regimes of Theorem \ref{Main_Result}, it is still a slowly varying quantity with flat gradient, which is fluctuating on the macroscopic energy scale $B$. Hence, this term is of the order $B^2$ compared to the normal state, too.
%
%As roughly explained in part (a), the quartic term in the Ginzburg--Landau functional is itself of the size $B$.

%\item When proving Theorem \ref{Main_Result}, we actually need and provide a finer decomposition of $\alpha$. \notiz{Woanders}The reason for this is that the calculation of the Ginzburg--Landau functional from the BCS functional needs an $H^2$-regularity on $\psi$. For the upper bound, we take a Ginzburg--Landau minimizer so that this condition is fulfilled. However, the lower bound forces us to employ an energy cut-off at energies of the order $B^{\nicefrac 13}$. The resulting explicit ``bad'' term in the decomposition satisfies a certain orthogonality condition but provides worse norm bounds. We defer the reader to Section XX for the precise result.
\end{enumerate}
\end{bems}

==> 1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1_Introduction_and_Main_Result.tex <==
%auto-ignore  % for ArXiv to process correctly

\section{Introduction and Main Results}

\input{../BCS-Theory_Duke/1_Introduction_and_Main_Result/1.1_Introduction}

\input{1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.2_Gauge-periodic_samples}

\input{1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.3_BCS-functional}

\input{../BCS-Theory_Duke/1_Introduction_and_Main_Result/1.4_Critical_temperature_of_BCS-functional}

\input{1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.5_Translation_Invariant_BCS-functional}

\input{../BCS-Theory_Duke/1_Introduction_and_Main_Result/1.6_Ginzburg-Landau_functional}

\input{1_BCS-Theory_in_a_weak_homogeneous_magnetic_field/1.7_Main_Results}

\input{../BCS-Theory_Duke/1_Introduction_and_Main_Result/1.8_Organization_of_paper}

==> 3_Decomposition_degenerate_case.tex <==
%auto-ignore  % for ArXiv to process correctly

\chapter{A decomposition result in the degenerate case}
\label{Chapter:Degenerate_Case}

\section{Setup and Main Result}

Let
\begin{align}
m = \dim \ker (K_\Tc - V)
\end{align}
and let 
\begin{align}
\alpha_* := (\alpha_*^{(1)}, \ldots, \alpha_*^{(m)}) \label{DEG:alpha_star_ev-equation}
\end{align}
be a fixed ONB of $\ker(K_\Tc - V)$. Accordingly,
\begin{align}
P := \sum_{i=1}^m |\alpha_*^{(i)} \rangle \langle \alpha_*^{(i)}| \label{DEG:Ground_state_projection}
\end{align}
is the orthogonal projection onto $\ker(K_\Tc - V)$. Let also 
\begin{align}
U := \e^{-\i \frac r2 \cdot P_X} \label{DEG:U_definition}
\end{align}
with $P_X := -\i \nabla_X$.

\begin{itemize}
\item Da muss man jetzt bissl aufpassen ob man $\alpha_*$ oder $\hat\alpha_*$ schreiben muss!
\end{itemize}


\begin{thm}
\label{DEG:Structure_of_almost_minimizers}
Let Assumptions \ref{DHS1:Assumption_V} and \ref{DHS1:Assumption_KTc} hold. For given $D_0, D_1 \geq 0$, there is a constant $h_0>0$ such that for all $0 <h \leq h_0$ the following holds: If the wave function $\alpha\in \Lsymm$ satisfies
\begin{align}
&\langle \alpha, [U(1 - P)(1 + p_r^2)(1 - P)U^* + U^*(1 - P)(1 + p_r^2)(1 - P)U] \alpha \rangle \notag\\
%
&\hspace{200pt} + \Tr\bigl[(\alpha^* \alpha)^2\bigr] \leq C h^2 \Vert \alpha\Vert_2^2 + D_1h^4, \label{DEG:Main_Result_Assumption}
\end{align}
then there are $\Psi\in \Hmag^1(Q_h)$ and $\xi\in \Hsymm$ such that
\begin{align}
\alpha(X,r) = \alpha_*(r)^t \Psi(X) + \xi(X,r), %\label{DHS1:Second_Decomposition_alpha_equation}
\end{align}
where
\begin{align}
\sup_{0< B\leq B_0} \Vert \alpha_*^t\Psi\Vert_{\Hsymm}^2 &\leq C, \notag \\
%
\Vert \xi\Vert_\Hsymm^2 &\leq CB^2 \bigl( \Vert \alpha_*^t \Psi\Vert_\Hsymm^2 + D_1\bigr). %\label{DHS1:Second_Decomposition_Psi_xi_estimate}
\end{align}
\end{thm}



\begin{lem}
\label{DEG:Schatten_estimate}
Let $B>0$, let $\Psi$ be a gauge-periodic function on $Q_h$ and let $\tau$ be an even and real-valued function on $\Rbb^3$. Moreover, let the operator $\alpha$ be defined via its integral kernel $\alpha(X,r) := \tau(r)\Psi(X)$, i.e., $\alpha$ acts as
\begin{align*}
\alpha f(x) &= \int_{\Rbb^3} \dd y \; \tau(x - y) \Psi\bigl(\frac{x+y}{2}\bigr) f(y), & f &\in L^2(\Rbb^3).
\end{align*}

\begin{enumerate}[(a)]
\item Let $p \in \{2,4,6\}$. If $\Psi\in \Lmag^p(Q_B)$ and $\tau \in L^{\frac {p}{p-1}}(\Rbb^3)$, then $\alpha \in \Scal^p$ and
\begin{align*}
\Vert \alpha\Vert_p \leq C \; \Vert \tau\Vert_{\frac{p}{p-1}} \; \Vert \Psi\Vert_p.
\end{align*}

\item For any $\nu > 3$, there is a $C_\nu >0$, independent of $B$, such that if $(1 +|\cdot|)^\nu \tau\in L^{\nicefrac 65}(\Rbb^3)$ and $\Psi\in \Lmag^6(Q_B)$, then $\alpha \in \Scal^\infty$ and
\begin{align*}
\Vert \alpha\Vert_\infty &\leq C_\nu \, B^{-\nicefrac 14} \; \max\{1 , B^{\nicefrac \nu 2}\} \; \Vert (1 + |\cdot|)^\nu \tau\Vert_{\nicefrac 65} \; \Vert \Psi\Vert_6.
\end{align*}
\end{enumerate}
\end{lem}

\begin{proof}
The case $p = 2$ of part (a) holds trivially with $C = 1$. Since $\tau$ is even and real-valued, the kernel of $\alpha^*\alpha$ is given by
\begin{align*}
\alpha^* \alpha(x,y) &= \int_{\Rbb^3} \dd z \; \tau(x-z) \ov{\Psi\bigl( \frac{x+z}{2}\bigr)} \tau(z - y) \Psi\bigl( \frac{z+y}{2}\bigr).
\end{align*}
Using $\Vert \alpha\Vert_4^4 = \Vert \alpha^* \alpha\Vert_2^2$ and the change of variables $z \mapsto x-z$ and $y \mapsto x-y$, we see that
\begin{align*}
\Vert \alpha\Vert_4^4 &= \frac{1}{|Q_B|} \iint_{Q_B\times \Rbb^3} \dx \dy \; \Bigl| \int_{\Rbb^3} \dd z \; \tau(z) \, \tau(y-z) \,  \ov{\Psi\bigl( x - \frac z2\bigr)}\, \Psi\bigl( x-\frac{y+z}{2}\bigr)\Bigr|^2.
\end{align*}
By Hölder's inequality, Young's inequality and 
%Expanding the square, pulling the modulus inside the integral, and using 
the fact that $|\Psi|$ is periodic, we see that
\begin{align*}
\Vert \alpha\Vert_4^4 &\leq \Vert \Psi\Vert_4^4 \; \int_{\Rbb^3} \dd y \, \Bigl| \int_{\Rbb^3} \dd z \; |\tau(z) \tau(y-z)|\Bigr|^2 \leq C  \; \Vert \tau\Vert_{\nicefrac 43}^4\; \Vert \Psi\Vert_4^4
\end{align*}
holds. This proves part (a) for $p =4$. If $p =6$ we use $\Vert \alpha\Vert_6^6 = \Vert \alpha \,\alpha^*\alpha\Vert_2^2$ and a similar change of variables to write
\begin{align*}
\Vert \alpha \alpha^* \alpha\Vert_2^2 &= \frac{1}{|Q_B|} \iint_{Q_B\times \Rbb^3} \dd x \dd y\; \Bigl| \iint_{\Rbb^3\times \Rbb^3} \dd z_1 \dd z_2 \; \tau(z_1) \, \tau(z_2 - z_1) \, \tau(y - z_2) \mathop \times \\
%
&\hspace{120pt} \times \Psi\bigl(x - \frac{z_1}{2}\bigr) \ov{ \Psi\bigl( x - \frac{x_1+ z_2}{2}\bigr)} \Psi\bigl( x - \frac{z_2 + y}{2}\bigr)\Bigr|^2.
\end{align*}
We thus obtain $\Vert \alpha\Vert_6^6 \leq \Vert \Psi\Vert_6^6 \; \Vert \tau * \tau * \tau \Vert_2^2$, which, in combination with Young's inequality, proves the claimed bound.

In case of part (b), we follow closely the strategy of the proof of \cite[Eq. (5.51)]{Hainzl2012}. Let $f,g\in L^2(\Rbb^3)$ and let $\chi_j$ denote the characteristic function of the cube with side length $\sqrt{2\pi B^{-1}}$ centered at $j\in \Lambda_B$. We estimate
\begin{align}
|\langle f, \alpha g\rangle| &\leq \sum_{j,k\in \Lambda_B}\iint_{\Rbb^3\times \Rbb^3} \dd x\dd y\; \bigl|\chi_j(x) f(x) \Psi\bigl( \frac{x+y}{2}\bigr) \tau(x - y)\chi_k(y)g(y)\bigr|. \label{DEG:Schatten_estimate_1}
\end{align}
Let $|\cdot|_\infty$ and $| \cdot |$ denote the maximum norm and the euclidean norm on $\Rbb^3$, respectively. We observe that the estimates $|x - j|_\infty \leq \frac 12\sqrt{2\pi B^{-1}}$ and $|y - k|_\infty \leq \frac 12\sqrt{2\pi B^{-1}}$ imply $| \frac{x + y}{2} - \frac{j + k}{2}|_\infty \leq \frac 12\sqrt{2\pi B^{-1}}$. Accordingly, if $\chi_j(x)\chi_k(y)$ equals $1$, so does $\chi_{\frac{j+k}{2}}(\frac{x+y}{2})$ and we may replace $\Psi$ on the right side of \eqref{Schatten_estimate_1} by $\chi_{\frac{j+k}{2}}\Psi$ without changing the term. The above bounds for $|x - j|_\infty$ and $|y - k|_\infty$ also imply $|j - k| \leq |x - y| + \sqrt{6\pi B^{-1}}$, which yields the lower bound
\begin{align}
|x - y| \geq \bigl[ |j -k| - \sqrt{6\pi B^{-1}}\bigr]_+. \label{DEG:Schatten_estimate_2}
\end{align}
We choose $\nu >3$, insert the factor $(\sqrt{2\pi B^{-1}} + |x-y|)^\nu$ and its inverse in \eqref{Schatten_estimate_1}, use \eqref{Schatten_estimate_2} to estimate the inverse, apply Cauchy--Schwarz in the $x$-coordinate, and obtain
\begin{align*}
|\langle f, \alpha g\rangle| &\leq \sum_{j,k\in \Lambda_B} \bigl( \sqrt{2\pi B^{-1}} + \bigl[|j-k| - \sqrt{6\pi B^{-1}}\bigr]_+\bigr)^{-\nu} \; \Vert \chi_jf\Vert_2 \mathop \times \\
%
&\hspace{-20pt} \times \Bigl( \int_{\Rbb^3} \dd x \, \Bigl| \int_{\Rbb^3} \dd y\; \bigl| (\chi_{\frac{j+k}{2}} \Psi)\bigl( \frac{x+y}{2}\bigr) \bigl( \sqrt{2\pi B^{-1}} + |x-y| \bigr)^\nu \tau(x-y) \chi_k(y)g(y)\bigr| \; \Bigr|^2\Bigr)^{\nicefrac 12}.
\end{align*}
%Then
%\begin{align*}
%\int_{\Rbb^3} \dd x\; \Bigl|\int_{\Rbb^3} \dd y \; \bigl| \chi_{\frac{j+k}{2}}\bigl( \frac{x+y}{2}\bigr) \Psi\bigl( \frac{x+y}{2}\bigr) \bigl( \frac{\sqrt{2\pi}}{\sqrt{B}} + |x-y|\bigr)^\nu \tau(x-y) \chi_k(y)g(y)\bigr|\; \Bigr|^2 &\\
%%
%&\hspace{-200pt}\leq \Vert \Psi\Vert_{L^6(Q_B)} \; \Bigl\Vert \bigl|(1 + |\cdot|)^\nu \tau \bigr|^{\nicefrac 65} * |\chi_kg|^{\nicefrac 65} \Bigr\Vert_{L^{\nicefrac 53}(\Rbb^3)}^{\nicefrac 53}
%\end{align*}
An application of Hölder's inequality in the $y$-coordinate shows that the second line is bounded by 
\begin{align*}
\Bigl\Vert \bigl|(\sqrt{2\pi B^{-1}} + |\cdot|)^\nu \tau \bigr|^{\nicefrac 65} * |\chi_kg|^{\nicefrac 65} \Bigr\Vert_{\nicefrac 53}^{\nicefrac 56} &\leq \bigl\Vert \bigl( \sqrt{2\pi B^{-1}} + |\cdot| \bigr)^\nu  \tau \bigr\Vert_{\nicefrac 65} \, \Vert \chi_kg \Vert_{2} %\\
%
%&= \bigl\Vert ( 1 + |\cdot|)^\nu \tau \bigr\Vert_{L^{\nicefrac 65}(\Rbb^3)}^2 \cdot \Vert \chi_kg\Vert_{L^2(\Rbb^3)}^2.
\end{align*}
times $|Q_B|^{\nicefrac 16} \Vert \Psi\Vert_{\Lmag^6(Q_B)}$. We highlight that the $\Lmag^6(Q_B)$-norm is defined via a normalized integral, whence we needed to insert the factor of $|Q_B|^{-\nicefrac 16}$ manually. 
%\notiz{We give more details here to see where the $L^2$-norm comes from with $g$}Applying Hölder in $y$ with $p = 6$ and $q = \nicefrac 65$ and Young's inequality to this,
Hence,
\begin{align*}
|\langle f, \alpha g\rangle| &\leq C B^{-\nicefrac 14} \, \Vert \Psi\Vert_6 \, \bigl\Vert \bigl( \sqrt{2\pi B^{-1}}  + |\cdot|\bigr)^\nu \tau\bigr\Vert_{\nicefrac 65}\mathop \times \\
%
&\hspace{50pt} \times \sum_{j,k\in \Lambda_B} \bigl( \sqrt{2\pi B^{-1}} + \bigl[ |j -k| - \sqrt{6\pi B^{-1}} \bigr]_+\bigr)^{-\nu} \; \Vert \chi_jf\Vert_2 \; \Vert \chi_kg\Vert_2 .
\end{align*}
For $\lambda >0$ we estimate $\Vert \chi_j f\Vert_2 \Vert \chi_k g\Vert_2 \leq \frac{\lambda}{2} \Vert \chi_j f\Vert_2^2 + \frac{1}{2 \lambda} \Vert \chi_kg\Vert_2^2$. In each term, we carry out one of the sums and optimize the resulting expression over $\lambda$. We find $\lambda = \Vert g\Vert_2 \; \Vert f\Vert_2^{-1}$ as well as
\begin{align*}
|\langle f, \alpha g\rangle| &\leq C B^{-\nicefrac 14}  \Vert f\Vert_2 \; \Vert g\Vert_2 \; \Vert \Psi\Vert_6 \; \frac{\Vert ( \sqrt{2\pi B^{-1}} +|\cdot|)^\nu \tau\Vert_{\nicefrac 65}}{(2\pi B^{-1})^{\nicefrac \nu 2}} \; \sum_{j\in \Zbb^3} \bigl( 1 + [ |j| - \sqrt{3}]_+\bigr)^{-\nu}.
\end{align*}
The fraction involving $\tau$ is bounded by $C_\nu\max\{1, B^{\nicefrac \nu 2}\} \Vert (1 + |\cdot|)^\nu \tau \Vert_{\nicefrac 65}$. This proves the claim.
\end{proof}



%\input{3_Decomposition_degenerate_case/5.1_A_priori_estimates}

\input{3_Decomposition_degenerate_case/5.2_First_decomposition_result}

\input{3_Decomposition_degenerate_case/5.3_Uniform_bound_on_Psi}

\input{3_Decomposition_degenerate_case/5.4_Proof_of_Thm_5.1}


\section{A comment on the nonzero-flux-case}






We decompose $L^2(\Rbb^3)$ into angular momentum sectors. To do this, we need the spherical harmonics, see \cite{FraLe2016},
\begin{align}
Y_\ell^m(\theta, \varphi) := \sqrt{\frac{(2\ell + 1)}{4\pi} \frac{(\ell - m)!}{(\ell + m)!}} \; P_\ell^m (\cos \theta) \e^{\i m \varphi},
\end{align}
where $P_\ell^m$ is the associated Legendre polynomial. Real-valued spherical harmonics:
\begin{align}
\Ycal_\ell^m := \begin{cases} \frac{\i}{\sqrt{2}} (Y_\ell^m - (-1)^m Y_\ell^{-m}), & m< 0, \\ Y_0^0, & m = 0, \\ \frac{1}{\sqrt{2}} (Y_\ell^m + (-1)^m Y_\ell^{-m}), & m >0. \end{cases}
\end{align}
Let $\Scal_\ell := \spano\{ Y_\ell^m : m = -\ell, \ldots, \ell\}$ and define
\begin{align}
\Hcal_\ell := L^2(\Rbb_+ ; r^2\dr) \otimes \Scal_\ell,
\end{align}
where $r = |x|$. Then, we have the orthogonal decomposition
\begin{align}
L^2(\Rbb^3) = \bigoplus_{\ell=0}^\infty \Hcal_\ell.
\end{align}

Since $V$ is a radial function, it follows that $K_\Tc - V$ leaves this decomposition invariant. 

\begin{asmp}
We assume that $\ker (K_{\Tc} - V) = \Hcal_\ell$ for some $\ell\in \Nbb_0$.
\end{asmp}

In particular, we have
\begin{align*}
\dim \ker K_{\Tc} - V = 2\ell + 1
\end{align*}
and we may fix an arbitary ONB $\alpha_*^{(-\ell)} , \ldots,\alpha_*^{(\ell)}$ of $\ker K_{\Tc} - V$ such that
\begin{align}
K_\Tc \alpha_*^{(m)}  &= V \alpha_*^{(m)} & m &= -\ell , \ldots, \ell. \label{DEG:alpha_star_ev_equation}
\end{align}
Since $\ov {\alpha_*^{(m)} }$ is a solution of \eqref{alpha_star_ev_equation}, we may assume that $\alpha_*^{(m)}$ is real-valued. We normalize such that $\Vert \alpha_*^{(m)}\Vert_{L^2(\Rbb^3)} = 1$.







\section{Arbitrary Angular Momentum Sectors}


Set $n := \dim \ker (K_\Tc - V)$ and choose an ONB $\alpha_*^{(1)} , \ldots, \alpha_*^{(n)} \in \ker(K_\Tc - V)$. Set
\begin{align}
\alpha_* := (\alpha_*^{(1)} , \ldots, \alpha_*^{(n)})^t.
\end{align}
Assume we have the operator
\begin{align*}
R := \int_{\Rbb^3} \dd r \; \ov{\alpha_*(r)} \alpha_*(r)^t \, \cos( r\cdot \Pi)
\end{align*}
whose components are
\begin{align}
R^{(i,j)} := \int_{\Rbb^3} \dd r \; \ov{\alpha_*^{(i)}(r)} \alpha_*^{(j)}(r) \, \cos (r\cdot \Pi).
\end{align}

%Then, since $\ov{\alpha_*} \alpha_*^t$ is a Hermitian matrix, there is a $U \in \Cbb^{n\times n}$ such that
%\begin{align}
%\ov{\alpha_*} \alpha_*^t = U^* \; \diag \bigl( |\alpha_*^{(1)}|^2\;  , \ldots, \; |\alpha_*^{(n)}|^2\bigr)  \; U.
%\end{align}
%Thus, we define
%\begin{align}
%R^{(i)} &:= \int_{\Rbb^3} \dd r \; |\alpha_*^{(i)}(r) |^2 \; \cos(r\cdot\Pi) & i &= 1,\ldots, n
%\end{align}
%and obtain
%\begin{align}
%U R U^* = \diag \bigl( R^{(1)} , \ldots, R^{(n)} \bigr).
%\end{align}

\subsection*{Decomposition in Spherical harmonics}

Now, in terms of the spherical coordinates $\rho > 0$, $\theta\in (0,\pi)$ and $\varphi\in (0,2\pi)$, we have the decomposition
\begin{align}
\alpha_*^{(i)} (\rho, \theta, \varphi) = \sum_{\ell =0}^\infty \sum_{m = -\ell}^\ell \alpha_*^{(i , \mathrm{rad})}(\ell, m; \rho)\; Y_m^\ell(\theta, \varphi)
\end{align}
where $\alpha_*^{(i, \mathrm{rad})}$ is a radial function and $Y_m^\ell$ are the spherical harmonics
\begin{align}
Y_m^\ell(\theta, \varphi) =\frac{1}{\sqrt{2\pi}} \;  N_{\ell, m} \; P_{\ell, m}(\cos \theta) \; \e^{\i m\varphi}
\end{align}
with $P_{\ell, m}$ the associated Legendre polynomial and the normalization constant
\begin{align*}
N_{\ell, m} = \sqrt{\frac{2\ell + 1}{2} \frac{(\ell - m)!}{(\ell + m)!}}.
\end{align*}

\subsection*{Decomposition of $R^{(i,j)}$}

In terms of the spherical harmonics, we have
\begin{align}
R^{(i,j)} &= \sum_{\ell, \ell' =0}^\infty \sum_{m = -\ell}^\ell \sum_{m' = -\ell'}^{\ell'} \int_0^\infty \dd \rho \; \rho^2 \, \ov{\alpha_*^{(i, \mathrm{rad})}(\ell, m;\rho)}\;  \alpha_*^{(i, \mathrm{rad})}(\ell', m'; \rho) \notag \\
%
&\hspace{100pt} \times \int_0^\pi \dd \theta \; \sin \theta \int_0^{2\pi} \dd \varphi \; \ov{Y_m^\ell (\theta, \varphi)} \, Y_{m'}^{\ell'} (\theta, \varphi)\; \e^{\i \rho \omega \cdot \Pi},
\end{align}
where
\begin{align}
\omega = \begin{pmatrix} \sin \theta \cos \varphi \\ \sin \theta \sin \varphi \\ \cos \theta \end{pmatrix}.
\end{align}

\subsection*{Creation and annihilation operators}

Now with the creation and annihilation operators
\begin{align*}
a &= \frac{1}{2\sqrt{B}} (\Pi^{(1)} - \i \Pi^{(2)}) , & a^* &= \frac{1}{2\sqrt{B}} (\Pi^{(1)} + \i \Pi^{(2)}),
\end{align*}
we have $[a, a^*] = 1$ and
\begin{align*}
\Pi^{(1)} &= \sqrt{B} \, (a + a^*) & \Pi^{(2)} &= \i \sqrt{B} \, ( a - a^*).
\end{align*}
and
\begin{align*}
\e^{\i \rho \omega \cdot\Pi} &= \e^{\i \rho \cos\theta \Pi^{(3)}} \; \e^{\i \rho \sqrt{B} \sin \theta \cos \varphi (a + a^*) - \rho\sqrt{B} \sin\theta \sin \varphi (a - a^*)} \\
%
&= \e^{\i \rho \cos \theta \Pi^{(3)}} \; \e^{\i \rho \sqrt B \sin \theta (\e^{-\i \varphi} a^* + \e^{\i \varphi} a)}.
\end{align*}
With the Baker-Campbell-Hausdorff formula $\e^{X+Y} = \e^X \e^Y\e^{-\frac 12 [X, Y]}$, we get 
\begin{align*}
\e^{\i \rho \sqrt B \sin \theta (\e^{-\i \varphi} a^* + \e^{\i \varphi} a)} &= \e^{-\frac 12 \rho^2 B \sin^2\theta} \e^{\i \rho \sqrt{B} \sin \theta \e^{-\i\varphi} a^*} \e^{\i \rho \sqrt{B} \sin \theta \e^{\i \varphi} a} \\
%
&= \e^{-\frac 12 \rho^2 B \sin^2\theta} \sum_{n, n'=0}^\infty \frac{(\i \rho \sqrt{B} \sin\theta)^{n+n'}}{n!(n')!} (a^*)^n a^{n'} \; \e^{\i \varphi(n' -n)}
\end{align*}
We define
\begin{align}
R_{m,m'}^{\ell, \ell'}(\rho) &:= \int_0^\pi \dd\theta \; \sin \theta \int_0^{2\pi} \dd \varphi \; \ov{Y_m^\ell (\theta, \varphi)}\,  Y_{m'}^{\ell'} (\theta, \varphi)\notag  \\
%
&\hspace{50pt}\e^{-\frac 12 \rho^2 B \sin \theta} \sum_{n, n'=0}^\infty \frac{(\i \rho \sqrt{B} \sin\theta)^{n+n'}}{n!(n')!} (a^*)^n a^{n'} \; \e^{\i \varphi(n' -n)}
\end{align}
Then
\begin{align}
R^{(i,j)} = \sum_{\ell, \ell' =0}^\infty \sum_{m = -\ell}^\ell \sum_{m' = -\ell'}^{\ell'} \int_0^\infty \dd \rho \; \rho^2 \, \ov{\alpha_*^{(i, \mathrm{rad})}(\ell, m;\rho)} \; \alpha_*^{(j, \mathrm{rad})}(\ell', m'; \rho) \; \e^{\i \rho \cos \theta \Pi^{(3)}} \; R_{m,m'}^{\ell, \ell'}(\rho)
\end{align}

\subsection*{Analysis of $R_{m,m'}^{\ell, \ell'}(\rho)$}

Now use the form of the spherical harmonics to get
\begin{align*}
R_{m,m'}^{\ell, \ell'}(\rho) &= N_{\ell, m}^2 \int_0^{\pi} \dd \theta \; \sin\theta \, P_{\ell, m}(\cos \theta ) \, P_{\ell', m'}(\cos \theta) \; \e^{-\frac 12 \rho^2 B\sin \theta} \\%
%
&\hspace{50pt} \times \sum_{n,n'=0}^\infty \frac{(\i\rho \sqrt B \sin \theta)^{n+n'}}{n! (n')!} (a^*)^n a^{n'} \; \underbrace{\frac{1}{2\pi} \int_0^{2\pi} \dd \varphi \; \e^{\i (n' - n)\varphi} \e^{\i (m'- m)\varphi}}_{= \delta_{n+m, n'+m'} = \delta_{0, n'-n + m'-m}}
\end{align*}

\subsubsection*{Case $m'\geq m$}

In this case $n = n' + m' -m \geq m' - m \geq 0$. Hence
\begin{align*}
\sum_{n,n'=0}^\infty \frac{(\i\rho \sqrt B \sin \theta)^{n+n'}}{n! (n')!} (a^*)^n a^{n'} \; \delta_{0, n' -n + m' -m} = \sum_{n'=0}^\infty \frac{(\i \rho \sqrt{B} \sin \theta)^{2n' + m' - m}}{(n' + m' - m)! (n')!}  (a^*)^{n' + m' - m} a^{n'}
\end{align*}
Let $(a^*)^k (b^*)^p |0\rangle$ denote a basis of the $k$\tho\ Landau level $P_{2B}^{(k)}$. Then
\begin{align*}
(a^*)^{n+m'-m} a^n (a^*)^k (b^*)^p|0\rangle &= \begin{cases}
\frac{k!}{(k-n)!}  (a^*)^{k+ m' -m} (b^*)^p|0\rangle & n \leq k \\ 0 & \text{otherwise}
\end{cases}
\end{align*}
Hence, in this case
\begin{align*}
R_{m,m'}^{\ell, \ell'}(\rho) P_{2B}^{(k)} &= N_{\ell, m}^2 \int_0^{\pi} \dd \theta\; \sin \theta \; P_{\ell, m}(\cos\theta ) \, P_{\ell', m'}(\cos \theta) \; \e^{-\frac 12 \rho^2 B \sin\theta} \\
%
&\hspace{50pt} \times (\i \rho \sqrt{B} \sin \theta)^{m'- m} \sum_{n=0}^k \frac{(-\rho^2 B \sin \theta)^n}{(n+ m' - m)!} \binom kn \quad P_{2B}^{(k+m'-m)}
\end{align*}

\subsubsection*{Case $m' \leq m$}

In this case $n' = n + m - m' \geq m - m' \geq 0$. Hence
\begin{align*}
\sum_{n,n'=0}^\infty \frac{(\i\rho \sqrt B \sin \theta)^{n+n'}}{n! (n')!} (a^*)^n a^{n'} \; \delta_{0, n' -n + m' -m} = \sum_{n=0}^\infty \frac{(\i \rho \sqrt{B} \sin \theta)^{2n+m-m'}}{n! (n +m-m')!} (a^*)^n a^{n+m-m'}
\end{align*}
Likewise, we have
\begin{align*}
(a^*)^n a^{n+m-m} (a^*)^k (b^*)^p |0\rangle &\\
%
&\hspace{-80pt} = \begin{cases}
\frac{k!}{(k - (n+m-m'))!} (a^*)^n (a^*)^{k - (n+ m-m')} (b^*)^p |0\rangle & k \geq n + m - m' \\ 0 & \text{otherwise}
\end{cases}
\end{align*}
Hence, in this case
\begin{align*}
R_{m,m'}^{\ell, \ell'}(\rho) P_{2B}^{(k)} &= N_{\ell, m}^2 \int_0^{\pi} \dd \theta\; \sin \theta \; P_{\ell, m}(\cos\theta )\,  P_{\ell', m'}(\cos \theta)\; \e^{-\frac 12 \rho^2 B \sin\theta} \\
%
&\hspace{50pt} (\i \rho \sqrt{B} \sin \theta)^{m-m'} \sum_{n=0}^k \frac{(-\rho^2 B \sin \theta)^n}{n!} \binom{k}{n+m-m'} \quad P_{2B}^{(k-m+m')}
\end{align*}


\subsubsection*{Summary}

We obtain
\begin{align*}
R_{m,m'}^{\ell, \ell'}(\rho) P_{2B}^{(k)} &= N_{\ell, m}^2 (-\i \rho \sqrt{B})^{|m-m'|} \\
%
&\hspace{-30pt} \times \int_0^{\pi} \dd \theta\; (\sin \theta)^{1+|m-m'|} \; P_{\ell, m}(\cos\theta ) P_{\ell', m'}(\cos \theta) \e^{-\frac 12 \rho^2 B \sin\theta} \; P_{2B}^{(k-m+m')}\\
%
&\hspace{-30pt} \times \begin{cases}
\sum_{n=0}^k \frac{(-\rho^2 B \sin \theta)^n}{n!} \binom{k}{n+m-m'} & m'\geq m \\
%
\sum_{n=0}^k \frac{(-\rho^2 B \sin \theta)^n}{(n+ m' - m)!} \binom kn & m'\leq m
\end{cases}
\end{align*}

By index-shifting and summarizing, we thus obtain ($\underline m := \min \{m, m'\}$)
\begin{align*}
R_{m,m'}^{\ell, \ell'}(\rho) P_{2B}^{(k)} &= N_{\ell, m}^2 \; (-\i \rho \sqrt{B})^{|m-m'|} \\
%
&\hspace{30pt}\times \int_0^{\pi} \dd \theta\; (\sin \theta)^{1+|m-m'|} \; P_{\ell, m}(\cos\theta ) P_{\ell', m'}(\cos \theta)\; \e^{-\frac 12 \rho^2 B \sin\theta}  \\
%
&\hspace{30pt} \times \sum_{p = -\underline m}^{k - \underline m} \frac{(-\rho^2 B\sin^2\theta)^{p + \underline m}}{(p+ m')!} \binom k{p+m} \quad P_{2B}^{(k-m+m')}
\end{align*}














==> 3_Decomposition_degenerate_case/5.1_A_priori_estimates.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{A lower bound for the BCS functional}

We start the proof of Theorem \ref{Structure_of_almost_minimizers} with the following lower bound on the BCS functional.

%by writing the BCS functional as
%\begin{align*}
%\FBCS(\Gamma) - \FBCS(\Gamma_0) = \frac{T}{2} \Hcal_0(\Gamma, \Gamma_0) - \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; V(r) \, |\alpha(X,r)|^2
%\end{align*}
%with the relative entropy $\Hcal_0(\Gamma, \Gamma_0)$ in \eqref{Relative_Entropy} and the normal state $\Gamma_0$ in \eqref{Gamma0}. 

\begin{lem}
Let $\Gamma_0$ be the normal state in \eqref{Gamma0}. We have the lower bound
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \geq  \Tr\bigl[ (K_{T,\Abold, W} - V) \alpha  \alpha^*\bigr] + \frac{4T}{5} \Tr\bigl[ (\alpha^* \alpha)^2\bigr], \label{Lower_Bound_A_3}
\end{align}
where
\begin{align*}
K_{T, \Abold, W} = \frac{(-\i \nabla + \Abold_h)^2 + W_h- \mu}{\tanh (\frac{(-\i \nabla + \Abold_h)^2 + W_h - \mu}{2T})}
\end{align*}
$V\alpha(x,y) = V(x-y) \alpha(x,y)$.
\end{lem}

\begin{proof}
The statement follows from Eqs.~(5.3)--(5.12) in \cite{Hainzl2012} with the evident replacements. The argument uses the relative entropy inequality \cite[Lemma~1]{Hainzl2012}, which is a refinement of the bound \cite[Theorem~1]{Hainzl2008_Lewin}.
\end{proof}

In Proposition \ref{KTV_Asymptotics_of_EV_and_EF} in Appendix~\ref{KTV_Asymptotics_of_EV_and_EF_Section} we show that the magnetic field can lower the lowest eigenvalue zero of $K_{\Tc} - V$
%, which is equal to zero by assumption, 
at most by a constant times $B$. This information is used in the following lemma to bound $K_{T,B} - V$ from below by a nonnegative operator, up to a correction of the size $CB$. The inequality \eqref{KTB_Lower_bound_eq} below is stated for $K_{T,B} - V$ as a one-particle operator but it holds equally for the operator $K_{T,B} - V(x-y)$ in \eqref{Lower_Bound_A_3} because $V$ intertwines as $T(y)^* V(x) T(y) = V(x-y)$ with the magnetic translations $T(y)$ in \eqref{Magnetic_Translation}.

\textcolor{red}{Hier muss jetzt zusätzlich $W$ entfernt werden (à la 2012). Für $A$ kann man die Störungstheorie wiederholen und es dann aus $\pi_A^2$ entfernen durch simples abschätzen}

\begin{lem}
\label{KTB_Lower_bound}
Let Assumptions \ref{Assumption_V} and \ref{Assumption_KTc} be true.
%and let $U$ be as in \eqref{U_definition}. 
For any $D_0 \geq 0$, there are constants $B_0>0$ and $T_0>0$ such that for $0< B\leq B_0$ and $T>0$ with $T - \Tc \geq -D_0B$, the estimate
\begin{align}
%U^* (K_{T, B}^r - V) U + U(K_{T,B}^r - V) U^* & \notag\\
%%
%&\hspace{-165pt} \geq c \; \bigl[ U (1 - P) (1 + \pi_r^2) (1- P)U^* + U^* (1 - P)(1 + \pi_r^2) (1 - P) U\bigr] + c \; (T - \Tc)_+ - CB. \label{KTB_Lower_bound_eq}
K_{T, B} - V &\geq c \; (1 - P) (1 + \pi^2) (1- P) + c \, \min \{ T_0, (T - \Tc)_+\} - CB \label{KTB_Lower_bound_eq}
\end{align}
holds. Here, $P = |\alpha_*\rangle\langle \alpha_*|$ is the orthogonal projection onto the ground state $\alpha_*$ of $K_{\Tc} - V$.
\end{lem}

\begin{proof}
We prove two lower bounds on $K_{T,B} - V$, which we add up to etablish \eqref{KTB_Lower_bound_eq}.

\emph{Step 1.} We claim that there are $T_0, c, C >0$ such that
\begin{align}
K_{T,B} - V \geq c \; \min \{ T_0, (T - \Tc)_+\} - CB. \label{KTB_Lower_bound_5}
\end{align}
To prove \eqref{KTB_Lower_bound_5}, we note that the derivative of the symbol $K_T$ in \eqref{KT-symbol} with respect to $T$ equals
\begin{align}
\frac{\dd}{\dd T} K_T(p) = 2\;  \frac{( \frac{p^2 - \mu}{2T})^2}{\sinh^2(\frac{p^2-\mu}{2T})} \label{KTc_bounded_derivative}
\end{align}
%$2\, f(\frac \beta 2(p^2-\mu))$ with the function $f(x) = \frac{x^2}{\sinh^2(x)}$. 
and is bounded from above by 2. If $T \leq \Tc$, we infer $K_{T,B} - K_{\Tc,B} \geq -2D_0B$ as an operator inequality, which, in combination with Proposition~\ref{KTV_Asymptotics_of_EV_and_EF} in the appendix,  proves \eqref{KTB_Lower_bound_5} in this case. To treat the case $T \geq \Tc$, we denote by $e_0^{T,B}$ and $e_1^{T,B}$ the lowest and the second lowest eigenvalue of the operator $K_{T,B} - V$, respectively. Also let $P_{T,B}$ be the spectral projection corresponding to $e_0^{T,B}$ and define $Q_{T,B} = 1 - P_{T,B}$. We have 
\begin{align*}
	K_{T,B} - V \geq e_0^{T,B} P_{T,B} + e_{1}^{T,B} Q_{T,B}.
\end{align*}
Since $K_T(p) - K_{\Tc}(p) \geq 0$ for all $p \in \mathbb{R}^3$, which follows from \eqref{KTc_bounded_derivative}, we know the lower bound $e_{1}^{T,B} \geq e_{1}^{\Tc,B} \geq \kappa$ for some $\kappa > 0$. Here, the second inequality follows from Proposition~\ref{KTV_Asymptotics_of_EV_and_EF}. From Proposition~\ref{KTV_Asymptotics_of_EV_and_EF} we also know that the lowest eigenvalue of $K_{T,B} - V $ is simple. According to \eqref{KTc_bounded_derivative}, the function $T \mapsto K_T(p)$ is increasing and has a non-vanishing derivative for each $p \in \mathbb{R}^3$. Analytic perturbation theory therefore implies the lower bound $e_0^{T,B} \geq e_0^{\Tc,B} + c (T - \Tc)$ for some $c > 0$ as long as $|T - \Tc |$ is small enough. Since Proposition~\ref{KTV_Asymptotics_of_EV_and_EF} shows $e_0^{\Tc,B} \geq -CB$ these consideration prove \eqref{KTB_Lower_bound_5} in the case $T \geq \Tc$.
%If on the other hand $T \geq \Tc$, then choose $T_0 := \frac \kappa 3$, where $\kappa >0$ denotes the spectral gap of the operator $K_{\Tc,B} - V$ above its lowest eigenvalue $e_0^B$. For $B$ small enough, Proposition \ref{KTV_Asymptotics_of_EV_and_EF} ensures that $\kappa$ is independent of $B$, whence $e_0^B$ is simple. In order to prove \eqref{KTB_Lower_bound_5}, we may henceforth assume that $T \leq \Tc + \frac \kappa 3$ due to the monotonicity of $K_{T,B}$ in $T$, which implies $K_{T,B} \geq K_{\min\{T,\Tc+\frac \kappa 3\},B}$.
%
%We consider the minimization problem for the operator $K_{T, B} - V$, while we assume $\Tc \leq T\leq \Tc + \frac \kappa 3$. For a normalized $\varphi \in L^2(\Rbb^3)$, we split $\varphi = a\alpha_*^B + b \zeta$\notiz{Eigene Gleichung? Besser lesbar?} with $|a|^2 + |b|^2 = 1$ and $\langle \alpha_*^B , \zeta\rangle =0$. Here, $\alpha_*^B$ is the unique normalized ground state of $K_{\Tc,B} - V$. In fact, $a$, $b$, and $\zeta$ are dependent on $B$ but these dependencies play no role in what follows. Note that for $T \geq \Tc$, \eqref{KTc_bounded_derivative} implies the inequality of operators
%\begin{align}
%K_{T,B} - K_{\Tc, B} \leq 2(T - \Tc).
%\end{align}
%Therefore, an application of $uv \leq \frac \eta 2 \, u^2 + \frac{1}{2\eta} \, v^2$ for $u,v\geq 0$ and $0 < \eta < 1$ yields
%\begin{align}
%\langle \varphi, (K_{T,B} - V) \varphi\rangle \geq \frac 12\, |a_B|^2 \; \langle \alpha_*^B, (K_{T,B} - K_{\Tc,B}) \alpha_*^B\rangle + |b_B|^2 \; (\kappa - 2 (T-\Tc)) - |e_0^B|. \label{KTB_Lower_bound_8}
%\end{align}
%In view of \eqref{KTc_bounded_derivative}, it is easy to see that
%\begin{align*}
%\langle \alpha_*^B, (K_{T,B} - K_{\Tc, B}) \alpha_*^B\rangle &\geq \bigl\langle K_{\Tc,B} \alpha_*^B, \frac{1}{\cosh^2(\frac{\pi^2 - \mu}{2\Tc})} K_{\Tc,B} \alpha_*^B\bigr\rangle \; (T - \Tc).
%\end{align*}
%It remains to remove the magnetic field in every instance\notiz{Wortwahl} to show that
%\begin{align}
%\bigl\langle K_{\Tc,B} \alpha_*^B, \frac{1}{\cosh^2(\frac{\pi^2 - \mu}{2\Tc})} K_{\Tc,B} \alpha_*^B\bigr\rangle \geq \int_{\Rbb^3} \dd p \; |\hat{V\alpha_*}(p)|^2 \; \frac{1}{\cosh^2(\frac{p^2-\mu}{2\Tc})} - CB. \label{KTB_Lower_bound_6}
%\end{align}
%The first term on the right side equals $2\Tc E_2 >0$ with $E_2$ from \eqref{GL-coefficient_1}.\notiz{$E$ ersetzen}
%
%To see that \eqref{KTB_Lower_bound_6} is true, we start with the eigenvalue equation $(K_{\Tc,B} - V)\alpha_*^B = e_0^B \alpha_*^B$. By Proposition \ref{KTV_Asymptotics_of_EV_and_EF}, the estimates $|e_0^B| \leq CB$ and $\Vert \alpha_*^B - \alpha_*\Vert_2^2 \leq CB$ hold. Since $V$ and $\cosh(\frac{\pi^2-\mu}{2\Tc})^{-2}$ are bounded operators, we may therefore replace $\alpha_*^B$ by $\alpha_*$ and $e_0^B$ by zero in every occurrence for an error of $CB$, i.e.,
%\begin{align}
%\bigl\langle K_{\Tc,B} \alpha_*^B, \frac{1}{\cosh^2(\frac{\pi^2 - \mu}{2\Tc})} K_{\Tc,B} \alpha_*^B\bigr\rangle \geq \bigl\langle V \alpha_*, \frac{1}{\cosh^2(\frac{\pi^2 - \mu}{2\Tc})}  V\alpha_*\bigr\rangle - CB.\label{KTB_Lower_bound_7}
%\end{align}
%
%
%Furthermore, we use the identity \eqref{cosh2_Matsubara}, which expresses $\cosh(\frac \beta 2 z)^{-2}$ in terms of the Matsubara frequencies $\omega_n$ in \eqref{Matsubara_frequencies}. The resolvent equation
%\begin{align*}
%\frac{1}{(\i\omega_n - \pi^2)^2} - \frac{1}{(\i\omega_n - p^2)^2} = \frac{1}{(\i\omega_n - \pi^2)^2} \bigl[ \i\omega_n (\pi^2 - p^2) - (\pi^4 - p^4) \bigr] \frac{1}{(\i\omega_n - p^2)^2}
%\end{align*}
%leads us to investigate
%\begin{align*}
%\pi^4 - p^4 &= (\pi^2 + p^2) (\pi^2- p^2) + [\pi^2- p^2, p^2] \\ 
%%
%&\hspace{-35pt}= \bigl( 2\pi^2 - \frac 14 |\Bbold \wedge x|^2\bigr) \bigl( \Bbold \wedge x\cdot p + \frac 14 |\Bbold \wedge x|^2 \bigr) - (\Bbold \wedge x \cdot p)^2 - \frac 14 |\Bbold \wedge x|^2 (\Bbold \wedge x\cdot p) + B^2.
%%
%%\bigl( \Bbold \wedge x \cdot  p + \frac 14 |\Bbold \wedge x|^2 \bigr) p^2 + \pi^2 \bigl( \Bbold \wedge x \cdot p + \frac 14 |\Bbold \wedge x|^2\bigr)
%\end{align*}
%Here, we used $[\pi^2 - p^2,p^2] = \frac 14 [|\Bbold \wedge x|^2,p^2] = B^2$ as well as $p^2 = \pi^2 - \Bbold \wedge x\cdot p - \frac 14 |\Bbold \wedge x|^2$ and the fact that $\Bbold \wedge x\cdot p$ commutes with $\pi^2-p^2$. Since $|\cdot|^k V\alpha_*\in L^2(\Rbb^3)$ for $k\in \Nbb$ by \eqref{Decay_of_alphastar}, a tedious investigation of the kernels with the techniques introduced in Section~\ref{Proofs} shows that, in \eqref{KTB_Lower_bound_7}, $\pi^2$ may be replaced by $p^2$ for an error of the size $CB$. This shows \eqref{KTB_Lower_bound_6}.
%
%We apply \eqref{KTB_Lower_bound_6} to \eqref{KTB_Lower_bound_8}. Together with the estimates provided by Proposition \ref{KTV_Asymptotics_of_EV_and_EF} mentioned above and $|a|^2 + |b|^2 =1$, we finally obtain
%\begin{align*}
%\langle \varphi, (K_{T,B} - V)\varphi\rangle &\geq \min \Bigl\{ \frac 12 \int_{\Rbb^3} \dd p \; |\hat{V\alpha_*}(p)|^2 \smash{\frac{1}{\cosh^2(\frac{p^2-\mu}{2\Tc})}} \, (T - \Tc) \; , \; \kappa - 2(T- \Tc)\Bigr\} \\
%%
%&\hspace{300pt} - CB.
%\end{align*}
%Since $T\leq \Tc + \frac \kappa 3$ implies $\kappa - 2(T - \Tc) \geq T - \Tc$, this proves \eqref{KTB_Lower_bound_5}.

\emph{Step 2.} We claim there are $c,C>0$ such that
\begin{align}
K_{T,B} - V \geq c \; (1 - P) (1 + \pi^2) (1- P) - CB. \label{KTB_Lower_bound_9}
\end{align}
From the arguments in Step~1 we know that we can replace $T$ by $\Tc$ for a lower bound if we allow for a remainder of the size $-CB$. To prove \eqref{KTB_Lower_bound_9}, we choose $0 < \eta < 1$ and write
\begin{align}
K_{\Tc,B}-V = e_0^BP_B + (1-P_B) [(1-\eta) K_{\Tc,B} -V](1-P_B) + \eta (1-P_B) K_{\Tc,B} (1-P_B), \label{KTB_Lower_bound_1}
\end{align}
where $e_0^B$ denotes the ground state energy of $K_{\Tc, B} - V$ and $P_B = |\alpha_*^B\rangle \langle \alpha_*^B|$ is the spectral projection onto the corresponding unique ground state vector $\alpha_*^B$. From Proposition~\ref{KTV_Asymptotics_of_EV_and_EF} we know that the first term on the right side of \eqref{KTB_Lower_bound_1} is bounded from below by $-CB$. The lowest eigenvalue of $K_{\Tc} - V$ is simple and isolated from the rest of the spectrum.  Proposition~\ref{KTV_Asymptotics_of_EV_and_EF} therefore implies that the second term in \eqref{KTB_Lower_bound_1} is nonnegative as long as $\eta$ is chosen small enough --- this choice only depends on $V$ and the spectral gap $\kappa$, i.e., not on $B$ --- and can be dropped for a lower bound.
%As long as $\eta \leq \kappa\,  (\kappa + \Vert V\Vert_\infty)^{-1}$, the second term is nonnegative and can be dropped for a lower bound.
%\vspace{10cm}
%For the second term of \eqref{KTB_Lower_bound_1}, Proposition \ref{KTV_Asymptotics_of_EV_and_EF} (b) provides a uniform spectral gap $\kappa>0$ above $e_0^B$ for small $B$. This implies
%\begin{align*}
%(1 - \eta) K_{\Tc,B}^r - V = (1- \eta) (K_{\Tc,B}^r - V) - \eta V \geq (1 - \eta) e_0^B P_B + (1-\eta)\kappa (1 - P_B) - \eta V.
%\end{align*}
%Since $P_B(1 - P_B) =0$, we infer
%\begin{align*}
%(1 - P_B)[ (1 - \eta)K_{\Tc,B}^r - V] (1 - P_B)\geq [ (1-\eta)\kappa - \eta \Vert V\Vert_\infty](1 - P_B).
%\end{align*}
%Hence, the second term on the right side of \eqref{KTB_Lower_bound_1} is nonnegative provided $\eta \leq \frac{\kappa}{\kappa + \Vert V\Vert_\infty}$. 
%Thus, \eqref{KTB_Lower_bound_1} is bounded from below by
%\begin{align}
%K_{\Tc,B} - V \geq \eta (1 - P_B) K_{\Tc,B}^r (1 - P_B) - CB. \label{KTB_Lower_bound_3}
%\end{align}
To treat the third term, we note that the symbol $K_T(p)$ in \eqref{KT-symbol} satisfies the inequality $K_{\Tc}(p) \geq c' (1 + p^2)$ for some constant $c'$, and hence $K_{\Tc,B} \geq c' (1 + \pi^2)$. In combination, the above considerations prove
\begin{align*}
K_{\Tc,B}-V \geq  c' \; (1-P_B)(1+\pi^2)(1-P_B) - CB.
\end{align*}
It remains to replace $P_B$ by $P = |\alpha_*\rangle\langle \alpha_*|$. To this end, we write
\begin{align}
(1-P_B)(1+\pi^2)(1-P_B) - (1-P)(1+\pi^2)(1-P) &\notag \\
%
&\hspace{-160pt}= (P-P_B) +  (P - P_B)\pi^2(1-P_B) + (1-P)\pi^2(P-P_B) \label{KTB_Lower_bound_4}.
\end{align}
From Proposition \ref{KTV_Asymptotics_of_EV_and_EF} we know that $\Vert P_B - P\Vert_\infty \leq CB$ and $\Vert \pi^2(P_B- P)\Vert_\infty \leq CB$. Hence, the norm of the operator on the right side of \eqref{KTB_Lower_bound_4} is bounded by a constant times $B$. This shows \eqref{KTB_Lower_bound_9} and concludes our proof.
\end{proof}

We deduce two corollaries from \eqref{Lower_Bound_A_3} and Lemma \ref{KTB_Lower_bound}. The first statement is an a priori bound on Theorem \ref{Main_Result_Tc} (b).

\begin{kor}
\label{TcB_First_Upper_Bound}
Let Assumptions \ref{Assumption_V} and \ref{Assumption_KTc} be true. Then, there are constants $B_0>0$ and $C>0$ such that for all $0 < B \leq B_0$ and all temperatures $T\geq \Tc(1 + CB)$, we have $\FBCS(\Gamma) - \FBCS(\Gamma_0) >0$ unless $\Gamma = \Gamma_0$.
%we have $\ov{\Tc(B)} \leq \Tc(1+ CB)$.
\end{kor}

\begin{proof}
Let $D_0>0$ and assume that $T \geq \Tc (1 + D_0B)$. From \eqref{Lower_Bound_A_3} and Lemma~\ref{KTB_Lower_bound} we know that
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \geq (c \, \min\{T_0, \Tc D_0B\}  - CB) \, \Vert \alpha\Vert_2^2. \label{TcB_First_Upper_Bound_1}
\end{align}
For the choice $D_0 = \frac{2 C}{ c \Tc}$ and $B_0 = \frac{T_0}{D_0 \Tc} $ the right side of \eqref{TcB_First_Upper_Bound_1} is strictly positive unless $\alpha = 0$. We conclude that $\Gamma_0$ is the unique minimizer of $\FBCS$, which proves the claim. 
\end{proof}

The second corollary provides a bound for the Cooper pair wave functions of low energy BCS states in the sense of \eqref{Second_Decomposition_Gamma_Assumption}. It is based upon \eqref{Lower_Bound_A_3} and to state it we need to introduce the operator
\begin{align}
U  &:= \e^{-\i \frac r2 \Pi_X}. \label{U_definition}
\end{align}
We highlight that it acts on both, the relative coordinate $r = x-y$ and the center-of-mass coordinate $X = \frac{x+y}{2}$ of a function $\alpha(x,y)$. 

\begin{kor}
\label{cor:lowerbound}
Let Assumptions \ref{Assumption_V} and \ref{Assumption_KTc} be true. For any $D_0, D_1 \geq 0$, there is a constant $B_0>0$ such that if $\Gamma$ satisfies \eqref{Second_Decomposition_Gamma_Assumption}, if $0 < B\leq B_0$, and if $T$ is such that $T - \Tc \geq -D_0B$, then $\alpha = \Gamma_{12}$ obeys
\begin{align}
&\langle \alpha, [U(1 - P)(1 + \pi_r^2)(1 - P)U^* + U^*(1 - P)(1 + \pi_r^2)(1 - P)U] \alpha \rangle \notag\\
%
&\hspace{200pt} + \Tr\bigl[(\alpha^* \alpha)^2\bigr] \leq C B \Vert \alpha\Vert_2^2 + D_1B^2, \label{Lower_Bound_A_2}
\end{align}
where $P = | \alpha_* \rangle \langle \alpha_* |$ and $\pi_r = -\i \nabla_r + \frac 12\Bbold \wedge r$ both act on the relative coordinate.
\end{kor}

In the statement of the corollary and in the following, we refrain from equipping the projection $P = |\alpha_*\rangle \langle \alpha_*|$ with an index $r$ although it acts on the relative coordinate. This does not lead to confusion and keeps the formulas readable.

\begin{proof}
We recall that the operator $V$ acts by multiplication with $V(x-y)$ and that $K_T(p)$ is defined in \eqref{KT-symbol}. Using $\alpha(x,y) = \alpha(y,x)$ we write
\begin{align}
\Tr \bigl[ (K_{T,B} - V) \alpha \alpha^*\bigr] &= \frac 12 \fint_{Q_B} \dd x \int_{\Rbb^3} \dd y \; \overline{\alpha(x,y)} \bigl[ (K_T(\pi_x) - V) + (K_T(\pi_y) - V) \bigr] \alpha(x,y). \label{Lower_Bound_A_4}
\end{align}
We note that $\pi_x = \frac 12 \Pi_X + \tilde \pi_r = U \pi_rU^*$ and $\pi_y = \frac 12 \Pi_X - \tilde \pi_r = -U^*\pi_r U$, with $\tilde \pi_r$ and $\Pi_X$ in \eqref{Magnetic_Momenta_COM}. Using the above identities we see that
\begin{align}
K_T(\pi_x) - V(r) &= U^* ( K_{T}(\pi_r) - V(r) ) U, \notag \\ %\quad \text{ and }  
%
K_T(\pi_y) - V(r) &= U ( K_{T}(\pi_r) - V(r) ) U^*. \label{eq:idK_T^r} 
\end{align}
The result follows from a short computation or from Lemma~\ref{CommutationI} below.
%Lemma \ref{CommutationI} provides several intertwining relations of $U$ with $\pi_r$. In particular, $\pi_x = \tilde \pi_r + \frac 12 \Pi_X = U \pi_rU^*$ and $-\pi_y = \tilde \pi_r - \frac 12 \Pi_X = U^*\pi_r U$, where $\tilde \pi_r$ and $\Pi_X$ are given by \eqref{Magnetic_Momenta_COM}. 
We combine \eqref{Second_Decomposition_Gamma_Assumption}, \eqref{Lower_Bound_A_3}, \eqref{Lower_Bound_A_4} and \eqref{eq:idK_T^r} to show the inequality
\begin{align*}
\frac 12\langle \alpha, [U (K_{T}(\pi_r) - V(r))U^* + U^* (K_{T}(\pi_r) - V(r))U]\alpha\rangle + c \Tr \bigl[ (\alpha^* \alpha)^2\bigr] \leq D_1 B^2. %\label{Lower_Bound_A_1}
\end{align*}
Finally, we apply Lemma \ref{KTB_Lower_bound} to the first term on the left side and obtain \eqref{Lower_Bound_A_2}.
\end{proof}

==> 3_Decomposition_degenerate_case/5.2_First_decomposition_result.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The first decomposition result}

The proof of Theorem~\ref{Structure_of_almost_minimizers} is based on Corollary~\ref{cor:lowerbound} and is given in two steps. In the first step we drop the second term on the left side of \eqref{Lower_Bound_A_2} for a lower bound, and investigate the implications of the resulting inequality for $\alpha$. The result of the corresponding analysis is summarized in Proposition~\ref{DEG:First_Decomposition_Result} below. The second term on the left side of \eqref{Lower_Bound_A_2} is used later in Lemma~\ref{Bound_on_psi}. 

\begin{prop}
\label{DEG:First_Decomposition_Result}
Given $D_0, D_1 \geq 0 $, there is $h_0>0$ with the following properties. If, for some $0< h\leq h_0$, the wave function $\alpha\in \Lsymm$ satisfies
\begin{align}
\langle \alpha , [U^* (1-P)(1 + p_r^2)(1-P)U + U (1-P) (1 + p_r^2)(1-P)U^*] \alpha \rangle & \leq D_0 h^2 \Vert \alpha\Vert_2^2 + D_1 h^4  , \label{DEG:First_Decomposition_Result_Assumption}
\end{align}
then there are $\Psi\in \Hmag^1(Q_h)$ and $\xi_0\in \Hsymm$ such that
\begin{align}
\alpha(X,r) =  \alpha_*(r)^t \cos\bigl( \frac r2 \cdot P_X\bigr) \Psi(X) + \xi_0(X,r) \label{DEG:First_Decomposition_Result_Decomp}
\end{align}
with
\begin{align}
\langle \Psi, P_X^2 \Psi\rangle + \Vert \xi_0\Vert_{\Hsymm}^2 \leq C\bigl( h^2 \Vert \Psi \Vert_2^2 + D_1 h^4  \bigr).  \label{DEG:First_Decomposition_Result_Estimate}
\end{align}
%and
%\begin{align}
%C \Vert \alpha\Vert_2^2 \geq \Vert \Psi\Vert_2^2 \geq (1- C  h^2)\; \Vert \alpha\Vert_2^2 - Ch. \label{First_Decomposition_Result_Estimate_psi}
%\end{align}
\end{prop}
Before we give the proof of the a priori estimates in Proposition \ref{DEG:First_Decomposition_Result}, we define the decomposition, discuss the idea behind it, which originates from \cite{Hainzl2017}, and make the connection to other existing works. For this purpose, let the operator $A \colon \Lsymm \ra \Lmag^2(Q_h)$ be given by
\begin{align}
(A\alpha)(X) := \int_{\Rbb^3} \dd r\; \ov{\alpha_*(r)} \; \cos\bigl( \frac r2\cdot P_X\bigr) \alpha(X,r). \label{DEG:Def_A}
\end{align}
A short computation shows that its adjoint $A^*\colon \Lmag^2(Q_h) \ra \Lsymm$ is given by
\begin{align}
(A^*\Psi) (X,r) = \alpha_*(r)^t \cos\bigl( \frac r2\cdot P_X\bigr) \Psi(X). \label{DEG:Def_Astar}
\end{align}
We highlight that this is the form of the first term in \eqref{DEG:First_Decomposition_Result_Decomp}. For a given Cooper pair wave function $\alpha$, we use these operators to define the two functions $\Psi$ and $\xi_0$ by
\begin{align}
	\Psi &:= (AA^*)^{-1} A\alpha, & \xi_0 &:= \alpha - A^*\Psi. \label{DEG:Def_Psixi}
\end{align}
Lemma~\ref{DEG:AAstar_Positive} below guarantees that $AA^*$ is invertible, and we readily check that  \eqref{DEG:First_Decomposition_Result_Decomp} holds with these definitions. Moreover, this decomposition of $\alpha$ is orthogonal in the sense that $\langle A^* \Psi, \xi_0 \rangle = 0$ holds. The claimed orthogonality follows from
\begin{align}
	A\xi_0 =0, \label{DEG:fundamental_property}
\end{align}
which is a direct consequence of \eqref{DEG:Def_Psixi}. In the following we motivate our choice for $\Psi$ and $\xi_0$ and comment on its appearance in the literature.

The decomposition of $\alpha$ is motivated by the minimization problem for the low-energy operator $2 -UPU^* - U^*PU$, that is, the operator in \eqref{DEG:First_Decomposition_Result_Assumption} with $p_r^2$ replaced by zero. The operators $UPU^*$ and $U^*PU$ act as $A^*A$ on the space $\Lsymm$ of reflection symmetric functions in the relative coordinate. If $P_X$ is replaced by $P_X$ then $A^*A$ can be written as 
\begin{equation}
	A^* A \cong \int^{\oplus}_{[0,\sqrt{ 2 \pi B}]^3} \mathrm{d}P_X \; | a_{P_X} \rangle \langle a_{P_X} |, \label{DEG:eq:directintegralA}
\end{equation}
with $| a_{P_X} \rangle \langle a_{P_X} |$ the orthogonal projection onto the function $a_{P_X}(r) = \cos(r/2 \cdot P_X) \alpha_*(r)$. Here the variable $P_X$ is the dual of the center-of-mass coordinate $X$ in the sense of Fourier transformation and $r$ denotes the relative coordinate. That is, the function $a_{P_X}(r)$ minimizes $1-A^* A$ in each fiber, whence it is the eigenfunction with respect to the lowest eigenvalue of $1 - A^* A = 1 - (UPU^* + U^*PU)/2$. This discussion should be compared to \cite[Eq. (5.47)]{Hainzl2012} and the discussion before Lemma~20 in \cite{ProceedingsSpohn}.

If $B$ is present in the magnetic momentum operator $P_X$ the above picture changes because the components of $P_X$ cannot be diagonalized simultaneously (they do not commute), and hence \eqref{DEG:eq:directintegralA} has no obvious equivalent in this case. The decomposition of $\alpha$ in terms of the operators $A$ and $A^*$ above has been introduced in \cite{Hainzl2017} in order to study the operator $1 - V^{\nicefrac 12} L_{T,B} V^{\nicefrac 12}$ with $L_{T,B}$ in \eqref{LTB_definition}, see also the discussion below Theorem~\ref{Calculation_of_the_GL-energy}. The situation in this work is comparable to our case with $p_r^2$ replaced by zero in \eqref{DEG:First_Decomposition_Result_Assumption}. Our analysis below shows that the ansatz \eqref{DEG:Def_Psixi} is useful even if the full range of energies is considered, that is, if $p_r^2$ is present in \eqref{DEG:First_Decomposition_Result_Assumption}. 

In the following lemma we collect useful properties of the operator $A A^*$. It should be compared to \cite[Lemma~27]{Hainzl2017}.
%
%
%
%That is, the function $f$ is the eigenfunction w.r.t. the lowest eigenvalue 
%of $1 - A^* A$, which motivates the decomposition. See also the discussion before Lemma~20 in \cite{ProceedingsSpohn} and \cite[Eq. (5.47)]{Hainzl2012}. In the case of a constant magnetic field, this reasoning is not  
%
%The above decomposition in terms of the operators $A$ and $A^*$ has been introduced in the case with a constant magnetic case in \cite{Hainzl2017}.
%
%
%The generalization of the above decomposition using the operators $A$ and $A^*$, was first introduced in \cite{Hainzl2017}. 
%We use this construction as a candidate for an approximate minimizer of the whole operator in \eqref{First_Decomposition_Result_Assumption} and set
%\begin{align}
%\Psi &:= (AA^*)^{-1} A\alpha, & \xi_0 &:= \alpha - A^*\Psi. \label{Def_Psixi}
%\end{align}
%By Lemma \ref{AAstar_Positive} below, $AA^*$ is indeed invertible. Then, \eqref{First_Decomposition_Result_Decomp} holds and the immediate and fundamental property
%\begin{align}
%A\xi_0 =0 \label{fundamental_property}
%\end{align}
%resulting from \eqref{Def_Psixi} implies that $A^*\Psi + \xi_0$ is an  orthogonal decomposition of $\alpha$ with respect to the scalar product in $\Lsymm$.

\begin{lem}
\label{DEG:AAstar_Positive}
The operators
\begin{align*}
AA^* &= \int_{\Rbb^3} \dd r\; \ov{\alpha_*(r)} \alpha_*(r)^t \cos^2\bigl( \frac{r}{2} \cdot P_X\bigr), & 1-AA^* &= \int_{\Rbb^3} \dd r \; \ov{\alpha_*(r)} \alpha_*(r)^t \sin^2\bigl( \frac r2 \cdot P_X\bigr) 
\end{align*}
on $\Lmag^2(Q_h)$ are both bounded nonnegative matrix-valued functions of $P_X^2$ and satisfy the following properties:
\begin{enumerate}[(a)]
\item $0\leq AA^*\leq 1$ and $0 \leq 1 - AA^*\leq 1$.
\item There is a constant $c>0$ such that $AA^* \geq c$ and $1 - AA^* \geq c \; P_X^2\; (1 + P_X^2)^{-1}$.
\end{enumerate}
In particular, $AA^*$ and $1 - AA^*$ are boundedly invertible on $\Lmag^2(Q_h)$.
\end{lem}

\textbf{\textcolor{red}{Dieses Lemma ist der Knackpunkt des Ganzen! Es wird so nicht stimmen wenn $\alpha_*$ nicht radial ist. Frage: Was stimmt dann?}}

Strategy of Proof:
\begin{itemize}
\item Prove this in the ``whole-space-case'' using the spherical harmonics.
\item Use Andi's argument to lift it to the periodic case.
\end{itemize}


%\subsubsection{Proof of Lemma \ref{AAstar_Positive}}
%
%\begin{proof}
%Part (a) is a direct consequence of the fact that $\Vert \alpha_* \Vert_2 = 1$. In the following we reduce the proof of part (b) to known results in \cite{Hainzl2017}. To this end, we introduce the operator
%\begin{align}
%	R := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot P_X)
%	\label{eq:R}
%\end{align}
%and note that
%\begin{align*}
%	AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R).
%\end{align*}
%Let us also denote by $\widetilde{R}$ the operator in \eqref{eq:R} but with $P_X$ replaced by $\tilde P_X$, which is the same operator but understood to act on $L^2(\mathbb{R}^3)$ instead of $\Lmag^2(Q_h)$. In Lemma~28 in \cite{Hainzl2017} it has been shown that $\widetilde{R}$ is a function of $\tilde P_X^2$. Moreover, the statement of Lemma~27 in \cite{Hainzl2017} is equivalent to
%\begin{align}
%	1 - \widetilde{R}^2 \geq c\,  \frac{\tilde P_X^2}{1 + \tilde P_X^2}
%	\label{eq:R1}
%\end{align}
%for some $0<c<1$, and Eq.~(55) in the same reference implies
%\begin{align}
%	| \widetilde{R} | \leq 1 - c.
%	\label{eq:R2}
%\end{align}
%In combination, \eqref{eq:R1}, \eqref{eq:R2}, and $ \widetilde{R} \leq 1$ show
%\begin{align}
%	 1+\widetilde{R} &\geq c, & 1 - \widetilde{R} \geq \frac{1 - \widetilde{R}^2}{2} &\geq \frac{c}{2} \frac{\tilde P_X^2}{1 + \tilde P_X^2} .
%	 \label{eq:R3} 
%\end{align}
%It remains to argue that $R$ is a function of $P_X^2$ and that a version of \eqref{eq:R3} with $\tilde R$ and $\tilde P_X$ replaced by $R$ and $P_X$ holds. 
%
%The fact that $R$ is a function of $P_X^2$ follows from the argument that we used to show that the same statement is true for the operator in \eqref{eq:A29}. To show that \eqref{eq:R3} with $\tilde R$ and $\tilde P_X$ replaced by $R$ and $P_X$ holds, we conjugate both sides of the inequalities with the Bloch-Floquet transformation in \eqref{eq:ABF1} and \eqref{eq:ABF2}, and use \eqref{eq:ABF3}. The inequalities in \eqref{eq:R3} therefore hold equally in any fiber, that is, with $\tilde P_X$ on the left and on the right sides replaced by $P_X(k) = P_X + k$ acting on $\Lmag^2(Q_h)$. Since $\tilde P_X(0) = P_X$, this proves the claim. 
%\end{proof}
%We note that part (a) is trivial. In contrast, part (b) needs the spectral decomposition of the operator $P_X^2$ acting in the space $\Lmag^2(Q_h)$. In appendix \ref{Spectrum_Landau_Hamiltonian_Section}, we use a Bloch-Floquet decomposition, under which $P_X$ fibers as a direct integral over $\vartheta\in [0,1]$ with the fiber momenta $P_X(\vartheta) := -\i \nabla + 2\Abold + \sqrt{2 \pi B} \, \vartheta \, e_3$. Proposition \ref{Spectrum_Landau_Hamiltonian} shows that the spectrum of $P_X(\vartheta)^2$ is then given by the values $2B(2k+1) + 2P_X (p+ \vartheta)^2$ with $k\in \Nbb_0$ and $p\in \Zbb$. Moreover, there is a basis of the $k$\tho\ Landau level of the form $\{(a^*)^k |1\rangle, (a^*)^k |2\rangle\}$ with $a|1\rangle =0$ and $a|2\rangle =0$ and the well-known creation and annihilation operators in \eqref{Creation-Annihilation}.
%It fibers in the magnetic Bloch-Floquet decomposition and can be diagonalized fiberwise by using the well-known creation and annihilation operators.
%A short computation shows that, in this setting, the spectrum of $P_X^2$ consists of the infinitely degenerate eigenvalues
%\begin{align}
%E_{k, p_3} &:= 2h^2 (2k+1) + p_3^2 , & k &\in \Nbb_0, \; p_3\in \sqrt{2\pi B}\; \Zbb. \label{Landau_Levels}
%\end{align}


%The goal of this section is to prove Lemma \ref{AAstar_Positive}. 
%Since $P_X$ is left invariant by the magnetic lattice translations $T_B(v)$, given by \eqref{Magnetic_Translation_Charge2}, there is a magnetic Bloch-Floquet decomposition $\Ucal_{\mathrm{BF}}$ such that the Landau Hamiltonian $P_X^2$ fibers according to
%\begin{align*}
%\Ucal_{\mathrm{BF}} \, P_X^2 \, \Ucal_{\mathrm{BF}}^* = \int_{Q_h^*}^\oplus \dd \vartheta \; P_X^2(\vartheta)
%\end{align*}
%with the fiber Hamiltonians
%\begin{align*}
%P_X^2(\vartheta) := (-\i \nabla_X + 2\Abold(X) + \vartheta)^2,
%\end{align*}
%acting on the domain $\Hmag^2(Q_h)$ for any $\vartheta\in Q_h^*$. Here, $Q_h^*$ is the fundamental cell of the dual lattice of $\Lambda_B$. We refer the interested reader to \cite[Section XIII.16]{Reedsimon4} for an introduction into Bloch-Floquet transformations and to \cite{Stefan_Peierls} for a particular treatment of the magnetic case.
%
%We claim that $P_X^2$ can be explicitly diagonalized as a multiplication operator with the eigenvalues
%
%%Consequently, in the Bloch-Floquet representation, $P_X^2$ becomes multiplication with the same numbers. 
%This follows from the fiberwise diagonalization of $P_X^2(\vartheta)$ via of the well-known creation and annihilation operators built upon the magnetic momentum $P_X + \vartheta$, and a Fourier transform in the free $X_3$-variable.
%
%The operator
%\begin{align*}
%R := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot P_X)
%\end{align*}
%satisfies
%\begin{align*}
%AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R)
%\end{align*}
%and can be written as a direct integral over $\vartheta\in [0,1]$ with fiber operators
%\begin{align*}
%R(\vartheta) := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot P_X(\vartheta))
%\end{align*}
%in a similar way as $P_X^2$. Then, $R(\vartheta)$ is diagonal in the same representation used to diagonalize $P_X(\vartheta)^2$.
%
%The proofs of Lemmas 27 and 28 in \cite{Hainzl2017} show that there is a $c >0$, independent of $\vartheta$, such that
%\begin{align*}
%R(\vartheta) &\geq - 1 + c, & R(\vartheta) &\leq 1 - c \; \frac{P_X^2}{1 + P_X^2}.
%\end{align*}
%From this, we easily deduce Lemma \ref{AAstar_Positive}.


%To see \eqref{Landau_Levels}, define $P_X(\vartheta) := P_X + \vartheta$ and let us introduce
%\begin{align*}
%a(\vartheta) &:= \frac{1}{2\sqrt{B}} \bigl( P_X^{(1)}(\vartheta) - \i P_X^{(2)}(\vartheta)\bigr), & a^\dagger(\vartheta) & = \frac{1}{2\sqrt{B}} \bigl( P_X^{(1)}(\vartheta) + \i P_X^{(2)}(\vartheta)\bigr).
%\end{align*}
%It follows that $[a(\vartheta), a^\dagger(\vartheta)] = 1$. Furthermore,
%\begin{align}
%P_X^2(\vartheta) = 2 h^2 \bigl( 2a^\dagger(\vartheta) a(\vartheta) + 1\bigr) + (P^{(3)} + \vartheta_3)^2. \label{AAstar_positive_3}
%\end{align}
%Here, $P^{(3)} = -\i \partial_{X_3}$ on the interval $[0,\sqrt{2P_X B^{-1}})$ with periodic boundary conditions. The operator $P^{(3)} + \vartheta_3$ can be diagonalized by the Fourier transform
%\begin{align*}
%(\Ucal_\vartheta \varphi)_m &= \frac{1}{\sqrt{2P_X B^{-1}}} \int_0^{\sqrt{2P_X B^{-1}}} \dd x_3 \; \e^{\i (\sqrt{2P_X B} \, m - \vartheta_3)x_3} \varphi(x_3) , & m &\in \Zbb,
%\end{align*} 
%having eigenvalues $p_3\in \sqrt{2P_X B}\, \Zbb$. Combining this with \eqref{AAstar_positive_3}, we read off \eqref{Landau_Levels}. 

%Consequently, \eqref{Landau_Levels} follows from taking the direct integral of $a(\vartheta)$ and $a^\dagger(\vartheta)$ over $\vartheta$. The proof shows that $P_X^2$ can be diagonalized as well, being a multiplication operator by the numbers
%\begin{align}
%E_{k, p_3} := 2B(2k+1) + 2P_X h^2 \; p_3^2, \qquad k\in \Nbb_0, \; p_3\in \Rbb. \label{Landau_Levels}
%\end{align}

%For the proof of Lemma \ref{AAstar_Positive}, we borrow the following auxiliary result, which is proven in \cite[Lemma 27]{Hainzl2017}. Denote the first two compontents of $P_X$ by $P_X^\perp = (P_X^{(1)}, P_X^{(2)})^t$. Moreover, by $P_{2B}^{(k)}$ we denote the projections onto the $k$\tho\ Landau level and by $L_k = L_k^{(0)}$ the Laguerre polynomials.
%
%\begin{lem}
%For every $\rho >0$,
%\begin{align*}
%\frac{1}{2P_X} \int_{\Sbb^1} \dd \omega \; \cos(\rho \omega\; P_X^\perp) =\e^{-\frac 12 B\rho^2} \sum_{k=0}^\infty L_k(B\rho^2) P_{2B}^{(k)}.
%\end{align*}
%\end{lem}

%\begin{proof}[Proof of Lemma \ref{AAstar_Positive}]
%As noted above, part (a) is trivial. We remark that the proof of part (b) is very similar to the proof of Lemma 27 in \cite{Hainzl2017}, when $\varphi_*$ is replaced by $\alpha_*$. It actually provides the proof of Lemma \ref{AAstar_Positive} when we read it carefully enough, which we do now. Let us introduce the operator
%\begin{align*}
%R := \int_{\Rbb^3} \dd r\; \alpha_*(r)^2 \; \cos(r\cdot P_X).
%\end{align*}
%Then, the key observation is that
%\begin{align*}
%AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R).
%\end{align*}
%
%In the representation of \eqref{Landau_Levels}, the operator $R$ is diagonalized as well, acting as a multiplication operator by the numbers
%%The operator $R$ can be diagonalized explicitly by a Fourier transform in the $x_3$ variable and decomposing into Landau levels in the $(x_1,x_2)$ variables. Then $R$ acts as a multiplication operator by the numbers
%\begin{align*}
%R_{k,p_3} &= P_X \int_0^\infty \dd u \int_\Rbb \dd x_3\; \bigl| \alpha_*\bigl( \sqrt{u + x_3^2}\bigr)\bigr|^2 \cos(x_3p_3) \e^{-\frac 12Bu} L_k(Bu), & k&\in \Nbb_0, \, p_3\in \sqrt{2P_X B} \, \Zbb.
%\end{align*}
%This formula is obtained in the same way as Eq. (49) in \cite{Hainzl2017} and $L_k$ is the $k$\tho\ Laguerre polynomial.
%
%Since $P_X^2$ acts as multiplication by the numbers $E_{k,p_3}$ of \eqref{Landau_Levels}, it suffices to prove that there is a $c>0$ such that
%\begin{align}
%R_{k,p_3} &\geq -1 + c, & R_{k,p_3} &\leq 1 - c \frac{E_{k,p_3}}{1 + E_{k,p_3}}. \label{AAstar_positive_2}
%\end{align}
%We prove these inequalities separately for small, medium and large values of $E_{k,p_3}$. In fact, \eqref{AAstar_positive_2} is true for all $p_3\in \Rbb$.
%
\emph{Step 1.} We claim that there are $E_* >0$ and $c_\leq , c_\geq >0$ such that for all $B>0$, $k\in\Nbb_0$ and $p_3\in \Rbb$ with $E_{k,p_3} \leq E_*$, we have
\begin{align}
1 - c_\leq E_{k,p_3} \leq R_{k,p_3} \leq 1 - c_\geq E_{k,p_3}. \label{AAstar_positive_1}
\end{align}
To see this, use $1 - \frac 12 x^2 \leq \cos x \leq 1 - \frac 12x^2 + \frac{1}{24} x^4$ for all $x\in \Rbb$ to conclude that
\begin{align}
0 \leq R - \int_{\Rbb^3} \dd r \; |\alpha_*(r)|^2 \bigl( 1 - \frac 12 (r\cdot P_X)^2\bigr) \leq \frac{1}{24} \int_{\Rbb^3} \dd r \; |\alpha_*(r)|^2 (r\cdot P_X)^4. \label{AAstar_positive_4}
\end{align}
Set
\begin{align*}
\langle |r|^{2m}\rangle &:= \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; r^{2m}, & m & = 1,2.
\end{align*} 
These numbers are finite by the decay properties \eqref{Decay_of_alphastar} of $\alpha_*$. An explicit computation using the fact that the angular average of $r_ir_j$ equals $\frac{1}{3} r_i^2 \delta_{ij}$ shows
\begin{align*}
\int_{\Rbb^3} \dd r \; \alpha_*(r)^2 (r\cdot P_X)^2 = \frac 13 \langle |r|^2\rangle \; P_X^2.
\end{align*}
Furthermore, using the operator inequality \eqref{ZPiX_inequality_quartic}, we get
\begin{align*}
\int_{\Rbb^3} \dd r \; \alpha_*(r)^2 (r\cdot P_X)^4 \leq C\langle |r|^4\rangle \; (P_X^4 + h^4 ).
\end{align*}
Combining this with \eqref{AAstar_positive_4}, we obtain
\begin{align*}
1 - \frac 16 \langle |r|^2\rangle P_X^2 \leq R \leq 1 - \frac 16 \langle |r|^2 \rangle P_X^2 + C\langle |r|^4\rangle (P_X^4 +  h^4 )
\end{align*}
or, equivalently,
\begin{align*}
1 - \frac 16 \langle |r|^2\rangle E_{k,p_3} \leq R_{k,p_3} \leq 1 - \frac 16\langle |r|^2 \rangle E_{k,p_3} + C\langle |r|^4\rangle (E_{k,p_3}^2 + h^4 ).
\end{align*}
To obtain \eqref{AAstar_positive_1} from this, we note that $B\leq E_{k,p_3}$ for every $k\in \Nbb_0$ and $p_3\in \Rbb$.
%
%Steps 2 and 3 in the proof of \cite[Lemma 28]{Hainzl2017} carry over to our situation. 
%
%\emph{Step 2} shows that $R_{k,p_3}\to 0$ as $E_{k,p_3}\to \infty$ uniformly for sufficiently small $B>0$. That is, for every $B_0>0$ and $\varepsilon>0$, there is $E_*>0$ such that for all $0\leq B\leq B_0$, all $k\in \Nbb_0$ and $p_3 \in \Rbb$ with $E_{k,p_3}\geq E_*$, we have $|R_{k,p_3}|\leq \varepsilon$.
%
%\emph{Step 3} shows that for any $E_\leq < E_\geq$ and any $B_0>0$, there is a $c>0$ such that for all $0 < B\leq B_0$, $k\in \Nbb_0$ and $p_3\in \Rbb$ with $E_\leq \leq E_{k,p_3}\leq E_\geq$, we have $|R_{k,p_3}| \leq 1 - c$.
%
%Putting the estimates together implies \eqref{AAstar_positive_2} and concludes the proof.
%\end{proof}


The remainder of this subsection is devoted to the proof of Proposition~\ref{DEG:First_Decomposition_Result}. We start with a lower bound on the operator in \eqref{DEG:First_Decomposition_Result_Assumption} when it acts on wave functions of the form $A^*\Psi$, see Lemma~\ref{DEG:MainTerm} below. 

\subsubsection{Step one -- lower bound on the range of \texorpdfstring{$A^*$}{A*}}

The main result of this subsection is the following lemma.

\begin{lem}
\label{DEG:MainTerm}
For any $\Psi\in \Lmag^2(Q_h)$, with $A$ and $A^*$ given by \eqref{DEG:Def_A} and \eqref{DEG:Def_Astar}, with $U$ given by \eqref{DEG:U_definition}, and $P = \sum_{i=1}^m  |\alpha_*^{(i)}\rangle \langle \alpha_*^{(i)}|$ in \eqref{DEG:Ground_state_projection} with $\alpha_*$ from \eqref{DEG:alpha_star_ev-equation} acting on the relative coordinate, we have
\begin{align}
\frac 12 \langle A^* \Psi, [ U^* (1 - P) (1 + p_r^2) (1- P) U + U(1 - P) (1 + p_r^2)(1-P) U^* ] A^*\Psi\rangle \hspace{-340pt}& \notag\\
%
&=  \langle \Psi, AA^* (1 - AA^*)(1 + P_X^2) \Psi\rangle \notag\\
%
&\hspace{10pt} +  \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \cos^2 \bigl(\frac r2 P_X\bigr) \; (1 - AA^*)\Psi(X) \notag \\
%
&\hspace{10pt}+ \fint_{Q_h} \dd X \int_{\Rbb^3} \dr \; \ov{AA^*\Psi(X)} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \sin^2 \bigl(\frac r2  P_X\bigr) \; AA^*\Psi(X). \label{DEG:MainTerm_5}
\end{align}
In particular, we have the lower bound
\begin{align}
\frac 12 \langle A^* \Psi, [ U^* (1 - P) (1 + p_r^2) (1- P) U + U(1 - P) (1 + p_r^2)(1-P) U^* ] A^*\Psi\rangle %& \notag\\
%
%&\hspace{-200pt}\geq \langle \Psi, AA^*(1 - AA^*)(1 + P_X^2)\Psi\rangle
\geq c\, \langle \Psi, P_X^2\Psi\rangle . \label{DEG:MainTerm_LowerBound}
\end{align}
\end{lem}

\begin{proof}
We start by defining
\begin{align}
\Tcal_1 &:= U^* p_r^2 U + Up_r^2 U^* = 2\, p_r^2 + \frac 12 \, P_X^2, & \Tcal_2 &:= U^*Pp_r^2PU + UPp_r^2PU^*, \notag \\
%
\Tcal_3 &:= U^* Pp_r^2U + UPp_r^2U^*, & \Tcal_4 &:= U^* p_r^2 PU + Up_r^2PU^*. \label{DEG:MainTerm_6}
\end{align}
Then, \eqref{DEG:MainTerm_5} can be written as
\begin{align}
\langle A^* \Psi, [ U^* (1 - P) (1 + p_r^2) (1- P) U + U(1 - P) (1 + p_r^2)(1-P) U^* ] A^*\Psi\rangle  & = \notag\\
%
&\hspace{-330pt}= 2\langle A^*\Psi, (1 - A^*A)A^*\Psi\rangle \notag \\
%
&\hspace{-300pt} + \langle A^*\Psi, \Tcal_1 A^*\Psi\rangle + \langle A^*\Psi, \Tcal_2 A^*\Psi\rangle - \langle A^*\Psi, \Tcal_3 A^*\Psi\rangle - \langle A^*\Psi, \Tcal_4 A^*\Psi\rangle. \label{DEG:Tcal_first_line}
\end{align}
The first term on the right side equals $2\langle AA^*\Psi, (1 - AA*)\Psi\rangle$, which is in its final form. 

The $P_X^2$ term in $\Tcal_1$ reads
\begin{align*}
\langle A^* \Psi , P_X^2 A^* \Psi \rangle = \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \alpha^*(r) \; \cos\bigl( \frac r2 P_X\bigr) P_X^2 \cos\bigl( \frac r2 P_X\bigr) \; \alpha_*(r) \Psi(X).
\end{align*}
and since all components of $\Pi_X$ commute, the result is
\begin{align}
\langle A^*\Psi, P_X^2 A^*\Psi\rangle = \langle AA^* , P_X^2 \Psi\rangle. \label{DEG:PX-term}
\end{align}
Next, we investigate the term proportional to $p_r^2$ in $\Tcal_1$, which reads
\begin{align*}
\langle A^*\Psi, p_r^2 A^*\Psi\rangle &= \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r \;  \ov{\Psi(X)^t} \alpha_*(r) \; \cos\bigl( \frac r2 P_X\bigr) \, p_r^2 \, \cos\bigl( \frac r2 P_X\bigr) \; \alpha_*(r)^t \Psi(X)
\end{align*}
We use
\begin{align}
p_r \cos\bigl( \frac r2 P_X\bigr) = \cos\bigl( \frac r2 P_X\bigr) p_r + \i \sin\bigl( \frac r2 P_X\bigr) \frac{P_X}{2} \label{DEG:pr_cos}
\end{align}
to move the operators $p_r$ from the middle to the outer positions and find
\begin{align*}
\cos\bigl( \frac r2 P_X\bigr) \, p_r^2 \, \cos\bigl( \frac r2 P_X\bigr) &= p_r \, \cos\bigl( \frac r2 P_X\bigr) \, p_r + \sin^2\bigl( \frac r2 P_X\bigr) \frac{P_X^2}{4} \\
%
&\hspace{-30pt} +\i \bigl[ p_r \, \sin\bigl( \frac r2 P_X\bigr)  \cos\bigl( \frac r2 P_X\bigr) \frac{P_X}{2} - \sin\bigl( \frac r2 P_X\bigr)  \cos\bigl( \frac r2 P_X\bigr) \frac{P_X}{2} \, p_r\bigr].
\end{align*}
Since this equation is self-adjoint apart from the term in square brackets, we conclude that this term vanishes. When we combine this with \eqref{DEG:PX-term}, we obtain
\begin{align}
\langle A^* \Psi, \Tcal_1 A^*\Psi\rangle &= \langle \Psi , AA^*P_X^2\Psi\rangle \notag \\
%
&\hspace{10pt}+ 2\fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)^t}\;  \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \cos^2\bigl( \frac r2 P_X\bigr)\;  \Psi(X) \label{DEG:Tcal1-Result}
\end{align}
and completes our computation of the term involving $\Tcal_1$.

A short computation shows that
\begin{equation}
\langle A^*\Psi , \Tcal_2A^*\Psi\rangle = 2\, \fint_{Q_h}\dd X \int_{\Rbb^3} \ov{AA^*\Psi(X)^t} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; AA^*\Psi(X). \label{DEG:Tcal2_result}
\end{equation}
It remains to compute the terms in \eqref{DEG:Tcal_first_line} involving the operators $\Tcal_3$ and $\Tcal_4$, where $\Tcal_4^* = \Tcal_3$.

In the following we compute the term with $\Tcal_3$. A short computation shows
\begin{align}
\langle A^* \Psi, \Tcal_3A^*\Psi\rangle & \notag\\ 
%
&\hspace{-30pt}= 2\fint_{Q_h}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; p_r\cos^2\bigl( \frac r2 P_X\bigr) \; \alpha_*(r) \; \Psi(X). \label{DEG:Tcal3_eq3}
\end{align}
We use \eqref{DEG:pr_cos} twice to commute $p_r$ with the squared cosine and find
\begin{align}
p_r\cos^2\bigl( \frac r2 P_X\bigr) %&= \cos^2\bigl( \frac r2 P_X\bigr)p_r + \i \cos\bigl( \frac r2 P_X\bigr)\sin\bigl( \frac r2 P_X\bigr)\frac{P_X}{2} + \i \frac{P_X}{2} \sin\bigl( \frac r2 P_X\bigr)\cos\bigl( \frac r2 P_X\bigr) \notag\\
%
&= \cos^2\bigl( \frac r2 P_X\bigr)p_r + \i \sin\bigl( \frac r2 P_X\bigr) P_X \cos\bigl( \frac r2 P_X\bigr). \label{DEG:Tcal3_eq1}
\end{align}
The first term is final and its quadratic form with $p_r \alpha_* AA^*\Psi$ and $\alpha_*\Psi$ reads
\begin{align}
2 \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)^t} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \cos^2\bigl( \frac r2P_X\bigr) \; \Psi(X). \label{DEG:MainTerm_4}
\end{align}
Let us continue with the second term on the right side of \eqref{DEG:Tcal3_eq1}. We multiply it with $p_r$ from the left, use \eqref{DEG:pr_cos} twice to commute $p_r$ to the right, and obtain
\begin{align*}
\i p_r \sin\bigl( \frac r2 P_X\bigr) P_X \cos\bigl( \frac r2 P_X\bigr) &= \i \sin\bigl( \frac r2 P_X\bigr)P_X\cos\bigl( \frac r2 P_X\bigr) p_r \\
%
&\hspace{50pt} - \sin^2 \bigl( \frac r2 P_X\bigr)\frac{P_X^2}{2} + \cos^2\bigl( \frac r2 P_X\bigr) \frac{P_X^2}{2}.
\end{align*}
We plug the second term of \eqref{DEG:Tcal3_eq1}, written in this form, back into \eqref{DEG:Tcal3_eq3} and obtain
%When evaluated in the inner product with $2 AA^*\Psi\alpha_*$ and $\Psi\alpha_*$, the second term on the right side of \eqref{Tcal3_eq1} therefore reads
\begin{align}
2 \i \fint_{Q_h}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)^t} \; \ov{p_r\alpha_*(r)} \; \sin\bigl( \frac r2 P_X\bigr) P_X  \cos\bigl( \frac r2 P_X\bigr)\; \alpha_*(r)^t\; \Psi(X) \hspace{-350pt}& \notag\\
%
&= 2 \i \fint_{Q_h}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^* \Psi(X)^t} \; \alpha_*(r) \; \sin\bigl( \frac r2 P_X\bigr) P_X \cos\bigl( \frac r2 P_X\bigr) \; p_r\alpha_*(r)^t\; \Psi(X) \notag \\
%
&\hspace{40pt} + \fint_{Q_h}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)^t} \;  \alpha_*(r) \; \cos^2\bigl( \frac r2 P_X\bigr)P_X^2 \; \alpha_*(r)^t\; \Psi(X) \notag \\
%
&\hspace{40pt} - \fint_{Q_h}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)^t} \; \alpha_*(r) \; \sin^2\bigl( \frac r2 P_X\bigr)P_X^2 \; \alpha_*(r)^t \; \Psi(X).\label{DEG:MainTerm_7}
\end{align}
Notice that the first term on the right side equals $(-1)$ times the term on the left side. Thus, the left side equals $\frac 12$ times the third line plus the fourth line. Accordingly, the left side of \eqref{DEG:MainTerm_7} is given by
\begin{align}
&\frac 12 \langle AA^*\Psi, AA^* P_X^2\Psi\rangle - \frac 12 \langle AA^*\Psi, (1 -AA^*) P_X^2\Psi\rangle. \label{DEG:Tcal3_eq4}
\end{align}
Adding this to \eqref{DEG:MainTerm_4}, we find
\begin{align}
\langle A^*\Psi, \Tcal_3 A^*\Psi\rangle &= \frac 12 \langle \Psi, AA^* AA^* P_X^2 \Psi\rangle - \frac 12 \langle \Psi, AA^* (1 - AA^*) P_X^2 \Psi\rangle  \notag\\
%
&\hspace{30pt} + 2 \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 P_X\bigr) \; \Psi(X). \label{DEG:Tcal3_result}
\end{align}
The corresponding result for $\langle A^*\Psi, \Tcal_4 A^*\Psi\rangle$ is obtained by taking the complex conjugate of the right side of \eqref{DEG:Tcal3_result}, which amounts to interchanging the roles of $AA^*\Psi$ and $\Psi$ in the last two lines.

We are now prepared to collect our results and to provide the final formula for \eqref{DEG:Tcal_first_line}. We need to collect the terms in \eqref{DEG:Tcal1-Result}, \eqref{DEG:Tcal2_result}, \eqref{DEG:Tcal3_result} and the complex conjugate of \eqref{DEG:Tcal3_result}. The terms involving $\nabla \alpha_* \, \nabla \alpha_*^t$ read
\begin{align}
&2\fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)^t}\;  \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \cos^2\bigl( \frac r2 P_X\bigr) \; \Psi(X) \notag \\
%
&\hspace{20pt} + 2 \fint_{Q_h} \dd X \int_{\Rbb^3} \ov{AA^*\Psi(X)^t} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; AA^*\Psi(X) \notag \\
%
&\hspace{20pt} - 2 \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)^t} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \cos^2\bigl( \frac r2 P_X\bigr) \; \Psi(X) \notag \\
%
&\hspace{20pt} - 2 \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)^t} \; \nabla \alpha_*(r) \, \nabla \alpha_*(r)^t \; \cos^2\bigl( \frac r2 P_X\bigr) \;  AA^*\Psi(X). \label{DEG:nablaterms}
\end{align}
When we insert the factor $1 = \cos^2(\frac r2 P_X) + \sin^2(\frac r2P_X)$ in the second term, we obtain the final result for the terms proportional to $\nabla \alpha_* \, \nabla \alpha_*^t$.

Finally, we collect the terms proportional to $\alpha_* \, \alpha_*^t$. Taking into account the first term in \eqref{DEG:Tcal_first_line}, we find
\begin{align*}
&2\langle \Psi, AA^*(1 - AA^*)\Psi\rangle + \langle \Psi, AA^*P_X^2\Psi\rangle + \langle \Psi, AA^*(1 - AA^*)P_X^2\Psi\rangle - \langle \Psi, AA^* AA^* P_X^2 \Psi\rangle \\
%
&\hspace{50pt}= 2\langle \Psi, AA^*(1 - AA^*)(1 + P_X^2)\Psi\rangle.
\end{align*}
To obtain the result, we used that the terms coming from $\Tcal_3$ and $\Tcal_4$ are actually the same because $AA^*$ and $1 - AA^*$ commute with $P_X^2$, see Lemma \ref{DEG:AAstar_Positive}. This proves \eqref{DEG:MainTerm_5} and the lower bound \eqref{DEG:MainTerm_LowerBound} is implied by the operator bounds in Lemma \ref{DEG:AAstar_Positive} as well.
%
%The estimate is true because the terms proportional to $|\nabla \alpha_*|^2$ and $|\Bbold \wedge r|^2\alpha_*^2$ are written in a commutative way. Hence, they are nonnegative.
\end{proof}

\subsubsection{Step two -- estimating the cross terms}

In the second step of the proof of Proposition \ref{DEG:First_Decomposition_Result} we estimate the cross terms that we obtain when the decomposition in \eqref{DEG:First_Decomposition_Result_Decomp} with $\Psi$ and $\xi_0$ in \eqref{DEG:Def_Psixi} is inserted into the left side of \eqref{DEG:First_Decomposition_Result_Assumption}. 

\begin{lem}
\label{DEG:Decomp_Low_Momenta_Crossterms}
Given $D_0, D_1 \geq 0$, there is $B_0>0$ with the following properties. If, for some $0< B\leq B_0$, the wave function $\alpha\in \Lsymm$ satisfies
\begin{align*}
\frac 12 \langle \alpha , [U^* (1 - P)U + U(1 - P)U^* ]\alpha \rangle \leq D_0 h^2\, \Vert \alpha \Vert_2^2 + D_1 h^4,
\end{align*}
then $\Psi$ and $\xi_0$ in \eqref{DEG:Def_Psixi} satisfy the estimate
\begin{align}
\langle \Psi, AA^*(1 - AA^*)\Psi\rangle + \Vert \xi_0\Vert_2^2 \leq C \bigl( h^2  \Vert \Psi \Vert_2^2 + D_1 h^4 \bigr). \label{DEG:Estimate_Low_Momenta}
\end{align}
Furthermore, for any $\eta >0$ we have
\begin{align}
|\langle \xi_0, [U(1-P)(1+p_r^2)(1-P)U^* + U^* (1-P)(1+p_r^2)(1-P)U] A^*\Psi\rangle| & \notag \\
%
&\hspace{-180pt}\leq \eta \, \Vert P_X\Psi\Vert^2 + C \left(1+ \eta^{-1} \right)\, \bigl( h^2 \Vert \Psi \Vert_2^2 + D_1 h^4 \bigr). \label{DEG:Tcal_CrossTerms} 
\end{align}
\end{lem}

\begin{proof}
We start by noting that $A\xi_0 =0$ implies $\langle \xi_0, A^*\Psi\rangle =0$, and hence
\begin{align}
\Vert \alpha\Vert_2^2 = \Vert A^*\Psi\Vert_2^2 + \Vert \xi_0\Vert_2^2 \leq \Vert \Psi\Vert_2^2 + \Vert \xi_0\Vert_2^2. \label{DEG:Decomp_Low_Momenta_1}
\end{align}
We use $\alpha \in \Lsymm$ and $A(1 - A^*A)A^* = AA^*(1 - AA^*)$ to see that
\begin{align}
D_0 h^2 \Vert \alpha\Vert_2^2 + D_1 h^4 &\geq \frac 12 \langle \alpha, [U^* (1 - P)U + U(1 - P)U^* ]\alpha \rangle = \langle \alpha, (1 - A^*A) \alpha\rangle \notag\\
%
&= \langle A^*\Psi, (1 - A^*A)A^*\Psi\rangle + \langle \xi_0, (1- A^*A) A^*\Psi\rangle + \langle A^*\Psi, (1- A^*A)\xi_0\rangle \notag \\
%
&\hspace{230pt} + \langle \xi_0 , (1- A^*A)\xi_0\rangle \notag \\
%
&= \langle \Psi, AA^*(1 - AA^*) \Psi\rangle + \Vert \xi_0\Vert_2^2. \label{DEG:Decomp_Low_Momenta_9}
\end{align}
From Lemma~\ref{DEG:AAstar_Positive} we know that the first term on the right side is nonnegative and hence
\begin{equation*}
	\Vert \xi_0\Vert_2^2 \leq D_0 h^2 \Vert \alpha\Vert_2^2 + D_1 h^4.
\end{equation*}
Together with \eqref{DEG:Decomp_Low_Momenta_1}, this also proves
\begin{equation*}
(1 - D_0h^2)\Vert \alpha\Vert_2^2 \leq \Vert \Psi\Vert_2^2 + D_1 h^4 . %\label{Bound_on_Psi_First}
\end{equation*}
Finally, this last bound \eqref{DEG:Decomp_Low_Momenta_9} prove \eqref{DEG:Estimate_Low_Momenta}.

Next we prove \eqref{DEG:Tcal_CrossTerms}. Let us define 
\begin{align}
\Tcal := U^* (1 - P)(1 + p_r^2)(1 - P)U + U(1 - P)(1 + p_r^2)(1 - P)U^* \label{DEG:Tcal_Op_Def}
\end{align}
and consider $\langle \xi_0, \Tcal A^*\Psi\rangle$. We note that $A\xi_0 =0$ implies $PU \xi_0 = 0 = PU^*\xi_0$, where the projection $P$ is understood to act on the relative coordinate. In combination with \eqref{DEG:MainTerm_6} this allows us to see that
\begin{align}
\langle \xi_0, \Tcal A^*\Psi\rangle &= \Bigl\langle \xi_0, \Bigl[2p_r^2 + \frac{P_X^2}{2} \Bigr] A^*\Psi\Bigr\rangle - \langle \xi_0, (U^* + U) p_r^2 \, \alpha_* AA^*\Psi\rangle \label{DEG:Decomp_Low_Momenta_2}
\end{align}
holds. First of all, since $A\xi_0 =0$, we have
\begin{align}
\frac 12\langle \xi_0, P_X^2 A^*\Psi\rangle &= \frac 12\langle A \xi_0, P_X^2\Psi\rangle = 0. \label{DEG:Decomp_Low_Momenta_4}
\end{align}
The first term on the right side vanishes because $A\xi_0 =0$. Similarly, we apply \eqref{DEG:pr_cos} to commute $p_r^2$ in the first term in \eqref{DEG:Decomp_Low_Momenta_2} to the right and find
\begin{align}
2\langle \xi_0, p_r^2A^*\Psi\rangle &= 2 \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \cos\bigl( \frac r2 P_X\bigr) \; p^2\alpha_*(r)^t \; \Psi(X) \notag \\ %\label{Decomp_Low_Momenta_5} \\
%
&\hspace{20pt} + 2\i \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r \, \ov{\xi_0(X,r)} \;  \sin\bigl( \frac r2 P_X\bigr) \; p\alpha_*(r)^t \; P_X\Psi(X). \label{DEG:Decomp_Low_Momenta_6}
\end{align}
%Using that $\alpha_*$ is radial, $p\alpha_*(r)$ is proportional to $e_r$, whence $p\alpha_*(r)\cdot \Bbold \wedge r =0$. Therefore, 
When we combine \eqref{DEG:Decomp_Low_Momenta_2}, \eqref{DEG:Decomp_Low_Momenta_4} and \eqref{DEG:Decomp_Low_Momenta_6}, we obtain
\begin{align*}
\langle \xi_0, \Tcal A^*\Psi\rangle &= 2 \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \cos\bigl( \frac r2 P_X\bigr) \; p_r^2\alpha_*(r)^t \; (1 - AA^*)\Psi(X) \\
%
&\hspace{30pt}+ 2\i \fint_{Q_h}\dd X\int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \sin\bigl( \frac r2 P_X\bigr) \; \bigl[ p - \frac 12\Bbold \wedge r\bigr] \alpha_*(r)^t \; P_X\Psi(X).
\end{align*}
Using Cauchy-Schwarz, we bound the absolute value of this by
\begin{align}
|\langle \xi_0, \Tcal A^*\Psi\rangle| \leq 2\Vert \xi_0\Vert_2 \; \bigl[ \Vert p^2\alpha_*\Vert_2 \; \Vert (1 - AA^*)\Psi\Vert_2 + \Vert \nabla \alpha_*\Vert_2 \, \Vert P_X\Psi\Vert_2\bigr], \label{DEG:Decomp_Low_Momenta_7}
\end{align}
and with the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar} we see that the norms of $\alpha_*$ on the right side are bounded. Moreover, Lemma~\ref{DEG:AAstar_Positive} and \eqref{DEG:Estimate_Low_Momenta} imply that there is a constant $c>0$ such that
\begin{equation}
	\Vert (1 - AA^*)\Psi\Vert_2^2 \leq \langle \Psi, (1-AA^*) \Psi \rangle \leq \frac{1}{c} \langle \Psi, A A^* (1-AA^*) \Psi \rangle \leq C \bigl( h^2  \Vert \Psi \Vert_2^2 +D_1 h^4\bigr).
\end{equation}
For $\eta >0$ we thus obtain
\begin{align}
|\langle \xi_0, \Tcal A^*\Psi\rangle| \leq C \bigl[ \eta\,  \Vert P_X\Psi\Vert_2^2 + \eta^{-1} \, \Vert \xi_0 \Vert_2^2 + \bigl( h^2 \Vert \Psi \Vert_2^2 +D_1 h^4 \bigr) \bigr] \label{DEG:Decomp_Low_Momenta_8}
\end{align}
and an application of \eqref{DEG:Estimate_Low_Momenta} proves the claim.
\end{proof}

\subsubsection{Proof of Proposition \ref{DEG:First_Decomposition_Result}}

We recall the decomposition $\alpha = A^*\Psi + \xi_0$ with $\Psi$ and $\xi_0$ in \eqref{DEG:Def_Psixi} as well as $\Tcal$ in \eqref{DEG:Tcal_Op_Def}. From \eqref{DEG:First_Decomposition_Result_Assumption} we know that
\begin{align}
D_0 h^2 \Vert\alpha\Vert_2^2 + D_1 h^4 \geq \langle A^*\Psi, \Tcal A^*\Psi\rangle + 2\Re\langle \xi_0, \Tcal A^*\Psi\rangle + \langle \xi_0, \Tcal\xi_0\rangle . \label{DEG:First_Decomposition_Result_1}
\end{align}
The identities $PU\xi_0 = 0 = PU^*\xi_0$ imply
\begin{align}
\langle \xi_0, \Tcal \xi_0 \rangle = \Bigl\langle \xi_0, \bigl(2 + \frac{P_X^2}{2} + 2p_r^2\bigr) \xi_0\Bigr\rangle \geq \frac 12 \, \Vert \xi_0\Vert_\Hsymm^2. \label{DEG:First_Decomposition_Result_2}
\end{align}
Lemma \ref{DEG:AAstar_Positive} guarantees the existence of a constant $\rho>0$ such that
\begin{align*}
AA^*(1 - AA^*)(1 + P_X^2) \geq \rho\; P_X^2.
\end{align*}
Therefore, \eqref{DEG:MainTerm_LowerBound} implies 
%that the first term of \eqref{First_Decomposition_Result_1} is bounded from below by
\begin{align}
\langle A^* \Psi, \Tcal A^*\Psi\rangle \geq 2\, \langle \Psi, AA^*(1 - AA^*) (1 + P_X^2)\Psi\rangle \geq 2\rho\, \langle \Psi, P_X^2\Psi\rangle. \label{DEG:First_Decomposition_Result_3}
\end{align}

To estimate the second term on the right side of \eqref{DEG:First_Decomposition_Result_1}, we note that $\Tcal$ is bounded from below by $U(1 - P)U^* + U^*(1-P)U$. Therefore, we may apply Lemma \ref{DEG:Decomp_Low_Momenta_Crossterms} with $\eta = \frac \rho2$ and find
\begin{align*}
2\Re \langle \xi_0, \Tcal A^*\Psi\rangle \geq -2\, |\langle \xi_0, \Tcal A^*\Psi\rangle| \geq - \rho \, \Vert P_X\Psi\Vert_2^2 - C\bigl( h^2 \Vert \Psi\Vert_2^2 + D_1 h^4 \bigr).
\end{align*}
In combination with \eqref{DEG:First_Decomposition_Result_1}, \eqref{DEG:First_Decomposition_Result_2} and \eqref{DEG:First_Decomposition_Result_3}, we thus obtain
\begin{align*}
C\bigl( h^2\Vert \Psi\Vert_2^2 + D_1h^4  \bigr)\geq \rho \, \Vert P_X\Psi\Vert_2^2 + \frac 12 \, \Vert \xi_0\Vert_\Hsymm^2.
\end{align*}
This proves \eqref{DEG:First_Decomposition_Result_Estimate}. %The estimate \eqref{First_Decomposition_Result_Estimate_psi} on $\Vert \Psi\Vert_2^2$ is \eqref{Bound_on_Psi_First}.

==> 3_Decomposition_degenerate_case/5.3_Uniform_bound_on_Psi.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Uniform estimate on \texorpdfstring{$\Vert\Psi\Vert_2$}{Psi}}

Up to now we neglected the nonlinear term on the left side of \eqref{Lower_Bound_A_2}. This term provides the inequality
\begin{align}
		\Tr\bigl[(\alpha^* \alpha)^2\bigr] \leq C \left( B \Vert \alpha\Vert_2^2 + B^2 \right). \label{Lower_Bound_A_2b}
\end{align}
In this section we will take this term and \eqref{Lower_Bound_A_2b} into account and show that it can be combined with Proposition~\ref{DEG:First_Decomposition_Result} to obtain a bound for $\Vert \Psi\Vert_2$. This will afterwards allow us to prove Theorem~\ref{Structure_of_almost_minimizers}.

\begin{lem}
\label{Bound_on_psi}
Given $D_0\geq0$, there is $B_0>0$ such that for all $0 < B \leq B_0$ the following holds. If the wave function $\alpha\in \Lsymm$ obeys \eqref{Lower_Bound_A_2} then $\Psi$ in \eqref{DEG:Def_Psixi} satisfies
\begin{align}
\Vert \Psi\Vert_2^2 &\leq CB. \label{Bound_on_psi_result}
\end{align}
\end{lem}

\begin{proof}
We recall the decomposition $\alpha = A^*\Psi + \xi_0$ with $\Psi$ and $\xi_0$ in \eqref{DEG:Def_Psixi}. Eq.~\eqref{Lower_Bound_A_2b} and an application of the triangle inequality imply
\begin{align}
C\bigl( B\Vert \Psi\Vert_2^2 + B^2\bigr)^{\nicefrac 14} \geq \Vert \alpha\Vert_4 \geq \Vert A^*\Psi\Vert_4 - \Vert \xi_0\Vert_4. \label{Nonlinearity_8}
\end{align}
Thus, it suffices to prove an upper bound for $\Vert \xi_0\Vert_4$ and a lower bound for $\Vert A^*\Psi\Vert_4$. Our proof follows closely the proof of \cite[Eq. (5.48)]{Hainzl2012}. 

\emph{Step 1.} Let us start with the upper bound on $\Vert \xi_0\Vert_4$. We claim the estimate
\begin{align}
\Vert \xi_0\Vert_4 \leq C \bigl( B^{\nicefrac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18} \Vert \Psi\Vert_2 + B^{\nicefrac 12}\bigr).
%C\bigl( B^{\nicefrac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18}\bigr) \;  \bigl(1 + B^{\nicefrac 12} \Vert \Psi\Vert_2\bigr)^{\nicefrac 12}. 
\label{Nonlinearity_1}
\end{align}
To see this, we first use Hölder's inequality to estimate $\Vert \xi_0\Vert_4^4 \leq \Vert \xi_0\Vert_2^2 \; \Vert \xi_0\Vert_\infty^2$. From Proposition~\ref{DEG:First_Decomposition_Result} we know that $\Vert \xi_0\Vert_2^2 \leq C(B\Vert \Psi\Vert_2^2+ B^2)$, and it thus remains to prove a bound for $\Vert \xi_0\Vert_\infty$. We claim that for any $\nu > 3$
\begin{align}
\Vert \xi_0\Vert_\infty \leq  1 + C_\nu\, B^{-\nicefrac 14} \, \Vert (1 + |\cdot |)^\nu \alpha_*\Vert_{\nicefrac 65} \; \Vert \Psi \Vert_6, \label{Claim_xi_infty}
\end{align}
where the right side is finite by the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar}. To prove \eqref{Claim_xi_infty}, we first note that \eqref{gamma_alpha_fermionic_relation} implies $\Vert \alpha\Vert_\infty\leq 1$, and hence $\Vert \xi_0\Vert_\infty \leq 1 + \Vert A^*\Psi\Vert_\infty$. We apply Lemma \ref{Schatten_estimate} (b) to $A^*\Psi$ and obtain \eqref{Claim_xi_infty}. We also combine \eqref{Magnetic_Sobolev} with Proposition \ref{DEG:First_Decomposition_Result} and obtain $
\Vert \Psi\Vert_6 \leq C( \Vert \Psi\Vert_2 + B^{\nicefrac 12})$. In combination, these considerations imply \eqref{Nonlinearity_1}. 

\emph{Step 2.} We claim that
\begin{align}
\Vert A^*\Psi\Vert_4^4 \geq \frac 1{16} \; \Vert \hat \alpha_* \Vert_4^4 \; \Vert \Psi\Vert_4^4 - C \bigl( B^{\nicefrac 18} \Vert \Psi\Vert_2 + B^{\nicefrac 58} \bigr)^4 \label{Nonlinearity_5}
\end{align}
holds. To prove \eqref{Nonlinearity_5}, we write $\Vert A^*\Psi\Vert_4^4 = \tr ((A^*\Psi)^* A^*\Psi)^2$. The fact that $\alpha_*$ is real-valued implies
\begin{align*}
\Vert A^*\Psi\Vert_4^4 &= \fint_{Q_B} \dd x \int_{\Rbb^3} \dd y \; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(x - z)\ov{ \left[ \cos\bigl( \frac{x - z}{2}\Pi_{\frac{x+z}{2}}\bigr)  \Psi\bigl( \frac{x+z}{2}\bigr) \right] } \mathop \times\\
%
&\hspace{150pt} \times \alpha_*(z-y) \left[ \cos\bigl( \frac{z-y}{2} \Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z+y}{2}\bigr) \right] \Bigr|^2.
\end{align*}
We use $\cos(x) = 1 - 2\sin^2(\frac x2)$ twice and find
\begin{align}
\Vert A^*\Psi\Vert_4^4 &\geq \frac 14 \Tcal_* - C \, (\Tcal_1 + \Tcal_2), \label{Nonlinearity_2}
\end{align}
where
\begin{align*}
\Tcal_* &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \;\Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(x - z) \ov{\Psi\bigl(\frac{x+z}{2}\bigr)} \alpha_*(z - y) \Psi\bigl( \frac{z+y}{2}\bigr)\Bigr|^2
\end{align*}
and 
\begin{align}
\Tcal_1 &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \;\Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(x - z) \ov{\Psi\bigl( \frac{x+z}{2}\bigr)} \mathop \times \notag\\
%
&\hspace{140pt} \times \alpha_*(z - y) \left[ \sin^2\bigl( \frac{z-y}{4} \Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z +y}{2}\bigr) \right] \Bigr|^2, \notag\\
%
\Tcal_2 &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \; \Bigl| \int_{\Rbb^3} \dd z\; \alpha_*(x - z)\ov{ \left[ \sin^2\bigl( \frac{x -z}{4} \Pi_{\frac{x+z}{2}}\bigr) \Psi\bigl( \frac{x + z}{2}\bigr) \right]} \mathop \times \notag \\
%
&\hspace{140pt} \times\alpha_*(z - y) \left[ \cos\bigl( \frac{z - y}{2}\Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z+y}{2}\bigr) \right] \Bigr|^2. \label{Nonlinearity_3}
\end{align}
In the following we derive a lower bound on $\Tcal_*$ and an upper bound on $\Tcal_1$ and $\Tcal_2$.

\emph{Lower bound on $\Tcal_*$.} We change variables $z\mapsto z + x$ and $y\mapsto y + x$ and afterwards replace $x$ by~$X$, which allows us to write
\begin{align}
\Tcal_* = \fint_{Q_B} \dd X \int_{\Rbb^3} \dy \; \Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(z) \ov{\Psi\bigl(X + \frac z2\bigr)} \alpha_*(z - y) \Psi\bigl(X + \frac{z+y}{2}\bigr)\Bigr|^2. \label{Nonlinearity_9}
\end{align}
Next, we combine $\Psi(X + \frac z2) = \e^{\i \frac z2P_X} \Psi(X)$ and the identity $\e^{\i \frac r2P_X} = \e^{\i \frac \Bbold 2 r\wedge X}\e^{\i \frac r2\Pi_X}$ in \eqref{representation_Ustar} to write $\Psi(X + \frac z2) = \e^{\i \frac \Bbold 2 z\wedge X} \e^{\i \frac z2\Pi_X} \Psi(X)$. 
%Similarly, $\Psi(X + \frac{z+y}{2}) = \e^{\i \frac{\Bbold }{2} (z+y)\wedge X} \e^{\i\frac{z+y}{2}\Pi_X}\Psi(X)$. 
We conclude that
\begin{align*}
\ov{\Psi\bigl( X + \frac z2\bigr)} \Psi\bigl(X + \frac{z+y}{2}\bigr) = \e^{\i \frac{\Bbold}{2} y\wedge X} \; \ov{\left[ \e^{\i \frac{z}{2}\Pi_X}\Psi(X) \right]} \; \left[ \e^{\i \frac{z+y}{2}\Pi_X} \Psi(X) \right],
\end{align*}
as well as
\begin{align*}
\Tcal_* = \fint_{Q_B} \dd X \int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(-z) \ov{ \left[ \e^{\i \frac z2\Pi_X} \Psi(X) \right]} \alpha_*(z - y) \left[ \e^{\i \frac{z+y}{2}\Pi_X} \Psi(X) \right] \Bigr|^2.
\end{align*}
This also implies
\begin{align}
\Tcal_* \geq \frac 14\Tcal_*^* - C(\Tcal_*^{(1)} + \Tcal_*^{(2)})
\label{eq:A1}
\end{align}
with
\begin{align*}
\Tcal_*^* := \fint_{Q_B}\dd X\int_{\Rbb^3}\dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(z)^t \ov{\Psi(X)} \alpha_*(z - y)^t \Psi(X)\Bigr|^2
\end{align*}
and
\begin{align}
\Tcal_*^{(1)} &:= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(z) \ov{\bigl[\e^{\i \frac{z}{2}\Pi_X}\Psi(X)\bigr]} \alpha_*(z - y) \bigl[\bigl( \e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X)\bigr]\Bigr|^2, \notag \\
%
\Tcal_*^{(2)} &:= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \;\alpha_*(z)  \ov{\bigl[\bigl( \e^{\i \frac z2\Pi_X} - 1\bigr) \Psi(X)\bigr]} \alpha_*(z - y) \Psi(X)\Bigr|^2. \label{Nonlinearity_10}
\end{align}
The term $\Tcal_*^*$ equals
\begin{align*}
\Tcal_*^* = \fint_{Q_B} \dd X\; |\Psi(X)|^4 \; \int_{\Rbb^3} \dd y\;\Bigl|\int_{\Rbb^3} \dd z\; \alpha_*(z)\alpha_*(y - z)\Bigr|^2 = \Vert \Psi\Vert_{L^4(Q_B)}^4 \; \Vert \alpha_* * \alpha_*\Vert_{L^2(\Rbb^3)}^2.
\end{align*}
By \eqref{Decay_of_alphastar}, the Fourier transform of $\alpha_**\alpha_*$ equals $|\hat \alpha_*|^2$. Thus, $\Vert \alpha_* *\alpha_*\Vert_2^2 = \Vert \hat \alpha_*\Vert_4^4>0$. This is the desired leading term of \eqref{Nonlinearity_5}. 

\emph{Upper bound on $\Tcal_*^{(1)}$ and $\Tcal_*^{(2)}$.} We start with $\Tcal_*^{(1)}$, expand the square and estimate
\begin{align}
&\Tcal_*^{(1)} \leq  \int_{\Rbb^3} \dd y  \int_{\Rbb^3} \dd z  \int_{\Rbb^3} \dd z' \;  | \alpha_*(z) \, \alpha_*(z') \, \alpha_*(z - y) \, \alpha_*(z' - y)| \label{Nonlinearity_13} \\
& \times \fint_{Q_B} \dd X \; \Bigl| \bigl[ \e^{\i \frac z2\Pi_X} \Psi(X) \bigr]  \bigl[ \e^{\i \frac {z'}2\Pi_X} \Psi(X) \bigr]  \bigl[ \bigl( \e^{\i \frac{z+y}{2}\Pi_X}-1\bigr) \Psi(X) \bigr]  \bigl[ \bigl( \e^{\i \frac{z'+y}{2}\Pi_X}-1\bigr) \Psi(X) \bigr] \Bigr|. \nonumber
\end{align}
When we use Hölder's inequality, \eqref{NTB-NtildeTB_3}, \eqref{ZPiX_inequality}, and \eqref{Magnetic_Sobolev} we see that the integral in the second line can be bounded by
\begin{align}
\Vert \e^{\i \frac{z}{2}\Pi} \Psi\Vert_6^2 \; \Vert (\e^{\i \frac{z+y}{2}\Pi} - 1) \Psi\Vert_6 \; \Vert (\e^{\i \frac{z+y}{2}\Pi} - 1) \Psi\Vert_2 \leq C\; \bigl|\frac{z+y}{2}\bigr| \; B^{-\nicefrac 32} \; \Vert \Pi\Psi\Vert_2^4. \label{Nonlinearity_11}
\end{align}
%
%
%
%Using Hölder in $X$, we obtain
%\begin{align*}
%\fint_{Q_B} \dd X \; |\e^{\i \frac{z}{2}\Pi_X} \Psi(X)|^2 \; \ov{\bigl(\e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X)} \; \bigl(\e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X) \leq &\\
%%
%&\hspace{-250pt} \leq \Bigl( \fint_{Q_B} \dd X \; |\e^{\i \frac z2\Pi_X} \Psi(X)|^6\Bigr)^{\nicefrac 13} \; \Bigl( \fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} - 1) \Psi(X)|^6\Bigr)^{\nicefrac 16} \mathop \times \\
%%
%&\hspace{-100pt} \times\Bigl( \fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} - 1) \Psi(X)|^2\Bigr)^{\nicefrac 12}.
%\end{align*}
%
%
%Use 
%
%
%
%For the first factor, note $|\e^{\i \frac z2\Pi_X}\Psi(X)| = |\Psi(X + \frac z2)|$, so that, since $|\Psi|$ is periodic, this term equals $\Vert \Psi\Vert_6^2$. As for the second factor.  For the last factor, we use the operator inequality \eqref{ZPiX_inequality} to obtain
%\begin{align*}
%\fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} -1)\Psi(X)|^2 &\leq \frac{|z+y|^2}{4} \; \Vert \Pi_X\Psi\Vert_2^2.
%\end{align*}
Proposition~\ref{DEG:First_Decomposition_Result} provides us with a bound for $\Vert \Pi \Psi \Vert_2$. In combination with \eqref{Nonlinearity_13}, \eqref{Nonlinearity_11}, Young's inequality, and the bound $|z + y| \leq 2|z| + |z- y|$, this implies
\begin{align}
\Tcal_*^{(1)} &\leq C \, B^{-\nicefrac 32}\,  \left( B^2 \Vert \Psi \Vert_2^4 + D_1 B^4 \right) \int_{\Rbb^3} \dd y \; \Bigl| \int_{\Rbb^3} \dd z\;  |z+y|\; |  \alpha_*(z) \alpha_*(y-z)|\Bigr|^2 \nonumber \\
&\leq C \left( B^{-\nicefrac 12} \Vert \Psi \Vert_2^4 + D_1 B^{ \nicefrac 52 } \right) \, \Vert \alpha_*\Vert_{\nicefrac 43} \, \Vert \, |\cdot|\alpha_*\Vert_{\nicefrac 43}, \label{Nonlinearity_12} 
\end{align}
where the right side is finite by \eqref{Decay_of_alphastar}. Similarly, we see that $\Tcal_*^{(2)}$ is bounded by the right side of \eqref{Nonlinearity_12}.
%\begin{align*}
%\int_{\Rbb^3} \dd z \Bigl( \int_{\Rbb^3} \dy \; \bigl| |z+y|\alpha_*(-z)\alpha_*(z-y)\bigr|^2 \Bigr)^{\nicefrac 12} \leq \sqrt{2} \Vert \alpha_*\Vert_1 \Vert |\cdot|^{\nicefrac 12}\alpha_*\Vert_2 + \Vert |\cdot|^{\nicefrac 12}\alpha_*\Vert_1 \Vert \alpha_*\Vert_2.
%\end{align*}
%All in all, we obtain a constant $0 < C < \infty$ with $\Tcal_*^{(1)} \leq C \; \Vert\Psi\Vert_6^3 \; \Vert \Pi_X\Psi\Vert_2$. Using  \eqref{Magnetic_Sobolev}, this implies the final result $\Tcal_*^{(1)} \leq C \; \Vert \Pi_X\Psi\Vert_2^4$. 
%For $\Tcal_*^{(2)}$, only \eqref{Nonlinearity_11} needs to be adjusted by the new right side $C |z| \, \Vert \Pi\Psi\Vert_2^4$. Then, \eqref{Nonlinearity_12} is estimated in the same way by $C \Vert \, |\cdot|\alpha_*\Vert_{\nicefrac 43} \Vert \alpha_*\Vert_{\nicefrac 43}$.

\emph{Upper bound on $\Tcal_1$ and $\Tcal_2$ in \eqref{Nonlinearity_3}.} Bounds for $\Tcal_1$ and $\Tcal_2$ can be obtain along the same lines as the bound for $\Tcal_*^{(1)}$. We apply the same change of variables as above and use estimates similar to the ones in \eqref{Nonlinearity_13}. In case of $\Tcal_1$, the bound in \eqref{Nonlinearity_11} needs to be replaced by
\begin{align}
\Vert \Psi\Vert_6^2 \, \bigl\Vert \sin^2\bigl( \frac{z - y}{2}  \Pi\bigr) \Psi \bigr\Vert_6 \, \bigl\Vert \sin^2\bigl( \frac{z - y}{2}  \Pi\bigr) \Psi \bigr\Vert_2 \leq C \; \frac{|z-y|}{2} \; B^{-\nicefrac 32}\,  \Vert \Pi\Psi\Vert_2^4. \label{Nonlinearity_14}
\end{align}
Here, we used $\sin^2(x) \leq |x|$ and the operator inequality in  \eqref{ZPiX_inequality} to estimate the third factor. For the first and the second factor, we used
\begin{align*}
\sin^2\bigl( \frac{z-y}{4} \Pi\bigr) = - \frac{1}{4} \bigl( 2+ \e^{\i\frac{z-y}{2} \Pi} + \e^{-\i \frac{z-y}{2}\Pi}\bigr)
\end{align*}
and \eqref{Magnetic_Sobolev} or \eqref{NTB-NtildeTB_3}, respectively. A bound for $\Tcal_2$ can be proved analogously. The final estimate we obtain in this way reads
\begin{equation}
	\Tcal_1 + \Tcal_2 \leq C \left( B^{-\nicefrac 12} \Vert \Psi \Vert_2^4 + D_1 B^{ \nicefrac 52 } \right). 
	\label{eq:A2}
\end{equation}
In combination with \eqref{Nonlinearity_2}, \eqref{eq:A1}, and \eqref{Nonlinearity_12}, this proves \eqref{Nonlinearity_5}.
%To bound $\Tcal_2$, \eqref{Nonlinearity_14} needs to be replaced by
%\begin{align*}
%\bigl\Vert \sin^2\bigl( \frac{z}{2} \Pi\bigr) \Psi \bigr\Vert_6 \, \bigl\Vert \sin^2\bigl( \frac{z}{2} \Pi\bigr) \Psi \bigr\Vert_2 \, \bigl\Vert \cos\bigl( \frac{z-y}{2} \Pi\bigr) \Psi\bigr\Vert_6^2 \leq C \; \frac{|z|}{2} \; B^{-\nicefrac 32} \, \Vert \Pi\Psi\Vert_2^4.
%\end{align*}
%Here, we used $\cos(x) = \frac 12 (\e^{\i x} + \e^{-\i x})$ and \eqref{NTB-NtildeTB_3}. Then, we obtain the bound \eqref{Nonlinearity_12} with $|z|$ instead of $|z+y|$, as for $\Tcal_*^{(2)}$.

\emph{Step 3.} We denote $c:= \frac 1{2} \Vert \hat\alpha_*\Vert_4$, insert \eqref{Nonlinearity_1} and \eqref{Nonlinearity_5} into \eqref{Nonlinearity_8} and obtain
%\begin{align*}
%C\bigl( B^{\frac 14}\Vert \Psi\Vert_2^{\nicefrac 12} + B^{\frac 18}\bigr)  &\geq  C\bigl(\Vert \Psi\Vert_2^2B + B^{\frac 12} \bigr)^{\nicefrac 14} \geq (\Vert\alpha\Vert_4^4)^{\nicefrac 14} \\
%%
%&\hspace{-80pt}\geq \bigl( c \Vert \Psi\Vert_4^4 - C( B^{\frac 12}\Vert \Psi\Vert_2 + B^{\frac 14})^4\bigr)_+^{\nicefrac 14} - C\bigl( B^{\frac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18}\bigr) (1 + B^{\nicefrac 12}\Vert \Psi\Vert_2)^{\nicefrac 12}.
%\end{align*}
%Using the inequality $(|x|^4 - |y|^4)_+^{\nicefrac 14} \geq |x| - |y|$, which can be seen by explicitly expanding the $4\tho$ power of the right side, employing $|y|\leq |x|$, we get
\begin{align}
C B^{\frac 14}\Vert \Psi\Vert_2^{\nicefrac 12}  \geq c \Vert \Psi\Vert_4 - CB^{\frac 18} \Vert \Psi\Vert_2 - CB^{\frac 12}, \label{Nonlinearity_6}
\end{align}
which holds for $B$ small enough. For $\eta >0$ the left side is bounded from above by a constant times $\eta \Vert \Psi\Vert_2 + \eta^{-1} B^{\frac 12}$ and Hölder's inequality implies $\Vert \Psi\Vert_4 \geq \Vert \Psi\Vert_2$. 
%\begin{align*}
%\Vert \Psi\Vert_{L^4(Q_B)} \geq B^{\frac 38} \; \Vert \Psi\Vert_{L^2(Q_B)}.
%\end{align*}
Accordingly,
\begin{equation}
C \left( \eta \Vert \Psi\Vert_2 + \eta^{-1} B^{\frac 12} \right) \geq (c - CB^{\frac 18}) \Vert \Psi\Vert_2 - CB^{\frac 12}.
\label{eq:A3}
\end{equation}
%Thus,
%\begin{align*}
%\geq c' B^{\frac 38} \Vert \Psi\Vert_2 - CB^{\frac 18}.
%\end{align*}\yexycolor
When we choose $\eta$ and $B$ in \eqref{eq:A3} small enough, this proves the claim.
%
%
%
%We may assume without loss that the right side is nonnnegative because if not, the proof is finished. If this is so, then we infer $\Vert \Psi\Vert_2 \geq CB^{-\nicefrac 14}$ so that
%\begin{align*}
%\Vert \Psi\Vert_2^{\nicefrac 12} &\leq C\bigl( B^{-\frac 18} + B^{-\frac 14} \; \Vert \Psi\Vert_2^{-\nicefrac 12}\bigr) \leq CB^{-\frac 18}.
%\end{align*}
%This proves the claim.
\end{proof}

==> 3_Decomposition_degenerate_case/5.4_Proof_of_Thm_5.1.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Proof of Theorem \ref{Structure_of_almost_minimizers}}

The assumption \eqref{Second_Decomposition_Gamma_Assumption} in Theorem~\ref{Structure_of_almost_minimizers}, Corollary~\ref{cor:lowerbound}, Proposition~\ref{DEG:First_Decomposition_Result}, \ifthenelse{\equal\masterfile{Diss}}{as well as}{and} Lemma~\ref{Bound_on_psi} imply the decomposition $\alpha = A^*\Psi + \xi_0$, where $\Psi$ and $\xi_0$ in \eqref{DEG:Def_Psixi} obey
\begin{align}
\Vert \Psi\Vert_{\Hmag^1(Q_B)}^2 = B^{-1} \Vert \Psi\Vert_2^2 + B^{-2} \Vert \Pi\Psi\Vert_2^2 \leq C  \label{Psi_estimate}
\end{align}
and
\begin{align}
\Vert \xi_0\Vert_{\Hsymm}^2 \leq C B^2 \bigl( \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2 + D_1\bigr). \label{xi0_estimate}
\end{align}
Define
\begin{align}
\xi &:= \xi_0 + \bigl( \cos\bigl( \frac r2 \Pi_X\bigr) - 1\bigr) \alpha_*(r) \Psi(X). \label{xi_definition}
\end{align}
Then, \eqref{Second_Decomposition_alpha_equation} holds and we claim that $\xi$ satisfies \eqref{Second_Decomposition_Psi_xi_estimate}. To prove this, we estimate the second term in \eqref{xi_definition}. We use $1 - \cos(x) \leq |x|$ and \eqref{ZPiX_inequality} to bound
\begin{align*}
\bigl\Vert \bigl( \cos\bigl( \frac r2\Pi_X\bigr) - 1\bigr) \Psi \alpha_*\bigr\Vert_2^2 &\leq  C\; \Vert |\cdot|\alpha_*\Vert_2^2 \; \Vert \Pi\Psi\Vert_2^2 \leq CB^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2,
\end{align*}
where the right side is finite by the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar}. Using \eqref{PiXcos} additionally, we also have
\begin{align*}
\bigl\Vert \Pi_X \bigl( \cos\bigl( \frac r2\Pi_X\bigr) -1\bigr) \alpha_* \Psi \bigr\Vert_2^2 &\leq \bigl\Vert \bigl[ \cos\bigl(\frac r2\Pi_X\bigr) - 1 \bigr] \Pi_X \alpha_* \Psi \bigr\Vert_2^2 + \bigl\Vert \sin\bigl( \frac r2\Pi_X\bigr) \Bbold \wedge r \alpha_* \Psi \bigr\Vert_2^2\\
%
&\leq C \bigl(\Vert \Pi\Psi\Vert_2^2 + B^2 \Vert \Psi \Vert_2^2\bigr) \leq CB^3 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2
\end{align*}
holds. Finally, an application of \eqref{DEG:pr_cos} and \eqref{ZPiX_inequality} allows us to estimate
\begin{align*}
\bigl\Vert \pi_r \bigl( \cos\bigl( \frac r2\Pi_X\bigr) - 1\bigr) \Psi \alpha_*\bigr\Vert_2^2 &= \bigl\Vert \bigl[ \bigl( \cos\bigl(\frac r2\Pi_X\bigr) - 1\bigr) \tilde \pi_r + \frac \i 2 \sin\bigl( \frac r2\Pi_X\bigr)\Pi_X\bigr] \Psi \alpha_*\bigr\Vert_2^2 \\
%
&\leq C \bigl( \Vert \Pi\Psi\Vert_2^2 + B^2 \Vert \Psi \Vert_2^2\bigr) \leq CB^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2.
\end{align*}
This proves that $\xi$ obeys \eqref{Second_Decomposition_Psi_xi_estimate} and ends the proof of Theorem \ref{Structure_of_almost_minimizers}. 



==> 3_Decomposition_degenerate_case/Abstellgleis.tex <==
%auto-ignore  % for ArXiv to process correctly

%%By Lemma \ref{AAstar_Positive}, $AA^*$ commutes with $P_X^2$ and the operator on the right side of \eqref{MainTerm_LowerBound} is bounded from below by a constant times $P_X^2$. This lower bound will allow us to prove the bound on the magnetic gradient of $\Psi$ in Proposition \ref{First_Decomposition_Result}.
%
%\begin{bem}
%Let us replace $p_r^2$ on the left side of \eqref{MainTerm_5} by zero for the moment. In this case, the substitute of \eqref{MainTerm_5} reads
%\begin{align}
%\frac 12 \langle A^*\Psi, [U^*(1 - P)U + U(1 - P)U^* ] A^*\Psi\rangle = \langle \Psi , AA^*(1 - AA^*) \Psi\rangle. \label{Low_Energy_Operator}
%\end{align}
%It follows from Lemma~\ref{AAstar_Positive} that the operator $AA^*(1 - AA^*)$ is bounded from below by $P_X^2$ only for small values of $P_X^2$, which is not enough for the proof of Proposition \ref{First_Decomposition_Result}. This justifies the term ``low-energy operator'' for $1 - A^*A$, which we used earlier in the discussion below \eqref{Def_Astar}. The additional factor $1 + P_X^2$ in the first term on the right side of \eqref{MainTerm_5} compensate for the problematic behavior of \eqref{Low_Energy_Operator} for high energies. The expression on the right side of \eqref{Low_Energy_Operator} also appears in \cite{Hainzl2017}. 
%%and serves us with the appropriate bound \eqref{MainTerm_LowerBound}.
%\end{bem}
%%In becomes clear in the proof of Lemma \ref{MainTerm} that there is no easy way to drop any term for a lower bound until one arrives at \eqref{MainTerm_5}. Every positive term, which drops out on the way, has to account for a corresponding negative term and the network of correspondences is intricate. This is the reason why the proof of Lemma \ref{MainTerm} requires considerably more effort than \eqref{Low_Energy_Operator}.
%
%Before we give the proof of Lemma~\ref{MainTerm}, we prove two technical lemmas, which provide intertwining relations for various magnetic momentum operators with $U$ and linear combinations of $U$. A part of the relations in the first lemma can be found in \cite[Lemma~24]{Hainzl2017}.
%
%\begin{lem}
%\label{CommutationI}
%Let $p_r := -\i \nabla_r$, $p_r = p_r + \frac 12\Bbold \wedge r$ and $\tilde p_r$ and $P_X$ be given by \eqref{Magnetic_Momenta_COM}. For $U$ in \eqref{U_definition}, we have the following intertwining relations:
%\begin{align*}
%\begin{split}
%U P_X U^* &= P_X - \Bbold\wedge r,\phantom{\frac 12}  \\  U^* P_X U &= P_X + \Bbold\wedge r, \phantom{\frac 12}
%\end{split} &
%\begin{split}
%U p_r U^* &= \tilde p_r + \frac{1}{2}P_X, \\ U^* p_r U &= \tilde p_r - \frac{1}{2}P_X, \phantom{\frac 12}
%\end{split} &
%\begin{split}
%U \tilde p_r U^* &= p_r + \frac{1}{2}P_X, \\ U^* \tilde p_r U &= p_r - \frac{1}{2}P_X.
%\end{split}
%\end{align*}
%\end{lem}
%
%\begin{proof}
%Let us denote $P_X := -\i \nabla_X$. We use the fact that $r\cdot P_X$ commutes with $r\cdot (\Bbold \wedge X)$ to see that
%\begin{align}
%U^* = \e^{\i \frac \Bbold 2 \cdot X\wedge r} \; \e^{\i \frac r2P_X} \label{representation_Ustar}
%\end{align}
%holds. To prove the first intertwining relation with $P_X$, we compute
%\begin{align*}
%P_XU^* &= (P_X + \Bbold\wedge X)U^* =  \e^{\i \frac \Bbold 2 \cdot X\wedge r} \Bigl[ P_X - \frac 12 \Bbold \wedge r + \Bbold\wedge X\Bigr] \e^{\i \frac r2P_X} \\
%%
%&= U^* \Bigl[ P_X - \frac 12 \Bbold \wedge r + \Bbold \wedge \bigl(X -\frac r2\bigr)\Bigr] = U^* [ P_X - \Bbold \wedge r].
%\end{align*}
%Here we used that $f(X)\, \e^{\i \frac r2P_X} = \e^{\i \frac r2 P_X}\, f(X-\frac r2)$. The second intertwining relation with $P_X$ is obtained by replacing $r$ by $-r$. 
%
%Next we consider the first intertwining relation with $p_r$ and compute
%\begin{align*}
%p_r U^* &= \bigl( p_r + \frac 12\Bbold \wedge r\bigr) U^* = \e^{\i \frac \Bbold 2 \cdot X\wedge r}\Bigl[ p_r + (-\i)\i \frac 12 \Bbold \wedge X + \frac 12 \Bbold \wedge r\Bigr] \e^{\i \frac r2P_X} \\
%%
%&= U^* \Bigl[ p_r + \frac{P_X}{2} + \frac 12 \Bbold \wedge \bigl( X - \frac r2\bigr) + \frac 12 \Bbold \wedge r\Bigr] = U^* \Bigl[ \tilde p_r + \frac{P_X}{2}\Bigr].
%\end{align*}
%The remaining relations can be proved similarly and we skip the details.
%\end{proof}
%
%\begin{lem}
%\label{CommutationII}
%\begin{enumerate}[(a)]
%\item We have the following intertwining relations for $P_X$:
%\begin{align}
%P_X \cos\bigl( \frac r2 P_X\bigr) &=  \cos\bigl( \frac r2 P_X\bigr)P_X - \i \sin\bigl( \frac r2 P_X\bigr) \Bbold\wedge r, \label{PiXcos} \\
%%
%P_X \sin\bigl( \frac r2 P_X\bigr) &= \sin\bigl( \frac r2 P_X\bigr) P_X + \i \cos\bigl( \frac r2 P_X\bigr) \Bbold\wedge r. \label{PiXsin}
%\end{align}
%
%\item The operators $p_r$, $\tilde p_r$ and $p_r$ intertwine according to
%\begin{align}
%\tilde p_r \cos\bigl( \frac r2 P_X\bigr) &= \cos\bigl( \frac r2 P_X\bigr) p_r + \i \sin\bigl( \frac r2 P_X\bigr) \frac{P_X}{2}, \label{pirtilde_cos_pr}\\
%%
%\tilde p_r \cos\bigl( \frac r2 P_X\bigr) &= \cos\bigl( \frac r2 P_X\bigr)p_r + \i \frac{P_X}{2} \sin\bigl( \frac r2 P_X\bigr), \label{pirtilde_cos_pir}
%\end{align}
%and
%\begin{align}
%\tilde p_r \sin\bigl( \frac r2 P_X\bigr)  &= \sin\bigl( \frac r2 P_X\bigr) p_r - \i \cos\bigl( \frac r2 P_X\bigr) \frac{P_X}{2}, \label{pirtilde_sin_pr}\\
%%
%\tilde p_r \sin\bigl( \frac r2 P_X\bigr) &= \sin\bigl( \frac r2 P_X\bigr) p_r - \i \frac{P_X}{2} \cos\bigl( \frac r2 P_X\bigr) \label{pirtilde_sin_pir}
%\end{align}
%\end{enumerate}
%\end{lem}
%
%It will be useful in the proof of Lemma \ref{MainTerm} to have displayed both, \eqref{pirtilde_cos_pr} and \eqref{pirtilde_cos_pir} as well as \eqref{pirtilde_sin_pr} and \eqref{pirtilde_sin_pir}, even though they follow trivially from each other and \eqref{PiXcos} or \eqref{PiXsin}.
%
%\begin{proof}
%The proof is a direct consequence of the representations
%\begin{align}
%	\cos\bigl( \frac r2 P_X\bigr) &= \frac 12 (U^* + U), & \sin\bigl( \frac r2 P_X\bigr) &= \frac 1{2\i} (U^*-U),
%\end{align}
%and the intertwining relations in Lemma~\ref{CommutationII}. We omit the details.
%%For example, \eqref{PiXcos} is obtained from Lemma \ref{CommutationI} by computing
%%\begin{align*}
%%P_X\cos\bigl( \frac r2 P_X\bigr) &= \frac{1}{2}P_X (U^* + U) = \frac{1}{2} U^* (P_X - \Bbold \wedge r) + \frac{1}{2} U (P_X + \Bbold \wedge r)\\
%%&= \frac{1}{2} (U^* + U) P_X - \frac{1}{2} (U^* - U) \Bbold \wedge r.
%%\end{align*}
%%Furthermore, \eqref{pirtilde_sin_pr} is obtained by
%%\begin{align*}
%%\tilde p_r \sin\bigl( \frac r2 P_X\bigr) &= \frac{1}{2\i} U^*\bigl( p_r + \frac{P_X}{2} \bigr) - \frac{1}{2\i} U \bigl( p_r - \frac{P_X}{2}\bigr) = \sin\bigl( \frac r2 P_X\bigr) p_r - \i \cos\bigl( \frac r2 P_X\bigr) \frac{P_X}{2} .
%%\end{align*}
%%Applying \eqref{PiXcos} to this yields \eqref{pirtilde_sin_pir}. The other equations are proved analogously.
%\end{proof}

==> commands.tex <==
%auto-ignore  % for ArXiv to process correctly



==> source/BCS-Theory_Duke/0_0_Title.tex <==
%auto-ignore  % for ArXiv to process correctly
%
Microscopic Derivation of Ginzburg--Landau Theory \\ and the BCS Critical Temperature Shift \\ in a Weak Homogeneous Magnetic Field
%
%
%
%\begin{abstract}
%Starting from the Bardeen--Cooper--Schrieffer (BCS) free energy functional, we derive the Ginzburg--Landau functional
%for the case of a weak homogeneous magnetic field. We also provide an asymptotic formula for the BCS critical temperature as a function of the magnetic field. This extends the previous works \cite{Hainzl2012, Hainzl2014} of Frank, Hainzl, Seiringer and Solovej to the case of external magnetic fields with non-vanishing magnetic flux through the unit cell. 
%%	
%%We consider a large periodic sample of fermionic particles in a weak homogeneous magnetic field $\Bbold \in \mathbb{R}^3$ that are described by the Bardeen--Cooper--Schrieffer (BCS) functional of superconductivity. The temperature $T$ of the sample is chosen such that $(\Tc - T)/\Tc = D |\textbf{B}|$ with $D \in \mathbb{R}$, and where $\Tc$ denotes the critical temperature of the system in the absence of external fields. We show that the correction of the BCS free energy of the system at the order $\Bbold^2$ is given by Ginzburg--Landau (GL) theory. Moreover, the Cooper pair wave function of the system is, to leading order in $|\textbf{B}|$, given by $\alpha_*(x-y) \Psi((x+y)/2)$, where $\Psi$ is described by GL theory and $\alpha_*$ is related to the Cooper pair wave function of the system in the absence of external fields. We also show that the BCS critical temperature shift caused by the external magnetic field equals $| \Bbold |$ times a constant that is determined by linearized GL theory. This extends previous results in \cite{Hainzl2012} and \cite{Hainzl2014} to the case of a magnetic field with a non-zero flux through the unit cell. The main new ingredient of our proof are a-priori bounds for certain low energy states of the BCS functional that include the magnetic field.
%\end{abstract}
%
%
%Proposals for titles:
%
%\begin{enumerate}
%\item Microscopic Derivation of Ginzburg-Landau Theory II
%
%\item BCS Theory for the weak homogeneous magnetic field
%
%\item The BCS density functional, its critical temperature, and derivation of Ginzburg-Landau Theory for the weak homogeneous magnetic field
%
%\item The BCS critical temperature and microscopic derivation of Ginzburg-Landau Theory in a weak homogeneous magnetic field
%\end{enumerate}

==> source/BCS-Theory_General_Field/0_0_Title.tex <==
%auto-ignore  % for ArXiv to process correctly
%
Microscopic Derivation of Ginzburg--Landau Theory \\ and the BCS Critical Temperature Shift \\ in the Presence of Weak Macroscopic External Fields
%
%\maketitle
%
%
%Proposals for titles:
%
%\begin{enumerate}
%\item Microscopic Derivation of Ginzburg-Landau Theory II
%
%\item BCS Theory for the weak homogeneous magnetic field
%
%\item The BCS density functional, its critical temperature, and derivation of Ginzburg-Landau Theory for the weak homogeneous magnetic field
%
%\item The BCS critical temperature and microscopic derivation of Ginzburg-Landau Theory in a weak homogeneous magnetic field
%\end{enumerate}

==> source/BCS-Theory_General_Field/4_Proofs/4.2_Representation_Formula.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Proof of Proposition \ref{BCS functional_identity}}
\label{BCS functional_identity_proof_Section}

We recall the definitions of $\Delta(X, r) = -2\, V\alpha_*(r) \Psi(X)$ in \eqref{Delta_definition}, the Hamiltonian $H_\Delta$ in \eqref{HDelta_definition} and $\Gamma_\Delta = (1 + \e^{\beta H_\Delta})^{-1}$ in \eqref{GammaDelta_definition}. Throughout this section we assume that the function $\Psi$ in the definition of $\Delta$ is in $\Hmag^1(Q_h)$. From  Lemma~\ref{Gamma_Delta_admissible}, which is proved in Section~\ref{sec:proofofadmissibility} below, we know that $\Gamma_{\Delta}$ is an admissible BCS state in this case. We define the anti-unitary operator
\begin{align*}
\Jcal &:= \begin{pmatrix} 0 & J \\ -J & 0\end{pmatrix} %, & \text{where }  \quad \begin{split} J \colon L^2(\Rbb^3) &\ra L^2(\Rbb^3), \\ f &\mapsto \ov f,\end{split}
\end{align*}
with $J$ defined below \eqref{Gamma_introduction}. The operator $H_\Delta$ obeys the relation $\Jcal H_\Delta \Jcal^* = - H_\Delta$, which implies $\Jcal\Gamma_\Delta \Jcal^* = 1 - \Gamma_\Delta$. Using this and the cyclicity of the trace, we write the entropy of $\Gamma_{\Delta}$ as
\begin{align}
S(\Gamma_\Delta) = \frac 12 \Tr[ \varphi(\Gamma_\Delta)] \label{entropy matrix},
\end{align}
where $\varphi(x) := -[x\ln(x) + (1 - x) \ln(1-x)]$ for $0 \leq x \leq 1$.
%The operator evaluated in the BCS functional is not locally trace class, in general. However, its diagonal entries are. Therefore, we need to switch to a weaker form of trace.

In order to rewrite the BCS functional, it is useful to introduce a weaker notion of trace per unit volume. More precisely, we call a gauge-periodic operator $A$ acting on $L^2(\Rbb^3)\oplus L^2(\Rbb^3)$ weakly locally trace class if $P_0AP_0$ and $Q_0AQ_0$ are locally trace class, where
\begin{align}
P_0 = \begin{pmatrix} 1 & 0 \\ 0 & 0 \end{pmatrix} \label{P0}
\end{align}
and $Q_0 = 1-P_0$, and we define its weak trace per unit volume by
\begin{align}
\Tr_0 (A):= \Tr\bigl( P_0AP_0 + Q_0 AQ_0\bigr). \label{Weak_trace_definition}
\end{align}
If an operator is locally trace class then it is also weakly locally trace class but the converse need not be true. It is true, however, in case of nonnegative operators. If an operator is locally trace class then its weak trace per unit volume and its usual trace per unit volume coincide. 

Before their appearance in the context of BCS theory in \cite{Hainzl2012,Hainzl2014}, weak traces of the above kind appeared in \cite{HLS05,FLLS11}. In \cite[Lemma 1]{HLS05} it has been shown that if two weak traces $\Tr_P$ and $\Tr_{P'}$ are defined via projections $P$ and $P'$ then $\Tr_{P}(A) = \Tr_{P'}(A)$ holds for appropriate $A$ if $P - P'$ is a Hilbert--Schmidt operator. 

% the trace is independent of the used basis, if the difference P_0-P_0’ is HS.
%
%We remark that this notion has been used earlier in the literature, see \cite{HLS05}, \cite{FLLS11}. In particular,  shows that if $P_0 - P_0'$ is locally Hilbert-Schmidt for some $P_0'$ then the sets of operators that are weakly locally trace class with respect to the analogue of \eqref{Weak_trace_definition} given by $P_0'$ and \eqref{Weak_trace_definition} itself coincide.

Let $\Gamma$ be an admissible BCS state and recall the normal state $\Gamma_0$ in \eqref{Gamma0}. 
%Writing $\alpha_\Delta(X,r)$ for the kernel of $\alpha_\Delta$, t
In terms of the weak trace per unit volume, the BCS functional can be written as
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \hspace{-90pt}& \notag\\
%
&= \frac 12 \Tr\bigl[  (H_0\Gamma - H_0\Gamma_0) - T \varphi(\Gamma) + T \varphi(\Gamma_0)\bigr] - \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; V(r)\, |\alpha(X,r)|^2 \notag\\
%
&= \frac 12 \Tr_0\bigl[ (H_\Delta\Gamma_\Delta - H_0\Gamma_0) - T\varphi(\Gamma_\Delta) + T\varphi(\Gamma_0)\bigr] \label{kinetic energy} \\
%
&\hspace{55pt} + \frac 12 \Tr_0\bigl[ (H_\Delta \Gamma - H_\Delta \Gamma_\Delta) - T \varphi(\Gamma) + T\varphi(\Gamma_\Delta)\bigr] \label{relative_entropy_term}\\
%
&\hspace{55pt} - \frac 12 \Tr_0 \begin{pmatrix}
0 & \Delta \\ \ov \Delta & 0 \end{pmatrix} \Gamma - \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; V(r)\, |\alpha(X,r)|^2. \label{interaction-term}
\end{align}
Note that we added and subtracted the first term in \eqref{kinetic energy} and that we added and subtracted the first term in \eqref{interaction-term} to replace the Hamiltonian $H_0$ in \eqref{relative_entropy_term} by $H_\Delta$. The operators inside the traces in \eqref{kinetic energy} and \eqref{relative_entropy_term} are not necessarily locally trace class, which is the reason we introduce the weak local trace. We also note that \eqref{relative_entropy_term} equals $\frac T2$ times the relative entropy $ \Hcal_0(\Gamma, \Gamma_\Delta)$ of $\Gamma$ with respect to $\Gamma_{\Delta}$, defined in \eqref{Relative_Entropy}. 
%Furthermore, , 
%
%, recall that $\Gamma_\Delta = (1 + \e^{\beta H_\Delta})^{-1}$ and note that
%\begin{align*}
% \beta H_\Delta  +  \ln(\Gamma_\Delta) = -\ln ( \e^{-\beta H_\Delta} (1 + \e^{\beta H_\Delta})) = -\ln (1 +\e^{-\beta H_\Delta}) = \ln (1 - \Gamma_\Delta).
%\end{align*}
%This implies
%\begin{align*}
%\beta H_\Delta  + \ln(\Gamma) = \ln(1 - \Gamma_\Delta) + \ln(\Gamma) - \ln(\Gamma_\Delta).
%\end{align*}
%Inserting this into \eqref{relative_entropy}, we conclude that
%\begin{align*}
%(\beta H_\Delta  + \ln(\Gamma))\,\Gamma - (\beta H_\Delta + \ln(\Gamma_\Delta)) \, \Gamma_\Delta + (1 - \Gamma)\ln(1 - \Gamma) - (1 - \Gamma_\Delta) \ln(1 - \Gamma_\Delta) &=  \\
%%
%&\hspace{-350pt} = \Gamma\ln(1- \Gamma_\Delta)- \Gamma_\Delta\ln(1 - \Gamma_\Delta)  + \Gamma(\ln(\Gamma) - \ln(\Gamma_\Delta))\\
%%
%&\hspace{-200pt} + (1 - \Gamma) \ln(1 - \Gamma) - (1 - \Gamma_\Delta)\ln(1 - \Gamma_\Delta)\\
%%
%&\hspace{-350pt} = \Gamma (\ln(\Gamma) - \ln(\Gamma_\Delta)) + (1- \Gamma) (\ln(1 - \Gamma) - \ln(1 - \Gamma_\Delta)) = \Hcal_0(\Gamma, \Gamma_\Delta).
%\end{align*}
%

The first term in \eqref{interaction-term} can be written as
\begin{align}
-\frac  12\Tr_0 \begin{pmatrix} 0 & \Delta \\ \ov \Delta & 0\end{pmatrix} \Gamma &
%= -\frac  12\Tr_0\begin{pmatrix} \Delta \ov \alpha & \Delta (1 - \ov \gamma) \\ \ov \Delta \gamma & \ov \Delta \alpha\end{pmatrix}
=2\Re \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; (V\alpha_*)(r) \Psi(X) \; \ov \alpha(X,r). \label{additional-term}
\end{align}
The integrands in \eqref{interaction-term} and \eqref{additional-term} are equal to
\begin{equation*}
-|\alpha(X,r)|^2 + 2\Re\alpha_*(r)\Psi(X) \; \ov \alpha (X,r)  = -\bigl|\alpha(X, r) - \alpha_*(r)\Psi(X)\bigr|^2 + \bigl|\alpha_*(r)\Psi(X)\bigr|^2. 
\end{equation*}
To rewrite \eqref{kinetic energy} we need the following identities, whose proofs are straightforward computations:
\begin{align}
\Gamma_\Delta &= \frac 12 - \frac 12 \tanh\bigl( \frac \beta 2 H_\Delta\bigr), & \ln(\Gamma_\Delta) &= -\frac \beta 2 H_\Delta - \ln\bigl( 2\cosh\bigl( \frac \beta 2 H_\Delta\bigr)\bigr), \notag\\
%
1 - \Gamma_\Delta &= \frac 12 + \frac 12 \tanh\bigl( \frac\beta 2H_\Delta\bigr), & \ln(1 - \Gamma_\Delta) &= \frac\beta 2H_\Delta - \ln\bigl( 2\cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr).  \label{GammaRelations}
\end{align}
Eq.~\eqref{GammaRelations} implies
\begin{align}
\Gamma_\Delta \ln(\Gamma_\Delta) + (1-\Gamma_\Delta)\ln(1-\Gamma_\Delta) =  -\ln\bigl( 2\cosh\bigl( \frac \beta 2H_\Delta\bigr) \bigr) + \frac{\beta}{2} H_\Delta \tanh\bigl( \frac\beta 2 H_\Delta\bigr)\bigr),
\label{GammaDeltaRelation}
\end{align}
as well as
\begin{align*}
\beta H_\Delta \Gamma_\Delta - \varphi(\Gamma_\Delta) &= \frac{\beta}{2} H_\Delta - \ln \bigl( 2 \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr).
\end{align*}
This allows us to rewrite \eqref{kinetic energy} as
\begin{align}
\frac 1{2\beta}\, \Tr_0\bigl[ (\beta H_\Delta\Gamma_\Delta - \beta H_0\Gamma_0) - \varphi(\Gamma_\Delta) + \varphi(\Gamma_0)\bigr] & \notag \\
%
&\hspace{-180pt}= \frac 14 \Tr_0 \bigl[ H_\Delta - H_0\bigr] - \frac 1{2\beta}\Tr_0 \bigl[ \ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac  \beta 2H_0\bigr)\bigr)\bigr]. \label{trace-difference-ln}
\end{align}
We note that $H_\Delta - H_0$ is weakly locally trace class and that its weak trace equals $0$. This, in particular, implies that the second term on the right side of \eqref{trace-difference-ln} is weakly locally trace class. To summarize, our intermediate result reads
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) \hspace{-60pt} & \notag\\
%
&= -\frac 1{2\beta}\Tr_0 \bigl[ \ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac  \beta 2H_0\bigr)\bigr)\bigr] \notag\\
%
&\hspace{30pt} + \Vert\Psi \Vert_{\Lmag^2(Q_B)} \, \langle \alpha_*, V\alpha_*\rangle_{L^2(\Rbb^3)} \notag \\
%
&\hspace{30pt} +\frac{T}{2} \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; V(r) \, \bigl|\alpha(X,r) - \alpha_*(r)^t \Psi(X)\bigr|^2.  \label{BCS functional-intermediate}
\end{align}

In order to compute the first term on the right side of \eqref{BCS functional-intermediate}, we need Lemma~\ref{BCS functional_identity_Lemma} below. It is the main technical novelty of our trial state analysis and should be compared to the related part in the proof of \cite[Theorem~2]{Hainzl2012}. The main difference between our proof of Lemma~\ref{BCS functional_identity_Lemma} and the relevant parts of the proof of \cite[Theorem~2]{Hainzl2012} is that we use the product representation of the hyperbolic cosine in \eqref{cosh-Product} below instead of a Cauchy integral representation of the function $z \mapsto \ln(1+e^{-z})$. In this way we obtain better decay properties in the subsequent resolvent expansion, which simplifies the analysis considerably. 

As already noted above, the admissibility of $\Gamma_{\Delta}$ implies that the difference between the two operators in the first term on the right side of \eqref{BCS functional-intermediate} is weakly locally trace class. We highlight that this is a nontrivial statement because each of the two operators separately does not share this property. We also highlight that our proof of Lemma~\ref{BCS functional_identity_Lemma} does not require this as an assumption, it implies the statement independently.

In combination with \eqref{BCS functional-intermediate}, Lemma~\ref{BCS functional_identity_Lemma} below proves Proposition~\ref{BCS functional_identity}.  Before we state the lemma, we recall the definitions of the operators $L_{T, \Abold, W}$ and $N_{T, \Abold, W}$ in \eqref{LTAW_definition} and \eqref{NTAW_definition}, respectively.

%To condude the proof of , we prove in the next result, Lemma \ref{BCS functional_identity_Lemma}, that  Proposition \ref{BCS functional_identity} then follows from and Lemma \ref{BCS functional_identity_Lemma}. 

\begin{lem}
\label{BCS functional_identity_Lemma}
Let $V\alpha_*\in L^{\nicefrac 65}(\Rbb^3)\cap L^2(\Rbb^3)$. For any $B>0$, any $\Psi\in \Hmag^1(Q_B)$, and any $T>0$, the operator
\begin{align*}
\ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr) 
\end{align*}
is weakly locally trace class and its weak local trace equals
\begin{align}
-\frac 1{2\beta} \Tr_0\Bigl[ \ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr) \Bigr] & \notag\\
%
&\hspace{-140pt}= -\frac 14\langle \Delta, L_{T, \Abold, W}\Delta\rangle + \frac 18 \langle \Delta, N_{T, \Abold, W}(\Delta)\rangle + \Tr\Rcal_{T, \Abold, W}^{(1)}(\Delta). \label{BCS functional_identity_Lemma_eq2}
\end{align}
The operator $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$ is locally trace class and its trace norm satisfies the bound
\begin{align*}
\Vert \Rcal_{T, \Abold, W}^{(1)}(\Delta) \Vert_1 &\leq C\; T^{-5} \; B^3 \; \Vert \Psi\Vert_{\Hmag^1(Q_B)}^6.
\end{align*}
\end{lem}

%Proposition \ref{BCS functional_identity} now follows from \eqref{BCS functional-intermediate} and \eqref{BCS functional_identity_Lemma_eq2}. 
%Proposition \ref{BCS functional_identity_rough} is obtained by setting $\Gamma= \Gamma_\Delta$ in \eqref{BCS functional-intermediate} and combining this with \eqref{BCS functional_identity_Lemma_eq1}.

%A desirable approach for the proof of Lemma \ref{BCS functional_identity_Lemma} would be to exploit the fact that the derivative of $\ln(\cosh(x))$ equals $\tanh(x)$ and use the representation \eqref{tanh-expansion}. Since $H_\Delta$ and $H_0$ do not commute, in general, the proof is a noncommutative analogue of this idea.

\begin{proof}[Proof of Lemma \ref{BCS functional_identity_Lemma}]
We recall the Matsubara frequencies in \eqref{Matsubara_frequencies} and write the hyperbolic cosine in terms of the following product expansion, see \cite[Eq. (4.5.69)]{Handbook}, 
\begin{align}
\cosh\bigl(\frac \beta 2x\bigr) &= \prod_{k=0}^\infty \Bigl( 1 + \frac{x^2}{\omega_k^2}\Bigr). %= \prod_{k=0}^\infty \bigl( 1 + \i \, \frac{x}{\omega_k}\bigr)\bigl( 1 - \i \, \frac{x}{\omega_k}\bigr). 
\label{cosh-Product}
\end{align}
We have
\begin{align*}
0 &\leq \sum_{k= 0}^\infty \ln \bigl( 1 + \frac{x^2}{\omega_k^2}\bigr) = \ln \bigl( \cosh\bigl( \frac \beta 2 x\bigr)\bigr) \leq \frac\beta 2 \; |x|, & x &\in \Rbb,
\end{align*}
and accordingly
\begin{align*}
\ln\bigl( \cosh\bigl( \frac{\beta}{2} H_\Delta\bigr)\bigr) =  \sum_{k=0}^\infty \ln \bigl( 1+ \frac{H_\Delta^2}{\omega_k^2}\bigr) %= \sum_{k=0}^\infty \ln \bigl( 1 + \i \frac{H_\Delta}{\omega_k}\bigr) + \ln\bigl( 1 - \i \frac{H_\Delta}{\omega_k}\bigr) 
%
\end{align*}
holds in a strong sense on the domain of $|H_\Delta|$. Since $\Delta$ is a bounded operator by Lemma \ref{Schatten_estimate}, the domains of $|H_\Delta|$ and $|H_0|$ coincide. The identity 
\begin{align}
\ln\bigl( \cosh\bigl( \frac{\beta}{2} H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac{\beta}{2} H_0\bigr)\bigr)  =  \sum_{k=0}^\infty \bigl[ \ln \bigl( \omega_k^2+ H_\Delta^2 \bigr) - \ln \bigl( \omega_k^2 + H_0^2 \bigr) \bigr] \label{BCS functional_identity_Lemma_1}
\end{align}
therefore holds in a strong sense on the domain of $|H_0|$. Elementary arguments show that
\begin{align}
\ln\bigl( \omega^2 + H_\Delta^2\bigr) - \ln\bigl(\omega^2 + H_0^2\bigr) = -\lim_{R\to\infty} \int_\omega^R \dd u \; \Bigl[\frac{2u}{u^2 + H_\Delta^2} - \frac{2u }{u^2 + H_0^2}\Bigr] \label{ln-integral}
\end{align}
holds for $\omega>0$ in a strong sense on the domain of $\ln(1+|H_0|)$. Therefore, by \eqref{BCS functional_identity_Lemma_1} and \eqref{ln-integral}, we have
%We claim that the integral on the right side also converges in the norm topology of $\Scal^\infty$, which, in particular implies that the operator on the left side is a bounded. To see this, we intend to show that the right side of \eqref{ln-integral} is a Cauchy sequence The limit of the operator on the right side exists in .
\begin{align}
\ln\bigl( \cosh\bigl(\frac \beta 2 H_\Delta\bigr)\bigr) - \ln\bigl( \cosh\bigl( \frac \beta 2 H_0\bigr)\bigr) & \notag \\
%
&\hspace{-100pt}= -\i \sum_{k=0}^\infty \int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_\Delta } - \frac{1}{\i u - H_0} + \frac{1}{\i u + H_\Delta} - \frac{1}{\i u + H_0}\Bigr] \label{lncosh-difference}
\end{align}
in a strong sense on the domain of $|H_0|$. By a slight abuse of notation, we have incorporated the limit in \eqref{ln-integral} into the integral.
%Here the integral $\int_{\omega_k}^\infty$ has to be understood as the limit in \eqref{ln-integral}.
%
%
%
%
%
%Since $\frac \dd\dx \ln(\cosh(x)) = \tanh(x)$, we may write
%\begin{align}
%\ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr)  &= \frac \beta 2 \int_0^1 \dt \; \tanh\bigl( \frac\beta 2H_{t\Delta} \bigr) \; \begin{pmatrix} 0 & \Delta \\ \ov \Delta & 0\end{pmatrix} \label{Trace_Class_1}.
%\end{align}
%Applying the expansion of $\tanh$ \eqref{tanh-expansion} with $H_\Delta$ replaced by $H_{t\Delta}$ and combining this with \eqref{Trace_Class_1}, we infer
%\begin{align*}
%\ln\bigl( \cosh\bigl( \frac \beta 2H_\Delta\bigr)\bigr) - \ln \bigl( \cosh\bigl( \frac \beta 2H_0\bigr)\bigr) = \int_0^1 \dt \; \sum_{n\in \Zbb} \frac{1}{\i \omega_n - H_{t\Delta}} \begin{pmatrix} 0 & \Delta \\ \ov \Delta & 0\end{pmatrix}.
%\end{align*}
%
%
%
%
%

In the next step we use the resolvent expansion
\begin{align}
(z-H_\Delta)^{-1} = (z-H_0)^{-1} + (z-H_0)^{-1} \; (H_\Delta - H_0)\; (z-H_\Delta)^{-1} \label{Resolvent_Equation}
\end{align}
to see that the right side of \eqref{lncosh-difference} equals
\begin{align*}
\Ocal_1 + \Dcal_2 + \Ocal_3 + \Dcal_4 + \Ocal_5 - 2\beta \,  \Rcal_{T, \Abold, W}^{(1)}(\Delta),
\end{align*}
with two diagonal operators $\Dcal_2$ and $\Dcal_4$, three offdiagonal operators $\Ocal_1$, $\Ocal_3$ and $\Ocal_5$ and a remainder term $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$. The index of the operators reflects the number of $\delta$ matrices appearing in their definition. The diagonal operators $\Dcal_2$ and $\Dcal_4$ are given by
\begin{align*}
\Dcal_2 &:=  -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} + \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0} \Bigr] , \\
%
\Dcal_4 &:=  -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{120pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr]
\end{align*}
and the offdiagonal operators read
\begin{align*}
\Ocal_1 &:= -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} + \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr], \\
%
\Ocal_3 &:= -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{85pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr],\\
%
\Ocal_5 &:=  -\i \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{85pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr].
\end{align*}
Since the operators $\Ocal_1$, $\Ocal_3$, and $\Ocal_5$ are offdiagonal, they are weakly locally trace class and their weak local trace equals $0$. We also note that the operator $\Ocal_1$ is not necessarily locally trace class, which is why we need to work with the weak local trace. The operator $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$ is defined by
\begin{align*}
\Rcal_{T, \Abold, W}^{(1)}(\Delta) & \\
%
&\hspace{-50pt}:= \frac{\i}{2\beta} \sum_{k=0}^\infty\int_{\omega_k}^\infty \dd u \; \Bigl[\frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_\Delta}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0}\delta \frac{1}{\i u - H_0} \\
%
&\hspace{40pt}+ \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_\Delta}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\delta \frac{1}{\i u + H_0}\Bigr].
\end{align*}

%First, we argue that the operators $\Ocal_1$, $\Ocal_2$, and $\Ocal_3$ are indeed offdiagonal. We have
%\begin{align*}
%\frac{1}{\i u \pm H_0} \, \delta = \begin{pmatrix} \frac{1}{\i u \pm \hfrak_h} \\ & \frac{1}{\i u \mp \ov{ \hfrak_h}}
%\end{pmatrix} \begin{pmatrix} &\Delta \\ \ov \Delta \end{pmatrix} = \begin{pmatrix} & \frac{1}{\i u \pm \hfrak_h} \, \Delta \\ \frac{1}{\i u \mp \ov{\hfrak_h}}\, \ov \Delta\end{pmatrix}
%\end{align*}
%and

It remains to compute the traces of $\Dcal_2$ and $\Dcal_4$, and to estimate the trace norm of $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$. We first consider $\Dcal_2$ and use Hölder's inequality in \eqref{Schatten-Hoelder} to estimate
\begin{align}
  \Bigl\Vert \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0}\Bigr\Vert_1 &\leq \Bigl\Vert \frac{1}{\i u \pm H_0} \Bigr\Vert_\infty^3 \; \Vert \delta\Vert_2^2 = \frac{2}{u^3} \; \Vert \Delta\Vert_2^2.
\end{align}
Therefore, Lemma \ref{Schatten_estimate} shows that the combination of series and integral defining $\Dcal_2$ converges absolutely in local trace norm.
%In combination with \eqref{Matsubara_frequencies} and an application of Lemma~\ref{Schatten_estimate}, this proves 
%\begin{equation}
%	\sum_{k=0}^\infty \int_{\omega_k}^\infty \dd u \Bigl\Vert \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0} \delta \frac{1}{\i u \pm H_0}\Bigr\Vert_1 \leq \frac{4 \Vert \Psi \Vert_2^2}{\pi^2 T^2} \sum_{k=0}^{\infty} \frac{1}{(2k+1)^2}.
%	\label{eq:A6}
%\end{equation}
In particular, $\Dcal_2$ is locally trace class and we may arbitrarily interchange the trace with the sum and the integral to compute its trace. We do this, use the cyclicity of the trace, and obtain
\begin{equation}
\Tr \Dcal_2 =  -\i \sum_{k=0}^\infty \int_{\omega_k}^\infty \dd u \; \Tr\Bigl[\Bigl(\frac{1}{\i u - H_0}\Bigr)^2 \delta \frac{1}{\i u - H_0}\delta + \Bigl(\frac{1}{\i u + H_0}\Bigr)^2\delta \frac{1}{\i u + H_0}\delta \Bigr]. \label{eq:A7}
\end{equation}
Integration by parts shows
\begin{align*}
\int_{\omega_k}^\infty \dd u \; \Bigl(\frac{1}{\i u \pm H_0}\Bigr)^2 \delta \frac{1}{\i u \pm H_0}\delta &= -\i\; \frac{1}{\i \omega_k \pm H_0} \delta \frac{1}{\i \omega_k \pm H_0} \delta \\
%
&\hspace{80pt}- \int_{\omega_k}^\infty \dd u \; \frac{1}{\i u \pm H_0} \delta \Bigl( \frac{1}{\i u \pm H_0}\Bigr)^2 \delta,
\end{align*}
and another application of the cyclicity of the trace yields
\begin{align}
\Tr \int_{\omega_k}^\infty \dd u \; \Bigl(\frac{1}{\i u \pm H_0}\Bigr)^2 \delta \frac{1}{\i u \pm H_0}\delta &= -\frac \i 2 \; \Tr \frac{1}{\i \omega_k \pm H_0} \delta \frac{1}{\i \omega_k \pm H_0} \delta. \label{BCS functional_identity_Lemma_2}
\end{align}
Note that
\begin{align}
\frac{1}{\i \omega_k \pm H_0}\,  \delta\,  \frac{1}{\i \omega_k \pm H_0} \, \delta 
%
&= \begin{pmatrix}
\frac{1}{\i \omega_k \pm \hfrak_h} \, \Delta \frac{1}{\i \omega_k \mp \ov{\hfrak_h}} \, \ov \Delta \\ & \frac{1}{\i \omega_k \mp \ov{\hfrak_h}}\,  \ov \Delta \frac{1}{\i \omega_k \pm \hfrak_h} \, \Delta
\end{pmatrix}. \label{Calculation-entry}
\end{align}
We combine this with \eqref{eq:A7} and \eqref{BCS functional_identity_Lemma_2} and summarize the cases $\pm$ into a single sum over $n\in \Zbb$. This yields
\begin{align*}
-\frac{1}{2\beta}\Tr \Dcal_2 &= \frac{1}{2\beta}\sum_{n\in \Zbb} \Bigl\langle \Delta, \frac{1}{\i\omega_n - \hfrak_h} \Delta \frac{1}{\i\omega_n + \ov{\hfrak_h}}\Bigr\rangle =  - \frac 14\langle \Delta, L_{T, \Abold, W}\Delta\rangle,
\end{align*}
where $L_{T, \Abold, W}$ is the operator defined in \eqref{LTAW_definition}.

We argue as above to see that the integrand in the series and integral defining $\Dcal_4$ is bounded by $C \Vert \Delta\Vert_4^4 \, u^{-5}$. Moreover, we have $\Vert \Delta\Vert_4^4 \leq CB^2 \Vert V\alpha_*\Vert_{\nicefrac 43}^4 \Vert \Psi\Vert_{\Hmag^1(Q_B)}^4$ by \eqref{Magnetic_Sobolev} and Lemma \ref{Schatten_estimate}. Therefore, $\Dcal_4$ is absolutely local trace norm convergent as well. The trace of $\Dcal_4$ is computed similar to that of $\Dcal_2$. With $N_{T, \Abold, W}$ defined in \eqref{NTAW_definition}, the result reads
\begin{align}
-\frac{1}{2\beta}\Tr \Dcal_4 &= \frac 18\langle \Delta, N_{T, \Abold, W}(\Delta)\rangle. \label{NTB_size_bound_2}
\end{align} 
In case of $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$, we bound the trace norm of the operator inside the integral by $u^{-7}\Vert \Delta\Vert_6^6$. Using \eqref{Magnetic_Sobolev} and Lemma~\ref{Schatten_estimate}, we estimate the second factor by a constant times $\Vert V\alpha_*\Vert_{\nicefrac 65}^6 B^{-3}\Vert \Pi\Psi\Vert_2^6 \leq CB^3 \Vert \Psi\Vert_{\Hmag^1(Q_B)}^6$. Finally, integration over $u$ yields the term $6\pi^{-6} T^{-6} (2k+1)^{-6}$, which is summable in $k$. This proves the claimed bound for the trace norm of $\Rcal_{T, \Abold, W}^{(1)}(\Delta)$.
\end{proof}

==> source/BCS-Theory_General_Field/5_Structure_of_Low-Energy_States/5.2_First_decomposition_result.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The first decomposition result}

The proof of Theorem~\ref{Structure_of_almost_minimizers} is based on Corollary~\ref{cor:lowerbound} and is given in two steps. In the first step we drop the second term on the left side of \eqref{Lower_Bound_A_2} for a lower bound, and investigate the implications of the resulting inequality for $\alpha$. The result of the corresponding analysis is summarized in Proposition~\ref{First_Decomposition_Result} below. The second term on the left side of \eqref{Lower_Bound_A_2} is used later in Lemma~\ref{Bound_on_psi}. 

\begin{prop}
\label{First_Decomposition_Result}
Given $D_0, D_1 \geq 0 $, there is $B_0>0$ with the following properties. If, for some $0< B\leq B_0$, the wave function $\alpha\in \Lsymm$ satisfies
\begin{align}
\langle \alpha , [U^* (1-P)(1 + \pi_r^2)(1-P)U + U (1-P) (1 + \pi_r^2)(1-P)U^*] \alpha \rangle & \leq D_0 B \Vert \alpha\Vert_2^2 + D_1 B^2 , \label{First_Decomposition_Result_Assumption}
\end{align}
then there are $\Psi\in \Hmag^1(Q_B)$ and $\xi_0\in \Hsymm$ such that
\begin{align}
\alpha(X,r) =  \alpha_*(r)^t \cos\bigl( \frac r2 \cdot \Pi_X\bigr) \Psi(X) + \xi_0(X,r) \label{First_Decomposition_Result_Decomp}
\end{align}
with
\begin{align}
\langle \Psi, \Pi^2 \Psi\rangle + \Vert \xi_0\Vert_{\Hsymm}^2 \leq C\bigl( B \Vert \Psi \Vert_2^2 + D_1 B^2 \bigr).  \label{First_Decomposition_Result_Estimate}
\end{align}
%and
%\begin{align}
%C \Vert \alpha\Vert_2^2 \geq \Vert \Psi\Vert_2^2 \geq (1- C  B)\; \Vert \alpha\Vert_2^2 - CB^{\nicefrac 12}. \label{First_Decomposition_Result_Estimate_psi}
%\end{align}
\end{prop}
Before we give the proof of the a priori estimates in Proposition \ref{First_Decomposition_Result}, we define the decomposition, discuss the idea behind it, which originates from \cite{Hainzl2017}, and make the connection to other existing works. For this purpose, let the operator $A \colon \Lsymm \ra \Lmag^2(Q_B)$ be given by
\begin{align}
(A\alpha)(X) := \int_{\Rbb^3} \dd r\; \ov{\alpha_*(r)} \; \cos\bigl( \frac r2\cdot \Pi_X\bigr) \alpha(X,r). \label{Def_A}
\end{align}
A short computation shows that its adjoint $A^*\colon \Lmag^2(Q_B) \ra \Lsymm$ is given by
\begin{align}
(A^*\Psi) (X,r) = \alpha_*(r)^t \cos\bigl( \frac r2\cdot \Pi_X\bigr) \Psi(X). \label{Def_Astar}
\end{align}
We highlight that this is the form of the first term in \eqref{First_Decomposition_Result_Decomp}. For a given Cooper pair wave function $\alpha$, we use these operators to define the two functions $\Psi$ and $\xi_0$ by
\begin{align}
	\Psi &:= (AA^*)^{-1} A\alpha, & \xi_0 &:= \alpha - A^*\Psi. \label{Def_Psixi}
\end{align}
Lemma~\ref{AAstar_Positive} below guarantees that $AA^*$ is invertible, and we readily check that  \eqref{First_Decomposition_Result_Decomp} holds with these definitions. Moreover, this decomposition of $\alpha$ is orthogonal in the sense that $\langle A^* \Psi, \xi_0 \rangle = 0$ holds. The claimed orthogonality follows from
\begin{align}
	A\xi_0 =0, \label{fundamental_property}
\end{align}
which is a direct consequence of \eqref{Def_Psixi}. In the following we motivate our choice for $\Psi$ and $\xi_0$ and comment on its appearance in the literature.

The decomposition of $\alpha$ is motivated by the minimization problem for the low-energy operator $2 -UPU^* - U^*PU$, that is, the operator in \eqref{First_Decomposition_Result_Assumption} with $\pi_r^2$ replaced by zero. The operators $UPU^*$ and $U^*PU$ act as $A^*A$ on the space $\Lsymm$ of reflection symmetric functions in the relative coordinate. If $\Pi$ is replaced by $P_X$ then $A^*A$ can be written as 
\begin{equation}
	A^* A \cong \int^{\oplus}_{[0,\sqrt{ 2 \pi B}]^3} \mathrm{d}P_X \; | a_{P_X} \rangle \langle a_{P_X} |, \label{eq:directintegralA}
\end{equation}
with $| a_{P_X} \rangle \langle a_{P_X} |$ the orthogonal projection onto the function $a_{P_X}(r) = \cos(r/2 \cdot P_X) \alpha_*(r)$. Here the variable $P_X$ is the dual of the center-of-mass coordinate $X$ in the sense of Fourier transformation and $r$ denotes the relative coordinate. That is, the function $a_{P_X}(r)$ minimizes $1-A^* A$ in each fiber, whence it is the eigenfunction with respect to the lowest eigenvalue of $1 - A^* A = 1 - (UPU^* + U^*PU)/2$. This discussion should be compared to \cite[Eq. (5.47)]{Hainzl2012} and the discussion before Lemma~20 in \cite{ProceedingsSpohn}.

If $B$ is present in the magnetic momentum operator $\Pi$ the above picture changes because the components of $\Pi$ cannot be diagonalized simultaneously (they do not commute), and hence \eqref{eq:directintegralA} has no obvious equivalent in this case. The decomposition of $\alpha$ in terms of the operators $A$ and $A^*$ above has been introduced in \cite{Hainzl2017} in order to study the operator $1 - V^{\nicefrac 12} L_{T,B} V^{\nicefrac 12}$ with $L_{T,B}$ in \eqref{LTB_definition}, see also the discussion below Theorem~\ref{Calculation_of_the_GL-energy}. The situation in this work is comparable to our case with $\pi_r^2$ replaced by zero in \eqref{First_Decomposition_Result_Assumption}. Our analysis below shows that the ansatz \eqref{Def_Psixi} is useful even if the full range of energies is considered, that is, if $\pi_r^2$ is present in \eqref{First_Decomposition_Result_Assumption}. 

In the following lemma we collect useful properties of the operator $A A^*$. It should be compared to \cite[Lemma~27]{Hainzl2017}.
%
%
%
%That is, the function $f$ is the eigenfunction w.r.t. the lowest eigenvalue 
%of $1 - A^* A$, which motivates the decomposition. See also the discussion before Lemma~20 in \cite{ProceedingsSpohn} and \cite[Eq. (5.47)]{Hainzl2012}. In the case of a constant magnetic field, this reasoning is not  
%
%The above decomposition in terms of the operators $A$ and $A^*$ has been introduced in the case with a constant magnetic case in \cite{Hainzl2017}.
%
%
%The generalization of the above decomposition using the operators $A$ and $A^*$, was first introduced in \cite{Hainzl2017}. 
%We use this construction as a candidate for an approximate minimizer of the whole operator in \eqref{First_Decomposition_Result_Assumption} and set
%\begin{align}
%\Psi &:= (AA^*)^{-1} A\alpha, & \xi_0 &:= \alpha - A^*\Psi. \label{Def_Psixi}
%\end{align}
%By Lemma \ref{AAstar_Positive} below, $AA^*$ is indeed invertible. Then, \eqref{First_Decomposition_Result_Decomp} holds and the immediate and fundamental property
%\begin{align}
%A\xi_0 =0 \label{fundamental_property}
%\end{align}
%resulting from \eqref{Def_Psixi} implies that $A^*\Psi + \xi_0$ is an  orthogonal decomposition of $\alpha$ with respect to the scalar product in $\Lsymm$.

\begin{lem}
\label{AAstar_Positive}
The operators
\begin{align*}
AA^* &= \int_{\Rbb^3} \dd r\; \ov{\alpha_*(r)} \alpha_*(r)^t \cos^2\bigl( \frac{r}{2} \cdot \Pi\bigr), & 1-AA^* &= \int_{\Rbb^3} \dd r \; \ov{\alpha_*(r)} \alpha_*(r)^t \sin^2\bigl( \frac r2 \cdot \Pi\bigr) 
\end{align*}
on $\Lmag^2(Q_B)$ are both bounded nonnegative matrix-valued functions of $\Pi^2$ and satisfy the following properties:
\begin{enumerate}[(a)]
\item $0\leq AA^*\leq 1$ and $0 \leq 1 - AA^*\leq 1$.
\item There is a constant $c>0$ such that $AA^* \geq c$ and $1 - AA^* \geq c \; \Pi^2\; (1 + \Pi^2)^{-1}$.
\end{enumerate}
In particular, $AA^*$ and $1 - AA^*$ are boundedly invertible on $\Lmag^2(Q_B)$.
\end{lem}

Strategy of Proof:
\begin{itemize}
\item Prove this in the ``whole-space-case'' using the spherical harmonics.
\item Use Andi's argument to lift it to the periodic case.
\end{itemize}


%\subsubsection{Proof of Lemma \ref{AAstar_Positive}}

%\begin{proof}
%Part (a) is a direct consequence of the fact that $\Vert \alpha_* \Vert_2 = 1$. In the following we reduce the proof of part (b) to known results in \cite{Hainzl2017}. To this end, we introduce the operator
%\begin{align}
%	R := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot \Pi)
%	\label{eq:R}
%\end{align}
%and note that
%\begin{align*}
%	AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R).
%\end{align*}
%Let us also denote by $\widetilde{R}$ the operator in \eqref{eq:R} but with $\Pi$ replaced by $\tilde \Pi$, which is the same operator but understood to act on $L^2(\mathbb{R}^3)$ instead of $\Lmag^2(Q_B)$. In Lemma~28 in \cite{Hainzl2017} it has been shown that $\widetilde{R}$ is a function of $\tilde \Pi^2$. Moreover, the statement of Lemma~27 in \cite{Hainzl2017} is equivalent to
%\begin{align}
%	1 - \widetilde{R}^2 \geq c\,  \frac{\tilde \Pi^2}{1 + \tilde \Pi^2}
%	\label{eq:R1}
%\end{align}
%for some $0<c<1$, and Eq.~(55) in the same reference implies
%\begin{align}
%	| \widetilde{R} | \leq 1 - c.
%	\label{eq:R2}
%\end{align}
%In combination, \eqref{eq:R1}, \eqref{eq:R2}, and $ \widetilde{R} \leq 1$ show
%\begin{align}
%	 1+\widetilde{R} &\geq c, & 1 - \widetilde{R} \geq \frac{1 - \widetilde{R}^2}{2} &\geq \frac{c}{2} \frac{\tilde \Pi^2}{1 + \tilde \Pi^2} .
%	 \label{eq:R3} 
%\end{align}
%It remains to argue that $R$ is a function of $\Pi^2$ and that a version of \eqref{eq:R3} with $\tilde R$ and $\tilde \Pi$ replaced by $R$ and $\Pi$ holds. 
%
%The fact that $R$ is a function of $\Pi^2$ follows from the argument that we used to show that the same statement is true for the operator in \eqref{eq:A29}. To show that \eqref{eq:R3} with $\tilde R$ and $\tilde \Pi$ replaced by $R$ and $\Pi$ holds, we conjugate both sides of the inequalities with the Bloch-Floquet transformation in \eqref{eq:ABF1} and \eqref{eq:ABF2}, and use \eqref{eq:ABF3}. The inequalities in \eqref{eq:R3} therefore hold equally in any fiber, that is, with $\tilde \Pi$ on the left and on the right sides replaced by $\Pi(k) = \Pi + k$ acting on $\Lmag^2(Q_B)$. Since $\tilde \Pi(0) = \Pi$, this proves the claim. 
%\end{proof}
%We note that part (a) is trivial. In contrast, part (b) needs the spectral decomposition of the operator $\Pi^2$ acting in the space $\Lmag^2(Q_B)$. In appendix \ref{Spectrum_Landau_Hamiltonian_Section}, we use a Bloch-Floquet decomposition, under which $\Pi$ fibers as a direct integral over $\vartheta\in [0,1]$ with the fiber momenta $\Pi(\vartheta) := -\i \nabla + 2\Abold + \sqrt{2\pi B} \, \vartheta \, e_3$. Proposition \ref{Spectrum_Landau_Hamiltonian} shows that the spectrum of $\Pi(\vartheta)^2$ is then given by the values $2B(2k+1) + 2\pi (p+ \vartheta)^2$ with $k\in \Nbb_0$ and $p\in \Zbb$. Moreover, there is a basis of the $k$\tho\ Landau level of the form $\{(a^*)^k |1\rangle, (a^*)^k |2\rangle\}$ with $a|1\rangle =0$ and $a|2\rangle =0$ and the well-known creation and annihilation operators in \eqref{Creation-Annihilation}.
%It fibers in the magnetic Bloch-Floquet decomposition and can be diagonalized fiberwise by using the well-known creation and annihilation operators.
%A short computation shows that, in this setting, the spectrum of $\Pi^2$ consists of the infinitely degenerate eigenvalues
%\begin{align}
%E_{k, p_3} &:= 2B (2k+1) + p_3^2 , & k &\in \Nbb_0, \; p_3\in \sqrt{2\pi B}\; \Zbb. \label{Landau_Levels}
%\end{align}


%The goal of this section is to prove Lemma \ref{AAstar_Positive}. 
%Since $\Pi$ is left invariant by the magnetic lattice translations $T_B(v)$, given by \eqref{Magnetic_Translation_Charge2}, there is a magnetic Bloch-Floquet decomposition $\Ucal_{\mathrm{BF}}$ such that the Landau Hamiltonian $\Pi^2$ fibers according to
%\begin{align*}
%\Ucal_{\mathrm{BF}} \, \Pi^2 \, \Ucal_{\mathrm{BF}}^* = \int_{Q_B^*}^\oplus \dd \vartheta \; \Pi^2(\vartheta)
%\end{align*}
%with the fiber Hamiltonians
%\begin{align*}
%\Pi^2(\vartheta) := (-\i \nabla_X + 2\Abold(X) + \vartheta)^2,
%\end{align*}
%acting on the domain $\Hmag^2(Q_B)$ for any $\vartheta\in Q_B^*$. Here, $Q_B^*$ is the fundamental cell of the dual lattice of $\Lambda_B$. We refer the interested reader to \cite[Section XIII.16]{Reedsimon4} for an introduction into Bloch-Floquet transformations and to \cite{Stefan_Peierls} for a particular treatment of the magnetic case.
%
%We claim that $\Pi^2$ can be explicitly diagonalized as a multiplication operator with the eigenvalues
%
%%Consequently, in the Bloch-Floquet representation, $\Pi^2$ becomes multiplication with the same numbers. 
%This follows from the fiberwise diagonalization of $\Pi^2(\vartheta)$ via of the well-known creation and annihilation operators built upon the magnetic momentum $\Pi + \vartheta$, and a Fourier transform in the free $X_3$-variable.
%
%The operator
%\begin{align*}
%R := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot \Pi_X)
%\end{align*}
%satisfies
%\begin{align*}
%AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R)
%\end{align*}
%and can be written as a direct integral over $\vartheta\in [0,1]$ with fiber operators
%\begin{align*}
%R(\vartheta) := \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; \cos( r \cdot \Pi_X(\vartheta))
%\end{align*}
%in a similar way as $\Pi^2$. Then, $R(\vartheta)$ is diagonal in the same representation used to diagonalize $\Pi(\vartheta)^2$.
%
%The proofs of Lemmas 27 and 28 in \cite{Hainzl2017} show that there is a $c >0$, independent of $\vartheta$, such that
%\begin{align*}
%R(\vartheta) &\geq - 1 + c, & R(\vartheta) &\leq 1 - c \; \frac{\Pi^2}{1 + \Pi^2}.
%\end{align*}
%From this, we easily deduce Lemma \ref{AAstar_Positive}.


%To see \eqref{Landau_Levels}, define $\Pi(\vartheta) := \Pi + \vartheta$ and let us introduce
%\begin{align*}
%a(\vartheta) &:= \frac{1}{2\sqrt{B}} \bigl( \Pi^{(1)}(\vartheta) - \i \Pi^{(2)}(\vartheta)\bigr), & a^\dagger(\vartheta) & = \frac{1}{2\sqrt{B}} \bigl( \Pi^{(1)}(\vartheta) + \i \Pi^{(2)}(\vartheta)\bigr).
%\end{align*}
%It follows that $[a(\vartheta), a^\dagger(\vartheta)] = 1$. Furthermore,
%\begin{align}
%\Pi^2(\vartheta) = 2 B \bigl( 2a^\dagger(\vartheta) a(\vartheta) + 1\bigr) + (P^{(3)} + \vartheta_3)^2. \label{AAstar_positive_3}
%\end{align}
%Here, $P^{(3)} = -\i \partial_{X_3}$ on the interval $[0,\sqrt{2\pi B^{-1}})$ with periodic boundary conditions. The operator $P^{(3)} + \vartheta_3$ can be diagonalized by the Fourier transform
%\begin{align*}
%(\Ucal_\vartheta \varphi)_m &= \frac{1}{\sqrt{2\pi B^{-1}}} \int_0^{\sqrt{2\pi B^{-1}}} \dd x_3 \; \e^{\i (\sqrt{2\pi B} \, m - \vartheta_3)x_3} \varphi(x_3) , & m &\in \Zbb,
%\end{align*} 
%having eigenvalues $p_3\in \sqrt{2\pi B}\, \Zbb$. Combining this with \eqref{AAstar_positive_3}, we read off \eqref{Landau_Levels}. 

%Consequently, \eqref{Landau_Levels} follows from taking the direct integral of $a(\vartheta)$ and $a^\dagger(\vartheta)$ over $\vartheta$. The proof shows that $\Pi^2$ can be diagonalized as well, being a multiplication operator by the numbers
%\begin{align}
%E_{k, p_3} := 2B(2k+1) + 2\pi B \; p_3^2, \qquad k\in \Nbb_0, \; p_3\in \Rbb. \label{Landau_Levels}
%\end{align}

%For the proof of Lemma \ref{AAstar_Positive}, we borrow the following auxiliary result, which is proven in \cite[Lemma 27]{Hainzl2017}. Denote the first two compontents of $\Pi$ by $\Pi^\perp = (\Pi^{(1)}, \Pi^{(2)})^t$. Moreover, by $P_{2B}^{(k)}$ we denote the projections onto the $k$\tho\ Landau level and by $L_k = L_k^{(0)}$ the Laguerre polynomials.
%
%\begin{lem}
%For every $\rho >0$,
%\begin{align*}
%\frac{1}{2\pi} \int_{\Sbb^1} \dd \omega \; \cos(\rho \omega\; \Pi^\perp) =\e^{-\frac 12 B\rho^2} \sum_{k=0}^\infty L_k(B\rho^2) P_{2B}^{(k)}.
%\end{align*}
%\end{lem}

%\begin{proof}[Proof of Lemma \ref{AAstar_Positive}]
%As noted above, part (a) is trivial. We remark that the proof of part (b) is very similar to the proof of Lemma 27 in \cite{Hainzl2017}, when $\varphi_*$ is replaced by $\alpha_*$. It actually provides the proof of Lemma \ref{AAstar_Positive} when we read it carefully enough, which we do now. Let us introduce the operator
%\begin{align*}
%R := \int_{\Rbb^3} \dd r\; \alpha_*(r)^2 \; \cos(r\cdot \Pi).
%\end{align*}
%Then, the key observation is that
%\begin{align*}
%AA^* &= \frac 12 (1 + R), & 1 - AA^* &= \frac 12 (1 - R).
%\end{align*}
%
%In the representation of \eqref{Landau_Levels}, the operator $R$ is diagonalized as well, acting as a multiplication operator by the numbers
%%The operator $R$ can be diagonalized explicitly by a Fourier transform in the $x_3$ variable and decomposing into Landau levels in the $(x_1,x_2)$ variables. Then $R$ acts as a multiplication operator by the numbers
%\begin{align*}
%R_{k,p_3} &= \pi \int_0^\infty \dd u \int_\Rbb \dd x_3\; \bigl| \alpha_*\bigl( \sqrt{u + x_3^2}\bigr)\bigr|^2 \cos(x_3p_3) \e^{-\frac 12Bu} L_k(Bu), & k&\in \Nbb_0, \, p_3\in \sqrt{2\pi B} \, \Zbb.
%\end{align*}
%This formula is obtained in the same way as Eq. (49) in \cite{Hainzl2017} and $L_k$ is the $k$\tho\ Laguerre polynomial.
%
%Since $\Pi^2$ acts as multiplication by the numbers $E_{k,p_3}$ of \eqref{Landau_Levels}, it suffices to prove that there is a $c>0$ such that
%\begin{align}
%R_{k,p_3} &\geq -1 + c, & R_{k,p_3} &\leq 1 - c \frac{E_{k,p_3}}{1 + E_{k,p_3}}. \label{AAstar_positive_2}
%\end{align}
%We prove these inequalities separately for small, medium and large values of $E_{k,p_3}$. In fact, \eqref{AAstar_positive_2} is true for all $p_3\in \Rbb$.
%
%\emph{Step 1.} We claim that there are $E_* >0$ and $c_\leq , c_\geq >0$ such that for all $B>0$, $k\in\Nbb_0$ and $p_3\in \Rbb$ with $E_{k,p_3} \leq E_*$, we have
%\begin{align}
%1 - c_\leq E_{k,p_3} \leq R_{k,p_3} \leq 1 - c_\geq E_{k,p_3}. \label{AAstar_positive_1}
%\end{align}
%To see this, use $1 - \frac 12 x^2 \leq \cos x \leq 1 - \frac 12x^2 + \frac{1}{24} x^4$ for all $x\in \Rbb$ to conclude that
%\begin{align}
%0 \leq R - \int_{\Rbb^3} \dd r \; |\alpha_*(r)|^2 \bigl( 1 - \frac 12 (r\cdot \Pi)^2\bigr) \leq \frac{1}{24} \int_{\Rbb^3} \dd r \; |\alpha_*(r)|^2 (r\cdot \Pi)^4. \label{AAstar_positive_4}
%\end{align}
%Set
%\begin{align*}
%\langle |r|^{2m}\rangle &:= \int_{\Rbb^3} \dd r \; \alpha_*(r)^2 \; r^{2m}, & m & = 1,2.
%\end{align*} 
%These numbers are finite by the decay properties \eqref{Decay_of_alphastar} of $\alpha_*$. An explicit computation using the fact that the angular average of $r_ir_j$ equals $\frac{1}{3} r_i^2 \delta_{ij}$ shows
%\begin{align*}
%\int_{\Rbb^3} \dd r \; \alpha_*(r)^2 (r\cdot \Pi)^2 = \frac 13 \langle |r|^2\rangle \; \Pi^2.
%\end{align*}
%Furthermore, using the operator inequality \eqref{ZPiX_inequality_quartic}, we get
%\begin{align*}
%\int_{\Rbb^3} \dd r \; \alpha_*(r)^2 (r\cdot\Pi)^4 \leq C\langle |r|^4\rangle \; (\Pi^4 + B^2).
%\end{align*}
%Combining this with \eqref{AAstar_positive_4}, we obtain
%\begin{align*}
%1 - \frac 16 \langle |r|^2\rangle \Pi^2 \leq R \leq 1 - \frac 16 \langle |r|^2 \rangle \Pi^2 + C\langle |r|^4\rangle (\Pi^4 +  B^2)
%\end{align*}
%or, equivalently,
%\begin{align*}
%1 - \frac 16 \langle |r|^2\rangle E_{k,p_3} \leq R_{k,p_3} \leq 1 - \frac 16\langle |r|^2 \rangle E_{k,p_3} + C\langle |r|^4\rangle (E_{k,p_3}^2 + B^2).
%\end{align*}
%To obtain \eqref{AAstar_positive_1} from this, we note that $B\leq E_{k,p_3}$ for every $k\in \Nbb_0$ and $p_3\in \Rbb$.
%
%Steps 2 and 3 in the proof of \cite[Lemma 28]{Hainzl2017} carry over to our situation. 
%
%\emph{Step 2} shows that $R_{k,p_3}\to 0$ as $E_{k,p_3}\to \infty$ uniformly for sufficiently small $B>0$. That is, for every $B_0>0$ and $\varepsilon>0$, there is $E_*>0$ such that for all $0\leq B\leq B_0$, all $k\in \Nbb_0$ and $p_3 \in \Rbb$ with $E_{k,p_3}\geq E_*$, we have $|R_{k,p_3}|\leq \varepsilon$.
%
%\emph{Step 3} shows that for any $E_\leq < E_\geq$ and any $B_0>0$, there is a $c>0$ such that for all $0 < B\leq B_0$, $k\in \Nbb_0$ and $p_3\in \Rbb$ with $E_\leq \leq E_{k,p_3}\leq E_\geq$, we have $|R_{k,p_3}| \leq 1 - c$.
%
%Putting the estimates together implies \eqref{AAstar_positive_2} and concludes the proof.
%\end{proof}


The remainder of this subsection is devoted to the proof of Proposition~\ref{First_Decomposition_Result}. We start with a lower bound on the operator in \eqref{First_Decomposition_Result_Assumption} when it acts on wave functions of the form $A^*\Psi$, see Lemma~\ref{MainTerm} below. 

\subsubsection{Step one -- lower bound on the range of $A^*$}

The main result of this subsection is the following lemma.

\begin{lem}
\label{MainTerm}
For any $\Psi\in \Lmag^2(Q_B)$, with $A$ and $A^*$ given by \eqref{Def_A} and \eqref{Def_Astar}, with $U$ given by \eqref{U_definition}, and $P = |\alpha_*\rangle \langle \alpha_*|$ with $\alpha_*$ from \eqref{alpha_star_ev-equation} acting on the relative coordinate, we have
\begin{align}
\frac 12 \langle A^* \Psi, [ U^* (1 - P) (1 + \pi_r^2) (1- P) U + U(1 - P) (1 + \pi_r^2)(1-P) U^* ] A^*\Psi\rangle \hspace{-340pt}& \notag\\
%
&=  \langle \Psi, AA^* (1 - AA^*)(1 + \Pi^2) \Psi\rangle \notag\\
%
&\hspace{10pt} +  \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2 \bigl(\frac r2 \Pi_X\bigr) \; (1 - AA^*)\Psi(X) \notag \\
%
&\hspace{10pt}+ \fint_{Q_B} \dd X \int_{\Rbb^3} \dr \; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2\; \sin^2 \bigl(\frac r2  \Pi_X\bigr) \; AA^*\Psi(X)\notag \\
%
&\hspace{10pt} + \frac 14 \fint_{Q_B}\dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2 \; \sin^2 \bigl(\frac r2 \Pi_X\bigr) \; (1 - AA^*)\Psi(X) \notag\\
%
&\hspace{10pt} + \frac 14\fint_{Q_B}\dd X\int_{\Rbb^3} \dr \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2 \;  \cos^2 \bigl(\frac r2 \Pi_X\bigr) \; AA^*\Psi(X). \label{MainTerm_5}
\end{align}
In particular, we have the lower bound
\begin{align}
\frac 12 \langle A^* \Psi, [ U^* (1 - P) (1 + \pi_r^2) (1- P) U + U(1 - P) (1 + \pi_r^2)(1-P) U^* ] A^*\Psi\rangle %& \notag\\
%
%&\hspace{-200pt}\geq \langle \Psi, AA^*(1 - AA^*)(1 + \Pi^2)\Psi\rangle
\geq c\, \langle \Psi, \Pi^2\Psi\rangle . \label{MainTerm_LowerBound}
\end{align}
\end{lem}

%By Lemma \ref{AAstar_Positive}, $AA^*$ commutes with $\Pi^2$ and the operator on the right side of \eqref{MainTerm_LowerBound} is bounded from below by a constant times $\Pi^2$. This lower bound will allow us to prove the bound on the magnetic gradient of $\Psi$ in Proposition \ref{First_Decomposition_Result}.

\begin{bem}
Let us replace $\pi_r^2$ on the left side of \eqref{MainTerm_5} by zero for the moment. In this case, the substitute of \eqref{MainTerm_5} reads
\begin{align}
\frac 12 \langle A^*\Psi, [U^*(1 - P)U + U(1 - P)U^* ] A^*\Psi\rangle = \langle \Psi , AA^*(1 - AA^*) \Psi\rangle. \label{Low_Energy_Operator}
\end{align}
It follows from Lemma~\ref{AAstar_Positive} that the operator $AA^*(1 - AA^*)$ is bounded from below by $\Pi^2$ only for small values of $\Pi^2$, which is not enough for the proof of Proposition \ref{First_Decomposition_Result}. This justifies the term ``low-energy operator'' for $1 - A^*A$, which we used earlier in the discussion below \eqref{Def_Astar}. The additional factor $1 + \Pi^2$ in the first term on the right side of \eqref{MainTerm_5} compensate for the problematic behavior of \eqref{Low_Energy_Operator} for high energies. The expression on the right side of \eqref{Low_Energy_Operator} also appears in \cite{Hainzl2017}. 
%and serves us with the appropriate bound \eqref{MainTerm_LowerBound}.
\end{bem}
%In becomes clear in the proof of Lemma \ref{MainTerm} that there is no easy way to drop any term for a lower bound until one arrives at \eqref{MainTerm_5}. Every positive term, which drops out on the way, has to account for a corresponding negative term and the network of correspondences is intricate. This is the reason why the proof of Lemma \ref{MainTerm} requires considerably more effort than \eqref{Low_Energy_Operator}.

Before we give the proof of Lemma~\ref{MainTerm}, we prove two technical lemmas, which provide intertwining relations for various magnetic momentum operators with $U$ and linear combinations of $U$. A part of the relations in the first lemma can be found in \cite[Lemma~24]{Hainzl2017}.

\begin{lem}
\label{CommutationI}
Let $p_r := -\i \nabla_r$, $\pi_r = p_r + \frac 12\Bbold \wedge r$ and $\tilde \pi_r$ and $\Pi_X$ be given by \eqref{Magnetic_Momenta_COM}. For $U$ in \eqref{U_definition}, we have the following intertwining relations:
\begin{align*}
\begin{split}
U \Pi_X U^* &= \Pi_X - \Bbold\wedge r,\phantom{\frac 12}  \\  U^* \Pi_X U &= \Pi_X + \Bbold\wedge r, \phantom{\frac 12}
\end{split} &
\begin{split}
U \pi_r U^* &= \tilde \pi_r + \frac{1}{2}\Pi_X, \\ U^* \pi_r U &= \tilde \pi_r - \frac{1}{2}\Pi_X, \phantom{\frac 12}
\end{split} &
\begin{split}
U \tilde \pi_r U^* &= p_r + \frac{1}{2}\Pi_X, \\ U^* \tilde \pi_r U &= p_r - \frac{1}{2}\Pi_X.
\end{split}
\end{align*}
\end{lem}

\begin{proof}
Let us denote $P_X := -\i \nabla_X$. We use the fact that $r\cdot P_X$ commutes with $r\cdot (\Bbold \wedge X)$ to see that
\begin{align}
U^* = \e^{\i \frac \Bbold 2 \cdot X\wedge r} \; \e^{\i \frac r2P_X} \label{representation_Ustar}
\end{align}
holds. To prove the first intertwining relation with $\Pi_X$, we compute
\begin{align*}
\Pi_XU^* &= (P_X + \Bbold\wedge X)U^* =  \e^{\i \frac \Bbold 2 \cdot X\wedge r} \Bigl[ P_X - \frac 12 \Bbold \wedge r + \Bbold\wedge X\Bigr] \e^{\i \frac r2P_X} \\
%
&= U^* \Bigl[ P_X - \frac 12 \Bbold \wedge r + \Bbold \wedge \bigl(X -\frac r2\bigr)\Bigr] = U^* [ \Pi_X - \Bbold \wedge r].
\end{align*}
Here we used that $f(X)\, \e^{\i \frac r2P_X} = \e^{\i \frac r2 P_X}\, f(X-\frac r2)$. The second intertwining relation with $\Pi_X$ is obtained by replacing $r$ by $-r$. 

Next we consider the first intertwining relation with $\pi_r$ and compute
\begin{align*}
\pi_r U^* &= \bigl( p_r + \frac 12\Bbold \wedge r\bigr) U^* = \e^{\i \frac \Bbold 2 \cdot X\wedge r}\Bigl[ p_r + (-\i)\i \frac 12 \Bbold \wedge X + \frac 12 \Bbold \wedge r\Bigr] \e^{\i \frac r2P_X} \\
%
&= U^* \Bigl[ p_r + \frac{P_X}{2} + \frac 12 \Bbold \wedge \bigl( X - \frac r2\bigr) + \frac 12 \Bbold \wedge r\Bigr] = U^* \Bigl[ \tilde \pi_r + \frac{\Pi_X}{2}\Bigr].
\end{align*}
The remaining relations can be proved similarly and we skip the details.
\end{proof}

\begin{lem}
\label{CommutationII}
\begin{enumerate}[(a)]
\item We have the following intertwining relations for $\Pi_X$:
\begin{align}
\Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) &=  \cos\bigl( \frac r2 \Pi_X\bigr)\Pi_X - \i \sin\bigl( \frac r2 \Pi_X\bigr) \Bbold\wedge r, \label{PiXcos} \\
%
\Pi_X \sin\bigl( \frac r2 \Pi_X\bigr) &= \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X + \i \cos\bigl( \frac r2 \Pi_X\bigr) \Bbold\wedge r. \label{PiXsin}
\end{align}

\item The operators $p_r$, $\tilde \pi_r$ and $\pi_r$ intertwine according to
\begin{align}
\tilde \pi_r \cos\bigl( \frac r2 \Pi_X\bigr) &= \cos\bigl( \frac r2 \Pi_X\bigr) p_r + \i \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}, \label{pirtilde_cos_pr}\\
%
\tilde \pi_r \cos\bigl( \frac r2 \Pi_X\bigr) &= \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r + \i \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr), \label{pirtilde_cos_pir}
\end{align}
and
\begin{align}
\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr)  &= \sin\bigl( \frac r2 \Pi_X\bigr) p_r - \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}, \label{pirtilde_sin_pr}\\
%
\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr) &= \sin\bigl( \frac r2 \Pi_X\bigr) \pi_r - \i \frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr) \label{pirtilde_sin_pir}
\end{align}
\end{enumerate}
\end{lem}

It will be useful in the proof of Lemma \ref{MainTerm} to have displayed both, \eqref{pirtilde_cos_pr} and \eqref{pirtilde_cos_pir} as well as \eqref{pirtilde_sin_pr} and \eqref{pirtilde_sin_pir}, even though they follow trivially from each other and \eqref{PiXcos} or \eqref{PiXsin}.

\begin{proof}
The proof is a direct consequence of the representations
\begin{align}
	\cos\bigl( \frac r2 \Pi_X\bigr) &= \frac 12 (U^* + U), & \sin\bigl( \frac r2 \Pi_X\bigr) &= \frac 1{2\i} (U^*-U),
\end{align}
and the intertwining relations in Lemma~\ref{CommutationII}. We omit the details.
%For example, \eqref{PiXcos} is obtained from Lemma \ref{CommutationI} by computing
%\begin{align*}
%\Pi_X\cos\bigl( \frac r2 \Pi_X\bigr) &= \frac{1}{2}\Pi_X (U^* + U) = \frac{1}{2} U^* (\Pi_X - \Bbold \wedge r) + \frac{1}{2} U (\Pi_X + \Bbold \wedge r)\\
%&= \frac{1}{2} (U^* + U) \Pi_X - \frac{1}{2} (U^* - U) \Bbold \wedge r.
%\end{align*}
%Furthermore, \eqref{pirtilde_sin_pr} is obtained by
%\begin{align*}
%\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr) &= \frac{1}{2\i} U^*\bigl( p_r + \frac{\Pi_X}{2} \bigr) - \frac{1}{2\i} U \bigl( p_r - \frac{\Pi_X}{2}\bigr) = \sin\bigl( \frac r2 \Pi_X\bigr) p_r - \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} .
%\end{align*}
%Applying \eqref{PiXcos} to this yields \eqref{pirtilde_sin_pir}. The other equations are proved analogously.
\end{proof}

\begin{proof}[Proof of Lemma \ref{MainTerm}]
The proof is a tedious computation that is based on the intertwining relations in Lemma \ref{CommutationII}. 
%We have to keep track of the following strategy:
%\begin{enumerate}[(1)]
%\item We want to resolve the entanglement of the coordinates $X$ and $r$ that is created by the operator in \eqref{MainTerm_5}. To do this, we display every term best possible with the functions $AA^*$ and $1 - AA^*$ of $\Pi_X^2$, which we know from Lemma \ref{AAstar_Positive}. Since $A^*\Psi$ contains the operator $\cos(\frac r2\Pi_X)$, the cosine is the left-most and right-most factor in each term. Roughly speaking, we have to move it into the center in order to get $AA^*$. However, in doing so, we should never separate powers of $\Pi_X^2$, since they obviously are a function of $\Pi_X^2$ already.
%
%\item In the relative coordinate, it turns out that the natural momentum operator is the nonmagnetic $p_r = -\i \nabla_r$ and the magnetic field in $\pi_r$ should be viewed as a perturbation that leads to a positive correction in the energy. Thus, we are going to separate the magnetic field from the relative momenta.
%
%\item We make frequent use of two trivial facts. Firstly, $\Bbold \wedge r$ commutes with all of $\pi_r$, $\tilde \pi_r$, and $p_r$ because $\divv \Bbold \wedge r =0$. Secondly, $\cos( \frac r2 \Pi_X)$ and $\sin( \frac r2 \Pi_X)$ commute with any function of $r$.
%
%\item We will end up having three sorts of terms: The ones proportional to $\alpha_*^2$ having no relative magnetic field. These contribute to the main term, the first term on the right side of \eqref{MainTerm_5}. The ones proportional to $|\nabla \alpha_*|^2$ and the ones proportional to $|\Bbold\wedge r|^2\; \alpha_*^2$ are positive corrections which we are dropping later in \eqref{MainTerm_LowerBound}.
%\end{enumerate}
We start by defining
\begin{align}
\Tcal_1 &:= U^* \pi_r^2 U + U\pi_r^2 U^* = 2\, \tilde \pi_r^2 + \frac 12 \, \Pi_X^2, & \Tcal_2 &:= U^*P\pi_r^2PU + UP\pi_r^2PU^*, \notag \\
%
\Tcal_3 &:= U^* P\pi_r^2U + UP\pi_r^2U^*, & \Tcal_4 &:= U^* \pi_r^2 PU + U\pi_r^2PU^*. \label{MainTerm_6}
\end{align}
Then, \eqref{MainTerm_5} can be written as
\begin{align}
\langle A^* \Psi, [ U^* (1 - P) (1 + \pi_r^2) (1- P) U + U(1 - P) (1 + \pi_r^2)(1-P) U^* ] A^*\Psi\rangle  & = \notag\\
%
&\hspace{-330pt}= 2\langle A^*\Psi, (1 - A^*A)A^*\Psi\rangle \notag \\
%
&\hspace{-300pt} + \langle A^*\Psi, \Tcal_1 A^*\Psi\rangle + \langle A^*\Psi, \Tcal_2 A^*\Psi\rangle - \langle A^*\Psi, \Tcal_3 A^*\Psi\rangle - \langle A^*\Psi, \Tcal_4 A^*\Psi\rangle. \label{Tcal_first_line}
\end{align}
The first term on the right side equals twice the term in \eqref{Low_Energy_Operator}, which is in its final form. 

We start by computing the $\Pi_X^2$ term in $\Tcal_1$, which reads
\begin{align*}
\langle A^* \Psi , \Pi_X^2 A^* \Psi \rangle = \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \alpha^*(r) \; \cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \Psi(X).
\end{align*}
Our goal is to move $\Pi_X^2$ to the right. To that end, we apply \eqref{PiXcos} twice and obtain
\begin{align*}
\Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) = \cos\bigl( \frac r2 \Pi_X\bigr)\Pi_X^2 - \i \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\Bbold \wedge r - \i \Pi_X \sin\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r.
\end{align*}
We multiply this from the left with $\cos( \frac r2 \Pi_X)$, use \eqref{PiXcos} to commute $\Pi_X$ to the left in the last term, and find
\begin{align}
\cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2\cos\bigl( \frac r2 \Pi_X\bigr) &= \cos^2\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 + \sin^2\bigl( \frac r2 \Pi_X\bigr) |\Bbold\wedge r|^2 \notag\\
&\hspace{-60pt}- \i \bigl[ \Pi_X\cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) + \cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\bigr]\Bbold\wedge r. \label{PiX-term_1}
\end{align}
The operator $| \Bbold \wedge r |^2$ in the second term on the right side commutes with $\sin^2( \frac r2 \Pi_X)$. The operator in square brackets is self-adjoint and commutes with $\Bbold \wedge r$. When we add \eqref{PiX-term_1} and its own adjoint, we obtain
%\begin{align*}
%&\hspace{-30pt}- \i \bigl[ \Pi_X\cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) + \cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\bigr]\Bbold\wedge r.
%\end{align*}
%We evaluate this term in the scalar product with $\alpha_*\Psi$ on both sides and make the following observations. The left-hand side is a real number. The first term on the right side equals $\langle \Psi, AA^* \Pi_X^2 \Psi\rangle$. Since $AA^*$ commutes with $\Pi_X^2$, see Lemma~\ref{AAstar_Positive}, this is a real number as well. The same is true for the second term on the right side because $|B\wedge r|$ commutes with $\sin^2(\frac r2\Pi_X)$. The operator in square brackets in the third term on the right side is self-adjoint and commutes with $\Bbold \wedge r$. In view of the $\i$ in front of the square bracket, the expectation of this term w.r.t. $\alpha_*\Psi$ is purely imaginary, and hence equals zero. This proves
\begin{align}
\cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2\cos\bigl( \frac r2 \Pi_X\bigr) & \notag\\
%
&\hspace{-50pt}= \frac 12 \cos^2\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 + \frac 12 \, \Pi_X^2 \cos^2\bigl( \frac r2 \Pi_X\bigr) + \sin^2\bigl( \frac r2 \Pi_X\bigr) |\Bbold\wedge r|^2. \label{PiX-term_2}
\end{align}
We evaluate \eqref{PiX-term_2} in the inner product with $\alpha_*\Phi$ and $\alpha_*\Psi$ on the left and right side, respectively, use the fact that $AA^*$ commutes with $\Pi^2$, see Lemma \ref{AAstar_Positive}, and obtain
\begin{align}
\langle A^*\Phi, \Pi_X^2A^*\Psi\rangle &= \langle \Phi, AA^* \Pi^2\Psi\rangle \notag\\
%
&\hspace{10pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Phi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X). \label{PiX-term}
\end{align}
When we choose $\Phi = \Psi$ we obtain the result for the term proportional to $\Pi_X^2$ in $\Tcal_1$.
%The left-hand side is a real number. The first term of the right side equals $\langle \Psi, AA^* \Pi^2 \Psi\rangle$, with $AA^*$ from Lemma \ref{AAstar_Positive}. Since $AA^*$ commutes with $\Pi^2$, this is a real number as well. As for the second term, since $|B\wedge r|$ commutes with $\sin^2(\frac r2\Pi_X)$, it is real.  In view of the $\i$ in front, the quadratic form of this term with $\alpha_*\Psi$ on both sides is a purely imaginary number and thus equal to zero. We end up with the quadratic form of the first and second term, i.e.,


Next, we investigate the term proportional to $\tilde\pi_r^2$ in $\Tcal_1$. We use \eqref{pirtilde_cos_pir} to move the operators $\tilde \pi_r$ from the middle to the outer positions and find
\begin{align}
\langle A^*\Psi, \tilde \pi_r^2A^*\Psi\rangle &= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)} \alpha_*(r)\left[ \pi_r\cos\bigl( \frac r2 \Pi_X\bigr) -\i \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}\right] \notag\\
%
&\hspace{80pt} \times \left[ \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r + \i \frac{\Pi_X}{2}\sin\bigl( \frac r2 \Pi_X\bigr)\right]\alpha_*(r) \Psi(X). \label{tildepir_eq1}
\end{align}
We multiply out the brackets and obtain four terms. The terms proportional to $\cos^2$ and $\sin^2$ read
\begin{align}
&\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)}\;  |\pi_r\alpha_*(r)|^2\;  \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag\\
%
&\hspace{20pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; \alpha_*(r)\;  \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4} \sin\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X).\label{tildepir_eq4}
\end{align}
For the moment the second line remains untouched. It is going to be canceled by a term in \eqref{tildepir_eq5} below. The term in the first line equals
%In the first line, we want to separate the magnetic field from $\pi_r= -\i \nabla_r + \frac 12 \Bbold \wedge r$. When we multiply out the square, the cross terms vanish because $\nabla_r\alpha_*(r)$ is proportional to $e_r$, since $\alpha_*$ is radial. Therefore, $\nabla_r\alpha_*(r) \cdot \Bbold \wedge r = 0$. Hence, the first line equals
\begin{align}
%\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\pi_r\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) = & \notag\\
%
&\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\ %\label{tildepir_eq3}\\
%
&\hspace{50pt} + \frac 14\fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X). \label{tildepir_eq2}
\end{align}
To obtain this result, we used $(\nabla \alpha_*)(r) \cdot \Bbold \wedge r =0$, which holds because $\alpha_*$ is radial. This term is in its final form.

Now we have a closer look at the terms proportional to $\sin $ times $\cos$ in \eqref{tildepir_eq1}. The operator inside the relevant quadratic form is given by
\begin{align}
\i \pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) - \i \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r. \label{MainTerm_1}
\end{align}
We intend to interchange $\sin( \frac r2 \Pi_X)$ and $\cos( \frac r2 \Pi_X)$ in the first term. To do this, we use \eqref{PiXsin} to move $\Pi_X$ out of the center so that the first term equals
%If we move $\pi_r$ into the center afterwards, we have a cancellation. To do this, we need to move in the first term, by using . Performing this, the first term of \eqref{MainTerm_1} equals
\begin{align*}
\i \pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} -\frac 12\pi_r\cos^2\bigl( \frac r2 \Pi_X\bigr) \Bbold \wedge r.
\end{align*}
%
%Meanwhile, in the second term, we move $\pi_r$ into the center. Thus, \eqref{MainTerm_1} is equal to
%\begin{align*}
%&\pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \bigl[ \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} + \frac \i2 \cos\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r\bigr] \\
%%
%&\hspace{60pt} - \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2}\bigl[ \tilde \pi_r \cos\bigl( \frac r2 \Pi_X\bigr) - \i \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr)\bigr].
%\end{align*}
In the first term we may now commute the sine and the cosine and use \eqref{PiXcos} and \eqref{pirtilde_sin_pir} to bring $\pi_r$ and $\Pi_X$ in the center again. We also move $\pi_r$ into the center in the second term in \eqref{MainTerm_1}. As a result, \eqref{MainTerm_1} equals
\begin{align}
%\pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r & =\\
%
&\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}\cos\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}\sin\bigl( \frac r2 \Pi_X\bigr) \notag \\
%
&\hspace{40pt}+ \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{4} \sin\bigl( \frac r2 \Pi_X\bigr) \Bbold \wedge r \notag \\ %\label{MainTerm_2} \\
%
&\hspace{80pt}- \frac 12 \pi_r \cos^2\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r - \frac 12 \sin\bigl( \frac r2 \Pi_X\bigr)\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r. \label{MainTerm_3}
\end{align}
We use \eqref{pirtilde_sin_pir} to move $\tilde \pi_r$ to the left in the last term in \eqref{MainTerm_3}. One of the terms we obtain in this way cancels the third term in \eqref{MainTerm_3}. We also use $\cos( \frac r2 \Pi_X)^2 + \sin( \frac r2 \Pi_X)^2=1$ to rewrite the fourth term in \eqref{MainTerm_3}. In combination, these considerations imply that the terms in \eqref{MainTerm_3} equal
%\begin{align*}
%&\frac \i2 \pi_r \cos^2\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r + \frac \i2 \sin\bigl( \frac r2 \Pi_X\bigr)\tilde \pi_r \sin\bigl( \frac r2 \Pi_X\bigr)\Bbold \wedge r \\
%%
%&\hspace{170pt} + \frac 12 \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) \Bbold \wedge r = \frac \i2 \pi_r \Bbold \wedge r.
%\end{align*}
\begin{align}
\begin{split}
%&\pi_r\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} \cos\bigl( \frac r2 \Pi_X\bigr)\pi_r = \\
%
\cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}\cos\bigl( \frac r2 \Pi_X\bigr) - \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{4}\sin\bigl( \frac r2 \Pi_X\bigr) - \frac 12 \pi_r\Bbold \wedge r. \end{split} \label{tildepir_eq5}
\end{align}
The expectation of the second term with respect to $\alpha_*(r) \Psi(X)$ cancels the second term in \eqref{tildepir_eq4}. We multiply the last term from the left and from the right with $\alpha_*(r)$, integrate over $r$ and find 
\begin{align}
\frac 12\int_{\Rbb^3} \dd r\; \alpha_*(r) \pi_r \Bbold \wedge r \alpha_*(r) = \frac 12 \int_{\Rbb^3} \ov{p_r\alpha_*(r)} \Bbold \wedge r\alpha_*(r) + \frac 14\int_{\Rbb^3} \dd r\; |\Bbold \wedge r|^2 \alpha_*(r)^2. \label{Tcal3_eq2}
\end{align}
The first term on the right side vanishes because $\alpha_*$ is radial, see the remark below \eqref{tildepir_eq4}. Let us summarize where we are. We combine \eqref{tildepir_eq1}--\eqref{Tcal3_eq2} to see that
\begin{align}
\langle A^*\Psi, \tilde \pi_r^2A^*\Psi\rangle &= \fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\
%
&\hspace{-30pt} + \frac 14 \fint_{Q_B} \dd X \int_{\Rbb^3}\dd r\; \ov{\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \; \bigl( \cos^2 \bigl( \frac r2 \Pi_X\bigr) -1 \bigr) \; \Psi(X) \notag \\
%
&\hspace{-30pt} + \frac 14 \fint_{Q_B} \dd X \int_{\Rbb^3}\dd r \; \ov{\alpha_*(r) \Psi(X)} \; \cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \Psi(X). \label{eq:1}
\end{align}
The term in the last line equals $\langle A^*\Psi, \Pi_X^2A^*\Psi\rangle$ and we use \eqref{PiX-term} to rewrite it. This allows us to show 
%Namely, we investigate the last term of \eqref{tildepir_eq5}. 
%Using that $p$ commutes with $\Bbold \wedge r$, we see by integrating by parts that the first term vanishes. 
%We are left with the first term of \eqref{PiX-term}, times $\frac 14$, and the first term of \eqref{tildepir_eq2}.
%The last term cancels the magnetic fields obtained in \eqref{tildepir_eq2} and by commuting $\Pi_X^2$ through $\cos( \frac r2 \Pi_X)$, see \eqref{PiX-term}, multiplied by $\frac 14$. The remaining terms are \eqref{tildepir_eq3} and the nonmagnetic part of \eqref{PiX-term}, times $\frac 14$. 
\begin{align*}
\langle A^*\Psi, \tilde \pi_r^2A^*\Psi\rangle &= \frac 14 \langle \Psi, AA^* \Pi^2\Psi\rangle + \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\;  \ov{\Psi(X)}\;  |\nabla \alpha_*(r)|^2\;  \cos^2\bigl( \frac r2 \Pi_X\bigr)\; \Psi(X).
\end{align*}
In combination with \eqref{MainTerm_6} and \eqref{PiX-term}, this yields
\begin{align}
\langle A^* \Psi, \Tcal_1 A^*\Psi\rangle &= \langle \Psi , AA^*\Pi^2\Psi\rangle \notag \\
%
&\hspace{10pt}+ 2\fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)}\;  |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr)\;  \Psi(X) \notag \\
%
&\hspace{10pt} + \frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X)  \label{Tcal1-Result}
\end{align}
and completes our computation of the term involving $\Tcal_1$.

A short computation shows that
\begin{equation}
\langle A^*\Psi , \Tcal_2A^*\Psi\rangle = 2\, \langle AA^*\Psi , AA^*\Psi\rangle \Bigl[ \Vert \nabla \alpha_*\Vert_2^2 + \frac 14 \int_{\Rbb^3} \dd r \; |\Bbold \wedge r|^2 \alpha_*(r)^2\Bigr]. \label{Tcal2_result}
\end{equation}
It remains to compute the terms in \eqref{Tcal_first_line} involving the operators $\Tcal_3$ and $\Tcal_4$, where $\Tcal_4^* = \Tcal_3$.
%The second equality holds because $\nabla\alpha_*(r) \cdot \Bbold \wedge r =0$, as argued below \eqref{tildepir_eq4}. 

In the following we compute the term with $\Tcal_3$. A short computation which uses the fact that $\alpha_*$ is radial shows
\begin{align}
\langle A^* \Psi, \Tcal_3A^*\Psi\rangle &= \langle \alpha_* A A^*\Psi, \pi_r^2 (U^* + U) A^*\Psi \rangle \notag\\
%
&\hspace{-30pt}= 2\fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; p_r\cos^2\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X) \notag\\
%
&\hspace{-10pt} + \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2\;  \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X). \label{Tcal3_eq3}
\end{align}
%Since $\alpha_*$ is radial, $p\alpha_*(r)$ is orthogonal to the unit sphere and hence also to $\Bbold \wedge r$. Thus, $\pi_r^2\alpha_*(r) = p^2\alpha_*(r) + \frac 14|\Bbold \wedge r|^2\alpha_*(r)$. 
%
%Using again that $U^*P$ and $UP$ act as $A^*\langle \alpha_*|$ on symmetric functions, 
The second term on the right side is in its final form and will be canceled by a term below. We continue with the first term, use \eqref{pirtilde_cos_pr} twice to commute $p_r$ with the squared cosine, as well as \eqref{PiXcos} and \eqref{PiXsin} to commute $\Pi_X$ to the center in the emerging terms, and find
\begin{align}
p_r\cos^2\bigl( \frac r2 \Pi_X\bigr) %&= \cos^2\bigl( \frac r2 \Pi_X\bigr)p_r + \i \cos\bigl( \frac r2 \Pi_X\bigr)\sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X}{2} + \i \frac{\Pi_X}{2} \sin\bigl( \frac r2 \Pi_X\bigr)\cos\bigl( \frac r2 \Pi_X\bigr) \notag\\
%
&= \cos^2\bigl( \frac r2 \Pi_X\bigr)p_r + \i \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) - \frac 12 \Bbold \wedge r. \label{Tcal3_eq1}
\end{align}
We note that the last term, when inserted back into \eqref{Tcal3_eq3}, vanishes because $\alpha_*$ is radial. The first term is final and its quadratic form with $p_r \alpha_* AA^*\Psi$ and $\alpha_*\Psi$ reads
\begin{align}
2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2\Pi_X\bigr) \; \Psi(X). \label{MainTerm_4}
\end{align}
Let us continue with the second term on the right side of \eqref{Tcal3_eq1}. We multiply it with $p_r$ from the left and use \eqref{pirtilde_cos_pr} and \eqref{pirtilde_sin_pr} to commute $p_r$ to the right. In the two emerging terms we bring $\Pi_X$ to the center and obtain
\begin{align*}
p_r \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X\cos\bigl( \frac r2 \Pi_X\bigr) &= \sin\bigl( \frac r2 \Pi_X\bigr)\Pi_X\cos\bigl( \frac r2 \Pi_X\bigr) p_r + \i \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{2} \sin\bigl( \frac r2 \Pi_X\bigr) \\
%
&\hspace{145pt}- \i \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{2}\cos\bigl( \frac r2 \Pi_X\bigr).
\end{align*}
We plug the second term of \eqref{Tcal3_eq1}, written in this form, back into \eqref{Tcal3_eq3} and obtain
%When evaluated in the inner product with $2 AA^*\Psi\alpha_*$ and $\Psi\alpha_*$, the second term on the right side of \eqref{Tcal3_eq1} therefore reads
\begin{align}
2 \i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X  \cos\bigl( \frac r2 \Pi_X\bigr)\; \alpha_*(r)\; \Psi(X) \hspace{-350pt}& \notag\\
%
&= 2 \i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^* \Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) \; p_r\alpha_*(r)\; \Psi(X) \notag \\
%
&\hspace{20pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \;  \alpha_*(r) \; \cos\bigl( \frac r2 \Pi_X\bigr)\Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r)\; \Psi(X) \notag \\
%
&\hspace{20pt} - \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr)\Pi_X^2 \sin\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X).\label{MainTerm_7}
\end{align}
Notice that the first term on the right side equals $(-1)$ times the term on the left side. Thus, the left side equals $\frac 12$ times the third line plus the fourth line. To compute the third line of \eqref{MainTerm_7} we use \eqref{PiX-term} with the choice $\Phi = AA^*\Psi$. A short computation shows that \eqref{PiX-term_2} holds equally with $\cos$ and $\sin$ interchanged. Accordingly, $(-1)$ times the fourth line of \eqref{MainTerm_7} equals
\begin{equation*}
	\langle AA^*\Psi, (1 -AA^*) \Pi^2\Psi\rangle + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X). 
\end{equation*}
%\begin{align}
%\sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2\sin\bigl( \frac r2 \Pi_X\bigr) &= \sin^2\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 + \cos^2\bigl( \frac r2 \Pi_X\bigr) |\Bbold\wedge r|^2 \notag\\
%%
%&\hspace{-60pt}- \i \bigl[ \Pi_X\sin\bigl( \frac r2 \Pi_X\bigr)\cos\bigl( \frac r2 \Pi_X\bigr) + \sin\bigl( \frac r2 \Pi_X\bigr)\cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X\bigr]\Bbold\wedge r, \label{MainTerm_8}
%\end{align}
In combination, these considerations imply that the left side of \eqref{MainTerm_7} is given by
%=======
%When evaluated in the inner product with $AA^*\Psi\alpha_*$ and $\Psi\alpha_*$, the second term on the right side of \eqref{Tcal3_eq1} therefore reads
%\begin{align*}
%\i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; \ov{p_r\alpha_*(r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X  \cos\bigl( \frac r2 \Pi_X\bigr)\; \alpha_*(r)\; \Psi(X) \hspace{-350pt}&\\
%%
%&= \i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{AA^* \Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X \cos\bigl( \frac r2 \Pi_X\bigr) \; p_r\alpha_*(r)\; \Psi(X)\\
%%
%&\hspace{20pt} - \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; \alpha_*(r) \; \sin\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{2} \sin\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r) \; \Psi(X) \\
%%
%&\hspace{20pt} + \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \;  \alpha_*(r) \; \cos\bigl( \frac r2 \Pi_X\bigr)\frac{\Pi_X^2}{2} \cos\bigl( \frac r2 \Pi_X\bigr) \; \alpha_*(r)\; \Psi(X) .
%\end{align*}
%Notice that the first term on the right side equals $(-1)$ times the term on the left side. Thus, the left side equals $\frac 12$ times the third plus fourth line. We also note that the term in the last line equals \eqref{PiX-term} with the left $\Psi$ replaced by $AA^*\Psi$. Moreover, we claim that the term in the third line equals
%>>>>>>> Stashed changes
\begin{align}
&\frac 12 \langle AA^*\Psi, AA^* \Pi^2\Psi\rangle - \frac 12 \langle AA^*\Psi, (1 -AA^*) \Pi^2\Psi\rangle \notag \\
%
&\hspace{20pt}+ \frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X) \notag\\
%
&\hspace{20pt} - \frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold\wedge r|^2  \alpha_*(r)^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X). \label{Tcal3_eq4}
\end{align}
We note that the third term in \eqref{Tcal3_eq4} cancels the second term in \eqref{Tcal3_eq3}. Adding all this to \eqref{MainTerm_4}, we find
\begin{align}
\langle A^*\Psi, \Tcal_3 A^*\Psi\rangle &= \frac 12 \langle \Psi, AA^* AA^* \Pi^2 \Psi\rangle - \frac 12 \langle \Psi, AA^* (1 - AA^*) \Pi^2 \Psi\rangle  \notag\\
%
&\hspace{-10pt} + 2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\ 
%
&\hspace{-10pt}+ \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \;  \sin^2\bigl( \frac r2 \Pi_X\bigr)\; \Psi(X). \label{Tcal3_result}
\end{align}
The corresponding result for $\langle A^*\Psi, \Tcal_4 A^*\Psi\rangle$ is obtained by taking the complex conjugate of the right side of \eqref{Tcal3_result}, which amounts to interchanging the roles of $AA^*\Psi$ and $\Psi$ in the last two lines.

We are now prepared to collect our results and to provide the final formula for \eqref{Tcal_first_line}. We need to collect the terms in \eqref{Tcal1-Result}, \eqref{Tcal2_result}, \eqref{Tcal3_result} and the complex conjugate of \eqref{Tcal3_result}. The terms involving $|\nabla \alpha_*|^2$ read
\begin{align}
&2\fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)}\;  |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) + 2\langle AA^*\Psi, AA^*\Psi\rangle \Vert \nabla \alpha_*\Vert_2^2 \notag \\
%
&\hspace{50pt}-2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \notag \\
%
&\hspace{50pt}- 2 \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\Psi(X)} \; |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \;  AA^*\Psi(X). \label{nablaterms}
\end{align}
When we insert the factor $1 = \cos^2(\frac r2 \Pi_X) + \sin^2(\frac r2\Pi_X)$ in the second term, we obtain the final result for the terms proportional to $|\nabla \alpha_*|^2$.

%By summarizing the first two lines according to $(1 - AA^*)\Psi$, and writing
%\begin{align*}
%\langle AA^*\Psi, AA^*\Psi\rangle \Vert \nabla\alpha_*\Vert^2 &= \fint_{Q_B}\dd X\int_{\Rbb^3}\dd r \; \ov{AA^*\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%& \hspace{5pt} +\fint_{Q_B}\dd X\int_{\Rbb^3}\dd r \; \ov{AA^*\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X),
%\end{align*}
%we get that \eqref{nablaterms} is equal to
%\begin{align*}
%&2\fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{(1-AA^*)\Psi(X)}\;  |\nabla \alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X) \\
%%
%&\hspace{30pt}-2 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{(1 - AA^*)\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%&\hspace{30pt}+2\fint_{Q_B}\dd X\int_{\Rbb^3}\dd r \; \ov{AA^*\Psi(X)} \; |\nabla\alpha_*(r)|^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr)\; AA^*\Psi(X).
%\end{align*}
%Summarizing the first two lines gives the final result 

The terms proportional to $\alpha_*^2$ with magnetic fields read
\begin{align*}
%\begin{split}
&\frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; |\Bbold\wedge r|^2 \alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr)  \; \Psi(X) \\
%
&\hspace{30pt} + \frac 12\langle AA^*\Psi, AA^*\Psi\rangle \int_{\Rbb^3} \dd r \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \\
%
&\hspace{30pt}-  \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2 \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; \Psi(X)  \\
%
&\hspace{30pt}-  \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{\Psi(X)} \; |\Bbold \wedge r|^2\alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X).%\end{split} \label{magneticterms}
\end{align*}
When we insert $1 = \cos^2(\frac r2 \Pi_X) + \sin^2(\frac r2\Pi_X)$ in the second term we can bring these terms in the claimed form.

%Summarizing the first two terms according to $(1 - AA^*)\Psi$ and writing
%\begin{align*}
%\langle AA^*\Psi, AA^*\Psi\rangle \int_{\Rbb^3} \dd r \; |\Bbold \wedge r|^2 \alpha_*(r)^2 = &\\
%%
%&\hspace{-130pt}= \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \;  |\Bbold \wedge r|^2 \alpha_*(r)^2  \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%&\hspace{-120pt} + \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \;  |\Bbold \wedge r|^2 \alpha_*(r)^2 \;  \cos^2\bigl( \frac r2 \Pi_X\bigr)  \; AA^*\Psi(X), 
%\end{align*}
%we see that we can write \eqref{magneticterms} as
%\begin{align*}
%&\frac 12 \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r \; \ov{(1-AA^*)\Psi(X)} \;  |\Bbold\wedge r|^2 \alpha_*(r)^2\; \sin^2\bigl( \frac r2 \Pi_X\bigr)\;  \Psi(X) \\
%%
%&\hspace{30pt} - \frac 12 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{(1-AA^*)\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2  \; \sin^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X) \\
%%
%&\hspace{30pt}+ \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{AA^*\Psi(X)} \; |\Bbold \wedge r|^2 \alpha_*(r)^2  \; \cos^2\bigl( \frac r2 \Pi_X\bigr) \; AA^*\Psi(X).
%\end{align*}
%Combining the first two lines yields the claimed equation. 

Finally, we collect the terms proportional to $\alpha_*^2$ but without magnetic field. Taking into account the first term in \eqref{Tcal_first_line}, we find
\begin{align*}
&2\langle \Psi, AA^*(1 - AA^*)\Psi\rangle + \langle \Psi, AA^*\Pi^2\Psi\rangle + \langle \Psi, AA^*(1 - AA^*)\Pi^2\Psi\rangle - \langle \Psi, AA^* AA^* \Pi^2 \Psi\rangle \\
%
&\hspace{50pt}= 2\langle \Psi, AA^*(1 - AA^*)(1 + \Pi^2)\Psi\rangle.
\end{align*}
To obtain the result, we used that the terms coming from $\Tcal_3$ and $\Tcal_4$ are actually the same because $AA^*$ and $1 - AA^*$ commute with $\Pi^2$, see Lemma \ref{AAstar_Positive}. This proves \eqref{MainTerm_5} and the lower bound \eqref{MainTerm_LowerBound} is implied by the operator bounds in Lemma \ref{AAstar_Positive} as well.
%
%The estimate is true because the terms proportional to $|\nabla \alpha_*|^2$ and $|\Bbold \wedge r|^2\alpha_*^2$ are written in a commutative way. Hence, they are nonnegative.
\end{proof}

\subsubsection{Step two -- estimating the cross terms}

In the second step of the proof of Proposition \ref{First_Decomposition_Result} we estimate the cross terms that we obtain when the decomposition in \eqref{First_Decomposition_Result_Decomp} with $\Psi$ and $\xi_0$ in \eqref{Def_Psixi} is inserted into the left side of \eqref{First_Decomposition_Result_Assumption}. 

%Our result, that is Lemma~\ref{Decomp_Low_Momenta_Crossterms} should be compared to 
%\cite[Lemma 29]{Hainzl2017} It turns out that these can be bounded in terms of the operator $1 -A^*A$, which is the operator on the left side of \eqref{First_Decomposition_Result_Assumption}, with $\pi_r^2$ dropped for a lower bound. The result can be viewed as a low-energy estimate on $\Psi$ because the operator $AA^*(1 - AA^*)$ is bounded from below by $\Pi^2$ only for small values of $\Pi^2$, see Lemma \ref{AAstar_Positive}. Parts of Lemma \ref{Decomp_Low_Momenta_Crossterms} were already obtained in . 
%
%It turns out that these can be estimated in terms of the low-energy operator $1 - A^*A$, which we 
%This is the content of Lemma \ref{Decomp_Low_Momenta_Crossterms}. It contains a bound on $\langle \Psi, AA^*(1 - AA^*)\Psi\rangle$ and the $\Lsymm$ norm of $\xi_0$. 
%Roughly speaking, this preliminary lemma provides a low-energy estimate on $\Psi$, because the operator $AA^*(1 - AA^*)$ is bounded from below by $\Pi^2$ only for small values of $\Pi^2$, see Lemma \ref{AAstar_Positive}. However, this will be enough to bound the cross-terms that will arise when we insert the decomposition \eqref{Def_Psixi} of $\alpha$ into the operator in \eqref{First_Decomposition_Result_Assumption}.
\begin{lem}
\label{Decomp_Low_Momenta_Crossterms}
Given $D_0, D_1 \geq 0$, there is $B_0>0$ with the following properties. If, for some $0< B\leq B_0$, the wave function $\alpha\in \Lsymm$ satisfies
\begin{align*}
\frac 12 \langle \alpha , [U^* (1 - P)U + U(1 - P)U^* ]\alpha \rangle \leq D_0 B\, \Vert \alpha \Vert_2^2 + D_1B^2,
\end{align*}
then $\Psi$ and $\xi_0$ in \eqref{Def_Psixi} satisfy the estimate
\begin{align}
\langle \Psi, AA^*(1 - AA^*)\Psi\rangle + \Vert \xi_0\Vert_2^2 \leq C \bigl( B  \Vert \Psi \Vert_2^2 +D_1 B^2\bigr). \label{Estimate_Low_Momenta}
\end{align}
Furthermore, for any $\eta >0$ we have
\begin{align}
|\langle \xi_0, [U(1-P)(1+\pi_r^2)(1-P)U^* + U^* (1-P)(1+\pi_r^2)(1-P)U] A^*\Psi\rangle| & \notag \\
%
&\hspace{-180pt}\leq \eta \, \Vert \Pi\Psi\Vert^2 + C \left(1+ \eta^{-1} \right)\, \bigl( B \Vert \Psi \Vert_2^2 + D_1B^2\bigr). \label{Tcal_CrossTerms} 
\end{align}
\end{lem}

\begin{proof}
We start by noting that $A\xi_0 =0$ implies $\langle \xi_0, A^*\Psi\rangle =0$, and hence
\begin{align}
\Vert \alpha\Vert_2^2 = \Vert A^*\Psi\Vert_2^2 + \Vert \xi_0\Vert_2^2 \leq \Vert \Psi\Vert_2^2 + \Vert \xi_0\Vert_2^2. \label{Decomp_Low_Momenta_1}
\end{align}
We use $\alpha \in \Lsymm$ and $A(1 - A^*A)A^* = AA^*(1 - AA^*)$ to see that
\begin{align}
D_0 B \Vert \alpha\Vert_2^2 + D_1 B^2 &\geq \frac 12 \langle \alpha, [U^* (1 - P)U + U(1 - P)U^* ]\alpha \rangle = \langle \alpha, (1 - A^*A) \alpha\rangle \notag\\
%
&= \langle A^*\Psi, (1 - A^*A)A^*\Psi\rangle + \langle \xi_0, (1- A^*A) A^*\Psi\rangle + \langle A^*\Psi, (1- A^*A)\xi_0\rangle \notag \\
%
&\hspace{230pt} + \langle \xi_0 , (1- A^*A)\xi_0\rangle \notag \\
%
&= \langle \Psi, AA^*(1 - AA^*) \Psi\rangle + \Vert \xi_0\Vert_2^2. \label{Decomp_Low_Momenta_9}
\end{align}
From Lemma~\ref{AAstar_Positive} we know that the first term on the right side is nonnegative and hence
\begin{equation*}
	\Vert \xi_0\Vert_2^2 \leq D_0 B \Vert \alpha\Vert_2^2 + D_1 B^2.
\end{equation*}
Together with \eqref{Decomp_Low_Momenta_1}, this also proves
\begin{equation*}
(1 - D_0B)\Vert \alpha\Vert_2^2 \leq \Vert \Psi\Vert_2^2 + D_1 B^2. %\label{Bound_on_Psi_First}
\end{equation*}
Finally, this last bound \eqref{Decomp_Low_Momenta_9} prove \eqref{Estimate_Low_Momenta}.

Next we prove \eqref{Tcal_CrossTerms}. Let us define 
\begin{align}
\Tcal := U^* (1 - P)(1 + \pi_r^2)(1 - P)U + U(1 - P)(1 + \pi_r^2)(1 - P)U^* \label{Tcal_Op_Def}
\end{align}
and consider $\langle \xi_0, \Tcal A^*\Psi\rangle$. We note that $A\xi_0 =0$ implies $PU \xi_0 = 0 = PU^*\xi_0$, where the projection $P$ is understood to act on the relative coordinate. In combination with \eqref{MainTerm_6} this allows us to see that
\begin{align}
\langle \xi_0, \Tcal A^*\Psi\rangle &= \Bigl\langle \xi_0, \Bigl[2\tilde \pi_r^2 + \frac{\Pi_X^2}{2} \Bigr] A^*\Psi\Bigr\rangle - \langle \xi_0, (U^* + U) \pi_r^2 \, \alpha_* AA^*\Psi\rangle \label{Decomp_Low_Momenta_2}
\end{align}
holds. We use \eqref{PiXcos} and \eqref{PiXsin} to commute $\Pi_X^2$ in the first term on the right side of \eqref{Decomp_Low_Momenta_2} to the right and find
%\begin{align*}
%\Pi_X^2 \cos\bigl( \frac r2 \Pi_X\bigr) = \cos\bigl( \frac r2 \Pi_X\bigr) \Pi_X^2 - 2\i \sin\bigl( \frac r2 \Pi_X\bigr)\Pi_X\Bbold \wedge r  + |\Bbold\wedge r|^2\cos\bigl( \frac r2 \Pi_X\bigr).
%\end{align*}
%The above implies
\begin{align}
\frac 12\langle \xi_0, \Pi_X^2 A^*\Psi\rangle &= \frac 12\langle \xi_0, A^*\Pi_X^2\Psi\rangle \notag \\
%
&\hspace{10pt}- \i \fint_{Q_B} \dd X\int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \; \Bbold \wedge r\; \alpha_*(r) \; \Pi_X \Psi(X) \notag \\
%
&\hspace{10pt}+ \frac 12\fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \; \ov{\xi_0(X,r)}  \; \cos\bigl( \frac r2 \Pi_X\bigr) \;  |\Bbold\wedge r|^2 \alpha_*(r) \; \Psi(X). \label{Decomp_Low_Momenta_4}
\end{align}
The first term on the right side vanishes because $A\xi_0 =0$. Similarly, we apply \eqref{pirtilde_cos_pr} and \eqref{pirtilde_sin_pr} to commute $\tilde \pi_r^2$ in the first term in \eqref{Decomp_Low_Momenta_2} to the right and find
%We obtain
%\begin{align*}
%\tilde \pi_r^2 \cos\bigl( \frac r2 \Pi_X\bigr) &= \cos\bigl( \frac r2 \Pi_X\bigr) p^2 + \i \sin\bigl( \frac r2 \Pi_X\bigr) \Pi_X p + \cos\bigl( \frac r2 \Pi_X\bigr) \frac{\Pi_X^2}{4}.
%\end{align*}
%Hence,
\begin{align}
2\langle \xi_0, \tilde \pi_r^2A^*\Psi\rangle &= 2 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \cos\bigl( \frac r2 \Pi_X\bigr) \; p^2\alpha_*(r) \; \Psi(X) \notag \\ %\label{Decomp_Low_Momenta_5} \\
%
&\hspace{20pt} + 2\i \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r \, \ov{\xi_0(X,r)} \;  \sin\bigl( \frac r2 \Pi_X\bigr) \; p\alpha_*(r) \; \Pi_X\Psi(X). \label{Decomp_Low_Momenta_6}
\end{align}
%Using that $\alpha_*$ is radial, $p\alpha_*(r)$ is proportional to $e_r$, whence $p\alpha_*(r)\cdot \Bbold \wedge r =0$. Therefore, 
When we combine $\pi_r^2 \alpha_*(r) = p_r^2\alpha_*(r) + \frac 14|\Bbold \wedge r|^2\alpha_*(r)$, which holds because $\alpha_*$ is radial, \eqref{Decomp_Low_Momenta_2}, \eqref{Decomp_Low_Momenta_4} and \eqref{Decomp_Low_Momenta_6}, we obtain
\begin{align*}
\langle \xi_0, \Tcal A^*\Psi\rangle &= 2 \fint_{Q_B} \dd X \int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \cos\bigl( \frac r2 \Pi_X\bigr) \; \pi_r^2\alpha_*(r) \; (1 - AA^*)\Psi(X) \\
%
&\hspace{30pt}+ 2\i \fint_{Q_B}\dd X\int_{\Rbb^3} \dd r\; \ov{\xi_0(X,r)} \; \sin\bigl( \frac r2 \Pi_X\bigr) \; \bigl[ p - \frac 12\Bbold \wedge r\bigr] \alpha_*(r) \; \Pi_X\Psi(X).
\end{align*}
Using Cauchy-Schwarz, we bound the absolute value of this by
\begin{align}
|\langle \xi_0, \Tcal A^*\Psi\rangle| \leq 2\Vert \xi_0\Vert_2 \; \bigl[ \Vert \pi_r^2\alpha_*\Vert_2 \; \Vert (1 - AA^*)\Psi\Vert_2 + \bigl(\Vert \nabla \alpha_*\Vert_2 + B \Vert \, | \cdot  |\alpha_*\Vert_2\bigr) \Vert \Pi\Psi\Vert_2\bigr], \label{Decomp_Low_Momenta_7}
\end{align}
%Since $\alpha_*$ is radial, $\Vert \pi_r^2\alpha_*\Vert_2 \leq \Vert p^2\alpha_*\Vert_2 + B \Vert \, |\cdot|^2\alpha_*\Vert_2$, so this expression is uniformly bounded in $B$ for bounded $B$. 
and with the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar} we see that the norms of $\alpha_*$ on the right side are bounded uniformly in $0 \leq B \leq B_0$. Moreover, Lemma~\ref{AAstar_Positive} and \eqref{Estimate_Low_Momenta} imply that there is a constant $c>0$ such that
\begin{equation}
	\Vert (1 - AA^*)\Psi\Vert_2^2 \leq \langle \Psi, (1-AA^*) \Psi \rangle \leq \frac{1}{c} \langle \Psi, A A^* (1-AA^*) \Psi \rangle \leq C \bigl( B  \Vert \Psi \Vert_2^2 +D_1 B^2\bigr).
\end{equation}
%Using the inequality $ab \leq \eta a^2 + \frac{1}{4\eta} b^2$ for $\eta>0$ and $a,b\geq 0$, we obtain
For $\eta >0$ we thus obtain
\begin{align}
|\langle \xi_0, \Tcal A^*\Psi\rangle| \leq C \bigl[ \eta\,  \Vert \Pi\Psi\Vert_2^2 + \eta^{-1} \, \Vert \xi_0 \Vert_2^2 + \bigl( B \Vert \Psi \Vert_2^2 +D_1 B^2\bigr) \bigr] \label{Decomp_Low_Momenta_8}
\end{align}
%By Lemma \ref{AAstar_Positive}, there is a constant $c>0$ such that
%\begin{align*}
%(1 - AA^*)^2 &\leq \frac 1c \; AA^* (1 - AA^*)^2 \leq \frac 1c \; AA^* (1- AA^*), %\label{Decomp_Low_Momenta_9}
%\end{align*}
%and $\Vert (1 - AA^*)\Psi\Vert^2 \leq \frac 1c \langle \Psi, AA^*(1 - AA^*)\Psi\rangle$. 
and an application of \eqref{Estimate_Low_Momenta} proves the claim.
\end{proof}

\subsubsection{Proof of Proposition \ref{First_Decomposition_Result}}

We recall the decomposition $\alpha = A^*\Psi + \xi_0$ with $\Psi$ and $\xi_0$ in \eqref{Def_Psixi} as well as $\Tcal$ in \eqref{Tcal_Op_Def}. From \eqref{First_Decomposition_Result_Assumption} we know that
\begin{align}
D_0 B \Vert\alpha\Vert_2^2 + D_1 B^2  \geq \langle A^*\Psi, \Tcal A^*\Psi\rangle + 2\Re\langle \xi_0, \Tcal A^*\Psi\rangle + \langle \xi_0, \Tcal\xi_0\rangle . \label{First_Decomposition_Result_1}
\end{align}
With the help of Lemma \ref{CommutationI}, the identities $PU\xi_0 = 0 = PU^*\xi_0$ imply
\begin{align}
\langle \xi_0, \Tcal \xi_0 \rangle = \Bigl\langle \xi_0, \bigl(2 + \frac{\Pi_X^2}{2} + 2\tilde \pi_r^2\bigr) \xi_0\Bigr\rangle \geq \frac 12 \, \Vert \xi_0\Vert_\Hsymm^2. \label{First_Decomposition_Result_2}
\end{align}
Lemma \ref{AAstar_Positive} guarantees the existence of a constant $\rho>0$ such that
\begin{align*}
AA^*(1 - AA^*)(1 + \Pi^2) \geq \rho\; \Pi^2.
\end{align*}
Therefore, \eqref{MainTerm_LowerBound} implies 
%that the first term of \eqref{First_Decomposition_Result_1} is bounded from below by
\begin{align}
\langle A^* \Psi, \Tcal A^*\Psi\rangle \geq 2\, \langle \Psi, AA^*(1 - AA^*) (1 + \Pi^2)\Psi\rangle \geq 2\rho\, \langle \Psi, \Pi^2\Psi\rangle. \label{First_Decomposition_Result_3}
\end{align}

To estimate the second term on the right side of \eqref{First_Decomposition_Result_1}, we note that $\Tcal$ is bounded from below by $U(1 - P)U^* + U^*(1-P)U$. Therefore, we may apply Lemma \ref{Decomp_Low_Momenta_Crossterms} with $\eta = \frac \rho2$ and find
\begin{align*}
2\Re \langle \xi_0, \Tcal A^*\Psi\rangle \geq -2\, |\langle \xi_0, \Tcal A^*\Psi\rangle| \geq - \rho \, \Vert \Pi\Psi\Vert_2^2 - C\bigl( B\Vert \Psi\Vert_2^2 + D_1 B^2\bigr).
\end{align*}
In combination with \eqref{First_Decomposition_Result_1}, \eqref{First_Decomposition_Result_2} and \eqref{First_Decomposition_Result_3}, we thus obtain
\begin{align*}
C\bigl( B\Vert \Psi\Vert_2^2 + D_1B^2 \bigr)\geq \rho \, \Vert \Pi\Psi\Vert_2^2 + \frac 12 \, \Vert \xi_0\Vert_\Hsymm^2.
\end{align*}
This proves \eqref{First_Decomposition_Result_Estimate}. %The estimate \eqref{First_Decomposition_Result_Estimate_psi} on $\Vert \Psi\Vert_2^2$ is \eqref{Bound_on_Psi_First}.

==> source/BCS-Theory_General_Field/5_Structure_of_Low-Energy_States/5.3_Uniform_bound_on_Psi.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Uniform estimate on \texorpdfstring{$\Vert\Psi\Vert_2$}{Psi}}

Up to now we neglected the nonlinear term on the left side of \eqref{Lower_Bound_A_2}. This term provides the inequality
\begin{align}
		\Tr\bigl[(\alpha^* \alpha)^2\bigr] \leq C \left( B \Vert \alpha\Vert_2^2 + B^2 \right). \label{Lower_Bound_A_2b}
\end{align}
In this section we will take this term and \eqref{Lower_Bound_A_2b} into account and show that it can be combined with Proposition~\ref{First_Decomposition_Result} to obtain a bound for $\Vert \Psi\Vert_2$. This will afterwards allow us to prove Theorem~\ref{Structure_of_almost_minimizers}.

\begin{lem}
\label{Bound_on_psi}
Given $D_0\geq0$, there is $B_0>0$ such that for all $0 < B \leq B_0$ the following holds. If the wave function $\alpha\in \Lsymm$ obeys \eqref{Lower_Bound_A_2} then $\Psi$ in \eqref{Def_Psixi} satisfies
\begin{align}
\Vert \Psi\Vert_2^2 &\leq CB. \label{Bound_on_psi_result}
\end{align}
\end{lem}

\begin{proof}
We recall the decomposition $\alpha = A^*\Psi + \xi_0$ with $\Psi$ and $\xi_0$ in \eqref{Def_Psixi}. Eq.~\eqref{Lower_Bound_A_2b} and an application of the triangle inequality imply
\begin{align}
C\bigl( B\Vert \Psi\Vert_2^2 + B^2\bigr)^{\nicefrac 14} \geq \Vert \alpha\Vert_4 \geq \Vert A^*\Psi\Vert_4 - \Vert \xi_0\Vert_4. \label{Nonlinearity_8}
\end{align}
Thus, it suffices to prove an upper bound for $\Vert \xi_0\Vert_4$ and a lower bound for $\Vert A^*\Psi\Vert_4$. Our proof follows closely the proof of \cite[Eq. (5.48)]{Hainzl2012}. 

\emph{Step 1.} Let us start with the upper bound on $\Vert \xi_0\Vert_4$. We claim the estimate
\begin{align}
\Vert \xi_0\Vert_4 \leq C \bigl( B^{\nicefrac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18} \Vert \Psi\Vert_2 + B^{\nicefrac 12}\bigr).
%C\bigl( B^{\nicefrac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18}\bigr) \;  \bigl(1 + B^{\nicefrac 12} \Vert \Psi\Vert_2\bigr)^{\nicefrac 12}. 
\label{Nonlinearity_1}
\end{align}
To see this, we first use Hölder's inequality to estimate $\Vert \xi_0\Vert_4^4 \leq \Vert \xi_0\Vert_2^2 \; \Vert \xi_0\Vert_\infty^2$. From Proposition~\ref{First_Decomposition_Result} we know that $\Vert \xi_0\Vert_2^2 \leq C(B\Vert \Psi\Vert_2^2+ B^2)$, and it thus remains to prove a bound for $\Vert \xi_0\Vert_\infty$. We claim that for any $\nu > 3$
\begin{align}
\Vert \xi_0\Vert_\infty \leq  1 + C_\nu\, B^{-\nicefrac 14} \, \Vert (1 + |\cdot |)^\nu \alpha_*\Vert_{\nicefrac 65} \; \Vert \Psi \Vert_6, \label{Claim_xi_infty}
\end{align}
where the right side is finite by the decay properties of $\alpha_*$ in \eqref{Decay_of_alphastar}. To prove \eqref{Claim_xi_infty}, we first note that \eqref{gamma_alpha_fermionic_relation} implies $\Vert \alpha\Vert_\infty\leq 1$, and hence $\Vert \xi_0\Vert_\infty \leq 1 + \Vert A^*\Psi\Vert_\infty$. We apply Lemma \ref{Schatten_estimate} (b) to $A^*\Psi$ and obtain \eqref{Claim_xi_infty}. We also combine \eqref{Magnetic_Sobolev} with Proposition \ref{First_Decomposition_Result} and obtain $
\Vert \Psi\Vert_6 \leq C( \Vert \Psi\Vert_2 + B^{\nicefrac 12})$. In combination, these considerations imply \eqref{Nonlinearity_1}. 

\emph{Step 2.} We claim that
\begin{align}
\Vert A^*\Psi\Vert_4^4 \geq \frac 1{16} \; \Vert \hat \alpha_* \Vert_4^4 \; \Vert \Psi\Vert_4^4 - C \bigl( B^{\nicefrac 18} \Vert \Psi\Vert_2 + B^{\nicefrac 58} \bigr)^4 \label{Nonlinearity_5}
\end{align}
holds. To prove \eqref{Nonlinearity_5}, we write $\Vert A^*\Psi\Vert_4^4 = \tr ((A^*\Psi)^* A^*\Psi)^2$. The fact that $\alpha_*$ is real-valued implies
\begin{align*}
\Vert A^*\Psi\Vert_4^4 &= \fint_{Q_B} \dd x \int_{\Rbb^3} \dd y \; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(x - z)\ov{ \left[ \cos\bigl( \frac{x - z}{2}\Pi_{\frac{x+z}{2}}\bigr)  \Psi\bigl( \frac{x+z}{2}\bigr) \right] } \mathop \times\\
%
&\hspace{150pt} \times \alpha_*(z-y) \left[ \cos\bigl( \frac{z-y}{2} \Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z+y}{2}\bigr) \right] \Bigr|^2.
\end{align*}
We use $\cos(x) = 1 - 2\sin^2(\frac x2)$ twice and find
\begin{align}
\Vert A^*\Psi\Vert_4^4 &\geq \frac 14 \Tcal_* - C \, (\Tcal_1 + \Tcal_2), \label{Nonlinearity_2}
\end{align}
where
\begin{align*}
\Tcal_* &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \;\Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(x - z) \ov{\Psi\bigl(\frac{x+z}{2}\bigr)} \alpha_*(z - y) \Psi\bigl( \frac{z+y}{2}\bigr)\Bigr|^2
\end{align*}
and 
\begin{align}
\Tcal_1 &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \;\Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(x - z) \ov{\Psi\bigl( \frac{x+z}{2}\bigr)} \mathop \times \notag\\
%
&\hspace{140pt} \times \alpha_*(z - y) \left[ \sin^2\bigl( \frac{z-y}{4} \Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z +y}{2}\bigr) \right] \Bigr|^2, \notag\\
%
\Tcal_2 &:= \fint_{Q_B} \dx \int_{\Rbb^3} \dy \; \Bigl| \int_{\Rbb^3} \dd z\; \alpha_*(x - z)\ov{ \left[ \sin^2\bigl( \frac{x -z}{4} \Pi_{\frac{x+z}{2}}\bigr) \Psi\bigl( \frac{x + z}{2}\bigr) \right]} \mathop \times \notag \\
%
&\hspace{140pt} \times\alpha_*(z - y) \left[ \cos\bigl( \frac{z - y}{2}\Pi_{\frac{z+y}{2}}\bigr)  \Psi\bigl( \frac{z+y}{2}\bigr) \right] \Bigr|^2. \label{Nonlinearity_3}
\end{align}
In the following we derive a lower bound on $\Tcal_*$ and an upper bound on $\Tcal_1$ and $\Tcal_2$.

\emph{Lower bound on $\Tcal_*$.} We change variables $z\mapsto z + x$ and $y\mapsto y + x$ and afterwards replace $x$ by~$X$, which allows us to write
\begin{align}
\Tcal_* = \fint_{Q_B} \dd X \int_{\Rbb^3} \dy \; \Bigl| \int_{\Rbb^3} \dd z \;  \alpha_*(z) \ov{\Psi\bigl(X + \frac z2\bigr)} \alpha_*(z - y) \Psi\bigl(X + \frac{z+y}{2}\bigr)\Bigr|^2. \label{Nonlinearity_9}
\end{align}
Next, we combine $\Psi(X + \frac z2) = \e^{\i \frac z2P_X} \Psi(X)$ and the identity $\e^{\i \frac r2P_X} = \e^{\i \frac \Bbold 2 r\wedge X}\e^{\i \frac r2\Pi_X}$ in \eqref{representation_Ustar} to write $\Psi(X + \frac z2) = \e^{\i \frac \Bbold 2 z\wedge X} \e^{\i \frac z2\Pi_X} \Psi(X)$. 
%Similarly, $\Psi(X + \frac{z+y}{2}) = \e^{\i \frac{\Bbold }{2} (z+y)\wedge X} \e^{\i\frac{z+y}{2}\Pi_X}\Psi(X)$. 
We conclude that
\begin{align*}
\ov{\Psi\bigl( X + \frac z2\bigr)} \Psi\bigl(X + \frac{z+y}{2}\bigr) = \e^{\i \frac{\Bbold}{2} y\wedge X} \; \ov{\left[ \e^{\i \frac{z}{2}\Pi_X}\Psi(X) \right]} \; \left[ \e^{\i \frac{z+y}{2}\Pi_X} \Psi(X) \right],
\end{align*}
as well as
\begin{align*}
\Tcal_* = \fint_{Q_B} \dd X \int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(-z) \ov{ \left[ \e^{\i \frac z2\Pi_X} \Psi(X) \right]} \alpha_*(z - y) \left[ \e^{\i \frac{z+y}{2}\Pi_X} \Psi(X) \right] \Bigr|^2.
\end{align*}
This also implies
\begin{align}
\Tcal_* \geq \frac 14\Tcal_*^* - C(\Tcal_*^{(1)} + \Tcal_*^{(2)})
\label{eq:A1}
\end{align}
with
\begin{align*}
\Tcal_*^* := \fint_{Q_B}\dd X\int_{\Rbb^3}\dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(z)^t \ov{\Psi(X)} \alpha_*(z - y)^t \Psi(X)\Bigr|^2
\end{align*}
and
\begin{align}
\Tcal_*^{(1)} &:= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \; \alpha_*(z) \ov{\bigl[\e^{\i \frac{z}{2}\Pi_X}\Psi(X)\bigr]} \alpha_*(z - y) \bigl[\bigl( \e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X)\bigr]\Bigr|^2, \notag \\
%
\Tcal_*^{(2)} &:= \fint_{Q_B} \dd X\int_{\Rbb^3} \dd y\; \Bigl| \int_{\Rbb^3} \dd z \;\alpha_*(z)  \ov{\bigl[\bigl( \e^{\i \frac z2\Pi_X} - 1\bigr) \Psi(X)\bigr]} \alpha_*(z - y) \Psi(X)\Bigr|^2. \label{Nonlinearity_10}
\end{align}
The term $\Tcal_*^*$ equals
\begin{align*}
\Tcal_*^* = \fint_{Q_B} \dd X\; |\Psi(X)|^4 \; \int_{\Rbb^3} \dd y\;\Bigl|\int_{\Rbb^3} \dd z\; \alpha_*(z)\alpha_*(y - z)\Bigr|^2 = \Vert \Psi\Vert_{L^4(Q_B)}^4 \; \Vert \alpha_* * \alpha_*\Vert_{L^2(\Rbb^3)}^2.
\end{align*}
By \eqref{Decay_of_alphastar}, the Fourier transform of $\alpha_**\alpha_*$ equals $|\hat \alpha_*|^2$. Thus, $\Vert \alpha_* *\alpha_*\Vert_2^2 = \Vert \hat \alpha_*\Vert_4^4>0$. This is the desired leading term of \eqref{Nonlinearity_5}. 

\emph{Upper bound on $\Tcal_*^{(1)}$ and $\Tcal_*^{(2)}$.} We start with $\Tcal_*^{(1)}$, expand the square and estimate
\begin{align}
&\Tcal_*^{(1)} \leq  \int_{\Rbb^3} \dd y  \int_{\Rbb^3} \dd z  \int_{\Rbb^3} \dd z' \;  | \alpha_*(z) \, \alpha_*(z') \, \alpha_*(z - y) \, \alpha_*(z' - y)| \label{Nonlinearity_13} \\
& \times \fint_{Q_B} \dd X \; \Bigl| \bigl[ \e^{\i \frac z2\Pi_X} \Psi(X) \bigr]  \bigl[ \e^{\i \frac {z'}2\Pi_X} \Psi(X) \bigr]  \bigl[ \bigl( \e^{\i \frac{z+y}{2}\Pi_X}-1\bigr) \Psi(X) \bigr]  \bigl[ \bigl( \e^{\i \frac{z'+y}{2}\Pi_X}-1\bigr) \Psi(X) \bigr] \Bigr|. \nonumber
\end{align}
When we use Hölder's inequality, \eqref{NTB-NtildeTB_3}, \eqref{ZPiX_inequality}, and \eqref{Magnetic_Sobolev} we see that the integral in the second line can be bounded by
\begin{align}
\Vert \e^{\i \frac{z}{2}\Pi} \Psi\Vert_6^2 \; \Vert (\e^{\i \frac{z+y}{2}\Pi} - 1) \Psi\Vert_6 \; \Vert (\e^{\i \frac{z+y}{2}\Pi} - 1) \Psi\Vert_2 \leq C\; \bigl|\frac{z+y}{2}\bigr| \; B^{-\nicefrac 32} \; \Vert \Pi\Psi\Vert_2^4. \label{Nonlinearity_11}
\end{align}
%
%
%
%Using Hölder in $X$, we obtain
%\begin{align*}
%\fint_{Q_B} \dd X \; |\e^{\i \frac{z}{2}\Pi_X} \Psi(X)|^2 \; \ov{\bigl(\e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X)} \; \bigl(\e^{\i \frac{z+y}{2}\Pi_X} - 1\bigr) \Psi(X) \leq &\\
%%
%&\hspace{-250pt} \leq \Bigl( \fint_{Q_B} \dd X \; |\e^{\i \frac z2\Pi_X} \Psi(X)|^6\Bigr)^{\nicefrac 13} \; \Bigl( \fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} - 1) \Psi(X)|^6\Bigr)^{\nicefrac 16} \mathop \times \\
%%
%&\hspace{-100pt} \times\Bigl( \fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} - 1) \Psi(X)|^2\Bigr)^{\nicefrac 12}.
%\end{align*}
%
%
%Use 
%
%
%
%For the first factor, note $|\e^{\i \frac z2\Pi_X}\Psi(X)| = |\Psi(X + \frac z2)|$, so that, since $|\Psi|$ is periodic, this term equals $\Vert \Psi\Vert_6^2$. As for the second factor.  For the last factor, we use the operator inequality \eqref{ZPiX_inequality} to obtain
%\begin{align*}
%\fint_{Q_B} \dd X\; |(\e^{\i \frac{z+y}{2}\Pi_X} -1)\Psi(X)|^2 &\leq \frac{|z+y|^2}{4} \; \Vert \Pi_X\Psi\Vert_2^2.
%\end{align*}
Proposition~\ref{First_Decomposition_Result} provides us with a bound for $\Vert \Pi \Psi \Vert_2$. In combination with \eqref{Nonlinearity_13}, \eqref{Nonlinearity_11}, Young's inequality, and the bound $|z + y| \leq 2|z| + |z- y|$, this implies
\begin{align}
\Tcal_*^{(1)} &\leq C \, B^{-\nicefrac 32}\,  \left( B^2 \Vert \Psi \Vert_2^4 + D_1 B^4 \right) \int_{\Rbb^3} \dd y \; \Bigl| \int_{\Rbb^3} \dd z\;  |z+y|\; |  \alpha_*(z) \alpha_*(y-z)|\Bigr|^2 \nonumber \\
&\leq C \left( B^{-\nicefrac 12} \Vert \Psi \Vert_2^4 + D_1 B^{ \nicefrac 52 } \right) \, \Vert \alpha_*\Vert_{\nicefrac 43} \, \Vert \, |\cdot|\alpha_*\Vert_{\nicefrac 43}, \label{Nonlinearity_12} 
\end{align}
where the right side is finite by \eqref{Decay_of_alphastar}. Similarly, we see that $\Tcal_*^{(2)}$ is bounded by the right side of \eqref{Nonlinearity_12}.
%\begin{align*}
%\int_{\Rbb^3} \dd z \Bigl( \int_{\Rbb^3} \dy \; \bigl| |z+y|\alpha_*(-z)\alpha_*(z-y)\bigr|^2 \Bigr)^{\nicefrac 12} \leq \sqrt{2} \Vert \alpha_*\Vert_1 \Vert |\cdot|^{\nicefrac 12}\alpha_*\Vert_2 + \Vert |\cdot|^{\nicefrac 12}\alpha_*\Vert_1 \Vert \alpha_*\Vert_2.
%\end{align*}
%All in all, we obtain a constant $0 < C < \infty$ with $\Tcal_*^{(1)} \leq C \; \Vert\Psi\Vert_6^3 \; \Vert \Pi_X\Psi\Vert_2$. Using  \eqref{Magnetic_Sobolev}, this implies the final result $\Tcal_*^{(1)} \leq C \; \Vert \Pi_X\Psi\Vert_2^4$. 
%For $\Tcal_*^{(2)}$, only \eqref{Nonlinearity_11} needs to be adjusted by the new right side $C |z| \, \Vert \Pi\Psi\Vert_2^4$. Then, \eqref{Nonlinearity_12} is estimated in the same way by $C \Vert \, |\cdot|\alpha_*\Vert_{\nicefrac 43} \Vert \alpha_*\Vert_{\nicefrac 43}$.

\emph{Upper bound on $\Tcal_1$ and $\Tcal_2$ in \eqref{Nonlinearity_3}.} Bounds for $\Tcal_1$ and $\Tcal_2$ can be obtain along the same lines as the bound for $\Tcal_*^{(1)}$. We apply the same change of variables as above and use estimates similar to the ones in \eqref{Nonlinearity_13}. In case of $\Tcal_1$, the bound in \eqref{Nonlinearity_11} needs to be replaced by
\begin{align}
\Vert \Psi\Vert_6^2 \, \bigl\Vert \sin^2\bigl( \frac{z - y}{2}  \Pi\bigr) \Psi \bigr\Vert_6 \, \bigl\Vert \sin^2\bigl( \frac{z - y}{2}  \Pi\bigr) \Psi \bigr\Vert_2 \leq C \; \frac{|z-y|}{2} \; B^{-\nicefrac 32}\,  \Vert \Pi\Psi\Vert_2^4. \label{Nonlinearity_14}
\end{align}
Here, we used $\sin^2(x) \leq |x|$ and the operator inequality in  \eqref{ZPiX_inequality} to estimate the third factor. For the first and the second factor, we used
\begin{align*}
\sin^2\bigl( \frac{z-y}{4} \Pi\bigr) = - \frac{1}{4} \bigl( 2+ \e^{\i\frac{z-y}{2} \Pi} + \e^{-\i \frac{z-y}{2}\Pi}\bigr)
\end{align*}
and \eqref{Magnetic_Sobolev} or \eqref{NTB-NtildeTB_3}, respectively. A bound for $\Tcal_2$ can be proved analogously. The final estimate we obtain in this way reads
\begin{equation}
	\Tcal_1 + \Tcal_2 \leq C \left( B^{-\nicefrac 12} \Vert \Psi \Vert_2^4 + D_1 B^{ \nicefrac 52 } \right). 
	\label{eq:A2}
\end{equation}
In combination with \eqref{Nonlinearity_2}, \eqref{eq:A1}, and \eqref{Nonlinearity_12}, this proves \eqref{Nonlinearity_5}.
%To bound $\Tcal_2$, \eqref{Nonlinearity_14} needs to be replaced by
%\begin{align*}
%\bigl\Vert \sin^2\bigl( \frac{z}{2} \Pi\bigr) \Psi \bigr\Vert_6 \, \bigl\Vert \sin^2\bigl( \frac{z}{2} \Pi\bigr) \Psi \bigr\Vert_2 \, \bigl\Vert \cos\bigl( \frac{z-y}{2} \Pi\bigr) \Psi\bigr\Vert_6^2 \leq C \; \frac{|z|}{2} \; B^{-\nicefrac 32} \, \Vert \Pi\Psi\Vert_2^4.
%\end{align*}
%Here, we used $\cos(x) = \frac 12 (\e^{\i x} + \e^{-\i x})$ and \eqref{NTB-NtildeTB_3}. Then, we obtain the bound \eqref{Nonlinearity_12} with $|z|$ instead of $|z+y|$, as for $\Tcal_*^{(2)}$.

\emph{Step 3.} We denote $c:= \frac 1{2} \Vert \hat\alpha_*\Vert_4$, insert \eqref{Nonlinearity_1} and \eqref{Nonlinearity_5} into \eqref{Nonlinearity_8} and obtain
%\begin{align*}
%C\bigl( B^{\frac 14}\Vert \Psi\Vert_2^{\nicefrac 12} + B^{\frac 18}\bigr)  &\geq  C\bigl(\Vert \Psi\Vert_2^2B + B^{\frac 12} \bigr)^{\nicefrac 14} \geq (\Vert\alpha\Vert_4^4)^{\nicefrac 14} \\
%%
%&\hspace{-80pt}\geq \bigl( c \Vert \Psi\Vert_4^4 - C( B^{\frac 12}\Vert \Psi\Vert_2 + B^{\frac 14})^4\bigr)_+^{\nicefrac 14} - C\bigl( B^{\frac 14} \Vert \Psi\Vert_2^{\nicefrac 12} + B^{\nicefrac 18}\bigr) (1 + B^{\nicefrac 12}\Vert \Psi\Vert_2)^{\nicefrac 12}.
%\end{align*}
%Using the inequality $(|x|^4 - |y|^4)_+^{\nicefrac 14} \geq |x| - |y|$, which can be seen by explicitly expanding the $4\tho$ power of the right side, employing $|y|\leq |x|$, we get
\begin{align}
C B^{\frac 14}\Vert \Psi\Vert_2^{\nicefrac 12}  \geq c \Vert \Psi\Vert_4 - CB^{\frac 18} \Vert \Psi\Vert_2 - CB^{\frac 12}, \label{Nonlinearity_6}
\end{align}
which holds for $B$ small enough. For $\eta >0$ the left side is bounded from above by a constant times $\eta \Vert \Psi\Vert_2 + \eta^{-1} B^{\frac 12}$ and Hölder's inequality implies $\Vert \Psi\Vert_4 \geq \Vert \Psi\Vert_2$. 
%\begin{align*}
%\Vert \Psi\Vert_{L^4(Q_B)} \geq B^{\frac 38} \; \Vert \Psi\Vert_{L^2(Q_B)}.
%\end{align*}
Accordingly,
\begin{equation}
C \left( \eta \Vert \Psi\Vert_2 + \eta^{-1} B^{\frac 12} \right) \geq (c - CB^{\frac 18}) \Vert \Psi\Vert_2 - CB^{\frac 12}.
\label{eq:A3}
\end{equation}
%Thus,
%\begin{align*}
%\geq c' B^{\frac 38} \Vert \Psi\Vert_2 - CB^{\frac 18}.
%\end{align*}\yexycolor
When we choose $\eta$ and $B$ in \eqref{eq:A3} small enough, this proves the claim.
%
%
%
%We may assume without loss that the right side is nonnnegative because if not, the proof is finished. If this is so, then we infer $\Vert \Psi\Vert_2 \geq CB^{-\nicefrac 14}$ so that
%\begin{align*}
%\Vert \Psi\Vert_2^{\nicefrac 12} &\leq C\bigl( B^{-\frac 18} + B^{-\frac 14} \; \Vert \Psi\Vert_2^{-\nicefrac 12}\bigr) \leq CB^{-\frac 18}.
%\end{align*}
%This proves the claim.
\end{proof}

==> source/BCS-Theory_General_Field/6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.1_BCS-energy_of_low-energy_states.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{The BCS energy of low-energy states}

In this section, we provide the lower bound on \eqref{ENERGY_ASYMPTOTICS} and the proof of Theorem~\ref{Main_Result_Tc}~(b), and thereby complete the proof of Theorems \ref{Main_Result} and \ref{Main_Result_Tc}. Let $D_1\geq 0$ and $D\in \Rbb$ be given and assume that $\Gamma$ is a gauge-periodic state at temperature $T = \Tc(1 - Dh^2)$ that satisfies \eqref{Second_Decomposition_Gamma_Assumption}. Corollary~\ref{Structure_of_almost_minimizers_corollary} provides us with a decomposition of the Cooper pair wave function $\alpha = [\Gamma]_{12}$ in terms of $\Psi_\leq$ in \eqref{PsileqPsi>_definition} and $\sigma$ in \eqref{sigma}, where $\Vert \Psi_\leq \Vert_{\Hmag^1(Q_h)} \leq C$ and where the bound
\begin{align}
	\Vert \Psi_\leq\Vert_{\Hmag^2(Q_h)}^2 &\leq C \, \varepsilon h^{-2} \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 \label{Lower_Bound_B_Psileq}
\end{align}
holds in terms of the function $\Psi$ in Theorem \ref{Structure_of_almost_minimizers}. 

With the function $\Psi_\leq$ we construct a Gibbs state $\Gamma_{\Delta}$ with the gap function $\Delta \equiv \Delta_{\Psi_\leq}$ as in \eqref{Delta_definition}. Using Proposition~\ref{BCS functional_identity}, we write the BCS free energy of $\Gamma$ as
\begin{align*}
	\FBCS(\Gamma) - \FBCS(\Gamma_0) &= - \frac 14 \langle \Delta, L_{T,B} \Delta\rangle + \frac 18 \langle \Delta, N_{T,B} (\Delta)\rangle + \Vert \Psi_\leq \Vert_2^2 \;  \langle \alpha_*, V\alpha_*\rangle \\
	%
	&\hspace{10pt}+ \Tr\bigl[\Rcal_{T,B}(\Delta)\bigr] + \frac T2 \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; V(r) \, |\sigma(X,r)|^2,
\end{align*}
where
\begin{equation*}
	\Vert \Rcal_{T,B}(\Delta) \Vert_1 \leq C \; h^6 \; \Vert \Psi \Vert_{\Hmag^1(Q_h)}^6.
\end{equation*}
We also apply Theorem~\ref{Calculation_of_the_GL-energy} to compute the terms in the first line on the right side, and find the lower bound
\begin{align}
		\FBCS(\Gamma) - \FBCS(\Gamma_0) &\geq h^4 \; \EGL(\Psi_\leq) -C \bigl( h^5 + \varepsilon h^4 \bigr) \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 \notag \\
		%
		&\hspace{30pt}+ \frac T2 \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_h} \dd X\int_{\Rbb^3} \dd r\; V(r) \, |\sigma(X,r)|^2. \label{Lower_Bound_B_2}
\end{align}
The relative entropy is nonnegative and the last term on the right side is nonpositive. In the next section we show that their sum is negligible.

==> source/BCS-Theory_General_Field/6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.2_Relative_entropy_estimates.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Estimate on the relative entropy}

In this section we prove a lower bound for the second line in \eqref{Lower_Bound_B_2}, showing that it is negligible. 
%\begin{lem}
%For all admissible BCS states $\Gamma$, we have
%\begin{align}
%T\Hcal_0(\Gamma, \Gamma_\Delta) &\geq \Tr \Bigl[ (\Gamma - \Gamma_\Delta) \frac{H_\Delta}{\tanh(\frac \beta 2H_\Delta)} (\Gamma - \Gamma_\Delta)\Bigr]. \label{LBpartB_1}
%\end{align}
%\end{lem}
%
%\begin{proof}
%The proof is given in \cite[Lemma 5]{Hainzl2012} and uses the fact that $\Gamma_\Delta$ is admissible, which follows from Lemma \ref{Gamma_Delta_admissible}.
%\end{proof}
%
%To be able to combine the term on the right side of \eqref{LBpartB_1} and the last term on the right side of \eqref{Lower_Bound_B_2}, we first need to replace the operator $H_{\Delta}$ in the second factor on the right side of \eqref{LBpartB_1} by $H_0$. To that end, we note that the estimate $H_\Delta^2\geq (1 - \delta)H_0^2 - \delta^{-1} \Vert \Delta\Vert_\infty^2$ holds for $0 < \delta < 1$ and we rewrite it as
%\begin{align}
%H_0 \leq (1 - \delta)^{-1} \bigl( H_\Delta^2 + \delta^{-1} \Vert \Delta\Vert_\infty^2\bigr). \label{LBpartB_4}
%\end{align}
%Furthermore, we note that the series expansion 
%\begin{align*}
%	\frac{x}{\tanh(\frac x2)} = 2+ \sum_{k=1}^\infty \bigl( 2 - \frac{8k^2\pi^2}{x^2 + 4k^2\pi^2}\bigr),
%\end{align*}
%see \cite[Eq. (5.14)]{Hainzl2012}, shows that the function $x \mapsto \frac{\sqrt{x}}{\tanh(\frac \beta 2\sqrt{x})}$ is operator monotone. We use this together with \eqref{LBpartB_4} and the monotonicity of the map $x \mapsto \tanh(x)$, which yields
% \begin{align*}
%	%K_{T,B} \otimes \Idbb_{\Cbb^2}
%	\begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix} = \frac{H_0}{\tanh(\frac \beta 2 H_0)}
%&\leq (1 - \delta)^{-\nicefrac 12} \frac{\sqrt{H_\Delta^2 + \delta^{-1}\Vert \Delta\Vert_\infty^2}}{\tanh(\frac \beta 2 \sqrt{H_\Delta^2 + \delta^{-1} \Vert\Delta\Vert_\infty^2})}.
%\end{align*}
%We may now Taylor expand this as
%\begin{align*}
%\begin{pmatrix}
%K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%\end{pmatrix} 
%&\leq (1 - \delta)^{-\nicefrac 12} \Bigl[\frac{H_\Delta}{\tanh(\frac \beta 2H_\Delta)} + \frac{\beta}{4} \int_0^{\delta^{-1} \Vert \Delta\Vert_\infty^2} \dd t \; g\bigl( \frac \beta 2 \sqrt{H_\Delta^2 + t}\bigr)\Bigr]
%\end{align*}
%with the nonnegative function 
%\begin{align*}
%g(x) &:= \frac{1}{x} \frac{1}{\tanh(x)} - \frac{1}{\tanh^2(x)} \frac{1}{\cosh^2(x)}.
%\end{align*}
%Using $\sup_{x \geq 0} g(x) \leq 1$ and $1 \leq \frac{x}{\tanh(x)}$, we conclude that
%\begin{align*}
%	%K_{T,B} \otimes \Idbb_{\Cbb^2} 
%	\begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix} \leq (1 - \delta)^{-\nicefrac 12} \bigl( 1 +  \frac{\delta^{-1} \beta^2}{8} \;  \Vert \Delta\Vert_\infty^2\bigr) \frac{H_\Delta}{\tanh(\frac \beta 2 H_\Delta)}
%\end{align*}
%holds. We choose $\delta := \Vert \Delta\Vert_\infty$ and note that Lemma~\ref{Schatten_estimate} and \eqref{Magnetic_Sobolev} imply 
%\begin{equation}
%	\Vert \Delta\Vert_\infty \leq C \; B^{\nicefrac 14} \; \Vert \Psi \Vert_{\Hmag^1(Q_h)}.
%	\label{eq:ABDelta}
%\end{equation} 
%In particular, $\delta < 1 $ as long as $B>0$ is sufficiently small, and we have
%\begin{align}
%	\frac{H_\Delta}{\tanh(\frac \beta 2 H_\Delta)} \geq \frac{\sqrt{1 - \Vert \Delta\Vert_\infty}}{1 + \frac{\beta^2}{8} \Vert \Delta\Vert_\infty} \; \begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix} 
%	%K_{T,B} \otimes \Idbb_{\Cbb^2} 
%	\geq (1 - C\Vert \Delta\Vert_\infty) \; \begin{pmatrix}
%		K_{T,B} & 0 \\ 0 & \ov{K_{T,B}}
%	\end{pmatrix}.
%	%K_{T,B} \otimes \Idbb_{\Cbb^2}.
%	\label{LBpartB_2}
%\end{align}
%Together, \eqref{LBpartB_1} and \eqref{LBpartB_2} show
%\begin{align*}
%\frac 12 \Tr \Bigl[(\Gamma - \Gamma_\Delta)\frac{H_\Delta}{\tanh(\frac \beta 2H_\Delta)} (\Gamma - \Gamma_\Delta)\Bigr] & \\
%%
%&\hspace{-160pt} \geq (1 - C\Vert \Delta\Vert_\infty) \langle \alpha - \alpha_\Delta , K_{T,B} (\alpha - \alpha_\Delta)\rangle + (1 - C\Vert \Delta\Vert_\infty) \Tr[ (\gamma - \gamma_\Delta) K_{T,B}(\gamma - \gamma_\Delta)],
%\end{align*}
%where we can drop the last term for a lower bound because it is nonnegative if $B$ is sufficiently small. This is the lower bound for the relative entropy of $\Gamma$ with respect to $\Gamma_{\Delta}$ we were looking for. 
%
% 
%
%
%It remains to combine the first term on the right side and the interaction term on the right side of \eqref{Lower_Bound_B_2}.
To start out with, let us define the function $\eta := \alpha_* \Psi_\leq - \alpha_\Delta$. By Corollary~\ref{Structure_of_almost_minimizers_corollary} we have $\alpha - \alpha_\Delta = \sigma + \eta$ and it follows from \cite[Eqs. (6.3)-(6.7)]{DeHaSc2021} that
\begin{align}
	&\frac T2 \Hcal_0(\Gamma, \Gamma_\Delta) - \fint_{Q_h} \dd X \int_{\Rbb^3} \dd r \; V(r)|\sigma(X, r)|^2 \notag\\
	%
	%&\hspace{20pt} \geq (1 - C\Vert \Delta\Vert_\infty) \langle \sigma + \eta, K_{T,B} (\sigma + \eta)\rangle - \langle \sigma , V\sigma\rangle \notag\\
	&\hspace{20pt} \geq (1 - C\Vert \Delta\Vert_\infty) \langle \sigma, (K_{T,\Abold, W} - V) \sigma \rangle - C\Vert \Delta\Vert_\infty \Vert V\Vert_\infty \Vert \sigma \Vert_2^2 - 2 \, | \langle\eta, K_{T, \Abold, W} \sigma\rangle|. \label{Lower_Bound_2_intermediate}
\end{align}
From \eqref{KTB_Lower_bound_5} we know that the lowest eigenvalue of $K_{T, \Abold, W} - V$ is bounded from below by $-Ch^2$. Furthermore, Lemma~\ref{Schatten_estimate} and \eqref{Magnetic_Sobolev} imply 
\begin{equation}
	\Vert \Delta\Vert_\infty \leq C \; h^{\nicefrac 12} \; \Vert \Psi \Vert_{\Hmag^1(Q_h)},
	\label{eq:ABDelta}
\end{equation}
which in combination with \eqref{Second_Decomposition_sigma_estimate} implies that the first two terms on the right side of \eqref{Lower_Bound_2_intermediate} are bounded from below by 
\begin{align}
	-C \varepsilon^{-1} h^{\nicefrac 92} \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}. \label{Lower_Bound_B_3}
\end{align}
To estimate the last term on the right side of \eqref{Lower_Bound_2_intermediate}, we use \eqref{KTc_bounded_derivative} to replace $K_{T, \Abold, W}$ by $ K_{\Tc, \Abold, W}$, which yields the estimate
\begin{align*}
|\langle \eta ,(K_{T,\Abold, W} - K_{\Tc, \Abold, W} )\sigma\rangle| &\leq 2D_0 h^2 \, \Vert \sigma\Vert_2 \, \Vert \eta\Vert_2 \\
%
&\leq C \, h^6 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}.
\end{align*}
To obtain the result we also used \eqref{Second_Decomposition_sigma_estimate},  Proposition~\ref{Structure_of_alphaDelta} and \eqref{Lower_Bound_B_Psileq}. Next, we decompose $\eta = \eta_0 + \eta_\perp$ with $\eta_0(\Delta)$ and $\eta_{\perp}(\Delta)$ as in Proposition~\ref{Structure_of_alphaDelta} and write
\begin{align}
	\langle \eta, K_{\Tc, \Abold, W} \sigma \rangle &= \langle \eta_0 , K_{\Tc, \Abold, W} \sigma\rangle + \langle \eta_\perp, K_{\Tc, \Abold, W} (\sigma - \sigma_0)\rangle + \langle \eta_\perp , K_{\Tc, \Abold, W} \sigma_0\rangle. \label{Lower_Bound_B_1}
\end{align}
Using \eqref{alphaDelta_decomposition_eq2} and \eqref{Second_Decomposition_sigma_estimate}, we see that the first term on the right side of \eqref{Lower_Bound_B_1} is bounded by
\begin{align}
	|\langle \eta_0, K_{\Tc, \Abold, W} \sigma \rangle| &\leq \bigl\Vert \sqrt{K_{\Tc, \Abold, W}}\, \eta_0\bigr\Vert_{2} \bigl\Vert \sqrt{K_{\Tc, \Abold, W}}\,\sigma\bigr\Vert_{2} \notag \\
	%
	&\leq C \varepsilon^{-\nicefrac 12} h^5 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}.
	\label{eq:A30}
\end{align}
We note that $\sigma - \sigma_0 = \xi$ and use \eqref{alphaDelta_decomposition_eq3}, \eqref{Second_Decomposition_Psi_xi_estimate}, and \eqref{Lower_Bound_B_Psileq} to estimate
\begin{align}
	|\langle \eta_\perp, K_{\Tc, \Abold, W} \xi \rangle| &\leq \bigl\Vert \sqrt{K_{\Tc, \Abold, W}} \, \eta_\perp\bigr\Vert_{2} \bigl\Vert \sqrt{K_{\Tc, \Abold, W}} \, \xi \bigr\Vert_{2} \notag \\
	&\leq C\varepsilon^{\nicefrac 12} h^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}. \label{eq:A31} 
\end{align}
It remains to estimate the last term on the right side of \eqref{Lower_Bound_B_1}, which we write as 
\begin{align}
\langle \eta_\perp, K_{\Tc, \Abold, W} \sigma_0\rangle &= \langle \eta_\perp, K_{\Tc}^r  \sigma_0\rangle + \langle \eta_\perp, [K_{\Tc, \Abold, W}^r - K_{\Tc}^r ] \sigma_0\rangle + \langle \eta_\perp, (U-1)K_{\Tc, \Abold, W}^r \sigma_0\rangle \notag \\
%
&\hspace{170pt}  + \langle \eta_\perp, UK_{\Tc, \Abold, W}^r (U^* - 1) \sigma_0\rangle. \label{LBpartB_3}
\end{align}
with the unitary operator $U$ in \eqref{U_definition}. We recall that the operators $K_{\Tc, \Abold, W}^r$ and $K_{\Tc}^r$ act on the relative coordinate $r = x-y$. Since $\Delta(X,r) = - 2 V(r) \alpha_*(r) \Psi_{\leq}(X)$ and $\sigma_{0}(X,r) = \alpha_*(r) \Psi_>(X)$ we know from Proposition~\ref{Structure_of_alphaDelta}~(c) that the first term on the right side of \eqref{LBpartB_3} vanishes. A bound for the remaining terms is provided by the following lemma.

\begin{lem}
	\label{Lower_Bound_B_remainings}
	We have the following estimates on the remainder terms of \eqref{LBpartB_3}:
	\begin{enumerate}[(a)]
		\item $|\langle \eta_\perp, [K_{\Tc,\Abold, W}^r - K_{\Tc}^r]\sigma_0\rangle| \leq C h^6 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2$,
		
		\item $|\langle \eta_\perp, (U - 1) K_{\Tc,\Abold, W}^r  \sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} h^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2$,
		
		\item $|\langle \eta_\perp, UK_{\Tc, \Abold, W}^r (U^* - 1)\sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} h^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2$.
	\end{enumerate}
\end{lem} 

\begin{proof}
The proof for the case $W =0$ and $A =0$ is given in \cite[Lemma 6.2]{DeHaSc2021}. The extension for general $A$ and $W$ is straightforward.
\end{proof}

Accordingly, we have
\begin{align*}
|\langle \sigma, K_{T, \Abold, W} \eta \rangle | &\leq C\bigl( \varepsilon^{-\nicefrac 12} h^5 + \varepsilon^{\nicefrac 12} h^4 \bigr) \, \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12}.
\end{align*}
We combine this with \eqref{Lower_Bound_B_2}, \eqref{Lower_Bound_2_intermediate}, and \eqref{Lower_Bound_B_3} to see that
\begin{align}
\FBCS(\Gamma) - \FBCS(\Gamma_0) & \geq h^4\, \EGL(\Psi_\leq) \notag\\
%
&\hspace{-90pt}  - C\bigl( \varepsilon^{-\nicefrac 12} h^5 + \varepsilon^{\nicefrac 12} h^4 + \varepsilon^{-1} h^{\nicefrac 92} \bigr) \Vert \Psi\Vert_{\Hmag^1(Q_h)} \bigl( \Vert \Psi\Vert_{\Hmag^1(Q_h)} + D_1 \bigr)^{\nicefrac 12}.  \label{Lower_Bound_B_8}
\end{align}
The optimal choice $\varepsilon = h^{\nicefrac 13}$ in \eqref{Lower_Bound_B_8} yields
\begin{align}
	&\FBCS(\Gamma) - \FBCS(\Gamma_0) \notag \\
	&\hspace{2cm}\geq h^4 \, \bigl(\EGL(\Psi_\leq) - C \,  h^{\nicefrac {1}{6}} \Vert \Psi\Vert_{\Hmag^1(Q_h)} \; \bigl(  \Vert \Psi\Vert_{\Hmag^1(Q_h)}^2 + D_1\bigr)^{\nicefrac 12} \bigr). \label{Lower_Bound_B_5}
\end{align}

==> source/BCS-Theory_General_Field/6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.3_Conclusion.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Conclusion}

We use \eqref{Lower_Bound_B_5} to complete the proofs of Theorem~\ref{Main_Result} and Theorem~\ref{Main_Result_Tc}. To prove the former, let an approximate minimizer $\Gamma$ of the BCS functional be given. This implies that \eqref{Second_Decomposition_Gamma_Assumption} holds with
\begin{align}
D_1 := \EGLGSE + \rho \label{Lower_Bound_B_4}
\end{align}
and $\rho\geq 0$. Since $\Vert \Psi\Vert_{\Hmag^1(Q_h)} \leq C$ by \eqref{Second_Decomposition_Psi_xi_estimate}, \eqref{Lower_Bound_B_5} implies
\begin{align*}
h^4 \bigl(\EGLGSE + \rho\bigr) \geq \FBCS(\Gamma) - \FBCS(\Gamma_0) \geq h^4 \bigl( \EGL(\Psi_\leq) - C\, h^{\nicefrac 16}\bigr)
\end{align*}
and this proves the remaining claims of Theorem \ref{Main_Result}.

We continue with the proof of Theorem~\ref{Main_Result_Tc}. We assume that the temperature $T$ obeys
\begin{align}
\Tc ( 1 - h^2 (\Dc - D_0 h^{\nicefrac 16})) < T \leq \Tc(1 + Ch^2), \label{TcB_Upper_Fine_1}
\end{align}
where $\Dc$ is defined in \eqref{Dc_Definition} and $D_0 > 0$. For such temperatures $T$, we claim that the BCS functional is minimized by the normal state if $D_0$ is choosen appropriately large. This concludes the proof of part (b) of Theorem \ref{Main_Result_Tc}, since Corollary \ref{TcB_First_Upper_Bound} covers the remaining temperature range.

To prove this claim, we use \eqref{Lower_Bound_B_5} as a basis and assume that \eqref{Second_Decomposition_Gamma_Assumption} holds with $D_1 =0$. For a lower bound, we may drop the nonnegative quartic term in the Ginzburg--Landau functional so that
\begin{align*}
	\EGL(\Psi_\leq) &\geq h^{-4}  \langle \Psi_\leq , (\Lambda_0 \, \Pi_\Abold^2 + \Lambda_1 \, W - Dh^2 \Lambda_2) \Psi_\leq\rangle \geq  \Lambda_2 \, ( \Dc - D) \; h^{-2} \, \Vert \Psi_\leq \Vert_2^2, 
\end{align*}
with the coefficients $\Lambda_0$, $\Lambda_1$, $\Lambda_2$, and $\Lambda_3$ in \eqref{GL-coefficient_1}-\eqref{GL_coefficient_3}, as well as $D \in \mathbb{R}$ determined by $T = \Tc(1-D h^2)$. We use the bound
\begin{align*}
\Vert \Pi \Psi\Vert_2 &\leq C \, h \, \Vert \Psi\Vert_2,
\end{align*}
whose proof is given by \cite[Eq. (5.26)]{DeHaSc2021} and combine this with \eqref{Psi>_bound} to see that
\begin{align*}
\Vert \Psi_\leq \Vert_2 \geq \Vert \Psi\Vert_2 - \Vert \Psi_>\Vert_2 \geq c \; h \; \Vert \Psi \Vert_{\Hmag^1(Q_h)} \, ( 1 - C \, h^{\nicefrac{5}{6}} ).
\label{eq:A32}
\end{align*}
We combine these observations with the lower bound \eqref{Lower_Bound_B_5} and obtain
\begin{equation}
0\geq \FBCS(\Gamma) - \FBCS(\Gamma_0) \geq c \; h^4 \; \Vert \Psi \Vert_{\Hmag^1(Q_h)}^2 \bigl( (\Dc - D)  - Ch^{\nicefrac {1}{6}}\bigr), \label{eq:A33}
\end{equation}
Since the lower bound in \eqref{TcB_Upper_Fine_1} is equivalent to
\begin{align}
\Dc - D > D_0 \, h^{\nicefrac 1{6}}, \label{TcB_Upper_Fine_2}
\end{align}
the choice $D_0 > C$ with $C>0$ in \eqref{eq:A33}, together with \eqref{TcB_Upper_Fine_2}, yields a lower bound for the right side of \eqref{eq:A33}. This proves that $\Psi =0$. By \eqref{Second_Decomposition_alpha_equation} and \eqref{Second_Decomposition_Psi_xi_estimate}, this implies that $\alpha = 0$, i.e., $\Gamma$ is a diagonal state. Therefore, $\Gamma_0$ is the unique minimizer of $\FBCS$ in the temperature range \eqref{TcB_Upper_Fine_1} provided $D_0$ is chosen as above. This proves Theorem \ref{Main_Result_Tc}.























==> source/BCS-Theory_General_Field/6_Lower_Bound_Asymptotics_and_Upper_Bound_Tc/6.4_Integral_representation_and_bound_rest_terms.tex <==
%auto-ignore  % for ArXiv to process correctly

\subsection{Proof of Lemma~\ref{Lower_Bound_B_remainings}}
\label{sec:A1}

In this section we prove Lemma~\ref{Lower_Bound_B_remainings}.
%\begin{lem}
%\label{Lower_Bound_B_remainings}
%We have the following estimates on the remainder terms of \eqref{LBpartB_3}:
%\begin{enumerate}[(a)]
%\item $|\langle \eta_\perp, [K_{\Tc,B}^r - K_{\Tc}^r]\sigma_0\rangle| \leq C B^3 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$,
%
%\item $|\langle \eta_\perp, (U - 1) K_{\Tc,B}^r  \sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$,
%
%\item $|\langle \eta_\perp, UK_{\Tc,B}^r (U^* - 1)\sigma_0\rangle| \leq C \varepsilon^{\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$.
%\end{enumerate}
%\end{lem}
Our proof of part (a) uses a Cauchy integral representation for the operator $K_{\Tc,B}- (\pi^2 -\mu)$, which is provided in Lemma~\ref{KT_integral_rep} below. Let us start by defining the contour for the Cauchy integral.

\begin{defn}[Speaker path]
\label{speaker path}
Let $R>0$, assume that $\mu \leq 1$ and define the following complex paths 
\begin{align*}
\begin{split}
u_1(t) &:= \frac{\pi\i}{2\betac} + (1 + \i)t\\
%
u_2(t) &:= \frac{\pi\i}{2\betac} - (\mu + 1)t\\
%
u_3(t) &:= -\frac{\pi\i}{2\betac}t - (\mu + 1)\\
%
u_4(t) &:= -\frac{\pi\i}{2\betac} - (\mu + 1)(1-t) \\
%
u_5(t) &:= -\frac{\pi\i }{2\betac} + (1 - \i)t
\end{split}
&
\begin{split}
\phantom{ \frac \i\betac }t&\in [0,R], \\
%
\phantom{ \frac \i\betac }t &\in [0,1], \\
%
\phantom{ \frac \i\betac }t&\in [-1,1],\\
%
\phantom{ \frac \i\betac }t &\in [0,1],\\
%
\phantom{ \frac \i \betac }t&\in [0,R].
\end{split}
%
& \begin{split} 
\text{\includegraphics[width=6cm]{../BCS-Theory_General_Field/Speaker_path.pdf}}
\end{split} 
\end{align*}
The speaker path is defined as the union of paths $u_i$, $i=1, \ldots, 5$, with $u_1$ taken in reverse direction, i.e.,
\begin{align*}
\speaker_R := \mathop{\dot -}u_1 \mathop{\dot +} u_2 \mathop{\dot +} u_3 \mathop{\dot +} u_4 \mathop{\dot +} u_5.
\end{align*}
If $\mu > 1$ we choose the same path as in the case $\mu = 1$.
\end{defn} 
This path has the property that certain norms of the resolvent kernel of $\pi^2$ are uniformly bounded for $z \in \speaker_R$ and $R > 0$. More precisely, Lemma~\ref{GAz-GtildeAz_decay} implies
\begin{align}
\sup_{0\leq B\leq B_0} \sup_{R>0} \sup_{w\in \speaker_R} \bigl[ \left\Vert \, |\cdot |^a g_B^w\right\Vert_1 + \left \Vert \, |\cdot|^a \nabla g_B^w\right\Vert_1 \bigr] < \infty. \label{g0_decay_along_speaker}
\end{align}
We could also choose a path parallel to the real axis in Lemma~\ref{KT_integral_rep} below. In this case the above norms would depend on $R$. Although our analysis also works in this case, we decided to use the path $\speaker_R$ because of the more elegant bound in \eqref{g0_decay_along_speaker}. 
%This is obtained by combining the strategy of proof of Lemmas \ref{g0_decay} and \ref{gB-g_decay} with the estimate $(\Re \sqrt{-z})^2 \geq |\Re z|$, which holds as long as $\Re z \leq 0$. For $B_0 > 0$ sufficiently small and any $a\geq 0$, it is thus easy to show that for all $0 \leq B \leq B_0$, we have
With the above definition at hand, we are prepared to state the following lemma.

%We remark that it is not necessary for the following lemma to follow the paths $u_1$ and $u_5$. On the level of operators alone, as it is in Lemma \ref{KT_integral_rep}, we could indeed follow paths parallel to the real line. However, since we want to argue with kernels, we want to use uniform bounds on the resolvent kernel along the used path, see Lemma \ref{Gz_decay_along_speaker}. For the proof of this result, we utilize Lemma \ref{gz_decay}, whose bounds deteriorate along constant distance to the real line. This is the reason why we need to increase this distance linearly.

%For a well-defined contour integral, it would be sufficient to define the path parallel to the real axis, since the resolvent of the Laplacian is uniformly bounded as an operator and the function we are integrating is decaying sufficiently fast to make the integral convergent, see Lemma \ref{KT_integral_rep}. This is not true for the resolvent kernel. 
%However, with the contour defined above, we do have a uniform bound of the resolvent kernel along the contour. 

%We could give up uniformity (in $w$) in this bound and profit from an easier path, which could then be laid parallel to the real axis. The convergence of the contour integral in the following lemma would still be fine, since the underlying function is decaying exponentially fast as the real part of $w$ grows along the positive real line. However, with the method used to prove Lemma \ref{g0_decay}, we found it convenient to work with the speaker shaped path.

%\begin{lem}
%\label{g0_decay_along_speaker}
%For $a\geq 0$, we have
%
%%Here, $C_{\mu, T} = 2\tan(\frac 12 \arctan(\frac{\pi T}{2\mu_+}))^{-1}$. Likewise, for $a> -1$, we have
%%\begin{align*}
%%\sup_{w\in \speaker_{T,\mu}} \left\Vert \, |\cdot |^a \nabla g_0^w\right\Vert_{L^1(\Rbb^3)} < \infty.
%%\end{align*}
%\end{lem}

%\begin{proof}
%We apply Lemma \ref{gz_decay} by defining $\theta \in (0, \frac \pi 4]$ as
%\begin{align*}
%\theta &:= \frac 12 \arctan\bigl( \frac{\pi \Tc}{2\mu_+}\bigr).
%\end{align*}
%A similar proof to that of Lemma \ref{g0_decay} shows that the traces of $u_2, u_3$ and $u_4$ from Definition \ref{speaker path} belong to $S_\theta$. Concerning the path $u_1$, we remark that it has an angle of $\frac \pi 4$ from the starting point $t=0$, while the sector has an angle of at most $\frac \pi 4$. Hence, they do not intersect. Likewise for $u_5$. Thus, the speaker path lies in $S_\theta$.
%
%With the exception of $u_3$, we have $|\Im w| \geq \frac{\pi}{2\beta_c}$. By Lemma \ref{gz_decay}, for any $w\in \speaker_R \setminus \{u_3\}$, we thus have
%\begin{align*}
%\Vert \, |\cdot|^a g_0^w\Vert_1 \leq \Gamma(a+2) \;  C_\theta^{1+\frac a2} \;  \bigl(\frac{\pi}{2\beta_c}\bigr)^{-1-\frac a2}.
%\end{align*}
%
%For the path $u_3$, we provide the following addendum to the proof of Lemma \ref{gz_decay}. Since , we infer $(\Re \sqrt{-(w+\mu)})^2 \geq |\Re (w+\mu)|$ as long as $\Re w < -\mu$. Along $u_3$, we have $\Re w+\mu = -1$. Applying this to \eqref{Resolvent_kernel_integration} for $w\in u_3$, we get $\Vert \, |\cdot|^a g_0^w\Vert_1 \leq \Gamma(a+2)$. This proves claimed estimate on the first term of \eqref{g0_decay_along_speaker_2}.
%
%For the second term of \eqref{g0_decay_along_speaker_2}, employ  $|\sqrt{-(w+\mu)}| \leq |\Re w+\mu|^{\nicefrac 12} + |\Im w|^{\nicefrac 12}$. Combining this with \eqref{g0_decay_2} and \eqref{Resolvent_kernel_integration}, we get
%\begin{align}
%\Vert \, |\cdot|^a \nabla g_0^w\Vert_1 \leq \frac{|\Re w+\mu|^{\nicefrac 12} + |\Im w|^{\nicefrac 12}}{|\Re \sqrt{-(w+\mu)}|^{2+a}} \Gamma(a+2) + \frac{\Gamma(a+1)}{|\Re \sqrt{-(w+\mu)}|^{1+a}}. \label{g0_decay_along_speaker_3}
%\end{align}
%Along $u_3$, we apply the estimate $|\Re \sqrt{-(w +\mu)}| \geq C_\theta^{-\nicefrac 12} |\Im w|^{\nicefrac 12}$ as in \eqref{g0_decay_3} once to accomodate for the factor $|\Im w|$. For the remaining powers, we apply the lower bound $|\Re \sqrt{-(w+\mu)}|^2 \geq |\Re w+\mu|$ again, since $\Re w+\mu < 0$ here. This implies
%\begin{align*}
%\Vert \, |\cdot|^a \nabla g_0^w\Vert_1 \leq \; \bigl( \Gamma(a+2) + \Gamma(a+1) + C_\theta^{\nicefrac 12}\bigr) \; |\Re w + \mu|^{-\frac 12 - \frac a2}.
%\end{align*}
%Since $\Re w + \mu = -1$ along $u_3$, we conclude the uniform bound. 
%
%On the remainder of the speaker path, we have $|\Im w|\geq \frac{\pi}{2\beta_c}$. Therefore, using \eqref{g0_decay_3} and \eqref{g0_decay_along_speaker_3},
%\begin{align}
%\Vert \, |\cdot|^a \nabla g_0^w\Vert_1 \leq \Bigl[ \Gamma(a+2) C_\theta^{1 + \frac a2} \frac{|\Re w+\mu|^{\nicefrac 12} + |\Im w|^{\nicefrac 12}}{|\Im w|^{\nicefrac 12}} + \Gamma(a+1) C_\theta^{\frac 12+\frac a2}\Bigr] |\Im w|^{-\frac 12 - \frac a2}. \label{g0_decay_along_speaker_1}
%\end{align}
%Inserting the explicit form of $w+\mu$ in the segments of $\speaker_R$ into \eqref{g0_decay_along_speaker_1}, we see that the term in square brackets is uniformly bounded.
%
%
%
%
%
%\begin{align}
%\Vert \, |\cdot|^a \nabla g_0^z\Vert_1 \leq \Bigl[ \Gamma(a+2) C_{\mu, T}^{1 + \frac a2} \frac{|\Re z+\mu|^{\nicefrac 12} + |\Im z|^{\nicefrac 12}}{|\Im z|^{\nicefrac 12}} + \Gamma(a+1) C_{\mu, T}^{\frac 12+\frac a2}\Bigr] |\Im z|^{-\frac 12 - \frac a2}
%%
%%
%%
%%
%%\frac{|\Re z+\mu|^{\nicefrac 12} + |\Im z|^{\nicefrac 12}}{|\Re \sqrt{-(z+\mu)}|^{2+a}} \Gamma(a+2) + \frac{\Gamma(a+1)}{|\Re \sqrt{-(z+\mu)}|^{1+a}}. 
%\label{g0_decay_along_speaker_1}
%\end{align}
%We applied the estimate $|\Re \sqrt{-(z +\mu)}| \geq C_{\mu, T}^{-\nicefrac 12} |\Im z|^{\nicefrac 12}$ as in \eqref{g0_decay_3}. 
%%For the remaining powers, we apply $|\Re \sqrt{-(z+\mu)}|^2 \geq |\Re z+\mu|$. This implies
%%\begin{align*}
%%\Vert \, |\cdot|^a g_0^z\Vert_1 \leq \Gamma(a+2) \; (2+ C_{\mu, T}^{\nicefrac 12}) \; |\Re z + \mu|^{-\frac 12 - \frac a2}.
%%\end{align*}
%%Since $\Re z + \mu = -1$ along $u_3$, we conclude the uniform bound. 
%Inserting the explicit form of $z+\mu$ in the segments of $\speaker_{T, \mu}$ in to \eqref{g0_decay_along_speaker_1}, we see that the term in square brackets is uniformly bounded.
%\end{proof}

%\notiz{We could give up uniformity of the bound \eqref{g0_decay_along_speaker} for simplifying the speaker path to a parallel-to-the-real-axis path. It does not disturb the convergence of the integral but makes the derivation of \eqref{g0_decay_along_speaker} more tedious, since we need to analyse the rate of deterioration of $\Vert g_0^w\Vert_1$. It will be linear in $\Re z$ for $\Re z \gg 1$. Shall we do that? Does not simplify much more than that, I think.}

\begin{lem}
\label{KT_integral_rep}
Let $H\colon \Dcal(H)\ra \Hcal$ be a self-adjoint operator on a separable Hilbert space~$\Hcal$ with $H\geq -\mu$. Then, we have
\begin{align}
\frac{H}{\tanh(\frac{\betac}{2} H)} = H + \lim_{R\to\infty} \int_{\speaker_R} \frac{\dd z}{2\pi\i} \Bigl( \frac{z}{\tanh(\frac{\betac}{2} z)} - z \Bigr) \frac{1}{z - H}, \label{KT_integral_rep_eq}
\end{align}
with the speaker path $\speaker_R$ in Definition~\ref{speaker path}. The above integral including the limit is understood as an improper Riemann integral with respect to the uniform operator topology.  
\end{lem}

\begin{proof}
We have that the function $f(z) = \frac{z}{\tanh(\frac{\betac }{2}z)} - z = \frac{2z}{\e^{\betac z} - 1}$ is analytic in the open domain $\Cbb \setminus 2\pi T \i \Zbb_{\neq 0}$. The construction of the Riemann integral over the path $\speaker_R$ with respect to the uniform operator topology is standard. The fact that the limit $R \to \infty$ exists in the same topology follows from the exponential decay of the function $f(z)$ along the speaker path. To check the equality in \eqref{KT_integral_rep_eq}, we evaluate both sides in the inner product with two vectors in $\ran \Idbb_{(-\infty, K]}(H)$ for $K > 0$ and use the functional calculus, the Cauchy integral formula and the fact that $\bigcup_{K>0} \ran \Idbb_{(-\infty, K]}(H)$ is a dense subset of $\Hcal$. This proves the claim.
\end{proof}


 

%and on the interval $[-\mu, \infty)$ we have $\Vert f\Vert_\infty = \frac{2\mu}{1 - \e^{-\betac \mu}}$. Therefore, $f(H)$ is a bounded operator.

%A straightforward computation shows that the limit on the right side of \eqref{KT_integral_rep_eq} exists in operator norm and defines a bounded operator that we denote by $g(H)$.
%We prove that the limit 
%\begin{align*}
%g(H) := \lim_{R\to\infty} \int_{\speaker_R} \frac{\dd z}{2\pi\i} \; f(z) \, \frac{1}{z - H}
%\end{align*}
%exists and defines a bounded operator on $\Hcal$. To do this, we investigate the tails of the paths $u_1$ and $u_5$. For example, we have to investigate the operator norm of
%\begin{align*}
%\int_R^\infty \frac{\dd t}{2\pi\i} \frac{2u_1(t)}{\e^{\betac u_1(t)} - 1} \frac{1}{u_1(t) - H} \;  u_1'(t).
%\end{align*}
%Note the following simple estimates for $t$ large enough
%\begin{align*}
%|u_1(t)| &\leq \frac{\pi}{2\betac} + \sqrt{2} t \leq Ct, & |u_1'(t)| &= \sqrt{2}, & \Re u_1(t) &= t,
%\end{align*}
%as well as
%\begin{align*}
%\Vert (u_1(t) - H)^{-1}\Vert_\infty &\leq \frac{1}{\Im u_1(t)} = \frac{1}{\frac{\pi}{2\betac} + t} \leq \frac 1t.
%\end{align*}
%This implies that
%\begin{align*}
%\Bigl\Vert \int_R^\infty \frac{\dd t}{2\pi\i} \frac{2u_1(t)}{\e^{\betac u_1(t)} - 1} \frac{1}{u_1(t) - H} \;  u_1'(t)\Bigr\Vert_\infty &\leq C \int_R^\infty \frac{1}{\e^{\betac t} - 1} \leq C \e^{-\betac R}.
%\end{align*}
%The contribution of $u_5$ is estimated in a similar fashion. This proves operator norm convergence of the limit and that $g(H)$ is bounded.

%Let $K \geq 0$ and choose $\eta\in \ran(\Idbb_{(-\infty, K-1]}(H))$. Take $R\geq K$ and close the speaker path by the contour $u_R(t) := R + (R+ \frac{\pi}{2\betac}) \i t$ where $t\in [-1,1]$. The Cauchy integral formula shows 
%\begin{align*}
%\langle \varphi, f(H) \eta\rangle = \int_{\speaker_R \dot + u_R} \frac{\dd z}{2\pi\i} \; f(z) \, \langle \varphi, (z - H)^{-1} \eta\rangle.
%\end{align*}
%for $\varphi\in \Hcal$. It remains to show that the integral over $u_R$ vanishes as $R \to \infty$. We use
%\begin{align*}
%\Bigl|\int_{u_R} \frac{\dd z}{2\pi\i} \; f(z) \langle \varphi, (z - H)^{-1}\eta\rangle\Bigr| &\leq \int_{-1}^1 \frac{\dt}{\pi} \frac{|u_R(t)|}{|\e^{\betac u_R(t)}| - 1} \;  |\langle \varphi, (u_R(t) - H)^{-1} \eta\rangle|\;  |u_R'(t)|.
%\end{align*}
%Since $\Re u_R(t) = R$, we have
%$|u_R(t) - (K-1)| \geq 1$ to see that $\sup_{t\in [-1,1]}\Vert (u_R(t) - H)^{-1}\Idbb_{(-\infty, K-1]}(H)\Vert_\infty \leq 1$. The claim follows from the decay of $f$ on the path $u_R(t)$. 
% Hence, we obtain
%\begin{align*}
%\sup_{\Vert \varphi\Vert = 1} \Bigl|\int_{u_R} \frac{\dd z}{2\pi\i} \; f_{\Tc}(z) \langle \varphi, (z - H)^{-1}\eta\rangle\Bigr| &\leq C \;  \frac{R^2}{\e^{\betac R} - 1} \;  \Vert\eta\Vert \xra{R\to\infty} 0.
%\end{align*}
%We conclude that the second term on the right side of \eqref{KT_integral_rep_eq} equals $f(H)$. This proves the claim. %Since both operators are bounded, this extends to all $\eta\in \Hcal$ by density. %Since $H$ and $\frac{H}{\tanh(\frac{\betac}{2} H)}$ have the same domain $\Dcal(H)$, the claim holds for all $\eta\in \Dcal(H)$.


Henceforth, we use the symbol $\int_{\speaker}$ to denote the integral on the right side of \eqref{KT_integral_rep_eq} including the limit and we denote $\speaker = \bigcup_{R > 0} \speaker_R$.

\begin{proof}[Proof of Lemma \ref{Lower_Bound_B_remainings}]
%Throughout we use the estimates of Theorems \ref{Structure_of_alphaDelta} and \ref{Structure_of_almost_minimizers}, as well as $B \leq \varepsilon \leq 1$.
We apply Cauchy-Schwarz to estimate
\begin{align}
|\langle \eta_\perp, (K_{\Tc,B}^r - K_{\Tc}^r)\sigma_0\rangle| \leq \Vert \eta_\perp\Vert_2 \, \Vert (K_{\Tc,B}^r- K_{\Tc}^r)\sigma_0\Vert_2
\label{eq:A34}
\end{align}
and claim that 
\begin{align}
\Vert [K_{{\Tc},B}^r - K_{\Tc}^r]\sigma_0\Vert_2 \leq C \varepsilon^{-\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)} \label{Lower_Bound_B_remainings_3}
\end{align}
holds. To see this, we apply Lemma~\ref{KT_integral_rep} and write
\begin{align}
K_{{\Tc},B}^r - K_{\Tc}^r = \pi_r^2 - p_r^2 + \int_\speaker \frac{\dd w}{2\pi\i} \; f(w) \;  \frac{1}{w + \mu - \pi_r^2} [\pi_r^2 - p_r^2] \frac{1}{w + \mu - p_r^2}, \label{Lower-bound-final_2}
\end{align}
where $\pi_r^2 - p_r^2 = \i \, \Bbold\wedge r\;  p_r + \frac 14 |\Bbold\wedge r|^2$. Using \eqref{Psi>_bound} and \eqref{Decay_of_alphastar}, we estimate the first term on the right side of \eqref{Lower-bound-final_2} by
\begin{align}
\Vert [\pi_r^2 - p_r^2]\sigma_0\Vert_2 &\leq B \, \Vert \, |\cdot|\nabla \alpha_*\Vert_2 \Vert \Psi_>\Vert_2 + B^2 \Vert \,|\cdot|^2\alpha_*\Vert_2 \Vert \Psi_>\Vert_2 \notag\\
%
&\leq C\varepsilon^{-\nicefrac 12} B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}. \label{Lower_Bound_B_remainings_1}
\end{align}
To estimate the second term in \eqref{Lower-bound-final_2}, we use Hölder's inequality in \eqref{Schatten-Hoelder} and find
\begin{align*}
\Bigl\Vert \int_\speaker \frac{\dd w}{2\pi\i} \, f(w)\;  \frac{1}{w + \mu - \pi_r^2} [\pi_r^2 - p_r^2]\frac{1}{w+\mu - p_r^2}\sigma_0\Bigr\Vert_2 &\\
%
&\hspace{-180pt}\leq \int_\speaker \frac{\dd |w|}{2\pi}\,  |f(w)| \, \Bigl\Vert \frac{1}{w + \mu- \pi_r^2} \Bigr\Vert_\infty \Bigl\Vert [\pi_r^2 - p_r^2]\frac{1}{w + \mu - p_r^2}\sigma_0\Bigr\Vert_2,
\end{align*}
where $\dd |w| = \dd t \; |w'(t)|$. Eq.~\eqref{g0_decay_along_speaker} implies that the operator norm of the magnetic resolvent is uniformly bounded for $w \in \speaker$. Since the function $f$ is exponentially decaying along the speaker path it suffices to prove a bound on the last factor that is uniform for $w \in \speaker$. We have
\begin{align*}
[\pi_r^2 - p_r^2] \frac{1}{w + \mu - p_r^2} \sigma_0(X,r) &= \int_{\Rbb^3} \dd s \; [\pi_r^2 - p_r^2] g_0^w(r - s) \alpha_*(s) \Psi_>(X),
\end{align*}
which implies
\begin{align}
\Bigl\Vert [\pi_r^2 - p_r^2] \frac{1}{w + \mu - p_r^2}\sigma_0\Bigr\Vert_2^2 &
%\leq\\
%%
%&\hspace{-100pt}\leq \int_{\Rbb^3} \dd r \int_{\Rbb^3} \dd s \int_{\Rbb^3} \dd s' \; |[\pi_r^2 - p_r^2]G^w(r - s) \alpha_*(s)|\cdot |[\pi_r^2 - p_r^2]G^w(r - s') \alpha_*(s')|\\
%%
%& \times \fint_{Q_B} \dd X \; \bigl| \cos\bigl(\frac{s}{2}\Pi_X\bigr) \Psi_>(X)\bigr| \;  \bigl|\cos\bigl( \frac{s'}{2}\Pi_X\bigr) \Psi_>(X)\bigr|\\
%
\leq \Vert \Psi_>\Vert_2^2 \int_{\Rbb^3} \dd r \, \Bigl| \int_{\Rbb^3} \dd s \; |[\pi_r^2 - p_r^2] g_0^w(r - s) \alpha_*(s)|\Bigr|^2. \label{Lower_Bound_B_remainings_2}
\end{align}
Moreover,
%note that
%\begin{align*}
%|[\pi_r^2 - p_r^2] G^w(r - s) \alpha_*(s)| &\leq B |r - s||G^w(r - s)| |\alpha_*(s)| + B |G^w(r - s)| \;  |s||\alpha_*(s)| \\
%%
%&\hspace{0pt} + B^2 |r - s|^2 |G^w(r - s)| |\alpha_*(s)| + B^2 |G^w(r - s)| |s|^2 |\alpha_*(s)|.
%\end{align*}
%This implies
\begin{align*}
\int_{\Rbb^3} \dd r \; \Bigl| \int_{\Rbb^3} \dd s \; |[\pi_r^2 - p_r^2] g_0^w(r - s) \alpha_*(s)|\Bigr|^2 & \\
%
&\hspace{-195pt} \leq CB^2 \bigl( \Vert \, |\cdot| \nabla g_0^w\Vert_1^2 \; \Vert \alpha_*\Vert_2^2 + \Vert \nabla g_0^w\Vert_1^2 \; \Vert \, |\cdot|\alpha_*\Vert_2^2 + \Vert \,  |\cdot|^2 g_0^w\Vert_1^2 \;  \Vert\alpha_*\Vert_2^2 + \Vert g_0^w\Vert_1^2 \;  \Vert \, |\cdot|^2\alpha_*\Vert_2^2\bigr).
\end{align*}
The right side is uniformly bounded for $w \in \speaker$ by \eqref{g0_decay_along_speaker} and \eqref{Decay_of_alphastar}. In combination with \eqref{Psi>_bound} and \eqref{Lower_Bound_B_remainings_2}, this implies
\begin{align*}
\Bigl\Vert [\pi_r^2 -p_r^2]\frac{1}{w + \mu - p_r^2} \sigma_0\Bigr\Vert_2^2 & \leq CB^2 \;  \Vert\Psi_>\Vert_2^2\leq C \varepsilon^{-1} B^4 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2.
\end{align*}
Using this and \eqref{Lower_Bound_B_remainings_1}, we read off \eqref{Lower_Bound_B_remainings_3}. Finally, we apply Proposition~\ref{Structure_of_alphaDelta} to estimate $\Vert \eta_\perp\Vert_2$ in \eqref{eq:A34}, which proves part (a).

%\item  $K_{T,B}^r - K_{\Tc,B}^r$ is a bounded operator of order $B$, as argued in \eqref{KTc_bounded_derivative}. Hence
%\begin{align*}
%|\langle \eta_\perp, [K_{T,B}^r - K_{\Tc,B}^r]\sigma_0\rangle| &\leq CB \;  \Vert \eta_\perp\Vert_2 \;  \Vert \sigma_0\Vert_2 \leq CB \varepsilon^{\nicefrac 12} B^{\nicefrac 14} \;  \varepsilon^{-\nicefrac 12} B^{\nicefrac 14} \leq CB^{\nicefrac 32}.
%\end{align*}

To prove part (b), we start by noting that
\begin{align*}
|\langle \eta_\perp, (U-1) K_{\Tc,B}^r\sigma_0 \rangle| &\leq \Vert \,  |r| \eta_\perp\Vert_2 \;  \Vert\, |r|^{-1} (U - 1) K_{\Tc,B}^r \, \sigma_0 \Vert_2. %\label{Lower_Bound_B_remainings_5}
\end{align*}
A bound for the left factor on the right side is provided by Proposition~\ref{Structure_of_alphaDelta}. To estimate the right factor, we use \eqref{Psi>_bound}, \eqref{Decay_of_alphastar} and the operator inequality in \eqref{ZPiX_inequality}, which implies $|U- 1|^2 \leq 3 r^2 \Pi_X^2$, and find
\begin{align*}
\Vert\, |r|^{-1} (U - 1) K_{\Tc,B}^r \, \sigma_0 \Vert_2 &\leq C \Vert K_{\Tc,B}^r \alpha_*\Vert_2 \; \Vert \Pi\Psi_>\Vert_2 \leq CB \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}.
\end{align*}
This proves part (b).
%Using $K_{\Tc,B}^r \leq C(1+\pi_r^2)$, we obtain
%\begin{align*}
%\bigl\Vert \sqrt{K_{\Tc,B}^r} \, \sigma_0\bigr\Vert^2 &= \langle \sigma_0, K_{\Tc,B}\sigma_0\rangle \leq C ( \Vert \sigma_0\Vert_2^2 + \Vert \pi_r\sigma_0\Vert_2^2) \leq C \varepsilon^{-1} B^ {\nicefrac 12}.
%\end{align*}
%\notiz{Indizes der Normen}Turning to the left factor in \eqref{Lower_Bound_B_remainings_5}, we have 
%\begin{align}
%\Vert \sqrt{K_{\Tc,B}} (U-1) \eta_\perp\Vert^2 &\leq \Vert (U-1) \eta_\perp\Vert^2 + \Vert \pi_r (U-1) \eta_\perp\Vert^2. \label{Lower_Bound_B_remainings_4}
%\end{align}
%Using Theorem \ref{Structure_of_alphaDelta} and \eqref{Psi_Higher_Derivatives} for $k =3$, the left term is bounded by
%\begin{align*}
%\Vert (U-1) \eta_\perp\Vert^2 &\leq \Vert \, |r\Pi_X| \eta_\perp\Vert^2 \leq C \, B^{\nicefrac 52} \;  (\varepsilon B^{-1})^2 \leq C \varepsilon^2 B^{\nicefrac 12}.
%\end{align*}
%By the intertwining relations in Lemma \ref{CommutationI}, we have
%\begin{align*}
%\pi_r (U-1) = (U-1) \tilde \pi_r - \frac 12 U \Pi_X - \frac 14 \Bbold \wedge r. %\label{Lower-bound-final_1}.
%\end{align*}
%Using this, the right term of \eqref{Lower_Bound_B_remainings_4} is bounded by
%\begin{align*}
%\Vert \pi_r (U-1) \eta_\perp \Vert^2 &\leq C \bigl( \Vert |r\Pi_X|\tilde \pi_r\eta_\perp\Vert^2 + \Vert \Pi_X\eta\Vert^2 + B^2 \Vert |r|\eta_\perp\Vert^2\bigr) \leq C \varepsilon^2 B^{\nicefrac 12}.
%\end{align*}

For part (c), we estimate
\begin{align}
|\langle \eta_\perp, UK_{\Tc,B}^r (U^* - 1) \sigma_0\rangle|  &\leq \bigl\Vert \sqrt{K_{\Tc,B}^r} \, U^* \eta_\perp \bigr\Vert_2 \;  \bigl\Vert \sqrt{K_{\Tc,B}^r}\, (U^* - 1)\sigma_0\bigr\Vert_2
\label{eq:A35}
\end{align}
and note that $K_{\Tc,B}^r \leq C(1+ \pi_r^2)$ implies
\begin{align}
\bigl\Vert \sqrt{K_{\Tc,B}^r} (U^* - 1)\sigma_0\bigr\Vert_2^2 &= \langle \sigma_0, (U - 1) K_{\Tc,B}^r (U^* - 1)\sigma_0\rangle \notag\\
%
&\leq C \Vert (U^* - 1)\sigma_0\Vert_2^2 + C\Vert \pi_r (U^* - 1)\sigma_0\Vert_2^2.\label{Lower-bound-final_3}
\end{align}
Using the bound for $|U-1|^2$ in part (b), \eqref{Psi>_bound} and \eqref{Decay_of_alphastar}, we see that the first term is bounded by $C\Vert |r|\alpha_* \Pi_X\Psi_>\Vert^2 \leq CB^2$. Lemma~\ref{CommutationI} allows us to write
\begin{align*}
\pi_r (U^* - 1) &= (U^* - 1) \tilde \pi_r + \frac 12 U^*\Pi_X - \frac 14 \Bbold \wedge r.
\end{align*}
Accordingly, we have
\begin{align*}
\Vert \pi_r (U^* - 1)\sigma_0\Vert_2^2 &\\
%
&\hspace{-50pt}\leq C\bigl( \Vert \, |r| p_r\alpha_*\Pi_X\Psi_>\Vert_2^2 + B \, \Vert \, |r|^2\alpha_* \Pi_X \Psi_> \Vert_2^2 + \Vert \alpha_*\Pi_X\Psi_>\Vert_2^2 + B \Vert \, |r|\alpha_* \Psi_>\Vert_2^2\bigr)\\
%
&\hspace{-50pt}\leq C \bigl( B^2 + \varepsilon^{-1} B^3 \bigr) \leq CB^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2.
\end{align*}
We conclude that the right side of \eqref{Lower-bound-final_3} is bounded by $CB^2 \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2$. 

With $K_T(p) \leq C (1+p^2)$ we see that the first factor on the right side of \eqref{eq:A35} is bounded by
\begin{align*}
\bigl\Vert \sqrt{K_{\Tc,B}^r} \, U^* \eta_\perp\bigr\Vert_2^2 &= \langle \eta_\perp , U K_{\Tc,B}^r U^* \eta_\perp\rangle \leq C \Vert \eta_\perp\Vert_2^2 + C\Vert \pi_rU^*\eta_\perp\Vert_2^2.
\end{align*}
From Lemma~\ref{CommutationI} we know that $\pi_r U^* = U^* [\tilde\pi_r + \frac 12 \Pi_X]$, and hence
\begin{align*}
\bigl\Vert \sqrt{K_{\Tc,B}^r} \, U^* \eta_\perp\bigr\Vert_2^2 &\leq C \bigl( \Vert \eta_\perp\Vert_2^2 + \Vert \tilde \pi_r\eta_\perp\Vert_2^2 + \Vert \Pi_X\eta_\perp\Vert_2^2\bigr) \leq C \varepsilon B^2 \, \Vert \Psi\Vert_{\Hmag^1(Q_B)}^2. 
\end{align*}
This proves part (c) and ends the proof.
\end{proof}

==> source/Exponential_estimates_for_the_adiabatic_theorem/Notes/18_Things_for_later.tex <==
%auto-ignore  % for ArXiv to process correctly

\newpage
\section[Things for later]{Things we would need later}

\begin{warn}
The notation is not streamlined to the previous section, since it refers to a version of the notes where $s = \nicefrac 12$ was fixed! No proof-reading was done in this section.
\end{warn}

\subsection{Estimating our decay function $\chi_b$}

\begin{lem}
\label{f-l-eps-1}
Let $\ell \in \frac 12\Nbb_0$ and $\varepsilon >0$. For $t\geq 0$, define
\begin{align*}
f_{\ell,\varepsilon}(t) := \max\{ 1, t\}^\ell \cdot  \e^{-\varepsilon \sqrt{t}}.
\end{align*}
Then:
\begin{align*}
\Vert f_{\ell,\varepsilon}\Vert_{L^\infty([0,\infty))} &\leq \begin{dcases} 1 & \frac{2\ell}{\varepsilon} \leq  \e, \\ \bigl( \frac{2\ell}{\e \cdot\varepsilon}\bigr)^{2\ell} & \frac{2\ell}{\varepsilon} \geq \e. \end{dcases}
\end{align*}
\end{lem}

\begin{proof}
It is clear that $g_{\ell,\varepsilon}$ defined by the $t$-case of the max has a unique maximum. To locate it, solve the critical equation
\begin{align*}
t^{\ell-1} \e^{-\varepsilon\sqrt{t}}\bigl[\ell - \frac{\varepsilon}{2} \cdot \sqrt{t}\bigr] =0.
\end{align*}
to obtain that the maximum sits at $\sqrt{t_0 } = \frac{2\ell}{\varepsilon}$. Inserting this gives the maximal value
\begin{align*}
g_{\ell,\varepsilon}(t_0) = \bigl(\frac{2\ell}{\e\cdot \varepsilon}\bigr)^{2\ell}.
\end{align*}
This is smaller than or equal to $1$ if and only if $\frac{2\ell}{\varepsilon} \leq \e$. In this case, $f_{\ell,\varepsilon}(t)\leq 1$. In the other case, $\Vert f_{\ell,\varepsilon}\Vert_\infty = g_{\ell,\varepsilon}(t_0)$.
\end{proof}




\begin{asmp}[Abel partial sum formula]
\label{Abel-partial-sum}
Let $(a_n)_{n\geq 0}$ be a sequence of real numbers and for any $t\in \Rbb$ define
\begin{align*}
A(t) := \sum_{n=0}^{\lfloor t\rfloor} a_n.
\end{align*}
Let $x < y$ be real and $\phi\in C^1[x,y]$. Then
\begin{align*}
\sum_{n = \lceil x\rceil}^{\lfloor y\rfloor} a_n \phi(n) = A(y)\phi(y) - A(x)\phi(x) - \int_x^y \du \; A(u) \phi'(u).
\end{align*}
\end{asmp}

\begin{lem}
\label{chi-n sum estimate}
Under Assumption \ref{Abel-partial-sum}, the following holds. Let $k\in \Nbb_0$, $b>0$ and $t\geq 0$. Then
\begin{align*}
\sum_{n = \lfloor t\rfloor +1}^\infty n^k \cdot \chi_b(n) & \leq \frac{1}{b^{2k+2}} \cdot (2k+3)! \cdot \max\{ 1, \, b^2t\}^{k+1} \cdot \chi_{b}(t).
\end{align*}
\end{lem}

\begin{proof}
Let $a_n = n^k$ for $n\geq 0$. It follows that
\begin{align*}
0 \leq A(t) = \sum_{n=1}^{\lfloor t\rfloor} n^k \leq t^{k+1}.
\end{align*}
Let $\phi(t) = \e^{-b \sqrt{t}}$. We have $\phi'(t) = -b\e^{-b\sqrt{t}}\cdot \frac{1}{2\sqrt{t}}$. Then, since $A(t) \phi(t)\geq 0$, by Assumption \ref{Abel-partial-sum} for $t<y$, we get
\begin{align*}
\sum_{n=\lceil t\rceil}^{\lfloor y\rfloor} n^k \cdot \e^{-b\sqrt{n}} \leq y^{k+1} \cdot \e^{-b\sqrt{y}} + \frac{b}{2} \int_t^y \dd u \; u^{k+\frac 12} \cdot \chi_b(u).
\end{align*}
Taking the limit $y\to \infty$, we have $y^{k+1}\e^{-b\sqrt{y}} \to 0$ and applying Lemma \ref{chi-estimate} (a) yields
\begin{align*}
\int_t^\infty \du \; u^{k+\frac 12}\cdot \chi_b(u) &\leq \frac{2}{b^{2k+3}}\cdot (2k+3)! \cdot \max\{1, b^2t\}^{k+1} \cdot \chi_b(t).
\end{align*}
%Finally, apply Lemma \ref{f-l-eps} with $\ell  = 1$ and $\varepsilon = \frac 12$. It follows that $\frac{2\ell}{\varepsilon} = 4 > \e$ so that
%\begin{align*}
%\int_t^\infty \du \; u^{k+\frac 12} \cdot \chi_b(u) &\leq \frac{32}{b^{2k+3} \cdot \e^2} \cdot (2k+3)! \cdot \max\{ 1, b^2t\}^k\cdot \chi_{\frac b2}(t).
%\end{align*}
Multiplying by $\frac b2$ gives the claim.
\end{proof}

\begin{note}
If all goes wrong, we have one thing: Let $x,y>0$ (think: large!), then $x^x\cdot y^y \leq (x+y)^{x+y}$. For,
\begin{align*}
x^xy^y &= \e^{x\log(x) +y\log(y)} = \exp\bigl((x+y)\bigl[ \frac{x}{x+y} \log(x) + \frac{y}{x+y}\log(y)\bigr]\bigr) \\
%
&\leq \exp\bigl( (x+y)\log\bigl( \frac{x^2+y^2}{x+y}\bigr)\bigr) \leq \e^{(x+y)\log(x+y)}.
\end{align*}
We used the concavity of the log and $x^2+y^2\leq (x+y)^2$.
\end{note}




==> source/Exponential_estimates_for_the_adiabatic_theorem/Notes/1_Introduction.tex <==
%auto-ignore  % for ArXiv to process correctly

\section{Introduction}

\subsection{How it came to this chapter}

In spring 2019, I had the opportunity to travel to the University of British Columbia (UBC) in Vancouver, Canada, for a research visit, which lasted four months. During the stay, my guest advisor Sven Bachmann and I started the project on proving exponential estimates for the adiabatic theorem in \cite{SvenAdiabatic}. Unfortunately, we could not finish the project in due time and planned to complete it in a second visit in 2020, which was then canceled due to the COVID-19 pandemic. Consequently, this project is still lying on my desk waiting to be completed and the progress we made so far forms the content of this chapter. As the time of my PhD studies is coming to an end, I feel that this thesis is a good opportunity to present the state of the project. I am also happy to hereby comply with a corresponding request by Stefan Teufel in Tübingen.

Since discussions on a regular basis are hard to organize between Sven and me due to the physical distance and the time shift, it is a pleasure to welcome the postdoc researcher Amanda Young, who we could recently (in September 2021) win to join the project. She is currently working at Technische Universität München. 

It is needless to say that I plan to undertake another attempt to bring the project to a successful conclusion in the remaining time after the submission of this thesis but I have to see if time permits enough commitment.

\subsection{Exponential estimates via optimal truncation}

Mathematically, the intention has been to prove exponential error estimates for the adiabatic theorem that has been proved in the work \cite{SvenAdiabatic}. We have in mind using a similar strategy to the one presented in the paper \cite{HagedornJoye}, namely to recursively provide an explicit estimate for the adiabatic error in the expansion after the $n$\tho\ step and then perform an optimal truncation argument. We will be somewhat more detailed below on what we mean by an optimal truncation argument. This goal has not been reached yet but we believe that the content of the chapter is helpful to understand the problem and needed to be applied in one way or the other by anybody in the future, who wants to complete the work.

Let us explain a bit further why we did not yet manage to prove the aimed result. When we began the project at the UBC, it soon became clear that the desired estimate would not be possible to prove within the by now standard locality setup that has already been used in \cite{AutomorphicEquivalence} and has worked its way through countless publications in the business of quantum lattice systems in the meantime. We only mention the recent publications \cite{BdRFL2021, BrunoQuasilocal, NWY2020} and point out to the reader the references therein as examples for communities using this framework. The reason why this setup fails in the context of our problem are the badly behaved ``continuity'' estimates, as we shall call them. Namely, when an operation like the commutator is applied to a pair of \emph{local Hamiltonians} (sometimes also called \emph{quasilocal operators}), the question is: What are the locality properties of the commutator provided the corresponding properties of the initial Hamiltonians are known and can we relate them quantitatively? In other words, if $G_1, G_2$ are the initial Hamiltonians, such a quantitative relation would be given by an estimate of the type
\begin{align}
\Vert \, [G_1, G_2]\, \Vert_{\mathrm{fin}} \leq C_{\mathrm{in}, \mathrm {fin}}([\cdot, \cdot]) \; \Vert G_1\Vert_{\mathrm {in}} \; \Vert G_2\Vert_{\mathrm {in}}. \label{AT:Continuity_estimate}
\end{align}
Here, $\Vert \cdot\Vert_{\mathrm{fin}}$ and $\Vert \cdot\Vert_{\mathrm{in}}$ are two possibly different initial and final norms, which should best be related in a convenient way and $C_{\mathrm{in}, \mathrm{fin}}([\cdot, \cdot]) >0$ is a constant independent of $G_1$ and $G_2$. We shall call \eqref{AT:Continuity_estimate} a ``continuity estimate'' for the operation $[\cdot, \cdot]$ for obvious reasons. The problem is often not to find such a constant but rather to gain precise control of it in that we have a formula at hand which is easy to work with. Additionally, the constant needs to behave well enough for the operation to be applied over and over again in an iterative procedure like the adiabatic expansion.

We remark that one is tempted to choose the operator norm $\Vert \cdot\Vert$ for $\Vert \cdot\Vert_{\mathrm{in}}$ and $\Vert \cdot\Vert_{\mathrm{fin}}$ but the reader familiar to extended quantum systems will immediately realize the problem of the volume dependence of this choice and the necessity of a norm that measures the ``locality'' of the local Hamiltonian. We will comment on this problem further below.

It turns out that the standard machinery mentioned above behaves too badly under repeated application of such operations and the constants that are stacking on the way grow much too fast. It is difficult to explain this phenomenon more precisely at this point without any notation at hand but we will provide some details below in Subsection \ref{AT:Norms_Section}.

When we sat in front of the problem in Vancouver, we realized that before we could even think about actually performing the adiabatic expansion in the manner of \cite[Lemma 4.3]{SvenAdiabatic}, we were forced to go back to the very beginning of the theory and tidy up the setup of locality within our quantum lattice system. After we defined the new norm, the first item on the list was then to provide a Lieb--Robinson bound for Hamiltonians that have a finite local norm. We realized that, within this new setup, it is actually possible to gain a pretty simple proof of a Lieb--Robinson bound even for tree graphs, which we shall present in Section \ref{AT:LR_bounds_Section}.

In Section \ref{AT:I_Section} we will introduce the map $\Ical$, which is the ``generator of the spectral flow'', ``local inverse of the Liouvillian'', or ``weighted integral operator'', depending on the convention within the respective community. This operator is a central tool in solving the Schrödinger equation in a locality preserving fashion and it requires the fact that the underlying Hamiltonian has a spectral gap. Under the assumption of a gap, we show that it provides an inverse of the map $G\mapsto [H, G]$, where $H$ is the Hamiltonian. In order to do this, we have to construct a new weight function which depends on the gap and satisfies an estimate in terms of our explicit decay functions. We are aware of and will not participate in the debate whether this restriction is too severe for realistic models to be true. Instead we will just stick to this assumption and see how far we get with it. It seems that already the (unsolved, after all) problem of this chapter in the presence of a gap is difficult enough and I encourage the reader to provide improvements in the gapless direction.

The continuity estimates are contained in Section \ref{AT:Estimating_Operations_Section}, starting with the (multi-) commutator. We further provide a well-behaved explicit estimate for the operation $\Ical$, showing the locality preserving property. For us, the main technical announcement is that we are able to provide the first explicit locality estimate for arbitrary high derivatives of $\Ical(G)$, provided the Hamiltonian for the underlying time evolution and $G$ are smooth. To the best of my knowledge, such an estimate is not known in the existing literature.

As an addendum, we also point out in Section \ref{AT:Analytic_Interactions_Section} how an analyticity property of the Hamiltonian $H$ allows to transport estimates on $H$ to higher derivatives of $H$. 

Unfortunately, to the present day, we were not able to perform the adiabatic expansion in its full generality in the sense of providing suitable estimates for the operators that are constructed iteratively. However, we present a sketch of a concept that in our opinion has the potential to provide the desired result when all ingredients are taken into account. We demonstrate this in Section \ref{AT:Concept_Section} with a toy estimate that discards the involvement of derivatives.

The reader should keep in mind that this chapter has the character of a working note, which means that the proofs may look a bit overdetailed sometimes. In particular, it should be noted that, in contrast to the previous chapters on BCS theory, one of the central interests in the endeavor here is the size and dependency of constants. For this reason, statements are always as explicit as possible and there is no ``constant $C$ that is allowed to change from line to line'' in this chapter.

\subsection{Basics of quantum spin systems}

\subsubsection{Lattice systems and their shape}

The prototype of a lattice system is, as the name suggests, the lattice $\Zbb^d$ with its graph norm\footnote{A graph is the tuple $(\Gamma, \Ecal)$ of $\Gamma$ with a set of edges $\Ecal$ where an element $e\in \Ecal$ connects two elements $x,y\in \Gamma$. The graph metric $d(x,y)$ is then defined as the cardinality of the smallest subset $e\in \Ecal$, which connects $x$ and $y$. If $\Gamma = \Zbb^d$, the standard graph metric is given by the 1-norm $|\cdot|_1$.} $|x|_1 := \sum_{i=1}^d |x_i|$. The reason why I don't like this picture so much is that it suggests the notion of a ``\emph{dimension}'' describing the shape of the lattice, namely $d$. However, it turns out that the dimension is not so relevant in this chapter in the sense that we never choose a basis for any space. Furthermore, this notion is not available for tree graphs and these are the reasons why I would rather like to think of the more general notion of ``\emph{growth relations}'' of the cardinality of a set in terms of its diameter. In this spirit, $\Zbb^d$ would be of polynomial growth with the power $d$ and a tree graph would be of exponential growth. We will comment on this a bit further below. 

That is why, in general, a lattice system for us will be a countable metric space $(\Gamma, d)$ with the graph metric. The ball of radius $n\in \Nbb_0$ about the point $x\in \Gamma$ is denoted by
\begin{align}
B_n(x) &:= \bigl\{ z\in \Gamma : d(x,z) \leq n\bigr\} \label{AT:Ball_definition}
\end{align}
and a set $Z\subset \Gamma$ has a (possibly infinite) \emph{diameter}, which we denote by
\begin{align}
\Dcal(Z) &:= \diam(Z) := \sup \bigl\{ d(x,y) : x,y\in Z\bigr\}. \label{AT:Diameter}
\end{align}
The set of finite and nonempty subsets
\begin{align}
\Fcal(\Gamma) &:= \bigl\{ \Lambda \subset \Gamma : 0 < |\Lambda| < \infty\bigr\} \label{AT:Finite_subsets_definition}
\end{align}
plays an important role throughout this chapter, where $|\Lambda|$ is the cardinality of the set $\Lambda$. Typically, to fix the shape of the lattice to be polynomial, we make assumptions of the following kind: There are constants $\kappa >0$ and $d \in \Nbb_0$ such that for every $Z\in \Fcal(\Gamma)$, we have
\begin{align}
|Z| \leq \kappa \, (1 + \Dcal(Z))^d. \label{AT:Growth_condition}
\end{align}
This means that $\Gamma$ has a polynomial growth of degree $d$, or is $d$-dimensional. Obviously, a tree graph violates \eqref{AT:Growth_condition}.

\subsubsection{The quantum setup}

We raise a quantum system upon $\Gamma$ by associating to each \emph{vertex} or \emph{lattice site} $x\in \Gamma$ a so-called \emph{on-site} Hilbert space $\Hcal_x$. Furthermore, to any subset $\Lambda \subset \Gamma$ (finite or infinite), the Hilbert space $\Hcal_\Lambda := \bigotimes_{x\in \Lambda} \Hcal_x$ is associated. Then, we also define the algebra of observables $\Acal_\Lambda := \Bcal(\Hcal_\Lambda)$, which consists of the bounded operators $\Hcal_\Lambda \ra \Hcal_\Lambda$, eqipped with the usual operator norm $\Vert \cdot \Vert$. There is a canonical embedding $\Acal_\Lambda \hookrightarrow \Acal_{\Lambda'}$ if $\Lambda \subset \Lambda'$, which is defined by $A \mapsto A \otimes \bigotimes_{x\in \Lambda'\setminus \Lambda} \Idbb \in \Acal_{\Lambda'}$ and which we use without comment. We also define the set of local observables by $\Acal_{\mathrm{loc}} := \bigcup_{\Lambda \in \Fcal(\Gamma)} \Acal_{\Lambda}$. For a local observable $A\in \Acal_{\mathrm{loc}}$, we may define its \emph{support} by the smallest set $X \in \Fcal(\Gamma)$ such that $A\in \Acal_X$, i.e.,
\begin{align}
\supp(A) &:= \bigcap \bigl\{ X\in \Fcal(\Gamma) : A\in \Acal_X \bigr\}.
\end{align}

Interesting quantum effects start becoming visible in the infinite volume limit, that is, when operators are considered that have an infinite support. This fact can be dealt with in two different ways:
\begin{enumerate}[(1)]
\item We can try to define all objects in infinite volume as limiting objects of their finite volume correspondents.
\item We try to restrict to a finite volume and execute the theory in such a way that the quantities of interest survive the infinite volume limit.
\end{enumerate}
It has turned out that option (1) suffers from the fact that several central objects such as the Hamiltonian do not possess a nice representation in the infinite volume and can only (if at all) be abstractly extended. However, we should not overlook that several other quantities like can indeed be extended. Nevertheless, option (2) is the method we will pursue. Therefore, all objects are introduced in finite volume and the theory is never allowed to depend on this finite volume.

To get started, an interaction is a map $\Phi \colon \Fcal(\Gamma) \ra \Acal_{\mathrm{loc}}$, which assigns $Z\mapsto \Phi(Z)$ with $\Phi(Z) \in \Acal_Z$. It is easy to see that the space of interactions inherits a complex vector space structure from the spaces of bounded operators via the canonical embedding. A sum of local terms
\begin{align}
\sum_{Z \in \Fcal(\Gamma)} \Phi(Z) \label{AT:Sum_of_local_terms}
\end{align}
is then an operator which has infinite operator norm unless $\Phi$ is \emph{compactly supported}, meaning that there is an $R>0$ such that $\Phi(Z) =0$ if $|Z| \geq R$ (example: nearest neighbor interactions). This raises the need for a locality setup, since the operator norm of a term $\Phi(Z)$ in \eqref{AT:Sum_of_local_terms} typically grows linearly in $|Z|$. Therefore, we need a different measure for the ``size'' of such an object, which encodes the fact that realistic interactions in quantum lattice systems merely feature nearest neighbor interactions in the most probable case and interactions of multituples of sites are suppressed with growing number of involved sites.

\subsubsection{Norms}
\label{AT:Norms_Section}

Mathematically speaking, the ``size'' of an object like \eqref{AT:Sum_of_local_terms} is expressed in terms of a norm. This is the point where is becomes technically delicate because the whole theory is very sensitive to the number of symbols and notions that are used in the definition of the norm. Therefore, there is inevitable need to keep this formula as concise as possible. To express the suppression of terms coming from large sets in the sum \eqref{AT:Sum_of_local_terms}, we need a bounded, non-increasing, positive function $\zeta\colon [0,\infty) \ra (0,\infty)$ that is logarithmically superadditive, i.e., for $x,y\geq 0$, we have
\begin{align}
\zeta(x + y) &\geq \zeta(x) \, \zeta(y).
\end{align}
In practice, $\zeta$ is a rapidly decaying function. The norm that we propose then reads
\begin{align}
\Vert \Phi\Vert_\zeta &:= \sup_{x\in \Gamma} \sum_{\substack{Z\subset \Gamma \\ x\in Z}} \frac{\Vert \Phi(Z)\Vert}{\zeta(\Dcal(Z))}. \label{AT:new_norm}
\end{align}
It should be noted that a norm which needs to be uniform in the lattice $\Gamma$ must have a point $x\in \Gamma$ which it is ``attached to'' and which is then suped over. Otherwise, we would sum over \emph{all} subsets in the lattice and even if we restrict to sets $Z\in \Fcal(\Gamma)$, we immediately realize that the number of sets of a given fixed diameter is heavily dependent on the shape of the lattice then.

Let us compare our definition to the one in \cite{SvenAdiabatic}, which reads
\begin{align}
\Vert \Phi\Vert_{\zeta, N} &:= \sup_{x, y\in \Gamma}  \frac{1}{F(d(x,y)) \, \zeta(d(x,y))} \sum_{\substack{Z \subset \Gamma \\ x,y\in Z}} |Z|^N \; \Vert \Phi(Z)\Vert, & F(r) &:= (1 + r)^{-(d+1)} \label{AT:old_norm}
\end{align}
In our opinion, \eqref{AT:old_norm} suffers from three facts that trigger a lot of problems:
\begin{enumerate}
\item The measure for locality is determined by two different parameters that are not comparable: a natural number $N\in \Nbb_0$, which indexes a volume moment $|Z|^N$ for a finite subset $Z$ of the lattice, as well as a rapidly decaying function $\zeta$, which by the factor $\zeta(d(x,y))^{-1}$ in the norm likewise indicates decay. It turns out that there is need to unify these decay parameters so that the local norm would only be determined by just one parameter. Since $|Z|$ and $d(x,y)$ are incomparable, however, we decided to replace $d(x,y)$ by the diameter $\Dcal(Z)$. In this way, the quantities $|Z|$ and $\Dcal(Z)$ become comparable --- provided we make a suitable assumption on shape of the lattice, like \eqref{AT:Growth_condition} --- and we do not need the volume factor $|Z|^N$ anymore, which had kept arising in each operation in the setup of \cite{SvenAdiabatic}. This turns out to cure the theory to a large extent and further makes it possible to leave away one point of $x,y\in Z$, which even more simplifies the business.

\item The existence of the decay function $F$, whose shape limits the theory to polynomially growing lattices from the very beginning, and whose so-called ``convolution property'' is used to prove a Lieb--Robinson bound, is a big problem in practice. We get rid of this function completely. \ifthenelse{\equal\masterfile{Diss}}{In the case of interest, the reader may have a look at Section \ref{AT:Old_norm_estimate_Section}, where we present a continuity estimate for $\Ical$ in the framework of the old norm in \cite{SvenAdiabatic}, which we obtained before we realized that iterating $\Ical$ with the help of this estimate is highly problematic on its own. This illustrates very well the problematic behavior of the function $F$, when it comes to precise continuity estimates and the proof shows that it is somewhat clumsy to work with the norm in \eqref{AT:old_norm}.}{}

\item The abstract class of rapidly decaying functions $\zeta$ makes it difficult to prove concise estimates. We choose an ``explicit'' class of rapidly decaying functions $\zeta$, namely the stretched exponential decay functions $\e^{-b x^s}$ for $b>0$ and $0 < s \leq 1$. Since $s$ is basically fixed throughout the theory, the norm effectively becomes determined by a single positive number $b >0$, which in our opinion purges the theory further and enables us to prove short, handy, and well-behaved continuity estimates for the relevant operations.
\end{enumerate}

\subsubsection{Preliminary note on the adiabatic theorem and optimal truncation}

So far, we have discussed locality setups for general quantum spin systems. Before we introduce the setup we will work with in the context of the adiabatic theorem, we take a somewhat closer look at the adiabatic theorem itself. The adiabatic theorem is a statement about the approximation of the time evolution of a state $\rho(u)$ given by a Hamiltonian $H(\varepsilon t)$, where $\varepsilon >0$ is the small \emph{adiabatic parameter} and $\rho(u)$ is initially given by a state $\rho_0$. The adiabatic parameter $\varepsilon$ measures the ``slowness'' of the variation of $H$ in time compared to the hopping it induces on the physical space, i.e., the system has a ``slow'' and a ``fast'' degree of freedom that are separated by the scale $\varepsilon$. The time evolution takes place according to the (adiabatic) Schrödinger equation
\begin{align}
\i \varepsilon \frac{\dd}{\dd u} \rho(u) &= [H(u), \rho(u)], & \rho(0) &= \rho_0. \label{AT:Schroedinger}
\end{align}
Here, we have already performed a rescaling of times $u = \varepsilon t$. The rescaled time is thus $u\in [0,1]$, which corresponds to the physical time $t \in [0 , \varepsilon^{-1}]$. The theorem has a long standing history which we will not repeat here (see \cite{SvenAdiabatic} for details), and has been proven in various different contexts and classes of problems.

Let $\rho_0 = P_0$ be the ground state projection of $H(0)$ and let $P(u)$ be the ground state projection of $H(u)$. A type of question one would then typically like to address is how much $\rho(u)$ differs from $P(u)$. In other words, are the operations ``take the ground state projection'' and ``evolve according to \eqref{AT:Schroedinger}'' commutative? Or, if we start with an instantaneous ground state and evolve it according to \eqref{AT:Schroedinger} for a time $u$, is the resulting state equal to $P(u)$ and, if not, how large is the error? The ``classical'' adiabatic theorem usually should answer this question in the following manner: We have
\begin{align}
\sup_{s\in [0,1]} \Vert \rho(u) - P(u) \Vert \leq C \varepsilon. \label{AT:Adiabatic_Thm_classic}
\end{align}
As pointed out earlier, the problem is that the constant $C$ in \eqref{AT:Adiabatic_Thm_classic} typically grows linearly with the number of lattice sites involved in the support of $H$ so \eqref{AT:Adiabatic_Thm_classic} becomes meaningless in the infinite volume limit, as long as $\varepsilon$ is nonzero, even if we restrict to finite volume initially. Therefore, to be able to prove a reasonable analogon for quantum spin systems, we have to replace the left side of \eqref{AT:Adiabatic_Thm_classic} by a volume independent quantity.
%On top of that, it is difficult to directly work in the thermodynamic limit since many of the central objects only have abstract extensions to infinite volume, if any. 
The revolutionary idea that has been introduced successfully in \cite{SvenAdiabatic} is to 
\begin{enumerate}
\item consider a finite volume $\Lambda$ and carry out the theory on the finite volume, proving uniform estimates in $|\Lambda|$.

\item do this by relaxing the topology from the operator norm to expectation values of observables with finite support within $\Lambda$. These do not probe the whole quantum system but only a small region.
\end{enumerate}
The reader is referred to \cite{SvenAdiabatic} for a thorough introduction into the business of the adiabatic theorem in the context of extended quantum systems and to \cite{SvenAdiabatic_Note} for further explanations around the topic.

Let us briefly sketch what we call an optimal truncation argument. Typically, under the assumption of a Hamiltonian that has an analytic extension to a complex strip around the real axis, \eqref{AT:Adiabatic_Thm_classic} can be improved to
\begin{align}
\Vert \rho(1) - P(1) \Vert &\leq C_m \varepsilon^m , & m&\in \Nbb, \label{AT:Intro_Optimal_truncation_1}
\end{align}
in terms of a constant $C_m$ that depends on $m$ as $C_m \lesssim m^m$. The function $f_\varepsilon(x) := x^x \varepsilon^x$, which can be written as $f_\varepsilon(x) = \exp( x \log(x\varepsilon))$, then has a unique global minimum at $x(\varepsilon) := (\e\varepsilon)^{-1}$ with value
\begin{align}
f_\varepsilon( x(\varepsilon)) = \e^{- \frac{\e^{-1}}{\varepsilon}},
\end{align}
which is exponentially decaying as $\varepsilon \to 0$. When we successfully deal with the subtlety that $x(\varepsilon)$ is not an integer in general, we can therefore choose $m\in \Nbb$ in \eqref{AT:Intro_Optimal_truncation_1} optimally in terms of $\varepsilon$ to improve the error to exponential decay in $\varepsilon^{-1}$.

\subsection{The setup of locality for this chapter}

We assume that the dimension of the on-site Hilbert spaces $\Hcal_x$ is uniformly bounded, that is,
\begin{align*}
\sup_{x\in \Gamma} \dim \Hcal_x < \infty.
\end{align*}

\subsubsection{Interactions and the new norm}

We are in position to introduce the locality setup suitable for the adiabatic theorem.

\paragraph{Time-independent setting.} An \emph{interaction} on $\Gamma$ is a family $\Phi = \{\Phi^\Lambda\}_{\Lambda \in \Fcal(\Gamma)}$ of maps $\Phi^\Lambda \colon \Fcal(\Lambda) \ra \Acal_\Lambda$, which assign $Z \mapsto \Phi^\Lambda(Z)$, where $\Phi^\Lambda(Z) \in \Acal_Z$. We denote the set of interactions by $\Bcal$.

A family of operators $G = \{G^\Lambda\}_{\Lambda\in \Fcal(\Gamma)}$ is called a \emph{local Hamiltonian} if there is an interaction $\Phi_G \in \Bcal$ such that for all $\Lambda\in \Fcal(\Gamma)$, we have
\begin{align}
G^\Lambda = \sum_{Z\subset \Lambda} \Phi_G^\Lambda (Z). \label{AT:Local_Hamiltonian_decomposition}
\end{align}
The set of local Hamiltonians is denoted by $\Lcal$. Note that $\Phi_G$ such that \eqref{AT:Local_Hamiltonian_decomposition} holds is not unique. For the sake of readability, we will mostly omit the dependence on $\Lambda$ in the rest of this chapter, since this does not cause any confusion. 

It is easy to verify that $\Bcal$ and $\Lcal$ are complex vector spaces with the usual operations that are inherited from the space of bounded operators.

With the help of the stretched exponential decay functions
\begin{align}
\chi_{s, b}(x) &:= \e^{-b \, x^s} , & 0 < s \leq 1, \quad  b\geq 0, \quad x \geq 0, \label{AT:chi_definition}
\end{align}
we define the \emph{local norm} of an interaction $\Phi\in \Bcal$ as
\begin{align}
\Vert \Phi\Vert_{s, b} &:= \sup_{\Lambda \in \Fcal(\Gamma)} \sup_{x\in \Lambda} \sum_{\substack{Z\subset \Lambda \\ Z \ni x}} \frac{\Vert \Phi^\Lambda(Z)\Vert}{\chi_{s, b}(\Dcal(Z))}.
\end{align}
Then, let us define the set of \emph{$(s, b)$-localized interactions} by
\begin{align*}
\Bcal_{s,b} := \bigl\{ \Phi \in \Bcal, \; \Vert \Phi \Vert_{s,b} < \infty\bigr\}.
\end{align*}
If $G\in \Lcal$ such that \eqref{AT:Definition_gapped_Hamiltonian} holds for some $\Phi\in \Bcal_{s, b}$, then $G$ is called \emph{$(s, b)$-localized} and the set of $(s, b)$-localized Hamiltonians is denoted by $\Lcal_{s, b}$. Since $\Phi_G$ is not unique, the term $\Vert G\Vert_{s, b}$ remains undefined but equals, per convention, $\Vert \Phi_G\Vert_{s, b}$ provided an interaction has been specified previously or is clear from the context.

\begin{lem}
For each $0 < s \leq 1$ and $b\geq 0$, the functional $\Vert \cdot \Vert_{s, b}$ is a norm on $\Bcal_{s, b}$, and $(\Bcal_{s, b}, \Vert \cdot\Vert_{s, b})$ is a Banach space. 
\end{lem}

\begin{proof}
Homogeneity and triangle inequality are inherited from the operator norm. Assume that $\Vert \Phi\Vert_{s, b} =0$ for some interaction $\Phi$. Then, for all $x\in \Lambda$, we have $\Vert \Phi^\Lambda(Z)\Vert =0$ for every set $Z\subset \Lambda$ that contains $x$. If a nonempty $Z'\subset \Lambda$ is given, choose an arbitrary point $x'\in Z'$ and obtain $\Vert \Phi^\Lambda(Z') \Vert =0$. This proves that $\Phi^\Lambda(Z') =0$ for every $Z'\subset \Lambda$, whence $\Phi =0$. The completeness property of $\Bcal_{s, b}$ is inherited from the completeness of $\Bcal(\Hcal_\Lambda)$.
\end{proof}

\begin{bem}
Since $\chi_{s, b_1} > \chi_{s, b_2}$ whenever $b_1 < b_2$, we have that $b \mapsto \Vert \Phi\Vert_{s, b}$ is a strictly increasing function on $[0, \infty)$ with values in $\Rbb \cup \{\infty\}$. Therefore, if there is an $0 < s \leq 1$ and a $b>0$ such that $\Vert \Phi\Vert_{s, b} < \infty$ then, either there is $b_0>0$ such that $\lim_{b \nearrow b_0}\Vert \Phi\Vert_{s, b} = \infty$ or we have $\lim_{b\nearrow \infty} \Vert \Phi\Vert_{s, b} = \infty$. In any case, we may assume without loss of generality that
\begin{align}
\Vert \Phi\Vert_{s, b} \geq 1. \label{AT:Hamiltonian_norm_greater_than_1}
\end{align}
\end{bem}

Let us denote the class of $s$-localized interactions by
\begin{align}
\Bcal_s &:= \bigcup_{b >0 } \Bcal_{s, b} , & 0 &< s \leq 1, \label{AT:Interactions_s-localized_definition}
\end{align}
and denote the corresponding classes of local Hamiltonians by $\Lcal_s$. Furthermore, define the classes of (stretched) exponentially localized interactions by
\begin{align}
\Ecal &:= \Bcal_1, & \Scal &:= \bigcup_{0 < s < 1} \Bcal_s, \label{AT:Interactions_stretched_exponentially_localized_definition}
\end{align}
respectively, and write $\Lcal_\Ecal$ and $\Lcal_\Scal$ for the corresponding sets of local Hamiltonians. 
%Then, the set of \emph{localized} interactions can be conveniently written as
%\begin{align}
%\Bcal_{\mathrm{loc}} &:= \Ecal \cup \Scal \label{AT:Interactions_localized_definition}
%\end{align}
%and, analogously, the set of localized local Hamiltonians is denoted by $\Lcal_{\mathrm{loc}}$.

\paragraph{Time-dependent setting.} Since we will be concerned with analytic interactions of time, we consider an open subset $I \subset \Cbb$. A \emph{time-dependent interaction} is a map $\Phi \colon I \ra \Bcal$ and we denote the set of time-dependent interactions by $\Bcal(I)$. A time-dependent local Hamiltonian is a map $G\colon I \ra \Lcal$ such that \eqref{AT:Local_Hamiltonian_decomposition} holds for $G(u)$ for every $u\in I$. The set of time-dependent local Hamiltonians is denoted by $\Lcal(I)$.

For $0 < s \leq 1$ and $b \geq 0$, we define the \emph{local norm} of an interaction $\Phi\in \Bcal(I)$ by
\begin{align}
\vvvert \Phi\vvvert_{I, s, b} := \sup_{u\in I} \Vert \Phi(u)\Vert_{s, b}
\end{align}
and the set of $(s, b)$-localized time-dependent interactions is defined by
\begin{align*}
\Bcal_{s, b}(I) := \bigl\{ \Phi\in \Bcal(I), \; \vvvert \Phi\vvvert_{I, s, b} < \infty\bigr\}.
\end{align*}
Likewise, we conclude that $\vvvert\cdot\vvvert_{I, s, b}$ is a norm on $\Bcal_{s, b}(I)$ and $(\Bcal_{s, b}(I), \vvvert \cdot \vvvert_{I, s, b})$ is a Banach space. We also define the symbols $\Bcal_s(I)$, $\Lcal_s(I)$, $\Ecal(I)$, $\Scal(I)$, $\Lcal_\Ecal(I)$, and $\Lcal_\Scal(I)$ as the obvious analoga to the symbols defined in \eqref{AT:Interactions_s-localized_definition} and \eqref{AT:Interactions_stretched_exponentially_localized_definition}.

An interaction $\Phi \in \Bcal(I)$ is called \emph{holomorphic} if for every $\Lambda \in \Fcal(\Gamma)$ and $Z\subset \Lambda$ the map
\begin{align*}
u \longmapsto \Phi(u)^\Lambda(Z),
\end{align*}
is holomorphic on $I$. For any set $\Xcal(I)$ of time-dependent interactions (or local Hamiltonians), we write $\Xcal^\hol(I)$ for the corresponding set of holomorphic interactions (or local Hamiltonians).

%
%
%In the following we will mix the notations $\Phi^\Lambda(Z, u) := \Phi_u^\Lambda(Z)$ when this is convenient.
%
% The omission of $I$ induces a similar notation for the time-independent setting.
%
%For the sake of readability, we will mostly omit the time index $u$ and the dependence on $\Lambda$ in the rest of this chapter, since this does not cause any confusion.

%%%%%%%%%%%%%%%%%%% OLD VESION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We are in position to introduce the locality setup suitable for the adiabatic theorem now. A time-dependent \emph{interaction} is a family $\Phi = \{\Phi^\Lambda\}_{\Lambda \in \Fcal(\Gamma)}$ of maps $\Phi^\Lambda \colon \Fcal(\Gamma) \times I \ra \Acal_{\mathrm{loc}}$ on an interval $I\subseteq \Rbb$, which assign $(Z, u) \mapsto \Phi_u^\Lambda(Z)$, where $\Phi_u^\Lambda(Z) \in \Acal_Z$ for all $u\in I$. In the following we will mix the notations $\Phi^\Lambda(Z, u) := \Phi_u^\Lambda(Z)$ when this is convenient.
%
%It is easy to verify that the set of interactions is a complex vector space with the usual operations that are inherited from the space of bounded operators. With the help of the stretched exponential decay functions
%\begin{align}
%\chi_{s, b}(x) &:= \e^{-b \, x^s} , & 0 < s \leq 1, \quad  b\geq 0, \quad x \geq 0, \label{AT:chi_definition}
%\end{align}
%we define the \emph{local norm} of an interaction $\Phi$ as
%\begin{align}
%\Vert \Phi\Vert_{s, b} &:= \sup_{\Lambda \in \Fcal(\Gamma)} \sup_{x\in \Lambda} \sum_{\substack{Z\subset \Lambda \\ Z \ni x}} \sup_{u\in I} \frac{\Vert \Phi_u^\Lambda(Z)\Vert}{\chi_{s, b}(\Dcal(Z))}.
%\end{align}
%Then, let us define the set $\Bcal_{s, b}(I)$ of time-dependent interactions on the interval $I\subseteq \Rbb$ by
%\begin{align*}
%\Bcal_{s,b}(I) := \bigl\{ \Phi = \{ \Phi^\Lambda\colon \Fcal(\Lambda) \times I \ra \Acal_\Lambda\}_{\Lambda\in \Fcal(\Gamma)} : \Phi_u^\Lambda(Z) \in \Acal_Z, \, Z\in \Fcal(\Lambda), \; \Vert \Phi \Vert_{s,b} < \infty\bigr\}.
%\end{align*}
%Likewise, we define $\Bcal_{s, b} := \Bcal_{s, b}(\{0\})$ and refer to this as the time-independent setting.
%
%\begin{lem}
%For each $0 < s \leq 1$ and $b\geq 0$, the functional $\Vert \cdot \Vert_{s, b}$ is a norm on $\Bcal_{s, b}(I)$, and $(\Bcal_{s, b}(I), \Vert \cdot\Vert_{s, b})$ is a Banach space. 
%\end{lem}
%
%\begin{proof}
%Homogeneity and triangle inequality are clear. Assume that $\Vert \Phi\Vert_{s, b} =0$ for some interaction $\Phi$. Then, for all $x\in \Lambda$ and $u\in I$, we have $\Vert \Phi_u^\Lambda(Z)\Vert =0$ for every set $Z\subset \Lambda$ that contains $x$. If a nonempty $Z'\subset \Lambda$ is given, choose an arbitrary point $x'\in Z'$ and obtain $\Vert \Phi_u^\Lambda(Z') \Vert =0$. This proves that $\Phi_u^\Lambda(Z') =0$ for every $Z'\subset \Lambda$, whence $\Phi =0$. The completeness property of $\Bcal_{s, b}(I)$ is inherited from the completeness of $\Bcal(\Hcal_\Lambda)$.
%\end{proof}
%
%
%
%\begin{bem}
%Since $\chi_{s, b_1} > \chi_{s, b_2}$ whenever $b_1 < b_2$, we have that $b \mapsto \Vert \Phi\Vert_{s, b}$ is a strictly increasing function on $[0, \infty)$ with values in $\Rbb \cup \{\infty\}$. Therefore, if there is an $0 < s \leq 1$ and a $b>0$ such that $\Vert \Phi\Vert_{s, b} < \infty$ then, either there is $b_0>0$ such that $\lim_{b \nearrow b_0}\Vert \Phi\Vert_{s, b} = \infty$ or we have $\lim_{b\nearrow \infty} \Vert \Phi\Vert_{s, b} = \infty$. In any case, we may assume without loss of generality that
%\begin{align}
%\Vert \Phi\Vert_{s, b} \geq 1. \label{AT:Hamiltonian_norm_greater_than_1}
%\end{align}
%\end{bem}
%
%A family of operators $G = \{G^\Lambda\}_{\Lambda\in \Fcal(\Gamma)}$ is called a \emph{local Hamiltonian} if there is an interaction $\Phi_G = \{\Phi_G^\Lambda\}_{\Lambda\in \Fcal(\Gamma)}$ such that
%\begin{align}
%G^\Lambda = \sum_{Z\subset \Lambda} \Phi_G^\Lambda (Z). \label{AT:Local_Hamiltonian_decomposition}
%\end{align}
%If additionally $\Phi_G\in \Bcal_{s,b}(I)$, we write $G\in \Lcal_{s, b}(I)$. Note that $\Phi_G$ such that \eqref{AT:Local_Hamiltonian_decomposition} holds is not unique, whence we always have to specify which interaction we agree on before we state results. 
%
%Let us denote the sets of $s$-localized interactions by
%\begin{align}
%\Bcal_s(I) &:= \bigcup_{b >0 } \Bcal_{s, b}(I) , & 0 &< s \leq 1, \label{AT:Interactions_s-localized_definition}
%\end{align}
%and denote the corresponding classes of local Hamiltonians by $\Lcal_s(I)$. Furthermore, define the classes of (stretched) exponentially localized interactions by
%\begin{align}
%\Ecal(I) &:= \Bcal_1(I), & \Scal(I) &:= \bigcup_{0 < s < 1} \Bcal_s(I), \label{AT:Interactions_localized_definition}
%\end{align}
%respectively, and write $\Lcal_\Ecal(I)$ and $\Lcal_\Scal(I)$ for the corresponding sets of local Hamiltonians. Then, the set of \emph{admissible} interactions can be conveniently written as
%\begin{align}
%\Bcal(I) &:= \Ecal(I) \cup \Scal(I) \label{AT:Interactions_admissible_definition}
%\end{align}
%and, analogously, the set of admissible local Hamiltonians is denoted by $\Lcal(I)$. The omission of $I$ induces a similar notation for the time-independent setting.
%
%For the sake of readability, we will mostly omit the time index $u$ and the dependence on $\Lambda$ in the rest of this chapter, since this does not cause any confusion.

==> source/Exponential_estimates_for_the_adiabatic_theorem/Notes/30_Exponential-Estimates.tex <==
%auto-ignore  % for ArXiv to process correctly

\chapter[Exponential Estimates]{A Setup for Exponential Estimates for the Adiabatic Theorem in Extended Quantum Systems}

\input{30_Exponential-Estimates/1_Technical_Preparations}
\newpage
\input{30_Exponential-Estimates/2_New-norm}
\newpage
\input{30_Exponential-Estimates/3_LR-bound}
\newpage
\input{30_Exponential-Estimates/4_Estimating_Operations}

\newpage
\input{30_Exponential-Estimates/5_Time-dependent_interactions}

\newpage
\input{30_Exponential-Estimates/6_Concept_Adiabatic_Expansion}

\newpage
\input{30_Exponential-Estimates/18_Things_for_later}
%
%\newpage
%\setcounter{section}{19}
%\input{30_Exponential-Estimates/20_Old-norm-estimates}

==> source/Exponential_estimates_for_the_adiabatic_theorem/Notes/99_Derivatives.tex <==
%auto-ignore  % for ArXiv to process correctly

%\section{A fresh look on derivatives}

%Let $I\subset \Rbb$ be an interval and let $X\subset \Lambda$. We denote the space of continuous sections $I\ra \Acal_X$ by $\Scal_I(\Acal_X)$ and equip it with the norm
%\begin{align*}
%\Vert A\Vert_{\Scal_I(\Acal_X)} := \sup_{t\in I} \Vert A(t)\Vert.
%\end{align*}
%Let $\Lcal$ be the vector space of local Hamiltonians and let $\Scal_I(\Lcal)$ be the space of continuous sections $I \ra \Lcal$, where $I\subset \Rbb$ is an interval. This means that $\Gcal\in \Scal_I(\Lcal)$ satisfies
%\begin{align*}
%\Gcal(t) = \sum_{Z\subset \Lambda} \Phi_\Gcal(Z)(t)
%\end{align*}
%pointwise for all $t\in I$.
%
%Furthermore, for $m,n\in \Nbb$ and $0 < b \leq b'$, we denote the space of bounded linear operators $\Bcal_{s', b'}^m \ra \Bcal_{s, b}$ by $\BL^m(s', b', s, b)$. If $s = s'$, we abbreviate $\BL^m(s, b',b)$. If $m =1$, we omit the corresponding index. We equip the space with the norms
%\begin{align*}
%\Vert \Rcal\Vert_{s', b', s, b}^m := \sup_{\substack{G_1, \ldots, G_m\in \Bcal_{s', b'} \\ G_1,\ldots, G_m\neq 0}} \frac{\Vert \Rcal(G_1, \ldots, G_m)\Vert_{s, b}}{\Vert G_1\Vert_{s', b'} \cdots \Vert G_m\Vert_{s', b'}}.
%\end{align*}
%
%Likewise, the space of bounded linear operators $\Scal_I(\Bcal_{s', b'})^m \ra \Scal_I(\Bcal_{s, b})$ is denoted by $\BL_I^m(s', b', s, b)$ and $\BL_I^m(s, b', b)$ in case $s = s'$. We likewise omit $m$ if $m=1$ and equip the space with the norm
%\begin{align*}
%\Vert \Rcal\Vert_{s', b', s, b}^{m, I} := \sup_{t\in I} \sup_{\substack{\Gcal_1, \ldots, \Gcal_m\in \Bcal_{s', b'} \\ \Gcal_1,\ldots, \Gcal_m\neq 0}} \frac{\Vert \Rcal(\Gcal_1, \ldots, \Gcal_m)(t)\Vert_{s, b}}{\Vert \Gcal_1(t)\Vert_{s', b'} \cdots \Vert \Gcal_m(t)\Vert_{s', b'}}.
%\end{align*}



%\begin{proof}
%Let $A$ be a section of local observables $A(t) \in \Acal_X$, $X\subset \Lambda$. Then $\Jcal(A)(t) \in \Acal_X$ for all $t\in I$ and $\Vert \Jcal(A)\Vert_{\Scal_I(\Acal_X)} \leq |I| \, \Vert A\Vert_{\Scal_I(\Acal_X)}$. A straightforward computation also shows that $\Vert \Phi_{\Jcal(\Gcal)}(t)\Vert_{s, b} \leq |I| \, \Vert \Phi_\Gcal(t)\Vert_{s, b}$, which proves the claim.
%\end{proof}

%\begin{proof}[Proof of Theorem \ref{AT:tau_estimate}]
%We first prove that $\tau(G)$ defines a local Hamiltonian. To see this, for each $Z\subset \Lambda$ and $n\in \Nbb_0$, define the $n$\tho\ fattening of $Z$ to be
%\begin{align}
%Z_n := \bigl\{ z\in \Lambda : \dist(z,Z) \leq \frac n2\bigr\}. \label{AT:Fattening_definition}
%\end{align}
%For a local observable $A\in \Acal_X$, where $X\subset \Lambda$, define
%\begin{align}
%\Delta_0(A) &:= \Ebb_{X}(\tau(A)), & \Delta_n(A) &:= \Ebb_{X_n}(\tau(A)) - \Ebb_{X_{n-1}}(\tau(A)), & n&\geq 1, \label{AT:Deltan_definition}
%\end{align}
%where $\Ebb_Z(B) = \frac{\tr_{Z^c}(B)}{\dim \Hcal_Z}$ is the normalized partial trace. Then, $\Delta_n(A) =0$ for all $n$ sufficiently large, since $\Lambda$ is finite, and $\supp(\Delta_n(A))\subseteq X_n\cap \Lambda$. In particular, $\tau(A) = \sum_{n=0}^\infty \Delta_n(A)$, where the sum is finite, in fact. It follows that
%\begin{align}
%\Phi_{\tau(G)} (Z) := \sum_{n=0}^\infty \sum_{\substack{Y\subset \Lambda \\ Y_n = Z}} \Delta_n(\Phi_G(Z)) \label{AT:tau_interaction}
%\end{align}
%defines an interaction for $\tau(G)$, i.e., we have
%\begin{align*}
%\tau(G) = \sum_{Z\subset \Lambda} \Phi_{\tau(G)} (Z).
%\end{align*}
%
%Let us now show the claimed estimate \eqref{AT:tau_estimate_eq1}. In order to do this, we first note that $\Vert \Delta_0(A)\Vert \leq \Vert A\Vert$. We further decompose $\Delta_n(A) = \tilde \Delta_n(A) - \tilde \Delta_{n-1}(A)$, where
%\begin{align*}
%\tilde \Delta_n(A) := \Ebb_{X_n}(\tau(A)) - \tau(A).
%\end{align*}
%On the one hand, we have the trivial estimate
%\begin{align*}
%\Vert \tilde \Delta_n(A)\Vert \leq 2\, \Vert A\Vert.
%\end{align*}
%On the other hand, since $d(X, X_n) \geq n$, the Lieb--Robinson bound Corollary \ref{AT:LR-bound_kor} implies that we may use Lemma \ref{AT:Partial_Trace_Lemma} with
%\begin{align*}
%\varepsilon := \frac{2}{V_{1, 1}(a' - a)} \; |X| \; \Vert A\Vert \; \bigl( \e^{a \Vcal_{1, a, 1}(a' -a)  |t|} - 1\bigr) \e^{-an}.
%\end{align*}
%Here, $V_{1,1}$ is the constant in \eqref{AT:Vkb_definition}, and $\Vcal_{1, a, 1}(a' - a)$ is the Lieb--Robinson velocity defined in \eqref{AT:LR-velocity_definition}. This yields
%\begin{align*}
%\Vert \tilde \Delta_n(A)\Vert \leq \frac{2 \, \e^{a}}{V_{1,1}(a' - a)} \; |X| \; \Vert A\Vert \; \e^{v |t| - a(n+1)},
%\end{align*}
%where $v := a\, \Vcal_{1,a,1}(a' - a)$. 
%\end{proof}



%\begin{bem}
%The fact that has been pointed out in part (c) of the preceding examples is a general observation. If $m\in \Nbb_0$ and $\ell\in \Nbb_0$ are given and $0 \leq n \leq \Vert \ell\Vert_1 + 1 - m$ is arbitrary, then
%\begin{align*}
%\Wcal^{m', \ell'} = \Wcal^{m, \ell},
%\end{align*}
%where $m' = m + n$, $\ell' = (\ell_1, \ldots, \ell_m, 0, \ldots, 0)\in \Nbb_0^{m'}$. In particular, this holds for $n = \Vert \ell\Vert_1 + 1 - m$. Therefore, we henceforth assume that
%\begin{align}
%m = \Vert \ell\Vert_1 + 1 \label{AT:Mountain_Range_admissible}
%\end{align}
%and write
%\begin{align*}
%\Wcal^\ell := \Wcal^{m, \ell}.
%\end{align*}
%In other words, a vector $\ell \in \Nbb_0^m$ is \emph{admissible} for the mountain range operator if \eqref{AT:Mountain_Range_admissible} holds. This allows for the interpretation ``a chain with length $\ell_i$ starts at position $i$ and the first operator to be inserted is $\Gcal_i$'', $i =1, \ldots, \Vert \ell\Vert_1 + 1$.
%\end{bem}
%
%\begin{bem}
%Let $\ell$ be an admissible vector. When we differentiate now and the derivative hits the $j$\tho\ position, then, if $\ell_j >0$, we have
%\begin{align*}
%\ell \longmapsto (\ell_1 , \ldots, \ell_{j-1} , \ell_j + 1, 0, \ell_{j+1} , \ldots, \ell_m , 0, \ldots, 0).
%\end{align*}
%Otherwise, we have
%\begin{align*}
%\ell \longmapsto (\ell_1, \ldots, \ell_{j-1} , 1, \ell_j =0, \ell_{j+1} , \ldots, \ell_m, 0, \ldots, 0).
%\end{align*}
%In both cases, the new vector is admissible as well.
%\end{bem}

%
%
%
%
%\begin{lem}
%Let $G$ and $H$ be time-dependent local Hamiltonians. Then
%\begin{align*}
%\frac{\dd }{\dd u } \tau(G) = \tau(\dot G) + (\tau^* \circ \Vcal_1) (\dot H, G).
%\end{align*}
%\end{lem}
%
%\begin{proof}
%Duhamel.
%\end{proof}













==> source/Exponential_estimates_for_the_adiabatic_theorem/Notes/99_New-norm.tex <==
%auto-ignore  % for ArXiv to process correctly

\section{A new norm}

Let $(\Gamma,d)$ be a countable metric space and let $\Fcal(\Gamma)$ denote the set of nonempty finite subsets of $\Gamma$. For an interaction $\Phi = \{\Phi^\Lambda \colon \Pcal(\Lambda) \lra \Acal_\Lambda\}_{\Lambda\in \Fcal(\Gamma)}$, given $0 < s \leq 1$ and $b \geq 0$, let us define the functional
\begin{align}
\Vert \Phi\Vert_{s, b} &:= \sup_{\Lambda \in \Fcal(\Gamma)} \sup_{x\in \Lambda} \sum_{\substack{Z\subset \Lambda \\ Z\ni x}}\frac{\Vert \Phi(Z)\Vert}{\chi_{s,b}(\Dcal(Z))}. \label{new norm def}
\end{align}
Here and in the sequel, we write $\Dcal(Z) := \diam(Z) := \max_{x,y\in Z}d(x,y)$ for any $Z\in \Fcal(\Gamma)$.

\begin{lem}
For each $0 < s \leq 1$ and $b\geq 0$, the functional $\Vert \cdot \Vert_{s, b}$ is a norm on the vector space of interactions $\Phi$. 
\end{lem}

\begin{proof}
Homogeneity and triangle inequality are clear. Assume that $\Vert \Phi\Vert_{s, b} =0$ for some interaction $\Phi$. Then, for all $x\in \Lambda$, we have $\Vert \Phi(Z)\Vert =0$ for every set $Z\subset \Lambda$ that contains $x$. If $Z'\subset \Lambda$ is given, choose an arbitrary point $x'\in Z'$ and obtain $\Vert \Phi(Z') \Vert =0$. This proves that $\Phi(Z') =0$ for every $Z'\subset \Lambda$, whence $\Phi =0$.
\end{proof}

Let us define the normed (Banach) spaces
\begin{align*}
\Bcal_{s, b} := \bigl\{ \{\Phi^\Lambda \colon \Pcal(\Lambda) \lra \Acal_\Lambda\}_{\Lambda\in \Fcal(\Gamma)} : \Vert \Phi\Vert_{s, b} < \infty\bigr\}.
\end{align*}
An operator $G$ for which there is a $\Phi_G$ such that
\begin{align}
G = \sum_{Z \subset \Lambda} \Phi_G(Z) \label{local Ham decomp}
\end{align}
holds, we call a \emph{local Hamiltonian}. If additionally $\Phi_G\in \Bcal_{s,b}$, we write $G\in \Lcal_{s, b}$. 

\begin{asmp}
For $k,b>0$, we assume that the constants
\begin{align}
V_{s,k}(b) := \sup_{Z\in \Fcal(\Gamma)} |Z| \cdot \chi_{s,\frac bk}(\Dcal(Z)) \label{Vkb}
\end{align}
are finite. Here, $|Z|$ is the number of points in $Z\in \Fcal(\Gamma)$.
\end{asmp}

\begin{varbems}
\begin{enumerate}[(i)]
\item Note that $V_{s,k}(b) \leq V_{s,k'}(b)$ for $k\leq k'$ and $b>0$ fixed.
\item We have that $V_{s,k}(b) \to \infty$ as soon as $\nicefrac{b}{k} \to 0$.

\item Let $0 \leq \ell \leq k$ be given. Then
\begin{align}
V_\ell(b)^\ell \leq V_k(b)^k. \label{V-estimate}
\end{align}
To see this, use $\frac{k}{\ell} \geq 1$ and $|Z|\geq 1$ for all $Z\in \Fcal(\Gamma)$
\begin{align*}
V_\ell(b)^\ell = \bigl(\sup_{Z\in \Fcal(\Gamma)} |Z| \cdot \chi_{\frac b\ell} (\Dcal(Z))\bigl)^\ell \leq \bigl(\sup_{Z\in \Fcal(\Gamma)} |Z|^{\frac k\ell} \cdot \chi_{\frac bk} (\Dcal(Z))^{\frac k\ell}\bigl)^\ell.
\end{align*}
Then, the expression in the supremum is bounded by $V_k(b)^{\frac k\ell}$ and the power $\ell$ outside yields the claim.
\end{enumerate}
\end{varbems}

==> source/Exponential_estimates_for_the_adiabatic_theorem/Notes/Titel.tex <==
%auto-ignore  % for ArXiv to process correctly

%\ThisTileWallPaper{\paperwidth}{\paperheight}{Baumwallpaper.pdf}

%\thispagestyle{plain}

\title{A Setup for Exponential Estimates for the Adiabatic Theorem in Extended Quantum Systems}

\maketitle

==> source/gauge-fixing/biber_setup.tex <==
%auto-ignore  % for ArXiv to process correctly

\usepackage[
	sorting=nyt, 
	backend=biber, 
    giveninits=true,	
	%style=alphabetic,
	%style=numeric, 
	%bibstyle=authoryear,
%	style=alphabetic, %citestyle=numeric,
	maxbibnames=99,
	%doi=false,
	%url=false,
	backref=true,
	eprint=true,
	isbn=false,
	%labelnumber,
	%defernumbers = true,
	date=year,
	]{biblatex}

%\addbibresource{../BCS-Theory_Duke/BCS-Theory.bib}
\addbibresource{gauge_fixing.bib}


%%Append keywords to identify different bibliography entries.
%\DeclareSourcemap{
%  \maps[datatype=bibtex]{
%    \map{
%      \perdatasource{10_appendix/A_research_profiles/HAI.bib}
%      \perdatasource{10_appendix/A_research_profiles/NAM.bib}
%      \perdatasource{10_appendix/A_research_profiles/POR.bib}
%      \perdatasource{10_appendix/A_research_profiles/SOR.bib}
%      \perdatasource{10_appendix/A_research_profiles/SPO.bib}
%      \perdatasource{10_appendix/A_research_profiles/TEU.bib}
%      \step[fieldset=KEYWORDS, fieldvalue=cv, append]
%    }
%    \map{
%      \perdatasource{03_projects/A03.bib}
%      \perdatasource{03_projects/A05.bib}
%      \step[fieldset=KEYWORDS, fieldvalue=project, append]
%    }
%  }
%}
%
\DeclareLabelalphaTemplate{
   \labelelement{
     \field[uppercase,final]{shorthand}     
     %\field[uppercase,strwidth=1,strside=left,ifnames=1]{labelname}
     \field[uppercase,strwidth=1,strside=left,names=-5,noalphaothers]{labelname}
   }
   \labelelement{
     \field[strwidth=2,strside=right]{year}
   }
   \labelelement{
		\field[uppercase]{label}
   }
}
%
%\DeclareFieldFormat{labelnumberwidth}{\mkbibbrackets{#1}}
%\renewbibmacro*{cite}{%
%  \printtext[bibhyperref]{%
%    \printfield{labelprefix}%
%    \ifkeyword{cv}{\printfield{labelnumber}}
%      {\printfield{labelalpha}%
%       \printfield{extraalpha}}}}
%
%\defbibenvironment{bibliographyNUM}
%  {\list
%     {\printtext[labelnumberwidth]{%
%        \printfield{prefixnumber}%
%        \printfield{labelnumber}}}
%     {\setlength{\labelwidth}{\labelnumberwidth}%
%      \setlength{\leftmargin}{\labelwidth}%
%      \setlength{\labelsep}{\biblabelsep}%
%      \addtolength{\leftmargin}{\labelsep}%
%      \setlength{\itemsep}{\bibitemsep}%
%      \setlength{\parsep}{\bibparsep}}%
%      \renewcommand*{\makelabel}[1]{\hss##1}}
%  {\endlist}
%  {\item}

\renewbibmacro*{note+pages}{%
  \printfield{note}%
  \setunit{\bibpagespunct}%
  \printfield{pages}%
  \setunit{\bibpagespunct}% this ...
  \printfield{pagetotal}% ... and this is new
  \newunit}


\DefineBibliographyStrings{english}{%
  backrefpage = {page}, % originally "cited on page"
  backrefpages = {pages}, % originally "cited on pages"
}


\renewbibmacro{in:}{} % Supress "in"
\DeclareFieldFormat{pages}{#1}
\DeclareFieldFormat{pagetotal}{#1~pages}
\DeclareFieldFormat[article]{volume}{\mkbibbold{#1}}
\DeclareFieldFormat[article,inbook,incollection,inproceedings,patent,thesis,unpublished]{title}{#1} %{\mkbibquote{#1\isdot}} % Suppress quotation marks

%\assignrefcontextkeyws[sorting=none]{cv}
%\assignrefcontextkeyws[sorting=none]{project}
\AtEveryBibitem{\clearfield{number}}
\AtEveryBibitem{\clearfield{issue}}


%\renewcommand{\bibfont}{\normalfont\footnotesize}







%%% Test MR Number stuff
%
%\makeatletter
%%% this creates a mathscinet URL using first part of MR... (...)
%\def\MR@URL#1{https://mathscinet.ams.org/mathscinet-getitem?mr=#1}
%
%\AtBeginDocument{
%\@ifpackageloaded{hyperref}
%{% make a link to mathscinet
%  \ifdefined\Link
%  % workarount for htlatex in texlive 2020
%  \def\MRnumber#1{\Link[\MR@URL{#1}]{}{}#1\EndLink}
%  \else
%  \def\MRnumber#1{\href{\MR@URL{#1}}{\nolinkurl{#1}}}
%  \fi
%}% else
%{
%\def\MRnumber#1{\texttt{#1}}% just typeset the MR number
%}
%\DeclareFieldFormat{mrnumber}{\mkbibacro{MR}\addcolon\space\MRnumber{#1}}
%\newbibmacro*{doi+eprint+url}{%
%  \iftoggle{bbx:doi}
%    {\printfield{doi}}
%    {}%
%  \newunit\newblock
%  \iftoggle{bbx:eprint}
%    {\usebibmacro{eprint}}
%    {}%
%  \newunit\newblock
%  \iftoggle{bbx:url}
%    {\usebibmacro{url+urldate}}
%    {}%
%  \newunit\newblock
%  \printfield{mrnumber}}
%}
%
%\makeatother


